Class Conditional Alignment for Partial Domain Adaptation

Adversarial adaptation models have demonstrated significant progress towards transferring knowledge from a labeled source dataset to an unlabeled target dataset. Partial domain adaptation (PDA) investigates the scenarios in which the source domain is large and diverse, and the target label space is a subset of the source label space. The main purpose of PDA is to identify the shared classes between the domains and promote learning transferable knowledge from these classes. In this paper, we propose a multi-class adversarial architecture for PDA. The proposed approach jointly aligns the marginal and class-conditional distributions in the shared label space by minimaxing a novel multi-class adversarial loss function. Furthermore, we incorporate effective regularization terms to encourage selecting the most relevant subset of source domain classes. In the absence of target labels, the proposed approach is able to effectively learn domain-invariant feature representations, which in turn can enhance the classification performance in the target domain. Comprehensive experiments on three benchmark datasets Office-31, Office-Home, and Caltech-Office corroborate the effectiveness of the proposed approach in addressing different partial transfer learning tasks.

==> data_etn_1.tex <==
x y label
-8 35 2
-8 35 2
-7 35 2
-10 36 2
-10 35 2
-9 35 2
-10 35 2
-9 35 2
-9 35 2
-9 34 2
-10 35 2
-8 37 2
-8 36 2
-8 36 2
-8 36 2
-8 37 2
-9 36 2
-8 36 2
-8 37 2
-8 36 2
-9 37 2
-8 36 2
-7 37 2
-7 36 2
-7 37 2
-7 36 2
-7 37 2
-8 37 2
-8 36 2
-7 36 2
-8 35 2
62 -1 4
62 -1 4
62 0 4
62 0 4
61 0 4
61 0 4
61 0 4
61 0 4
61 1 4
61 1 4
60 1 4
61 1 4
61 2 4
61 1 4
54 5 4
55 5 4
54 5 4
54 6 4
54 6 4
54 6 4
54 6 4
54 6 4
53 5 4
53 5 4
54 5 4
53 5 4
53 5 4
-47 3 5
-50 3 5
-50 3 5
-52 3 5
-52 3 5
-52 3 5
-52 2 5
-50 3 5
-51 3 5
-51 2 5
-29 8 5
-51 3 5
-50 2 5
-50 2 5
-52 2 5
-50 2 5
-50 2 5
-52 2 5
-52 2 5
-51 3 5
-52 1 5
-48 3 5
-51 1 5
-51 1 5
-52 1 5
-52 1 5
-51 1 5
-52 1 5
-52 0 5
-52 1 5
-18 -52 7
-17 -50 7
-17 -52 7
-16 -52 7
-17 -52 7
-18 -52 7
-17 -52 7
-17 -52 7
-16 -52 7
-16 -50 7
-16 -52 7
-17 -50 7
-14 -52 7
-13 -53 7
-14 -53 7
-14 -52 7
-14 -52 7
-13 -53 7
-16 -53 7
-16 -53 7
-15 -53 7
-15 -54 7
-16 -53 7
-16 -54 7
-16 -53 7
-15 -53 7
-15 -51 7
-15 -51 7
-15 -51 7
-15 -51 7
-34 -33 6
-34 -33 6
-33 -32 6
-32 -33 6
-31 -33 6
-32 -31 6
-33 -32 6
-35 -33 6
-35 -33 6
-35 -33 6
-35 -33 6
-36 -33 6
-35 -33 6
-32 -32 6
-34 -35 6
-32 -33 6
-31 -33 6
-34 -34 6
-31 -33 6
-35 -33 6
-35 -34 6
-33 -34 6
-34 -34 6
-33 -33 6
-31 -31 6
48 18 6
-31 -30 6
-33 -33 6
-34 -33 6
-34 -33 6
-34 -33 6
-32 -33 6
-30 -32 6
-33 -32 6
-30 -32 6
-34 -32 6
-35 -32 6
-34 -32 6
-31 -32 6
-31 -32 6
-30 -31 6
-30 -31 6
-31 -32 6
11 -49 8
11 -49 8
11 -49 8
11 -49 8
11 -49 8
14 -50 8
14 -50 8
14 -51 8
14 -50 8
13 -51 8
13 -50 8
12 -50 8
13 -50 8
13 -49 8
13 -49 8
13 -51 8
13 -51 8
13 -51 8
14 -50 8
13 -51 8
13 -51 8
11 -51 8
11 -51 8
11 -51 8
11 -51 8
12 -50 8
11 -51 8
-35 44 1
-34 43 1
-35 44 1
-36 45 1
-36 45 1
-36 44 1
-36 44 1
-35 45 1
-35 45 1
-35 45 1
-35 46 1
-35 45 1
-35 44 1
-35 45 1
-35 45 1
-35 44 1
-35 44 1
-35 45 1
-34 43 1
-35 44 1
-34 43 1
-54 23 0
-54 23 0
-53 23 0
-55 23 0
-55 22 0
-55 22 0
-55 24 0
-55 24 0
-54 24 0
-55 23 0
-55 24 0
-55 24 0
-54 23 0
-54 23 0
-54 23 0
-55 24 0
-55 24 0
-55 23 0
-54 25 0
-53 25 0
-52 25 0
-53 24 0
-53 24 0
-53 25 0
-53 25 0
-53 24 0
-52 25 0
-52 25 0
-54 25 0
29 38 9
30 38 9
29 39 9
30 39 9
29 38 9
29 38 9
29 38 9
29 38 9
31 28 9
31 29 9
31 30 9
31 30 9
31 29 9
31 29 9
31 29 9
31 30 9
31 29 9
32 29 9
31 30 9
31 30 9
32 29 9
32 28 9
32 28 9
20 12 9
20 12 9
20 12 9
20 12 9
20 12 9
20 13 9
20 12 9
47 -18 3
47 -18 3
46 -19 3
47 -19 3
46 -19 3
47 -16 3
47 -16 3
48 -16 3
48 -16 3
48 -16 3
47 -17 3
47 -17 3
47 -17 3
47 -17 3
47 -19 3
48 -18 3
47 -18 3
47 -16 3
48 -18 3
47 -17 3
47 -16 3
47 -16 3
48 -18 3
48 -18 3
48 -17 3
48 -17 3
49 -18 3
-41 -41 6
-38 -39 6
56 5 4
43 -17 3
-35 41 1
45 -24 3
-31 39 1
-49 31 0
36 32 9
-31 36 1
55 -3 4
-48 30 0
-39 -38 6
57 -2 4
58 -3 4
-42 1 5
-41 4 5
27 -18 4
54 -2 4
-9 42 2
-9 45 2
-29 37 1
-46 27 0
46 -23 3
-29 39 1
7 -60 8
-39 -42 6
2 -10 2
44 -17 3
7 -62 8
56 -2 4
-36 -37 6
-12 42 2
-32 39 1
-13 -40 7
-46 2 5
19 45 9
-47 2 5
-47 -1 5
34 35 9
-36 -40 6
46 -23 3
-49 25 0
-31 37 1
-29 34 1
12 -55 8
-44 27 0
10 -59 8
-48 25 0
34 33 9
58 0 4
60 2 4
42 -24 3
35 39 9
-16 -47 7
-11 -48 7
-39 4 5
33 35 9
42 -20 3
-46 25 0
-42 2 5
56 -1 4
-10 42 2
-15 44 2
10 -57 8
-14 -48 7
-11 -47 7
-46 0 5
43 -20 3
-46 24 0
-44 30 0
37 36 9
41 -19 3
33 37 9
-32 37 1
4 1 0
55 -1 4
9 -59 8
7 -62 8
-13 44 2
-10 -44 7
36 34 9
11 -59 8
58 -3 4
5 -58 8
41 -22 3
-42 -43 6
13 -32 8
41 -24 3
-12 -47 7
-17 42 2
-16 39 2
-13 47 2
-41 -42 6
27 -17 4
7 -60 8
-12 -46 7
-48 26 0
-13 -48 7
-41 -43 6
33 39 9
-45 3 5
-13 44 2
-29 35 1
-42 1 5
-15 -48 7
-38 2 6
33 39 9
11 -58 8
-14 -46 7
58 -2 4
53 -1 4
42 -22 3
-42 25 0
32 37 9
10 -60 8
56 -1 4
-12 43 2
-39 -42 6
62 -2 4
44 -22 3
-16 38 2
-11 45 2
-13 -49 7
42 -23 3
-49 -3 5
33 39 9
11 -61 8
10 -57 8
-47 26 0
-31 33 1
-34 40 1
56 -5 4
53 0 4
-43 26 0
54 2 4
-10 41 2
11 -63 8
-15 -48 7
-45 0 5
32 32 9
8 -57 8
-30 35 1
-48 25 0
-37 -39 6
-38 -39 6
55 2 4
-12 47 2
9 -59 8
-9 45 2
33 36 9
-17 -46 7
53 1 4
33 34 9
-13 40 2
53 1 4
-10 -46 7
-13 -45 7
45 -20 3
-37 -38 6
-28 34 1
10 -59 8
32 34 9
-37 -44 6
-39 -41 6
-45 2 5
-38 -38 6
9 -58 8
35 37 9
41 -23 3
9 -55 8
-49 27 0
-45 3 5
7 -61 8
-30 35 1
-15 -47 7
53 1 4
41 -21 3
-14 43 2
-37 -44 6
-45 -1 5
-16 44 2
58 -6 4
43 -24 3
45 -21 3
31 35 9
54 -2 4
-39 -39 6
-15 -43 7
-33 38 1
42 -19 3
-13 -46 7
-10 43 2
-36 -39 6
-33 40 1
-34 40 1
-42 27 0
-43 26 0
12 -55 8
-45 25 0
13 -61 8
-42 27 0
58 2 4
-45 0 5
58 0 4
-34 35 1
-49 -2 5
-47 25 0
32 35 9
43 -17 3
-48 24 0
-13 -46 7
14 -56 8
8 -40 8
-29 35 1
-29 39 1
14 -60 8
41 -23 3
12 -55 8
8 -56 8
-44 28 0
-42 25 0
34 35 9
34 36 9
41 -22 3
36 34 9
-15 -45 7
-39 4 5
-48 25 0
-35 38 1
-14 -49 7
58 -3 4
58 0 4
53 -1 4
60 -4 4
-30 33 1
-43 4 5
35 32 9
28 -11 2
-49 29 0
-45 30 0
-15 43 2
35 36 9
-42 28 0
56 -1 4
-30 34 1
7 -60 8
-37 -44 6
-15 46 2
42 -21 3
-12 47 2
32 34 9
42 -21 3
33 34 9
34 34 9
57 1 4
14 -56 8
13 -56 8
35 36 9
-38 -37 6
-46 27 0
-47 26 0
56 -2 4
54 -3 4
33 35 9
-16 45 2
56 -3 4
-39 -38 6
-31 37 1
-48 26 0
13 -53 8
10 -60 8
44 -20 3
-17 42 2
-13 -40 7
58 2 4
-28 36 1
56 -2 4
-50 -2 5
11 -59 8
-40 -44 6
-47 28 0
-12 42 2
-13 40 2
-38 -38 6
5 -58 8
-47 1 5
-49 27 0
-35 37 1
-28 36 1
-11 -49 7
-14 -48 7
-11 -49 7
57 1 4
-41 -39 6
-36 -30 6
-37 -44 6
-17 -46 7
-12 43 2
-45 1 5
-16 45 2
-45 1 5
-39 -40 6
40 -20 3
-16 41 2
-49 26 0
-32 35 1
41 -18 3
11 -55 8
-45 2 5
-13 -46 7
13 -54 8
-43 4 5
-43 4 5
-41 -39 6
-13 40 2
-18 -46 7
57 -2 4
60 -3 4
-35 41 1
-48 -1 5
-36 -41 6
-30 37 1
56 1 4
-15 45 2
34 38 9
-28 36 1
-13 45 2
-16 -46 7
-43 2 5
36 34 9
-49 27 0
-16 41 2
33 39 9
-12 47 2
-47 27 0
54 -5 4
-42 1 5
-11 45 2
44 -19 3
9 -60 8
-46 3 5
-50 -2 5
-49 31 0
-12 -49 7
-29 34 1
-42 3 5
43 -23 3
-44 1 5
44 -17 3
32 38 9
-41 -39 6
-16 38 2
-38 2 6
-42 -43 6
-44 27 0
-31 39 1
7 -58 8
58 4 4
-43 1 5
-44 0 5
-49 -3 5
-33 41 1
-47 2 5
55 -2 4
-49 25 0
-11 44 2
34 34 9
43 -21 3
-11 45 2
33 35 9
-49 25 0
-29 35 1
43 -22 3
34 37 9
-28 34 1
31 35 9
-12 42 2
-35 37 1
45 -20 3
56 1 4
-35 38 1
-49 30 0
-32 36 1
-13 47 2
-42 -39 6
7 -62 8
33 33 9
-35 38 1
-29 37 1
10 -60 8
12 -58 8
62 -2 4
34 34 9
-40 -41 6
-10 42 2
-13 -46 7
56 -3 4
-16 40 2
-37 -37 6
-42 3 5
53 -2 4
-11 44 2
-28 35 1
-45 26 0
11 -63 8
-40 -39 6
-13 44 2
-14 42 2
-12 42 2
-45 2 5
52 1 4
-43 2 5
-10 42 2
7 -62 8
42 -20 3
45 -23 3
44 -21 3
-11 44 2
-13 43 2
-36 -38 6
12 -54 8
-27 34 1
-32 41 1
-38 -41 6
42 -16 3
-32 39 1
-11 47 2
-12 40 2
-45 0 5
-43 4 5
-36 -40 6
44 -17 3
-30 38 1
-41 4 5
-45 30 0
35 39 9
53 1 4
-16 40 2
13 -55 8
30 35 9
-15 -46 7
11 -54 8
-11 -49 7
-44 27 0
37 36 9
8 -56 8
43 -17 3
-43 -42 6
-46 5 5
37 36 9
-36 -41 6
35 39 9
-15 -48 7
45 -23 3
-49 27 0
53 2 4
55 0 4
-30 37 1
41 -21 3
53 -1 4
-14 46 2
41 -22 3
-38 -40 6
12 -54 8
56 -2 4
7 -62 8
-40 4 5
41 -18 3
9 -60 8
43 -20 3
-12 -45 7
-11 -47 7
-45 3 5
-43 25 0
-49 25 0
-12 44 2
-31 36 1
56 -3 4
8 -57 8
-10 -46 7
-36 -31 6
31 35 9
-48 30 0
44 -18 3
-50 -2 5
-32 34 1
33 34 9
41 -24 3
58 -2 4
-46 27 0
8 -61 8
-12 42 2
-44 27 0
8 -60 8
-12 -49 7
-49 30 0
-41 5 5
-44 5 5
-44 28 0
-14 42 2
-32 35 1
-39 4 5
-41 -41 6
33 39 9
36 35 9
-15 -47 7
53 3 4
8 -61 8
11 -56 8
-13 42 2
2 -10 2
-32 38 1
-41 -41 6
36 34 9
-30 33 1
-15 -48 7
-47 2 5
-48 26 0
-49 27 0
-46 5 5
-11 47 2
41 -19 3
-43 26 0
13 -56 8
60 -3 4
12 -58 8
13 -56 8
-15 -49 7
-49 28 0
-27 35 1
11 -56 8
-14 43 2
35 36 9
-14 46 2
33 33 9
-31 36 1
-15 -49 7
11 -57 8
-13 -49 7
36 39 9
57 -4 4
-29 34 1
12 -56 8
-42 -40 6
42 -21 3
-45 1 5
-46 3 5
-18 -46 7
13 -61 8
-14 -44 7
-39 -38 6
-16 44 2
-10 43 2
-32 35 1
44 -21 3
-47 27 0
35 39 9
9 -58 8
36 39 9
-12 -48 7
57 2 4
-48 27 0
13 -57 8
44 -20 3
58 -3 4
-15 43 2
43 -23 3
-15 45 2
32 35 9
36 36 9
11 -53 8
-10 42 2
-41 -41 6
-41 -42 6
13 -58 8
34 34 9
-46 24 0
59 -1 4
-37 -38 6
-14 44 2
43 -23 3
11 -63 8
-14 45 2
54 2 4
9 -56 8
-14 -44 7
44 -19 3
-11 45 2
34 38 9
8 -56 8
9 -62 8
-13 44 2
11 -63 8
-38 -39 6
12 -54 8
34 34 9
9 -61 8
42 -22 3
-46 25 0
57 4 4
60 -3 4
-15 -49 7
-45 29 0
25 9 4
-36 -37 6
8 -20 4
-45 25 0
54 -2 4
-16 38 2
-43 1 5
42 -21 3
-9 43 2
7 -60 8
41 -22 3
-16 -46 7
-14 42 2
9 -55 8
-27 34 1
-50 -2 5
-35 41 1
36 36 9
19 11 9
-43 -43 6
-38 -39 6
45 -20 3
-43 -41 6
55 -1 4
-39 -42 6
-27 35 1
-16 -49 7
54 -3 4
-29 39 1
-45 1 5
-41 -41 6
32 37 9
-29 36 1
-37 -44 6
9 -56 8
53 0 4
-48 -1 5
-44 5 5
-14 -49 7
-31 36 1
-13 -47 7
60 1 4
-48 24 0
-27 37 1
-32 41 1
32 33 9
7 -60 8
-42 27 0
-37 -38 6
-32 38 1
-45 26 0
-14 45 2
11 -63 8
-48 26 0
11 -56 8
-45 1 5
-15 -48 7
12 -54 8
-48 28 0
-38 38 1
-28 34 1
-15 -50 7
7 -12 3
-44 26 0
58 4 4
-49 -3 5
54 -2 4
-48 25 0
-37 39 1
-41 -39 6
8 -12 3
-33 38 1
-45 1 5
58 4 4
-40 -38 6
-36 -37 6
-32 39 1
37 34 9
-35 38 1
57 -4 4
9 -58 8
-42 -39 6
-12 44 2
-47 30 0
-47 27 0
60 -4 4
-10 43 2
55 -1 4
45 -23 3
-42 -43 6
14 -60 8
36 35 9
-38 -40 6
-10 -46 7
55 0 4
31 33 9
13 -57 8
45 -20 3
11 -56 8
-46 25 0
-30 38 1
-44 1 5
12 -56 8
-47 29 0
-45 30 0
-12 43 2
59 -1 4
-40 -42 6
-45 2 5
-49 28 0
56 -3 4
43 -20 3
-45 1 5
7 -62 8
-29 37 1
-10 42 2
-45 30 0
-34 37 1
15 24 9
-47 31 0
8 -40 8
11 -53 8
-43 -43 6
44 -21 3
57 -3 4
43 -24 3
-8 45 2
-27 37 1
58 -2 4
-40 -39 6
-16 -49 7
55 -2 4
-7 0 0
-36 -41 6
-17 -46 7
-40 -43 6
-48 27 0
-31 38 1
8 -20 4
-11 -44 7
-15 -47 7
-33 38 1
33 35 9
-29 39 1
-41 -42 6
12 -54 8
10 -60 8
-36 -37 6
-42 28 0
58 -3 4
9 -56 8
-46 28 0
10 -56 8
-14 -44 7
-39 -41 6
45 -20 3
10 -58 8
-45 1 5
-13 -49 7
33 39 9
-45 25 0
-13 -47 7
-9 45 2
-11 -44 7
-16 41 2
-13 43 2
-13 -44 7
-42 5 5
36 36 9
33 36 9
-40 -44 6
-32 41 1
-50 -2 5
54 2 4
54 2 4
-42 3 5
-29 36 1
-41 -42 6
-44 27 0
-49 -4 5
-45 0 5
-37 38 1
-11 45 2
-16 -45 7
-11 -49 7
31 33 9
-40 -41 6
57 1 4
-29 36 1
-34 40 1
58 -6 4
33 37 9
42 -21 3
-29 35 1
7 -61 8
54 2 4
34 32 9
-41 -42 6
-30 35 1
-30 38 1
-11 45 2
-10 42 2
-28 34 1
-45 3 5
53 3 4
-46 1 5
-5 41 4
9 -61 8
-28 35 1
-49 31 0
12 -56 8
28 -9 8
-17 42 2
44 -22 3
11 -59 8
45 -24 3
-15 45 2
43 -17 3
-32 34 1
-12 -47 7
-36 -38 6
11 -57 8
-39 -39 6
-12 -46 7
-41 4 5
42 -19 3
36 37 9
58 -6 4
-11 -48 7
-38 38 1
-46 2 5
55 0 4
-9 43 2
-30 37 1
-14 -47 7
-18 -48 7
42 -23 3
43 -22 3
54 -5 4
-12 46 2
-14 -45 7
-44 29 0
-32 35 1
-36 -40 6
2 -10 2
35 35 9
8 -59 8
-13 -44 7
56 -3 4
-37 38 1
-11 47 2
-39 -42 6
-17 -46 7
-5 41 4
-40 -40 6
-46 3 5
53 -2 4
-29 39 1
34 36 9
-48 31 0
59 -3 4
8 -58 8
-46 29 0
-29 36 1
45 -23 3
12 -55 8
33 32 9
-31 33 1
-37 -44 6
-14 -48 7
-49 -3 5
-43 3 5
32 34 9
-13 -44 7
44 -20 3
-34 40 1
-17 -46 7
-10 44 2
-30 36 1
-16 39 2
-38 -37 6
-31 38 1
-11 43 2
-18 -47 7
-44 0 5
-41 -43 6
-37 38 1
-47 31 0
59 0 4
14 -56 8
-15 -48 7
-15 46 2
42 -16 3
-40 -42 6
-50 26 0
-11 42 2
52 1 4
33 35 9
52 1 4


==> data_etn_2.tex <==
x y label
-7.8174 34.916 0
-7.6151 34.667 0
-7.3822 34.822 0
-9.8794 36.064 0
-9.9044 35.24 0
-8.787 34.718 0
-9.9143 35.269 0
-9.096 34.504 0
-8.6453 34.535 0
-9.4539 34.484 0
-9.7453 35.229 0
-8.4228 37.15 0
-7.8152 35.851 0
-8.328 35.909 0
-7.823 35.521 0
-8.2626 37.034 0
-9.4485 36.056 0
-8.0047 35.667 0
-8.286 36.514 0
-7.8345 35.768 0
-8.9396 36.587 0
-7.8447 35.772 0
-6.6588 36.793 0
-6.9345 36.042 0
-6.6194 36.745 0
-6.8037 36.18 0
-6.6586 37.015 0
-7.5071 36.521 0
-7.6461 35.56 0
-7.0824 36.023 0
-7.6257 35.475 0
62.193 -0.91024 0
62.181 -0.88945 0
62.308 0.36941 0
61.504 0.32807 0
61.304 0.10382 0
61.433 0.087755 0
61.385 0.24759 0
61.478 -0.46238 0
61.092 1.3623 0
61.251 1.4403 0
60.445 0.61649 0
60.627 0.6881 0
61.022 1.5414 0
61.05 1.19 0
54.461 5.4274 0
54.511 5.4086 0
54.47 5.4102 0
54.33 5.6577 0
54.243 5.6044 0
54.233 5.651 0
54.248 5.632 0
54.411 5.6023 0
52.97 5.2696 0
52.982 5.228 0
53.569 5.1067 0
53.477 5.1852 0
53.159 5.1942 0
-47.36 3.1666 0
-49.814 2.8356 0
-49.697 2.9284 0
-52.232 3.2974 0
-52.212 3.3576 0
-52.195 3.0314 0
-52.36 2.4104 0
-49.715 2.7133 0
-50.82 2.6354 0
-50.99 1.8622 0
-29.36 7.8932 0
-51.251 2.5641 0
-49.8 1.8321 0
-49.791 2.1245 0
-51.529 2.3985 0
-50.166 2.0332 0
-50.458 2.0978 0
-51.738 2.4115 0
-51.733 2.2386 0
-50.854 3.4123 0
-51.785 0.93183 0
-47.863 3.058 0
-51.391 1.1942 0
-51.353 1.1073 0
-52.253 0.93507 0
-51.601 0.53535 0
-50.595 0.66617 0
-51.725 0.8754 0
-51.926 0.49758 0
-52.343 0.83649 0
-17.906 -52.475 0
-16.676 -49.802 0
-16.609 -52.173 0
-16.46 -52.089 0
-16.86 -52.334 0
-17.931 -52.481 0
-17.232 -51.966 0
-16.909 -51.791 0
-16.352 -51.814 0
-16.309 -50.498 0
-16.359 -51.985 0
-16.533 -49.897 0
-13.509 -52.463 0
-13.397 -52.574 0
-13.787 -52.745 0
-13.841 -52.418 0
-13.694 -52.499 0
-13.243 -52.573 0
-15.628 -53.315 0
-15.527 -53.047 0
-14.587 -52.801 0
-15.187 -53.577 0
-15.66 -52.87 0
-15.814 -53.744 0
-15.801 -52.963 0
-14.915 -53.23 0
-15.377 -51.146 0
-14.749 -51.347 0
-15.16 -51.181 0
-14.771 -51.477 0
-33.993 -32.921 0
-33.672 -33.125 0
-33.183 -32.147 0
-32.44 -32.73 0
-31.363 -32.658 0
-32.246 -31.162 0
-33.06 -32.26 0
-35.179 -32.693 0
-34.886 -32.864 0
-35.165 -32.786 0
-34.936 -32.983 0
-35.51 -32.635 0
-35.235 -32.576 0
-31.796 -31.714 0
-34.249 -34.514 0
-32.422 -33.416 0
-30.796 -32.628 0
-33.838 -34.286 0
-30.781 -32.667 0
-34.782 -32.708 0
-34.67 -33.733 0
-33.297 -33.506 0
-34.466 -33.676 0
-32.575 -33.369 0
-30.639 -30.735 0
48.236 18.029 0
-31.02 -30.42 0
-32.611 -32.879 0
-34.162 -32.616 0
-33.904 -32.504 0
-34.003 -32.604 0
-32.224 -32.57 0
-30.215 -32.374 0
-33.289 -32.421 0
-30.313 -32.435 0
-34.359 -32.145 0
-34.54 -31.807 0
-33.815 -31.893 0
-30.748 -31.894 0
-30.638 -31.646 0
-30.151 -31.166 0
-30.269 -31.465 0
-31.005 -32.457 0
11.495 -49.251 0
11.415 -49.444 0
11.302 -48.878 0
11.285 -49.295 0
11.323 -48.848 0
13.931 -50.287 0
13.87 -50.41 0
13.644 -50.513 0
13.615 -50.421 0
13.464 -50.647 0
12.567 -49.722 0
12.374 -49.758 0
12.544 -49.649 0
12.958 -49.37 0
13.161 -49.366 0
13.044 -51.28 0
13.187 -50.825 0
12.804 -51.323 0
13.775 -49.68 0
13.2 -50.652 0
13.07 -51.354 0
11.19 -50.772 0
11.017 -51.009 0
11.033 -50.771 0
10.893 -51.145 0
11.565 -50.281 0
11.121 -51.002 0
-34.53 44.405 0
-33.961 43.212 0
-34.625 43.902 0
-36.074 45.159 0
-35.648 44.616 0
-36.438 44.427 0
-36.459 44.47 0
-34.703 44.642 0
-35.41 44.724 0
-35.119 45.197 0
-35.011 45.66 0
-34.856 45.313 0
-35.062 44.301 0
-35.277 44.5 0
-35.388 44.969 0
-34.576 44.179 0
-34.775 44.293 0
-34.944 44.887 0
-34.113 43.489 0
-34.517 43.647 0
-33.826 43.123 0
-54.273 22.77 0
-53.668 22.537 0
-53.316 23.381 0
-55.4 22.918 0
-54.762 22.343 0
-54.815 22.258 0
-54.936 23.672 0
-54.638 23.741 0
-54.239 23.69 0
-54.796 23.388 0
-55.313 23.52 0
-54.592 23.679 0
-53.774 22.504 0
-54.45 23.35 0
-54.27 22.829 0
-55.097 24.228 0
-55.016 24.345 0
-54.61 22.596 0
-54.279 24.751 0
-52.72 24.565 0
-52.408 24.673 0
-52.818 24.408 0
-52.885 24.479 0
-53.156 24.715 0
-53.385 24.76 0
-53.169 24.215 0
-51.714 25.289 0
-51.954 25.225 0
-53.786 24.51 0
28.933 38.32 0
30.454 38.471 0
28.756 38.807 0
29.787 38.579 0
28.607 38.471 0
29.45 38.18 0
29.093 38.414 0
29.049 38.284 0
30.984 28.1 0
30.984 28.581 0
31.234 29.715 0
30.875 29.783 0
30.616 29.148 0
31.011 28.73 0
31.029 28.665 0
31.083 29.745 0
30.919 29.098 0
31.503 29.277 0
31.359 29.753 0
31.493 29.575 0
31.501 29.132 0
31.793 27.986 0
31.711 27.832 0
20.164 12.111 0
19.914 12.038 0
20.016 12.351 0
20.13 12.083 0
19.779 11.904 0
20.216 13.321 0
19.818 11.913 0
47.425 -18.281 0
46.582 -18.325 0
45.73 -18.783 0
47.376 -18.708 0
46.231 -18.684 0
47.324 -15.896 0
47.274 -16.069 0
47.961 -15.78 0
47.877 -15.856 0
47.94 -15.889 0
46.585 -17.387 0
46.569 -17.118 0
46.778 -17.382 0
46.633 -17.402 0
47.492 -18.846 0
47.531 -18.352 0
46.983 -17.504 0
46.984 -15.957 0
47.634 -17.502 0
47.354 -17.198 0
46.996 -16.026 0
46.817 -15.799 0
48.167 -17.95 0
48.131 -18.152 0
48.331 -17.196 0
48.458 -17.014 0
48.776 -17.524 0
-40.969 -41.393 1
25.411 -20.018 1
-25.146 12.615 1
-38.187 -39.373 1
-2.1156 -0.90304 1
-40.176 -19.083 1
-13.029 0.36724 1
-12.646 -7.4634 1
13.663 40.052 1
55.613 5.1805 1
-29.071 11.383 1
9.8318 7.0395 1
42.665 -16.558 1
-34.739 40.595 1
-14.624 23.852 1
13.153 -33.495 1
44.684 -24.281 1
-31.488 39.367 1
13.942 -7.34 1
-3.3741 -13.421 1
6.4189 -5.7717 1
-48.623 30.743 1
-23.651 -11.372 1
35.519 32.233 1
3.664 9.3529 1
-43.831 -21.817 1
18.276 44.291 1
-31.42 36.008 1
-1.8747 23.198 1
20.436 23.979 1
-27.436 13.272 1
-25.98 11.725 1
27.556 4.8751 1
40.991 19.765 1
-4.0035 21.735 1
55.437 -3.0765 1
-47.612 29.883 1
-12.77 5.3379 1
-39.415 -37.939 1
-39.799 -16.193 1
-8.717 6.0235 1
41.563 18.916 1
57.41 -1.8999 1
24.64 -19.52 1
20.301 24.586 1
57.914 -2.7329 1
-42.063 0.80878 1
34.218 -42.142 1
36.231 -43.984 1
-25.491 -12.864 1
-41.352 3.9103 1
27.089 -17.608 1
4.1241 6.5028 1
17.15 43.648 1
-22.342 -27.759 1
8.0599 -38.397 1
3.2384 7.8374 1
53.99 -2.0541 1
-33.398 -31.242 1
16.602 43.609 1
46.673 20.923 1
3.8779 -10.55 1
-8.8381 42.379 1
16.942 -30.114 1
14.376 -30.419 1
-8.6273 44.79 1
-26.738 -11.179 1
-13.41 -0.32204 1
-28.957 37.249 1
23.748 -18.245 1
-46.049 26.748 1
45.904 -22.567 1
13.396 -10.48 1
-7.1299 -31.379 1
-29.115 39.204 1
-12.988 21.395 1
7.8866 14.506 1
-4.6254 -22.041 1
-22.084 -8.8008 1
-5.0363 -3.7661 1
6.7573 -60.456 1
-39.239 -42.18 1
1.6676 -9.8074 1
-25.273 12.566 1
3.6642 12.746 1
-8.7972 -4.0396 1
-42.68 -15.936 1
14.976 0.3219 1
13.103 -2.475 1
6.6262 -7.5865 1
25.906 -3.3902 1
43.699 -17.119 1
7.0364 -62.319 1
-7.1745 -2.6582 1
-10.984 20.463 1
56.278 -2.4761 1
17.262 20.805 1
15.479 19.538 1
-28.385 12.441 1
-36.32 -36.884 1
8.2843 -41.432 1
-12.028 41.87 1
-32.269 39.498 1
21.326 0.65466 1
-26.083 -7.7703 1
-13.016 -40.049 1
-44.154 -16.795 1
-46.372 1.5399 1
19.027 42.342 1
18.601 44.788 1
-26.814 -13.107 1
16.882 -32.13 1
21.314 -11.413 1
-46.54 2.1787 1
12.7 41.313 1
4.7167 -38.904 1
-46.863 -1.4241 1
11.836 -32.655 1
12.203 40.718 1
-32.923 6.6402 1
-10.565 18.932 1
0.081786 -24.347 1
34.136 34.914 1
-35.55 -40.215 1
45.852 -22.534 1
-7.1324 -32.639 1
27.663 4.9642 1
18.409 -5.1677 1
13.825 41.118 1
16.952 43.371 1
-48.723 24.648 1
17.349 23.647 1
-43.182 -18.09 1
-31.483 37.071 1
-29.173 33.625 1
-11.935 7.2302 1
32.75 -43.75 1
24.258 4.3224 1
-13.75 18.581 1
11.607 -55.049 1
-44.256 26.76 1
7.0997 -38.236 1
-12.226 4.1703 1
10.4 -58.549 1
-19.642 -10.647 1
19.394 -2.9727 1
-26.831 13.451 1
-3.5199 -21.583 1
-48.22 25.141 1
-4.9935 -3.8153 1
8.9286 -37.035 1
21.137 1.1438 1
-12.913 24.544 1
7.3144 8.631 1
-13.272 -0.4948 1
-47.563 -18.309 1
33.95 33.315 1
-2.1568 -6.2991 1
57.715 -0.39785 1
17.304 -34.984 1
9.0007 11.564 1
-12 18.977 1
3.2366 -27.748 1
59.985 1.8923 1
41.888 -23.698 1
0.56845 -27.9 1
13.877 -28.694 1
34.972 38.931 1
-16.076 -47.499 1
-10.891 -48.029 1
-39.134 4.1936 1
-47.605 -17.436 1
46.229 18.393 1
48.79 19.138 1
29.188 -16.247 1
33.198 35.431 1
-13.007 19.162 1
42.391 -20.061 1
-7.261 -2.6085 1
3.623 12.734 1
-13.737 5.5803 1
25.345 -20.866 1
17.165 45.994 1
8.2466 12.635 1
6.2612 7.1888 1
-0.39215 10.511 1
-45.537 24.51 1
-42.174 2.4228 1
56.187 -1.1522 1
-10.37 41.687 1
0.52661 -15.03 1
-15.175 43.894 1
11.925 46.376 1
10.158 -57.255 1
-44.291 -15.391 1
-11.129 18.065 1
-13.699 -48.17 1
-10.664 -3.7414 1
-11.173 -46.633 1
-45.781 0.17618 1
-2.9057 -5.7577 1
16.16 18.445 1
23.27 -18.231 1
-10.516 -0.67769 1
42.896 -20.377 1
28.229 -7.0134 1
12.942 -7.6408 1
-45.814 23.993 1
-43.999 29.534 1
10.873 42.406 1
17.523 18.658 1
36.663 35.883 1
40.899 -18.595 1
33.196 36.648 1
-31.802 10.476 1
-15.308 22.295 1
-24.073 -11.21 1
-1.9741 23.193 1
3.2201 7.8212 1
31.885 -10.735 1
-39.153 -19.77 1
-32.037 36.984 1
17.985 -33.779 1
-25.664 14.111 1
3.9778 0.87824 1
-25.758 14.085 1
26.208 -19.97 1
10.567 45.892 1
-15.789 22.95 1
55.203 -1.3177 1
25.456 14.04 1
-27.438 -11.328 1
14.219 -33.953 1
8.6037 -59.368 1
-42.534 -19.582 1
-15.281 3.6803 1
7.0514 -62.242 1
-22.119 -9.9685 1
-29.518 12.008 1
-22.465 -27.786 1
-2.0387 23.462 1
13.286 43.673 1
2.8578 10.913 1
-13.035 44.189 1
43.882 20.371 1
9.4797 40.591 1
18.17 -34.276 1
-9.6724 -43.67 1
36.469 33.657 1
11.042 -59.37 1
-19.311 -29.312 1
-14.844 -10.956 1
15.124 0.40912 1
27.391 5.2803 1
57.969 -2.933 1
5.2427 -57.839 1
37.268 -44.492 1
11.085 -6.0181 1
-2.2224 24.023 1
41.344 -22.345 1
-42.214 -42.952 1
13.159 -31.774 1
40.791 -24.097 1
-2.5372 24.439 1
-3.6428 -31.931 1
-24.23 -5.8333 1
5.5384 -37.092 1
14.008 -7.3266 1
-12.075 -46.506 1
7.8374 12.347 1
-3.4734 -8.1138 1
24.85 1.2423 1
-16.288 5.4341 1
-17.39 41.872 1
-16.081 38.857 1
-12.905 46.735 1
-4.8885 -6.6165 1
25.544 -15.868 1
5.2338 11.264 1
19.847 9.6453 1
-41.398 -42.21 1
33.237 -44.747 1
14.549 0.63113 1
6.444 -15.454 1
-6.4362 -33.676 1
27.006 -17.466 1
6.722 -60.479 1
-8.1412 3.3258 1
-12.425 -46.448 1
-48.129 26.116 1
-12.556 -47.587 1
-40.535 -43.039 1
2.4162 27.052 1
45.21 19.625 1
11.448 -18.917 1
33.031 38.846 1
-23.053 -10.402 1
-19.292 -29.327 1
-33.108 5.2704 1
-8.6878 -31.03 1
-45.11 3.1156 1
-27.697 -11.729 1
-13.029 44.13 1
-43.486 -15.368 1
24.931 -8.9956 1
6.6508 -7.6377 1
-29.105 35.282 1
14.981 43.476 1
26.756 -0.51217 1
27.248 5.6979 1
21.844 -19.889 1
-42.321 0.97298 1
-15.025 -47.677 1
-38.484 2.2612 1
11.886 -29.349 1
2.8465 22.421 1
-32.06 9.218 1
-9.6004 -8.486 1
33.114 38.897 1
-12.767 24.568 1
18.228 -34.336 1
29.954 -12.053 1
-22.091 -25.502 1
46.17 18.211 1
-7.1958 -31.612 1
-25.812 -11.146 1
-12.745 -5.9024 1
41.731 18.992 1
11.874 46.369 1
13.818 -32.673 1
-11.814 -0.076685 1
10.603 -57.541 1
16.947 -17.623 1
-43.42 -17.619 1
0.71902 25.049 1
-2.0172 8.4935 1
-13.713 -46.026 1
-44.936 -18.89 1
57.956 -1.7163 1
5.6015 -36.939 1
53.056 -0.56429 1
42.015 -22.493 1
14.435 -0.58012 1
23.009 3.2968 1
-42.409 24.83 1
31.973 36.629 1
-11.495 -8.5191 1
2.4354 27.258 1
10.021 -60.179 1
3.4835 -4.56 1
55.785 -1.2036 1
49.381 19.101 1
-27.379 14.167 1
12.458 44.5 1
3.8633 -10.779 1
-16.11 2.6105 1
-0.12345 13.313 1
-12.088 42.675 1
21.549 23.904 1
16.034 -34.586 1
18.961 -16.439 1
2.9111 28.467 1
-39.43 -42.098 1
62.32 -1.7686 1
-5.4243 -5.5616 1
44.389 -21.993 1
-7.2359 -2.6382 1
-15.791 38.49 1
-11.297 45.369 1
-12.55 -48.564 1
-12.709 -7.8955 1
42.498 -23.398 1
15.966 44.646 1
8.9578 11.597 1
22.335 -2.3696 1
-20.732 -26.568 1
5.5954 16.451 1
-27.368 10.069 1
-49.043 -3.1706 1
-22.747 -8.631 1
2.8186 29.375 1
21.894 -19.899 1
42.817 15.92 1
-3.6549 -7.4499 1
-17.536 -25.42 1
-13.322 23.251 1
17.656 -17.131 1
4.9171 8.5865 1
33.077 38.868 1
-20.968 -26.188 1
7.76 15.627 1
17.846 1.2041 1
-13.075 0.38042 1
11.45 -60.895 1
9.8319 11.668 1
13.596 46.016 1
-44.691 -15.821 1
15.691 -0.86666 1
20.717 4.1549 1
32.763 -42.315 1
22.769 -18.163 1
-22.471 -27.842 1
10.202 -57.184 1
-23.634 -11.377 1
-47.101 25.735 1
-30.99 32.853 1
17.301 21.531 1
-33.585 40.312 1
11.655 -33.068 1
13.875 -28.749 1
55.582 -4.572 1
44.425 17.8 1
-21.484 -12.731 1
14.007 -3.9885 1
53.118 0.025473 1
-42.755 25.871 1
53.881 2.3929 1
-10.215 41.312 1
-7.3955 -27.214 1
10.983 -63.239 1
-14.78 -48.064 1
-45.447 -0.10265 1
8.6128 10.361 1
-8.4365 -31.185 1
1.0003 12.36 1
-21.538 -11.305 1
32.406 32.289 1
-12.198 -8.1155 1
16.237 41.8 1
-3.7631 7.2086 1
8.2362 -57.238 1
-30.484 34.743 1
-47.525 25.232 1
-11.893 -7.2623 1
-7.3078 -8.5916 1
4.038 6.4008 1
-37.051 -39.048 1
5.577 -9.1922 1
-37.884 -38.994 1
55.237 2.4766 1
25.284 2.1854 1
-12.387 23.264 1
47.816 17.963 1
-11.89 -5.8908 1
-11.813 46.642 1
17.168 45.986 1
-12.895 5.2429 1
-24.472 -27.697 1
27.72 -6.8765 1
-26.607 -10.86 1
-9.8122 19.69 1
5.6175 -9.1999 1
3.554 -11.826 1
0.92742 21.937 1
9.4064 -58.886 1
-9.2051 45.303 1
32.83 36.346 1
7.5313 13.52 1
-9.2698 -9.9275 1
-17.225 -46.193 1
14.359 -34.884 1
-13.044 24.228 1
25.203 -0.46609 1
34.322 -12.765 1
48.792 20.324 1
-14.443 1.5141 1
32.657 -45.654 1
-22.566 -29.326 1
52.691 0.71809 1
33.034 33.849 1
14.694 -10.191 1
18.214 22.11 1
8.7938 7.8603 1
-10.746 1.6636 1
15.027 0.39674 1
-32.246 8.2711 1
-12.566 40.131 1
12.271 39.1 1
25.35 2.1103 1
52.722 0.85297 1
-9.9988 -45.639 1
-16.654 4.2283 1
-9.8204 -1.9035 1
14.13 -34.021 1
-12.911 -45.309 1
45.005 -20.195 1
26.985 -2.8559 1
-4.5248 -19.15 1
-37.002 -38.049 1
-3.7652 -8.4133 1
-28.027 34.088 1
10.492 -58.77 1
31.897 34.236 1
3.9911 -9.9477 1
8.7371 42.368 1
-10.843 6.0891 1
0.7667 7.1242 1
-37.07 -43.574 1
26.026 4.3761 1
7.6052 -10.227 1
-8.1162 -10.864 1
-13.365 -2.1467 1
2.7681 29.357 1
-9.8998 23.31 1
34.255 -12.74 1
46.051 19.719 1
30.832 -48.023 1
-4.5516 -7.9863 1
-39.272 -41.211 1
-0.66323 -27.147 1
13.143 -7.4109 1
23.578 3.4781 1
26.21 -1.899 1
18.059 5.3611 1
-45.19 2.0083 1
31.893 -44.393 1
-38.447 -38.437 1
12.23 -23.706 1
-6.9105 22.808 1
7.4979 -10.235 1
31.824 -10.774 1
9.323 -58.251 1
25.837 -3.2709 1
35.303 36.768 1
34.971 -10.462 1
41.114 -23.349 1
-6.1408 -29.195 1
-5.7021 -15.905 1
15.834 -27.941 1
9.1595 -54.806 1
-3.9401 -28.775 1
16.73 19.757 1
-49.426 26.508 1
48.787 20.31 1
-45.169 2.5818 1
-29.456 12.017 1
-3.6204 -31.943 1
24.137 -18.933 1
3.5091 -11.814 1
6.7154 -61.442 1
15.814 -27.951 1
-15.674 1.9319 1
-26.812 -11.517 1
-27.5 13.522 1
6.8645 9.8504 1
-42.701 -17.936 1
11.484 -7.0841 1
11.587 45.872 1
-30.348 34.717 1
-24.247 -5.8466 1
-15.254 -47.158 1
33.115 -49.642 1
44.747 18.092 1
11.236 9.4713 1
53.038 1.1884 1
30.23 -43.421 1
-12.207 -3.4201 1
24.971 -25.349 1
-21.408 -11.402 1
41.497 -21.466 1
-23.828 -24.89 1
18.176 -13.428 1
2.9052 28.355 1
-5.6776 -15.942 1
-14.367 43.399 1
-37.063 -43.627 1
6.2184 -37.396 1
-22.673 -8.6315 1
24.518 -25.419 1
-3.6894 -8.4488 1
-43.877 -21.822 1
-45.25 -0.55019 1
43.066 18.099 1
-16.305 43.84 1
5.252 -39.61 1
10.674 -15.039 1
58.303 -6.009 1
0.72102 25.084 1
43.479 -23.639 1
-47.407 -17.461 1
46.917 21.705 1
-13.381 2.7683 1
17.702 -16.931 1
-13.192 23.082 1
45.258 -21.355 1
31.277 35.238 1
54.006 -2.0107 1
-39.196 -39.141 1
31.341 -46.055 1
-44.289 -14.468 1
-13.373 3.8265 1
-14.506 -43.475 1
-42.573 -12.612 1
8.3242 -41.483 1
0.80192 7.669 1
25.589 -25.469 1
30.752 -9.3187 1
11.983 43.996 1
3.4808 9.9946 1
14.159 1.019 1
2.1664 28.101 1
18.288 23.343 1
-32.608 38.088 1
31.974 -45.64 1
42.123 -19.279 1
12.404 -10.345 1
-17.777 -25.781 1
12.801 -34.403 1
-0.37293 20.749 1
2.8154 10.856 1
-12.732 -45.697 1
8.7035 10.828 1
-9.5973 43.015 1
27.062 -19.067 1
-36.26 -38.547 1
2.9066 24.751 1
-1.5282 23.654 1
-33.363 40 1
-42.106 -18.064 1
43.214 19.721 1
-27.284 14.19 1
-33.544 40.268 1
3.3689 -30.172 1
-42.156 26.862 1
13.309 42.577 1
-43.277 25.887 1
32.581 -44.798 1
-6.0653 -6.4393 1
-7.5945 -31.734 1
5.6633 7.846 1
12.197 -55.476 1
-45.453 25.139 1
-9.5038 -8.4254 1
29.35 -45.222 1
27.126 -19.731 1
12.555 -60.991 1
8.9415 -37.025 1
-42.137 26.899 1
-11.531 -8.3658 1
25.502 -19.668 1
30.619 -10.398 1
23.056 -0.78814 1
58.206 1.6875 1
1.7442 14.194 1
-45.295 -0.39683 1
-1.0254 23.974 1
15.749 -1.3703 1
-7.5584 -27.268 1
30.833 -9.0544 1
57.709 -0.4374 1
27.571 4.9466 1
-13.481 3.7686 1
-26.786 13.964 1
-30.167 9.2792 1
-33.558 35.377 1
-26.402 -12.859 1
-46.126 -16.712 1
-11.879 7.1837 1
-6.4745 -25.331 1
-1.5212 23.701 1
-6.4268 -33.669 1
47.006 21.77 1
-6.16 -29.276 1
-48.819 -2.1927 1
7.2204 -8.3149 1
18.448 -14.332 1
12.213 44.51 1
-47.413 24.912 1
1.7329 14.232 1
-9.5965 1.4134 1
32.852 -46.9 1
8.9644 -10.733 1
25.105 -0.86941 1
31.566 34.948 1
-13.226 23.193 1
42.674 -16.695 1
-16.493 -3.6126 1
29.882 -7.4826 1
-47.579 24.309 1
8.8496 -10.685 1
2.7419 11.263 1
-25.784 -13.059 1
-11.105 20.442 1
-33.07 10.533 1
-12.202 18.049 1
7.8628 40.759 1
-13.209 -45.647 1
13.663 -55.936 1
-45.301 -16.713 1
1.9347 11.044 1
8.4982 -39.51 1
17.793 -32.648 1
-32.425 7.2036 1
-29.321 34.68 1
32.082 -48.038 1
47.594 16.972 1
20.775 22.241 1
-29.059 39.123 1
-35.511 4.2894 1
31.795 -41.663 1
-45.526 -18.462 1
20.814 -1.7653 1
8.7043 10.775 1
44.223 20.084 1
-47.652 -17.693 1
14.223 -59.609 1
-45.163 -16.381 1
41.234 -23.405 1
11.897 -55.445 1
0.6873 -14.977 1
11.072 41.472 1
7.6657 -55.744 1
14.427 -31.995 1
11.523 -12.821 1
17.777 -16.395 1
43.735 17.222 1
-1.1651 15.928 1
-44.217 28.327 1
19.263 -30.853 1
-40.139 -14.06 1
-35.132 4.3971 1
0.87373 23.011 1
12.103 -30.798 1
21.429 23.514 1
-42.395 24.801 1
34.301 34.918 1
33.847 36.46 1
7.5792 -10.344 1
5.417 -26.101 1
-13.319 -2.242 1
16.13 -35.283 1
40.598 -21.983 1
36.149 33.846 1
24.682 -17.757 1
-15.22 -45.141 1
-31.995 10.404 1
13.991 -7.3106 1
24.934 -23.01 1
20.962 -17.034 1
2.4642 27.043 1
-15.941 4.5275 1
-9.8543 -1.8402 1
-38.987 4.1895 1
-48.252 25.249 1
22.718 -25.022 1
-11.957 23.809 1
-35.45 37.794 1
-13.504 -48.98 1
57.919 -3.4579 1
58.213 0.038714 1
5.82 -20.939 1
-0.63079 -29.264 1
31.581 -43.618 1
24.705 -18.868 1
52.615 -1.4562 1
13.477 -10.57 1
0.5964 -15.346 1
-22.636 -8.721 1
-10.122 18.842 1
-20.662 -26.684 1
16.559 23.834 1
-13.04 6.3962 1
32.603 -49.65 1
4.3838 -38.532 1
33.768 -43.307 1
59.597 -4.2663 1
-29.61 33.459 1
10.676 -15.061 1
-43.195 3.7728 1
32.009 -48.498 1
11.522 -32.847 1
5.6525 -38.346 1
45.12 18.539 1
30.695 -8.3546 1
5.3212 -40.628 1
-16.327 5.4378 1
35.489 32.264 1
5.62 -2.9262 1
27.527 -10.817 1
-7.6746 -27.048 1
-29.565 11.931 1
41.33 20.199 1
26.957 -25.39 1
-12.057 -8.0822 1
16.23 -2.2409 1
-21.588 -25.959 1
-20.213 -26.098 1
6.3117 9.6718 1
-31.07 8.4064 1
8.1998 -41.471 1
0.64078 -15.147 1
16.89 -30.112 1
-48.845 29.41 1
-27.353 13.603 1
-8.7979 -4.0543 1
-23.917 -9.2288 1
-45.376 29.945 1
27.523 -13.524 1
10.949 44.53 1
24.764 -1.5573 1
-14.871 43.197 1
-32.778 9.4583 1
34.746 36.458 1
7.6735 -38.66 1
23.491 5.3194 1
20.797 2.6712 1
16.172 22.125 1
11.213 9.4877 1
-0.14754 13.333 1
36.692 -44.449 1
-41.712 27.983 1
56.098 -1.123 1
24.914 -9.1116 1
-30.214 34.063 1
-1.4625 -21.515 1
7.4489 -59.635 1
27.681 5.0336 1
-6.8508 -15.846 1
-11.424 -5.9498 1
30.659 -11.638 1
-37.067 -43.591 1
-15.221 46.043 1
12.9 -34.499 1
11.848 -33.516 1
41.534 -21.449 1
15.645 44.557 1
31.816 -48.257 1
34.015 -42.818 1
34.331 -41.175 1
-11.638 46.581 1
-21.025 -27.927 1
32.377 33.94 1
-14.068 25.414 1
-42.502 -19.575 1
42.281 -21.164 1
34.883 -42.403 1
-0.9591 -9.4938 1
18.27 23.33 1
-43.698 -16.674 1
-7.4851 -24.252 1
27.582 -5.1736 1
12.597 0.58999 1
7.8601 -41.264 1
34.977 -10.455 1
-43.97 -15.419 1
30.801 -9.0434 1
32.687 34.08 1
33.843 34.033 1
56.857 0.78754 1
32.569 -49.504 1
21.318 -11.411 1
14.147 -55.882 1
12.767 -55.874 1
43.247 18.112 1
22.385 22.92 1
-24.377 -11.958 1
12.709 42.126 1
11.179 41.349 1
-8.7924 -31.408 1
34.159 -42.154 1
-47.278 -17.406 1
12.674 42.927 1
12.959 -7.6227 1
34.55 35.684 1
-38.304 -37.46 1
28.215 -6.9938 1
-46.05 26.731 1
-47.004 25.616 1
56.046 -2.0106 1
-25.903 -12.278 1
19.255 21.885 1
53.78 -3.0443 1
32.899 35.014 1
26.229 -0.83244 1
36.495 -43.73 1
-16.444 44.803 1
6.4726 -36.999 1
55.79 -2.5585 1
-38.78 -37.998 1
-30.737 37.471 1
-47.518 26.063 1
14.308 -30.431 1
21.702 -17.744 1
12.972 -52.815 1
22.974 -0.39718 1
13.721 21.027 1
-12.17 18.037 1
9.8837 -60.346 1
43.525 -20.369 1
42.961 21.071 1
-17.381 41.873 1
-13.052 24.132 1
-13.013 -40.043 1
58.219 1.6872 1
-28.117 35.59 1
55.937 -1.8592 1
31.776 -9.3743 1
-9.8622 -9.0286 1
20.854 9.1658 1
-49.579 -1.607 1
9.8689 11.684 1
11.009 -59.169 1
22.36 22.912 1
-39.698 -44.373 1
17.313 -33.423 1
-46.675 27.931 1
30.292 -44.299 1
-12.167 41.654 1
-12.78 40.336 1
-38.029 -37.706 1
5.258 -57.849 1
-47.099 0.86857 1
-26.109 -7.8003 1
-14.264 -9.4578 1
-48.664 26.922 1
-2.9678 -29.837 1
24.942 -9.1842 1
-7.76 -32.336 1
-34.938 36.973 1
-22.578 -10.428 1
-28.478 36.473 1
-2.2708 -6.3025 1
-47.581 -18.205 1
-11.141 -49.265 1
-12.238 7.0543 1
3.3186 29.002 1
-14.373 -48.042 1
28.874 -9.6243 1
33.332 -45.197 1
21.265 0.67106 1
6.5074 15.917 1
-3.2953 -8.174 1
-10.949 -49.436 1
-35.259 4.3864 1
56.855 0.86714 1
-40.694 -39.306 1
-31.886 10.53 1
-35.943 -30.499 1
-37.082 -43.609 1
21.359 23.648 1
26.222 -18.54 1
7.0921 15.662 1
11.14 44.183 1
-24.384 -10.388 1
-3.9983 21.652 1
0.77596 21.535 1
2.5134 23.405 1
5.2045 -39.658 1
-6.7457 -27.762 1
-13.749 3.4505 1
-17.244 -46.274 1
-12.056 42.776 1
-44.926 0.753 1
13.886 -2.6355 1
-16.38 44.854 1
-44.954 1.1591 1
-38.621 -40.036 1
2.6643 23.395 1
25.342 4.3115 1
40.381 -19.502 1
-7.1493 22.531 1
-13.043 19.172 1
32.719 -45.609 1
12.52 -4.7971 1
-5.4784 -29.522 1
-20.754 -27.35 1
-42.869 -16.335 1
-15.937 23.984 1
-16.157 40.916 1
0.94009 12.451 1
-48.646 26.349 1
12.753 42.903 1
-1.6013 -0.89066 1
8.9024 -37.074 1
18.067 5.3595 1
20.589 24.211 1
-3.6387 -7.3462 1
-15.189 22.261 1
37.616 -44.434 1
-7.3392 -5.9489 1
13.221 45.398 1
24.133 15.127 1
-7.2022 -2.6597 1
-32.11 35.081 1
11.628 -32.743 1
-0.90536 6.2335 1
41.065 -17.664 1
-15.442 3.5996 1
11.164 -54.82 1
-45.349 1.674 1
-42.544 -19.696 1
-2.9342 -5.8348 1
-11.763 3.882 1
-22.467 -27.954 1
12.723 44.543 1
-12.759 -45.934 1
34.296 -41.289 1
0.6583 -19.727 1
0.70565 -15.227 1
2.9377 24.764 1
12.504 -53.671 1
-43.231 3.7165 1
16.212 -36.533 1
-35.374 4.9118 1
-43.467 3.5176 1
-5.892 -15.806 1
0.28727 24.278 1
4.3743 -8.5347 1
0.15098 -24.37 1
-41.221 -39.101 1
-12.527 40.085 1
-44.128 -15.249 1
18.68 22.971 1
-17.541 -46.006 1
-43.732 -16.366 1
-9.0924 -10.107 1
-26.848 13.674 1
57.388 -1.8031 1
-12.537 6.9373 1
60.079 -2.6617 1
3.6584 12.743 1
-1.1268 5.7228 1
13.986 -3.995 1
-31.069 7.9553 1
15.804 20.677 1
-34.762 40.59 1
19.922 -16.309 1
-25.604 -11.346 1
47.418 19.352 1
-48.191 -1.2475 1
10.965 44.521 1
-35.545 -41.031 1
-20.73 -8.9296 1
26.755 -7.1948 1
-8.9074 -14.995 1
-14.803 23.144 1
-5.6228 -0.31775 1
-22.447 -29.285 1
-29.692 36.587 1
56.239 0.95017 1
-9.9712 23.39 1
-14.806 44.721 1
19.418 19.794 1
34.474 37.967 1
-28.166 35.907 1
-4.8595 -1.6602 1
-12.925 44.687 1
-16.151 -46.038 1
-43.381 1.8637 1
-6.4555 -16.191 1
36.066 33.811 1
4.6048 -39.392 1
-41.451 -15.801 1
-49.274 26.525 1
1.7497 14.205 1
19.895 23.092 1
-25.234 -11.165 1
-16.144 40.94 1
-0.78017 -2.3103 1
33.014 38.775 1
3.3624 -30.162 1
-4.5564 -29.503 1
-31.477 7.5616 1
-7.8692 -1.6396 1
13.191 -27.666 1
0.6593 -19.722 1
-11.625 46.526 1
-15.163 22.371 1
47.516 18.988 1
6.3534 8.5569 1
-34.878 4.8436 1
-8.1159 -23.781 1
-24.412 -12.174 1
0.11223 -24.337 1
2.5101 -7.9331 1
23.074 -0.76433 1
14.025 -3.9926 1
-14.522 2.5599 1
-0.28804 22.097 1
26.357 -1.6376 1
-6.9285 -30.706 1
16.187 18.501 1
-47.346 27.271 1
54.307 -4.8023 1
26.953 0.7947 1
-42.088 0.85666 1
24.221 -19.073 1
-5.5893 1.5797 1
-11.081 44.911 1
-15.206 4.5153 1
43.687 -18.759 1
9.2397 -60.207 1
-15.66 20.041 1
-21.506 -12.562 1
-45.586 3.4046 1
-49.645 -1.6226 1
-48.661 30.845 1
-1.4291 -9.2482 1
-12.458 -48.634 1
-29.159 34.475 1
30.945 -9.6795 1
-42.025 2.8625 1
42.588 -23.211 1
-2.988 -27.615 1
5.8691 -13.168 1
31.204 -10.537 1
-43.906 1.2219 1
43.733 -17.128 1
-22.862 -25.854 1
-25.175 -7.6148 1
-28.924 10.737 1
-8.1781 3.3446 1
32.449 38.033 1
0.64978 18.857 1
16.773 42.745 1
-40.984 -39.051 1
27.505 4.9221 1
-34.554 -27.813 1
-45.235 -15.766 1
14.437 -34.833 1
-16.232 38.424 1
31.828 -48.509 1
-26.465 -12.814 1
15.312 20.701 1
-38.488 2.2687 1
24.933 -23.005 1
-12.75 -5.9684 1
-42.387 -42.621 1
-44.202 26.829 1
44.672 18.064 1
-31.154 38.973 1
-10.641 -3.7369 1
7.1687 -57.647 1
57.751 3.5289 1
14.428 -15.982 1
2.0519 11.223 1
-42.903 1.3358 1
18.687 -3.8614 1
-43.519 -0.015586 1
24.132 15.117 1
-33.141 10.576 1
6.8478 9.7604 1
25.019 -23.181 1
12.778 -11.756 1
-49.046 -3.0779 1
19.94 18.339 1
-11.303 6.0707 1
8.3861 9.7324 1
34.645 -42.021 1
-33.398 40.634 1
16.124 -35.198 1
24.713 -17.804 1
-1.3347 23.675 1
-46.903 2.2742 1
55.283 -1.644 1
-42.234 -16.284 1
36.193 -45.029 1
24.554 -8.0478 1
-49.291 24.983 1
0.56021 18.913 1
0.42942 -15.243 1
46.399 17.851 1
27.706 5.0122 1
-10.933 43.733 1
12.957 -34.514 1
33.897 33.854 1
43.078 -20.985 1
23.592 5.2028 1
23.908 -0.11035 1
31.767 -41.136 1
24.394 -25.596 1
-10.954 44.988 1
5.6177 16.465 1
33.342 35.475 1
6.0015 -41.163 1
3.4787 9.9756 1
20.117 -16.63 1
11.447 -18.925 1
-48.855 24.979 1
-35.297 4.2761 1
-28.975 35.267 1
-6.4979 -16.182 1
5.4808 -26.077 1
43.442 -22.379 1
33.845 36.546 1
-27.886 34.361 1
26.964 -2.7757 1
31.352 35.27 1
-12.228 41.953 1
24.277 -25.641 1
19.959 22.54 1
-4.5818 -11.883 1
-28.913 12.356 1
12.671 41.243 1
-34.988 37.331 1
18.214 44.287 1
24.928 -9.0383 1
-13.684 18.588 1
25.354 -17.882 1
14.524 44.382 1
44.801 -20.223 1
-10.93 1.6761 1
-15.999 4.5603 1
-46.28 -15.946 1
1.6804 23.243 1
56.22 0.91377 1
-35.238 38.462 1
-48.825 29.507 1
13.99 -33.178 1
-44.584 -17.094 1
6.5974 9.2028 1
-32.466 36.181 1
-12.853 46.74 1
-41.873 -39.169 1
46.141 19.744 1
-13.821 23.983 1
-0.32294 10.417 1
7.2976 -61.66 1
-10.061 -0.10738 1
18.464 20.659 1
4.193 -38.433 1
1.1651 -26.624 1
15.696 44.675 1
5.8279 -20.937 1
2.9659 24.894 1
-45.042 -17.068 1
32.998 33.427 1
-35.468 37.794 1
-29.451 37.089 1
-19.728 -27.577 1
14.872 23.744 1
25.438 -20.033 1
9.9963 -60.279 1
-9.2386 7.2958 1
7.1752 -36.423 1
-11.975 19.054 1
41.175 20.02 1
-0.48931 -22.911 1
-6.7291 22.841 1
12.375 -58.43 1
-11.855 19.313 1
62.345 -1.7909 1
13.906 -32.723 1
8.8388 7.8625 1
-13.73 -3.9683 1
18.21 -13.427 1
14.312 1.2633 1
33.648 33.743 1
-39.96 -41.212 1
-9.8254 41.644 1
-12.936 -45.762 1
9.1347 -10.767 1
27.063 -19.002 1
-27.776 10.625 1
55.512 -2.5627 1
28.586 -10.269 1
-39.327 -17.854 1
33.198 -43.601 1
9.7652 -39.581 1
-16.404 39.557 1
-10.754 6.2041 1
-42.59 -19.785 1
14.077 1.1738 1
3.8966 -39.348 1
-37.334 -37.192 1
4.8721 -8.4671 1
-41.934 2.864 1
52.599 -1.5874 1
-11.066 43.504 1
-20.143 -25.004 1
25.703 -25.799 1
34.29 -12.746 1
-11.931 19.122 1
31.978 -48.082 1
-9.7794 20.314 1
-28.243 34.606 1
-44.939 25.987 1
10.992 -63.196 1
-7.634 -32.176 1
12.892 -29.269 1
-39.545 -38.529 1
41.032 19.926 1
3.3475 16.793 1
-20.355 -26.398 1
-6.35 -24.398 1
18.589 19.751 1
37.26 -44.529 1
-25.015 10.438 1
-13.138 44.083 1
-13.942 42.17 1
2.3129 -7.8644 1
-13.779 2.1774 1
-11.94 41.694 1
-7.8173 -32.515 1
-22.667 -8.6243 1
-44.626 2.4194 1
52.297 0.72742 1
31.604 -43.553 1
-43.433 1.9274 1
14.526 -1.5438 1
-10.426 41.645 1
-1.212 8.4123 1
7.0399 -62.23 1
-42.461 -15.727 1
-24.095 -27.585 1
42.221 -19.862 1
44.854 -22.565 1
-9.6311 19.416 1
25.461 14.06 1
11.447 -18.897 1
18.077 5.3529 1
31.722 -45.083 1
-2.9457 22.733 1
7.7643 -38.166 1
-9.5338 19.417 1
44.061 -21.4 1
11.897 -32.588 1
-30.914 7.8836 1
-13.179 21.404 1
-10.688 43.556 1
-12.69 42.635 1
2.6825 21.171 1
19.836 9.6429 1
-3.6359 -15.218 1
23.204 16.52 1
-1.3215 -19.747 1
18.419 -5.1475 1
24.8 -26.617 1
26.219 0.82031 1
-36.486 -37.726 1
21.029 3.2849 1
-23.657 -11.949 1
-14.806 1.8463 1
12.189 -53.634 1
17.161 1.1793 1
-34.561 -27.841 1
-27.307 33.863 1
-32.208 41.222 1
31.793 -44.122 1
13.258 45.171 1
-37.969 -41.068 1
42.415 -16.186 1
1.2121 -12.266 1
-32.166 8.3221 1
-31.52 39.435 1
-10.984 47.364 1
-12.474 40.199 1
-45.432 -0.2778 1
-43.373 3.5272 1
-35.555 -40.086 1
43.835 -17.456 1
-26.003 -13.243 1
-10.76 1.6579 1
-30.499 38.422 1
-23.571 -29.042 1
-24.94 10.383 1
22.646 1.0282 1
-43.833 -21.802 1
20.931 22.848 1
12.834 2.1149 1
-27.491 13.564 1
18.437 -2.3781 1
-41.207 4.232 1
-45.456 29.849 1
35.324 39.296 1
13.808 39.926 1
-5.5384 -29.575 1
25.473 13.991 1
52.662 0.85599 1
9.375 -10.884 1
25.512 -25.664 1
8.2291 8.0567 1
2.4123 27.88 1
-16.382 39.563 1
-41.302 -17.237 1
13.822 -32.67 1
12.563 -55.316 1
30.379 35.412 1
-15.032 -45.546 1
47.045 21.833 1
-4.7642 -1.6911 1
-11.937 -0.94413 1
-10.222 23.135 1
11.227 -53.912 1
-7.3779 -24.365 1
30.65 -8.3676 1
-7.3315 -8.5507 1
11.941 -29.365 1
-19.562 -10.593 1
21.815 -19.814 1
-27.605 10.29 1
-11.166 -48.695 1
24.632 -19.229 1
-21.83 -26.963 1
-7.906 -13.571 1
6.3361 -38.993 1
-8.1634 -10.854 1
21.901 -19.833 1
-0.42678 10.489 1
-4.5763 -4.1491 1
12.121 -30.797 1
-18.705 -27.954 1
3.4959 -4.5202 1
-44.201 26.709 1
-12.351 -4.3178 1
37.007 35.527 1
-12.746 -5.9473 1
-2.6896 -27.168 1
17.155 1.3293 1
19.17 -30.747 1
7.6267 -55.749 1
42.653 -16.519 1
-42.709 -42.46 1
-4.5828 -11.882 1
21.806 4.4384 1
-15.142 22.523 1
5.5856 -36.966 1
23.782 2.31 1
44.993 19.975 1
-0.1113 21.913 1
0.56128 22.824 1
-23.591 -11.837 1
3.475 5.9346 1
-4.4213 -29.41 1
-18.925 -23.067 1
-46.463 5.3879 1
36.91 35.523 1
-6.4374 -25.34 1
-35.684 -40.783 1
35.155 39.125 1
3.381 -11.812 1
0.6181 -15.273 1
19.407 -3.1402 1
-14.889 -48.212 1
-24.2 -9.1448 1
20.769 -2.2633 1
44.89 -22.53 1
-10.877 5.9012 1
28.855 -9.5152 1
-30.498 6.1226 1
-48.514 27.075 1
52.956 1.6753 1
-9.9438 -4.0155 1
18.731 1.5852 1
55.382 -0.087736 1
2.4353 -7.8021 1
44.878 16.65 1
-29.92 36.757 1
12.42 -8.1722 1
29.173 -16.285 1
-39.169 -19.781 1
13.269 -31.858 1
12.25 -23.746 1
40.847 -20.526 1
16.9 44.674 1
-1.5029 23.977 1
18.188 -32.933 1
52.661 -1.4522 1
-15.337 25.399 1
6.214 7.2814 1
-9.1424 -8.3916 1
-17.204 -10.653 1
-13.996 45.542 1
-9.7762 -29.104 1
5.655 16.435 1
40.852 -22.05 1
-0.79526 -2.3345 1
-10.183 22.999 1
24.058 2.905 1
-12.206 -3.5138 1
-37.954 -40.428 1
-0.82184 -30.685 1
3.9351 -39.338 1
12.021 -53.8 1
-45.371 -15.948 1
32.452 -43.117 1
55.992 -2.3156 1
-13.241 24.561 1
-4.667 -28.015 1
4.9936 11.265 1
-6.9842 -26.698 1
7.0448 -62.313 1
-40.242 4.1189 1
41.015 -17.734 1
21.312 -11.427 1
-37.562 4.6312 1
1.6167 22.767 1
16.25 41.362 1
9.2433 -60.257 1
17.217 -33.487 1
42.876 -20.021 1
-12.078 -45.331 1
6.3605 -5.6431 1
-11.149 -46.763 1
-21.87 -27.072 1
19.068 -21.119 1
-44.872 2.5561 1
0.611 -24.876 1
12.115 44.026 1
-1.0615 -4.7585 1
8.7046 42.375 1
-42.521 24.895 1
-32.734 9.439 1
25.582 -25.751 1
-48.544 24.572 1
40.498 17.662 1
-11.79 44.208 1
-31.019 7.8082 1
28.425 -12.632 1
6.4391 -5.8178 1
31.981 -46.223 1
1.892 14.19 1
-11.394 -5.9376 1
-31.334 35.835 1
18.114 22.206 1
8.0894 40.734 1
11.472 -2.2003 1
-6.0051 -15.05 1
32.204 -43.185 1
56.394 -3.4629 1
-32.217 8.2848 1
8.2819 -57.339 1
-22.47 -29.399 1
20.528 -4.0865 1
-10.022 -45.542 1
-35.936 -30.509 1
-22.107 -8.8151 1
-16.326 3.6903 1
-16.266 -10.006 1
7.8811 -41.241 1
-2.7281 -27.227 1
20.53 -0.53368 1
31.288 35.244 1
4.779 -38.897 1
20.728 4.1816 1
18.396 -11.841 1
30.081 -11.979 1
1.9614 11.296 1
18.94 11.238 1
-0.57088 -22.89 1
17.526 0.21141 1
-47.741 30.02 1
43.943 -18.258 1
-50.349 -1.8403 1
-30.46 9.2355 1
-1.7696 -20.339 1
-32.07 34.371 1
33.383 34.34 1
32.246 -45.171 1
41.319 -23.877 1
57.984 -1.7376 1
-10.966 23.207 1
40.908 16.907 1
-46.422 26.518 1
-2.069 8.4516 1
-2.3053 -20.01 1
47.508 16.952 1
2.5368 23.414 1
5.1566 -38.545 1
-26.744 13.917 1
-32.691 9.3912 1
2.2917 28.335 1
8.3822 -60.679 1
17.703 -4.3823 1
-11.98 41.792 1
-44.25 26.813 1
14.756 42.04 1
23.94 -0.049158 1
10.686 45.982 1
21.536 23.828 1
-24.94 -8.0611 1
27.221 5.7651 1
11.775 -33.114 1
7.979 -59.755 1
-11.508 -9.5412 1
14.185 -27.867 1
-1.4607 -19.975 1
-22.054 -25.481 1
24.453 -25.575 1
15.765 -0.6226 1
-3.0084 -29.843 1
5.7113 -37.942 1
14.098 20.431 1
-23.881 -9.724 1
0.71818 -15.247 1
-12.46 -48.614 1
-48.881 29.589 1
-41.497 4.8371 1
24.717 7.3344 1
-43.788 4.6495 1
5.0674 13.997 1
-44.14 28.485 1
-13.914 42.124 1
-31.795 34.672 1
19.268 -30.841 1
-20.056 -9.2712 1
-39.097 4.1445 1
-42.589 -14.738 1
-41.209 -41.113 1
-25.22 11.944 1
-21.318 -27.578 1
-18.792 -27.918 1
33.141 38.629 1
36.331 35.182 1
3.3372 16.801 1
26.145 1.5927 1
16.278 42.402 1
-7.6775 -27.024 1
-43.844 -21.809 1
15.525 19.401 1
-14.994 -46.527 1
-13.424 -3.5439 1
-14.598 23.26 1
2.1999 10.838 1
52.746 2.8278 1
8.2896 -60.679 1
10.563 -55.905 1
-13.353 42.059 1
1.7007 -9.7983 1
-32.452 37.933 1
18.123 20.05 1
-41.039 -41.418 1
-44.624 -17.084 1
0.5002 22.712 1
35.819 33.922 1
-29.645 33.395 1
-15.161 -47.668 1
-3.9119 -28.703 1
33.388 -43.732 1
-46.959 2.2873 1
-48.446 26.322 1
-49.186 27.436 1
-40.824 -17.908 1
-19.325 -29.399 1
-4.0848 -30.169 1
2.504 29.116 1
6.2536 -39.86 1
34.889 -42.356 1
-46.461 5.397 1
-11.066 47.313 1
-7.5122 -5.4548 1
29.355 -45.229 1
20.257 -15.288 1
-32.84 9.4344 1
41.077 -18.733 1
-0.7497 -10.253 1
-43.198 26.079 1
13.163 -56.333 1
43.217 19.945 1
60.009 -2.693 1
-24.322 -11.253 1
12.496 -57.587 1
-11.428 -9.6849 1
33.478 -41.933 1
-6.4523 -33.653 1
-12.782 6.7763 1
-6.0426 -6.4818 1
12.747 -56.335 1
-15.435 -48.529 1
-31.035 8.539 1
-0.094569 8.6858 1
-48.729 28.243 1
30.773 -45.233 1
-3.7736 7.2036 1
1.386 -15.812 1
-45.373 -14.999 1
14.218 40.845 1
24.131 -3.492 1
17.678 21.451 1
-27.48 34.93 1
11.403 -55.512 1
26.54 -24.387 1
-9.8141 19.492 1
25.304 -0.91347 1
7.1075 8.8442 1
-11.555 -5.8554 1
-14.41 43.441 1
14.689 -35.483 1
20.693 4.1979 1
34.665 35.81 1
13.773 40.054 1
33.535 -12.605 1
29.128 -11.386 1
-13.915 45.724 1
16.089 -34.679 1
33.008 33.437 1
14.666 -1.372 1
-34.945 4.9011 1
29.482 -11.04 1
-7.9248 -1.6846 1
47.037 21.947 1
12.243 -8.9176 1
-30.882 36.364 1
-9.7728 -29.116 1
-14.523 -48.595 1
26.729 -0.7293 1
-24.475 -27.622 1
10.909 -56.975 1
15.465 -27.68 1
20.529 -4.0813 1
48.29 21.585 1
-9.9152 19.84 1
-13.419 -49.055 1
35.515 38.987 1
12.337 41.537 1
56.631 -4.0017 1
-6.4541 -27.976 1
-29.116 33.534 1
12.106 -55.769 1
-1.105 -9.4378 1
26.267 -1.7149 1
-10.046 -0.074819 1
-41.556 -40.122 1
-47.604 -18.273 1
13.991 -7.3305 1
42.495 -21.109 1
-4.368 -13.785 1
-13.704 23.373 1
16.985 -30.108 1
-0.33857 20.831 1
16.874 -30.081 1
-25.061 12.57 1
-44.713 1.1332 1
-23.826 -24.939 1
-46.015 3.0964 1
-5.5619 -29.569 1
25.369 -0.89927 1
-47.256 -17.386 1
-2.5593 24.456 1
-4.6271 21.496 1
6.9802 15.678 1
18.055 5.3429 1
-19.514 -24.305 1
13.666 42.304 1
14.038 -7.2854 1
-17.565 -45.932 1
31.096 -10.512 1
-21.53 -12.709 1
25.512 -17.707 1
40.269 18.288 1
12.559 -60.994 1
26.038 1.3993 1
45.702 20.667 1
-41.462 -17.237 1
7.601 11.108 1
-5.3301 -26.087 1
-14.289 -43.699 1
-39.467 -38.306 1
-13.324 24.455 1
22.801 -18.196 1
-24.217 -5.8451 1
18.295 -34.344 1
-16.34 43.907 1
-7.24 -2.6668 1
-15.643 20.009 1
-10.408 42.727 1
18.428 23.417 1
-12.253 5.6457 1
19.03 42.338 1
-4.799 -6.9082 1
13.838 39.993 1
15.83 -27.95 1
14.407 46.083 1
-26.076 -11.151 1
19.935 -16.316 1
24.657 -20.238 1
-20.551 -27.66 1
-1.6339 9.0586 1
-32.426 35.206 1
44.202 -21.37 1
-30.384 9.2383 1
-47.253 27.307 1
35.266 38.871 1
-9.6997 23.258 1
-9.5756 19.954 1
9.419 -58.062 1
36.453 38.764 1
0.78068 21.421 1
-11.907 -48.163 1
57.169 1.6935 1
-47.72 27.227 1
17.111 1.2543 1
42.843 15.951 1
12.814 -56.601 1
43.755 -19.527 1
23.465 -17.83 1
0.3257 22.77 1
-3.3153 -7.2619 1
-23.764 -8.1352 1
16.159 -34.729 1
-20.993 -26.191 1
-39.95 -18.658 1
12.355 -9.4948 1
6.4636 -15.511 1
58.067 -3.263 1
-3.5699 -8.3041 1
15.162 -25.056 1
-15.273 43.062 1
11.741 42.659 1
20.655 1.8886 1
11.467 -2.2082 1
43.23 -23.454 1
-15.12 44.822 1
32.217 35.154 1
35.868 36.28 1
19.092 -21.11 1
10.75 -52.75 1
-9.7229 41.579 1
-34.914 4.3997 1
6.4757 -16.414 1
0.52883 -27.863 1
-7.5314 -5.4206 1
20.791 -1.7794 1
24.723 7.3917 1
-40.822 -40.565 1
-6.0025 -29.862 1
-41.466 -42.299 1
12.572 -57.634 1
33.704 33.704 1
19.949 18.309 1
36.494 -43.732 1
-45.812 24.002 1
-24.561 -27.648 1
59.203 -1.0413 1
4.5781 -22.663 1
-37.096 -37.988 1
25.513 -17.222 1
-14.433 44.337 1
17.472 43.806 1
8.7888 -9.5573 1
21.44 0.007779 1
43.244 -23.495 1
-40.079 -15.982 1
19.099 -21.109 1
20.26 23.586 1
23.499 3.8951 1
-26.925 10.225 1
-25.786 -12.565 1
10.992 -63.28 1
-14.344 44.974 1
5.6485 -37.009 1
17.816 -32.672 1
30.054 -11.987 1
-16.496 -3.6118 1
53.797 2.2987 1
-44.196 -17.817 1
-2.8982 -5.8037 1
19.114 1.8574 1
8.6987 -55.69 1
-10.763 23.468 1
16.705 19.775 1
26.918 -25.461 1
-24.305 -5.9297 1
4.3084 -8.4958 1
20.994 23.96 1
-13.983 -44.337 1
-2.5619 -14.187 1
44.235 -18.528 1
-11.282 45.352 1
-11.718 0.11214 1
34.433 37.966 1
-12.433 23.144 1
7.6682 -55.757 1
9.4958 -61.501 1
-13.002 44.163 1
46.411 16.935 1
9.4727 40.572 1
-28.553 9.3571 1
16.765 -32.21 1
-40.12 -14.116 1
11.004 -63.201 1
-38.026 -39.143 1
26.213 -18.861 1
45.419 21.058 1
12.471 -53.735 1
34.346 34.118 1
-15.795 23.095 1
9.4995 -61.407 1
42.059 -22.391 1
-45.78 25.251 1
31.608 -45.93 1
-5.4254 -5.5611 1
40.625 17.718 1
-13.558 21.538 1
33.116 -12.203 1
5.6752 -9.2166 1
27.383 5.6304 1
11.449 -32.936 1
57.259 4.1398 1
13.092 -33.486 1
32.334 -43.317 1
60.016 -2.6734 1
-10.349 18.806 1
-46.094 -16.633 1
5.9236 -13.15 1
-14.974 -48.858 1
-45.147 28.659 1
25.415 8.5827 1
-36.05 -36.566 1
8.1795 -19.966 1
-45.096 25.106 1
-2.9093 -29.767 1
18.078 20.777 1
-45.45 -16.565 1
53.907 -2.1932 1
-15.806 2.6508 1
-23.998 -11.198 1
-15.673 38.401 1
-42.9 1.3234 1
48.249 21.551 1
42.424 -21.469 1
-41.816 -19.262 1
-9.0357 42.549 1
13.974 -4.0152 1
13.196 46.538 1
15.656 46.029 1
3.419 -25.38 1
47.711 18.597 1
7.4402 -59.631 1
40.532 -21.98 1
14.632 43.168 1
-15.799 -45.895 1
8.0101 40.747 1
5.1012 13.999 1
-14.281 41.731 1
24.14 -17.673 1
24.425 4.1316 1
27.102 -7.876 1
9.1864 -54.831 1
6.9685 15.671 1
18.619 21.85 1
-16.292 -10.534 1
-27.34 33.93 1
-23.014 -10.491 1
25.461 14.035 1
-22.459 -27.862 1
-50.358 -1.8778 1
-34.847 40.682 1
35.951 36.337 1
-7.4937 -5.466 1
0.50377 24.189 1
10.326 -10.645 1
18.53 10.527 1
-40.143 -14.056 1
-42.761 -43.267 1
-11.064 18.735 1
-38.224 -39.368 1
45.404 -20.127 1
-9.5608 -29.253 1
-42.566 -40.884 1
8.8731 -10.689 1
54.509 -1.1561 1
-2.2371 24.122 1
-21.01 -27.941 1
-39.385 -41.982 1
-11.973 23.553 1
16.28 41.686 1
-20.681 -26.54 1
19.247 -1.3121 1
-0.77034 23.592 1
7.8146 12.385 1
-26.812 34.941 1
32.644 -49.413 1
-16.073 -48.546 1
53.729 -2.9863 1
-29.11 39.094 1
-44.957 0.93061 1
45.336 19.625 1
12.767 -11.778 1
41.923 16.827 1
44.174 18.896 1
-40.973 -41.361 1
-42.322 -18.053 1
-11.901 -0.79093 1
31.858 37.413 1
-16.463 -3.6174 1
16.865 44.624 1
23.543 3.95 1
-4.7748 -1.6087 1
22.411 22.828 1
-20.833 -28.787 1
-28.873 36.066 1
-21.026 -11.505 1
3.8386 -10.77 1
-37.125 -43.544 1
47.784 18.683 1
15.979 -32.015 1
-18.509 -10.758 1
33.311 -45.209 1
5.2559 16.564 1
8.6592 -55.83 1
52.968 0.26686 1
-48.141 -1.2013 1
28.869 -9.6563 1
12.731 -1.3276 1
-1.4912 -21.458 1
14.018 42.803 1
13.36 -10.49 1
2.5487 27.887 1
26.795 -25.282 1
33.137 -45.847 1
3.851 -10.695 1
23.596 5.2517 1
-42.724 -14.768 1
-11.124 -8.5436 1
-43.716 4.5212 1
-7.0178 -31.779 1
24.04 2.9037 1
-8.79 5.9812 1
-17.732 -25.677 1
-14.363 -48.624 1
6.7267 2.5729 1
24.926 -23.005 1
-31.203 35.887 1
16.081 -35.291 1
-3.031 -29.811 1
19.035 42.32 1
-0.31198 2.3883 1
-13.267 -47.327 1
59.929 0.54112 1
-0.56802 -22.917 1
6.8107 2.6269 1
-39.317 -17.9 1
3.2367 -27.73 1
-6.781 -9.321 1
-10.675 4.5166 1
-47.526 24.28 1
5.8918 -13.138 1
-27.243 14.246 1
-27.196 37.283 1
-31.863 10.48 1
-32.371 41.199 1
-14.023 25.468 1
12.247 -23.747 1
0.68197 24.711 1
24.73 7.3869 1
32.402 32.981 1
6.7334 -60.462 1
-10.537 -8.3132 1
24.918 -24.839 1
-42.061 27.091 1
-34.914 4.9333 1
18.746 22.594 1
-7.1424 -31.31 1
-36.83 -38.021 1
0.33719 1.0647 1
34.241 -12.738 1
-31.698 38.108 1
-43.964 -16.134 1
2.8241 11.12 1
-44.944 26.006 1
-13.763 45.429 1
-14.679 1.6137 1
16.612 44.878 1
10.933 -63.233 1
-48.083 26.275 1
10.9 -56.234 1
-44.846 1.3199 1
-24.64 -13.074 1
0.96357 12.388 1
12.565 45.694 1
-15.207 -47.884 1
12.483 -54.436 1
15.466 19.603 1
14.311 -30.396 1
0.8226 20.484 1
32.053 -9.4948 1
-48.309 27.741 1
-1.931 22.487 1
22.587 4.3894 1
4.9867 11.167 1
-2.9732 -27.57 1
-11.44 21.033 1
4.5848 11.015 1
29.974 -11.67 1
43.647 17.125 1
-37.552 38.166 1
12.41 42.986 1
16.953 -30.123 1
-27.715 34.233 1
-14.779 -49.629 1
28.181 8.0478 1
-26.136 -7.7979 1
-42.511 -14.772 1
7.3592 -11.756 1
6.7326 2.5853 1
-43.714 26.453 1
6.1004 -41.178 1
13.632 40.53 1
-8.0676 -32.899 1
57.756 3.5759 1
26.794 -0.39104 1
-49.04 -3.1793 1
53.977 -2.0302 1
-22.816 -10.6 1
2.5302 3.1412 1
-1.4027 -4.8367 1
-48.17 25.237 1
5.9908 -25.849 1
28.988 -11.441 1
-37.376 38.547 1
-41.243 -39.414 1
8.2985 -11.641 1
-34.56 -27.844 1
-33.375 38.246 1
18.48 -15.491 1
-11.377 -5.8568 1
-44.84 1.088 1
57.743 3.5712 1
22.269 3.4105 1
6.8751 9.8238 1
-40.433 -38.191 1
-36.063 -36.564 1
-31.952 39.333 1
36.512 33.663 1
-35.165 37.767 1
56.665 -4.1495 1
24.93 -9.0544 1
2.892 28.529 1
9.269 -58.277 1
18.402 -2.4337 1
-7.7135 -1.0849 1
-41.992 -39.041 1
-11.859 44.161 1
-46.6 30.022 1
2.6683 21.158 1
3.0481 5.7455 1
16.685 23.765 1
-47.371 27.417 1
-24.109 -9.1128 1
4.3054 -8.4986 1
26.018 -17.541 1
59.597 -4.2008 1
-10.039 42.954 1
55.008 -1.4194 1
-6.3561 -15.126 1
44.825 -23.014 1
25.586 -24.547 1
-6.7851 -28.243 1
14.605 -1.14 1
-20.624 -24.705 1
26.076 -24.679 1
-42.379 -42.98 1
14.231 -59.606 1
30.537 -9.8338 1
36.063 35.078 1
-37.648 -39.558 1
-26.168 14.057 1
32.677 -44.673 1
12.835 1.9634 1
-9.8545 -8.9893 1
-9.9933 -45.639 1
26.576 1.1416 1
0.34093 1.0659 1
28.744 -8.6045 1
5.6218 -2.929 1
55.387 -0.079178 1
-6.0057 -15.09 1
30.926 33.283 1
-14.934 24.568 1
-5.1585 -3.6687 1
12.506 -57.143 1
45.299 -20.124 1
16.131 40.664 1
-7.3132 21.504 1
10.914 -55.796 1
8.1847 -41.409 1
-45.982 24.645 1
-29.612 37.905 1
-43.85 0.95596 1
12.3 -56.273 1
21.429 23.45 1
-47.208 28.52 1
7.1833 8.3535 1
-45.492 29.666 1
26.787 -7.1319 1
-11.635 42.526 1
2.9471 10.936 1
4.9758 -38.983 1
-43.297 -17.525 1
59.179 -1.0852 1
-39.544 -42.085 1
-44.675 2.2051 1
-48.686 28.189 1
-44.387 -14.576 1
55.954 -3.096 1
-19.923 -26.438 1
44.353 18.917 1
-9.8466 20.345 1
43.463 -19.521 1
-44.793 0.63194 1
45.284 19.957 1
-17.302 -10.697 1
4.8805 9.3604 1
-19.641 -27.707 1
11.217 46.062 1
6.711 -40.841 1
12.265 -23.802 1
7.0247 -62.334 1
-28.7 36.907 1
-4.8837 -25.282 1
17.564 20.734 1
-16.051 2.5811 1
3.4312 -4.6762 1
47.209 20.161 1
-4.031 21.669 1
-35.395 4.8833 1
-10.021 42.401 1
-24.535 -27.637 1
-45.34 29.85 1
-29.051 11.313 1
-3.8051 7.2004 1
-13.61 5.6269 1
-33.556 37.487 1
44.846 16.592 1
14.877 23.659 1
-8.5238 -15.015 1
-46.509 30.51 1
7.8154 14.661 1
-0.25194 10.155 1
5.1733 -31.942 1
30.182 -43.404 1
-42.519 -15.883 1
8.4983 -39.572 1
11.253 -53.174 1
-12.262 7.0535 1
31.901 -45.574 1
-42.605 -17.805 1
-4.5112 -19.17 1
-42.555 -42.739 1
44.169 -21.332 1
57.262 -3.3431 1
-19.65 -26.319 1
43.4 -24.307 1
-27.148 -10.681 1
5.363 -12.303 1
-11.301 21.678 1
46.718 20.481 1
10.076 -9.0427 1
-8.304 44.966 1
41.117 19.973 1
24.673 -18.75 1
-25.445 12.051 1
-33.125 10.537 1
12.318 42.913 1
-3.4888 -8.1375 1
5.7925 -38.335 1
-27.112 37.148 1
57.832 -1.7534 1
-40.493 -38.74 1
31.734 -48.22 1
-0.26371 2.1373 1
-16.456 -49.393 1
1.761 -18.568 1
32.423 -43.208 1
-29.013 12.235 1
26.205 -20.002 1
-21.493 -12.706 1
55.456 -1.6709 1
-6.806 0.0014181 1
-3.0606 -27.652 1
31.264 -43.086 1
6.7241 -36.835 1
-3.4938 -21.593 1
-36.232 -41.208 1
-17.053 -46.432 1
-40.418 -43.15 1
-47.633 27.023 1
-0.65816 23.716 1
-1.1572 15.916 1
-7.9529 -1.728 1
-4.6204 -6.9129 1
18.43 -14.307 1
-12.323 7.0904 1
12.764 -1.3037 1
-16.427 -10.893 1
-37.851 -17.159 1
33.905 -44.201 1
3.2144 29.541 1
-21.591 -11.459 1
-31.846 10.469 1
-12.154 4.2751 1
17.512 20.581 1
11.765 43.029 1
0.61263 -14.87 1
-12.153 18.387 1
-31.242 37.688 1
8.1667 -19.983 1
4.5969 -22.66 1
-10.854 -44.224 1
-42.582 -12.611 1
26.066 -18.048 1
46.805 17.885 1
-35.265 4.6085 1
-14.965 23.107 1
-14.92 -46.546 1
-22.468 -29.491 1
-32.537 37.978 1
-35.348 4.9532 1
32.605 34.828 1
-29.264 39.172 1
44.743 16.584 1
-25.012 -11.271 1
11.907 41.755 1
20.757 22.823 1
-41.483 -42.219 1
-5.0426 -28.211 1
2.7506 11.242 1
8.9475 -6.5085 1
29.98 -9.7816 1
-27.175 14.224 1
1.0985 -26.587 1
-39.911 -18.541 1
11.772 -54.39 1
9.951 -60.154 1
-19.239 -25.803 1
-36.2 -36.726 1
45.5 20.61 1
-41.729 27.95 1
14.444 -15.982 1
26.199 -18.454 1
20.382 -14.837 1
-4.5161 -19.177 1
-19.68 -27.655 1
-4.5153 -19.173 1
57.645 -3.138 1
-17.529 -10.851 1
8.6698 -55.816 1
4.0124 6.3999 1
-7.2751 -27.594 1
-8.087 -32.885 1
-1.7388 -24.895 1
-27.77 -11.815 1
11.506 -13.058 1
-25.34 12.595 1
3.4214 -25.37 1
31.57 -43.605 1
48.773 19.144 1
23.783 2.1661 1
-46.075 28.314 1
-8.7702 38.838 1
6.4776 -16.352 1
10.467 -55.922 1
-18.746 -29.001 1
11.446 -18.915 1
-14.357 -43.629 1
-39.121 -41.392 1
26.221 -17.463 1
5.2587 -12.194 1
-7.87 -13.665 1
44.502 -20.199 1
9.7816 -57.959 1
12.714 -1.3159 1
-12.437 23.337 1
3.252 29.584 1
19.28 -1.3941 1
15.595 -33.128 1
4.8745 9.3296 1
20.694 21.365 1
3.3727 -30.168 1
-45.032 0.82822 1
-9.4837 -1.9979 1
-12.529 -48.611 1
4.6596 -22.549 1
14.215 41.777 1
14.095 -33.477 1
32.873 38.753 1
-22.542 -29.4 1
26.992 1.5976 1
-45.12 24.972 1
17.305 -5.9265 1
-13.25 -47.312 1
7.816 10.079 1
-9.2068 45.174 1
-10.968 -44.047 1
32.569 -47.103 1
-16.164 40.956 1
31.936 -48.6 1
30.805 -9.2068 1
26.155 -0.9025 1
19.055 1.8478 1
-13.008 42.579 1
-12.087 24.208 1
-12.663 -43.766 1
5.2795 -39.646 1
-41.782 5.0195 1
23.496 4.7611 1
35.831 36.456 1
40.671 17.628 1
-6.2793 -23.903 1
4.6769 -36.98 1
33.363 35.614 1
12.354 -9.6063 1
-2.4127 -19.913 1
-4.8303 -14.936 1
-11.968 -5.6683 1
-39.668 -44.389 1
14.277 41.776 1
23.59 5.1394 1
30.838 -48.028 1
13.649 39.989 1
23.888 -3.3515 1
-32.353 41.216 1
16.129 -32.105 1
-49.626 -1.6536 1
6.7308 2.591 1
54.411 2.474 1
-12.11 18.641 1
53.786 2.3237 1
-42.225 3.1037 1
-5.8283 -15.028 1
2.9172 24.731 1
24.817 -17.085 1
-13.187 2.16 1
-28.676 36.067 1
17.383 0.20464 1
-41.455 -42.174 1
14.625 -1.0568 1
22.776 -25.028 1
-43.628 27.036 1
-48.848 -3.6383 1
44 20.375 1
25.78 -15.549 1
30.531 -11.557 1
-44.936 -0.23951 1
0.46005 -15.123 1
-12.169 -8.8024 1
12.608 41.437 1
-12.364 -4.3203 1
18.455 -33.046 1
-37.489 38.221 1
13.913 -7.369 1
-0.69236 -30.642 1
-12.164 5.6518 1
-11.057 44.93 1
-27.477 -11.255 1
-7.694 -31.734 1
-4.8132 -1.4002 1
6.5089 10.44 1
21.699 -19.745 1
-2.8293 -5.971 1
25.121 -25.565 1
-10.008 20.328 1
-16.334 -44.932 1
-3.5846 -15.312 1
10.082 -9.044 1
27.309 5.6894 1
-11.246 -48.656 1
30.887 33.209 1
-33.087 5.2586 1
6.4765 -16.31 1
4.9963 11.251 1
-1.4254 -4.8477 1
14.361 -30.351 1
-10.724 4.2872 1
-19.825 -24.579 1
-0.67359 -28.747 1
7.0149 15.669 1
-37.822 -17.172 1
-40.05 -41.231 1
45.894 18.302 1
-15.892 4.4818 1
16.722 -32.131 1
-42.589 -12.629 1
18.457 22.39 1
56.689 0.94639 1
-28.807 36.155 1
-34.274 40.092 1
58.316 -6.0163 1
-26.977 -12.878 1
19.328 23.557 1
-15.348 25.471 1
-19.163 -26.739 1
32.787 36.55 1
-26.312 -13.076 1
42.474 -21.197 1
-29.282 34.923 1
7.8327 12.419 1
-3.2749 -13.412 1
7.2065 -61.284 1
-7.8476 -10.87 1
53.884 2.3257 1
30.798 -44.68 1
34.467 31.924 1
12.807 1.9584 1
-41.344 -42.148 1
10.544 42.456 1
42.871 20.006 1
-13.278 3.8015 1
-43.311 -15.804 1
11.358 42.459 1
-29.81 35.4 1
24.545 -8.0896 1
-30.363 38.429 1
-22.07 -25.658 1
-11.479 45.313 1
-10.48 41.508 1
-3.7827 7.2003 1
31.565 -9.2037 1
18.526 22.503 1
-28.387 33.997 1
-45.009 3.1957 1
7.2059 8.2152 1
52.738 2.8848 1
-46.095 1.301 1
13.503 40.646 1
12.545 -4.7875 1
26.001 -17.643 1
-4.6027 41.391 1
-22.616 -10.368 1
9.4564 -61.474 1
-28.403 35.32 1
20.75 1.7499 1
20.683 21.344 1
43.191 19.121 1
-12.64 -7.4527 1
-23.448 -10.354 1
-20.64 -24.741 1
-48.663 30.795 1
48.752 20.322 1
25.521 -25.486 1
29.093 -9.5474 1
12.084 -55.911 1
12.724 -1.7932 1
-11.298 -1.7162 1
27.772 -9.3839 1
-17.395 41.866 1
19.976 -16.51 1
-44.787 -18.893 1
17.092 20.666 1
43.592 -22.375 1
10.523 -58.926 1
44.711 -24.327 1
3.2906 29.068 1
3.266 29.663 1
32.068 -8.6111 1
0.85657 22.875 1
-37.85 -17.182 1
-14.832 21.645 1
-15.24 44.856 1
42.68 -16.512 1
-31.89 34.342 1
-11.815 -46.645 1
-36.085 -38.466 1
47.156 20.968 1
6.6172 -7.6178 1
10.581 -57.49 1
5.8986 -13.152 1
-13.747 2.1668 1
-39.031 -39.463 1
2.5546 29.118 1
-1.2579 -19.929 1
11.719 43.386 1
-12.391 23.419 1
-12.096 -45.514 1
23.419 4.2013 1
37.476 -44.424 1
-3.6474 -15.246 1
-13.347 24.967 1
-41.147 4.4283 1
42.214 -19.219 1
19.345 -1.3149 1
-4.1313 -6.5913 1
-6.7409 -9.3474 1
26.258 -19.945 1
35.731 37.263 1
-27.657 -13.291 1
58.318 -6.0371 1
42.979 21.095 1
-10.994 -47.991 1
14.728 -35.368 1
0.73794 7.6911 1
-25.152 -11.258 1
16.093 -35.273 1
-38.175 37.795 1
-21.362 -23.966 1
32.576 -43.039 1
-46.346 2.3512 1
29.459 -11.099 1
-41.725 -18.149 1
-23.153 -27.031 1
-17.168 -10.656 1
44.29 17.685 1
29.312 -45.266 1
-13.079 23.994 1
55.349 -0.072883 1
6.1264 -39.806 1
17.357 -33.375 1
-9.3304 43.371 1
27.113 1.6249 1
-7.5096 -5.3705 1
11.248 9.4741 1
-42.616 -19.56 1
-29.504 37.352 1
-43.716 -15.569 1
20.922 22.961 1
26.84 -6.2644 1
-14.313 -46.858 1
-17.52 -47.596 1
42.809 20.285 1
-0.43717 10.458 1
25.738 -15.607 1
43.415 18.935 1
11.941 -29.378 1
42.274 -22.837 1
-7.5054 -5.4522 1
3.6607 -4.0622 1
-13.077 2.1674 1
43.279 -22.314 1
54.32 -4.78 1
26.908 -1.0484 1
17.624 -17.115 1
0.67807 -19.725 1
-12.087 46.275 1
6.2332 7.2556 1
24.823 -19.065 1
42.642 19.382 1
-14.149 -45.33 1
-2.5895 24.527 1
23.871 2.0531 1
-44.174 28.521 1
14.055 46.149 1
-14.45 2.6446 1
16.637 44.865 1
-32.409 35.245 1
-21.315 -23.856 1
46.972 21.894 1
24.756 -18.681 1
14.11 -33.972 1
-23.769 -24.958 1
13.368 4.0877 1
1.2357 -12.281 1
-16.697 4.2074 1
0.22181 1.7303 1
31.132 -10.603 1
-28.945 10.801 1
-29.106 11.316 1
19.88 18.435 1
37.783 -44.429 1
-11.077 1.7542 1
-35.52 -39.871 1
1.7391 -9.8176 1
15.56 -33.638 1
-21.847 -8.3792 1
0.299 1.1191 1
35.34 35.253 1
31.661 -43.519 1
7.9874 -59.183 1
-0.72698 -28.804 1
22.744 -2.6509 1
-12.703 -43.743 1
55.951 -3.0907 1
-37.472 38.205 1
-2.5799 -14.165 1
17.413 0.33444 1
-10.685 47.366 1
-27.524 -11.169 1
-38.643 -41.921 1
16.587 23.793 1
-14.559 3.1719 1
-17.241 -46.158 1
-4.5901 41.397 1
19.108 -2.032 1
-39.641 -40.156 1
13.735 21.047 1
-39.4 -17.953 1
-43.758 -16.174 1
-46.062 3.0337 1
6.7399 2.5893 1
11.771 46.489 1
16.143 -34.699 1
-5.5914 1.5723 1
52.544 -1.6907 1
-13.179 21.404 1
7.1219 14.955 1
-40.793 -18.034 1
-24.145 -9.1681 1
-28.964 39.143 1
34.351 36.145 1
-47.982 30.848 1
58.547 -2.7835 1
-0.933 6.2369 1
-22.269 -9.9178 1
8.441 -58.492 1
-21.32 -24.073 1
19.239 23.47 1
-46.127 28.5 1
-1.7908 -25.078 1
-1.6159 23.819 1
26.914 -19.559 1
19.186 24.714 1
11.526 -12.816 1
0.75934 25.08 1
-29.163 36.383 1
-40.422 -18.226 1
5.18 -31.959 1
32.63 -49.6 1
2.1238 23.359 1
44.726 -22.506 1
-10.096 -9.3826 1
-15.906 4.3723 1
11.651 -55.088 1
29.788 -9.0437 1
32.559 31.501 1
-31.071 32.888 1
-37.157 -43.521 1
-9.927 -5.5199 1
-16.238 -9.8973 1
20.242 22.755 1
47.144 20.068 1
-14.053 -48.307 1
0.62592 -27.921 1
-43.734 -21.751 1
7.7638 15.541 1
-49.002 -3.2037 1
5.6497 16.437 1
31.654 -45.683 1
16.779 -6.7107 1
-43.37 3.3095 1
11.077 -5.988 1
2.5468 3.1435 1
4.6047 6.8886 1
2.1168 27.993 1
32.267 34.083 1
-2.0542 8.452 1
-7.3662 -14.704 1
-12.696 -43.755 1
25.768 -25.958 1
-8.1945 -32.859 1
44.095 -20.298 1
15.786 -0.6649 1
2.8587 10.908 1
-34.298 40.099 1
-17.2 -46.164 1
-9.9592 44.041 1
-1.8998 22.53 1
23.225 16.488 1
25.427 -24.943 1
27.272 5.6793 1
-29.655 35.671 1
14.7 40.588 1
-16.05 38.731 1
-37.66 -37.451 1
-30.92 37.552 1
13.627 -32.109 1
-10.757 42.882 1
-43.72 -14.601 1
-9.9235 -5.5179 1
-17.633 -47.04 1
-13.738 -3.9846 1
-44.24 -18.391 1
-43.507 -0.095254 1
-41.074 -42.9 1
0.90717 12.435 1
36.708 -44.548 1
25.632 -6.5684 1
8.9463 -6.4616 1
23.488 3.2252 1
-2.3282 -7.8915 1
-9.8453 -1.8435 1
-26.173 13.955 1
-34.785 4.7342 1
30.647 -9.8691 1
11.93 46.397 1
-23.561 -26.721 1
-37.474 38.225 1
-46.521 30.577 1
59.021 -0.48683 1
1.1388 -26.625 1
14.065 -56.002 1
-32.752 9.4767 1
-15.137 -47.635 1
7.2634 8.3906 1
29.326 -8.1665 1
-2.8578 -12.322 1
3.0244 24.806 1
-15.234 45.994 1
-28.21 11.069 1
-0.17196 22.629 1
11.404 40.901 1
4.0289 -9.9598 1
5.1758 -39.581 1
42.335 -16.087 1
7.533 -10.232 1
25.626 -20.386 1
21.214 24.588 1
19.218 24.735 1
-40.257 -42.202 1
-49.638 26.347 1
20.998 1.3096 1
-10.552 42.321 1
21.911 -17.814 1
-6.3928 -27.771 1
-10.85 5.9052 1
-22.395 -27.941 1
20.188 -16.726 1
11.552 42.456 1
13.859 -2.6675 1
45.161 17.857 1
-8.1724 3.3572 1
52.232 0.77411 1
15.176 -25.05 1
33.298 34.507 1
52.213 0.79039 1
-43.975 -15.244 1
11.538 44.686 1
-3.4245 -7.3641 1
42.557 20.851 1


==> data_pada_1.tex <==
x y label
32 28 2
-5 30 8
25 17 3
-42 -16 6
31 32 2
5 -44 2
-40 -15 6
-13 -46 1
21 -38 9
-30 45 5
6 -50 2
11 -32 7
33 29 2
-30 44 5
-42 -16 6
33 -24 0
7 -44 2
44 13 4
-6 0 2
-1 -9 9
-30 44 5
24 -43 9
34 33 2
-28 39 5
-40 -18 6
24 14 8
47 11 4
35 -23 0
-30 48 5
-28 43 5
-5 29 8
10 -27 7
-26 40 5
10 -30 7
24 15 3
-29 44 5
11 -32 7
-8 33 8
45 10 4
5 -49 2
15 -24 7
23 15 8
-38 -10 9
-16 -47 1
28 17 3
-16 -41 1
-41 -15 6
-40 -16 6
44 12 4
-8 30 8
-9 33 8
-11 8 6
-7 33 8
27 15 3
34 34 2
-41 -12 6
-42 -15 6
11 -30 7
24 16 3
26 -43 9
14 -27 7
25 15 3
-42 -13 6
-27 44 5
5 -48 2
5 -49 2
-41 -15 6
-29 44 5
24 16 3
13 -30 7
-28 40 5
-1 0 1
-26 43 5
-2 -1 0
-41 -18 6
37 -28 0
37 -27 0
33 31 2
-27 42 5
-1 1 0
12 -32 7
38 -25 0
36 -27 0
-42 -18 6
32 29 2
-41 -17 6
-3 32 8
11 -32 7
2 -48 9
22 19 3
33 -24 0
-15 -44 1
-32 12 4
36 -24 0
-7 34 8
25 -39 9
24 -39 9
35 -22 0
11 -29 7
32 29 2
47 11 4
2 -50 9
41 11 4
47 11 4
27 14 3
35 -27 0
-39 -17 6
35 -23 0
13 -32 7
24 16 3
-38 -18 5
34 30 2
-2 2 4
-43 -17 6
-41 -16 6
-28 40 5
-42 -16 6
24 17 3
22 -39 9
35 -23 0
10 -30 7
-14 -48 1
-7 35 8
36 -24 0
-27 42 5
11 -25 7
-7 33 8
-41 -16 6
-3 3 1
48 13 4
-45 -17 6
-38 -15 6
-29 46 5
12 -27 7
23 -40 9
5 -48 2
10 2 9
37 34 2
13 -28 7
46 11 4
-1 0 7
6 -46 2
-16 -45 1
36 35 2
-13 -47 1
-8 34 8
38 -25 0
36 35 2
25 16 3
9 -32 7
-3 32 8
34 -22 0
34 -22 0
20 -44 9
23 16 3
6 0 9
24 -40 9
36 -27 0
11 -30 7
23 17 3
-7 33 8
-42 -15 6
37 -27 0
22 -41 9
49 10 4
25 -43 9
36 -27 0
-42 -13 6
47 9 4
50 10 4
26 14 3
46 11 4
-43 -15 6
13 -30 7
-15 -43 1
-51 1 6
-44 -15 6
-38 -15 6
33 33 2
27 17 3
-13 -46 1
27 18 3
28 17 3
-13 -46 1
33 32 2
-40 -16 6
35 -24 0
26 20 3
5 -48 2
10 -33 7
21 17 8
11 -30 7
11 -32 7
-8 35 8
12 -33 7
-14 -47 1
-23 -30 6
6 0 9
44 12 4
33 -22 0
-15 -48 1
49 10 4
-13 -44 1
7 -44 2
-39 -15 6
24 -43 9
23 14 3
44 13 4
-17 9 6
-18 -45 1
43 11 4
-41 -16 6
35 -24 0
-30 44 5
-45 -15 6
-8 35 8
-16 -19 9
-5 30 8
-28 40 5
-6 34 8
42 11 4
37 34 2
24 16 3
-25 -1 6
32 32 2
-9 31 8
27 15 3
20 -42 9
36 -27 0
44 13 4
-13 -47 1
37 -25 0
4 0 9
34 -23 0
-18 -45 1
45 10 4
-15 -43 1
24 16 3
44 10 4
-43 -17 6
-28 44 5
-15 -10 4
-2 -1 7
-30 47 5
-38 -10 6
35 32 2
-28 39 4
23 16 3
-6 34 8
11 -33 7
10 -30 7
3 -49 2
21 17 8
13 -32 7
-2 -2 7
24 -43 9
46 10 4
25 18 3
-15 -16 5
-16 -46 1
22 -41 9
-40 -15 6
13 -25 7
37 34 2
-49 -1 9
2 -50 9
33 29 2
6 -1 9
32 29 4
-27 41 5
-43 -17 6
-27 46 5
-43 -17 6
-27 44 5
-16 -19 9
-40 -15 6
-7 35 8
26 15 3
-6 33 8
-27 39 6
-43 -15 6
37 -23 0
-27 44 5
21 -37 9
-4 3 8
-29 40 5
-27 44 5
-29 41 5
20 17 8
26 16 3
-15 -42 1
-41 -16 6
-6 4 5
36 -11 0
44 11 4
11 -31 7
-7 32 8
-8 34 8
-5 35 8
22 -40 9
33 -22 0
26 -44 9
33 31 2
24 -39 9
-16 -44 1
45 14 4
35 -25 0
-14 -47 1
11 -31 7
-27 45 5
22 -40 9
13 -27 7
14 -31 7
25 16 3
12 -31 7
38 -27 0
12 -26 7
-39 -13 6
-27 41 5
-5 35 8
-31 45 5
25 16 3
11 -26 7
33 30 2
33 32 2
-31 46 5
38 -27 0
-3 32 8
-8 36 8
-7 34 8
-27 42 5
23 -42 9
-7 36 8
34 34 2
47 8 4
33 -25 0
13 -27 7
-15 -44 1
35 -24 0
38 -26 0
21 -39 9
34 29 2
-10 31 8
26 18 3
-16 -45 1
24 19 3
27 17 3
25 16 3
-38 -13 6
-29 46 5
23 -42 9
36 33 2
-5 33 8
35 33 2
33 -26 0
20 -39 9
-43 -19 6
25 15 3
24 -42 9
-8 32 8
26 18 3
-17 -46 1
-27 42 5
22 14 3
24 13 3
36 36 2
-5 -3 9
34 -27 0
48 10 4
-4 3 6
-40 -14 6
-13 -46 1
-45 -15 6
-31 44 5
34 -24 0
-39 -15 6
46 12 4
-43 -14 6
41 14 4
-26 41 5
11 -28 7
-5 30 8
-28 40 5
26 15 3
26 -41 9
35 34 2
-14 -47 1
13 -31 7
-17 -44 1
36 -26 0
9 -31 7
-29 46 5
22 -40 9
-6 31 8
-29 43 5
48 10 4
24 18 3
-7 35 8
34 31 2
-31 46 5
12 -26 7
12 -26 7
34 32 2
11 -29 7
36 -24 0
-28 41 5
-11 32 8
-40 -13 6
44 10 4
47 12 4
45 14 4
-31 42 5
-28 41 5
-29 42 5
-39 -13 6
-7 32 8
37 34 2
-17 -3 1
33 32 2
-40 -14 6
45 13 4
-17 -43 1
-7 8 3
-14 -46 1
14 -28 7
46 9 4
-6 34 8
46 13 4
-37 -13 6
-6 33 8
-38 -14 6
-3 33 8
-8 31 8
-43 -18 6
21 -39 9
-16 -43 1
12 -28 7
23 -43 9
-14 -43 1
11 -26 7
-13 -47 1
34 32 2
33 31 2
32 -22 0
24 -44 9
-29 43 5
32 31 2
-14 -47 1
-9 36 8
-9 30 8
-29 43 5
23 -40 9
35 33 2
25 -40 9
34 -22 0
-30 44 5
25 -41 9
14 -30 7
-28 40 5
20 -43 9
27 17 3
-8 32 8
35 -23 0
24 -43 9
-40 -14 6
34 -25 0
44 11 4
37 -26 0
-17 -42 1
10 -32 7
47 8 4
-29 42 5
11 -32 7
34 32 2
-16 -49 1
38 -27 0
44 9 4
-15 -47 1
-5 35 8
23 -38 9
22 -42 9
37 -24 0
36 33 2
26 18 3
-6 31 8
37 -23 0
-17 -43 1
45 12 4
-14 -46 1
47 12 4
-31 46 5
-8 31 8
-8 32 8
44 13 4
11 -27 7
-29 42 5
-5 34 8
-29 42 5
13 -28 7
-28 41 5
49 13 4
23 -40 9
-31 46 5
22 -38 9
35 -23 0
-30 45 5
26 -42 9
-25 39 5
28 18 3
26 18 3
37 34 2
25 -43 9
26 18 3
-17 -43 1
48 11 4
-15 -46 1
-43 -13 6
-7 34 8
-15 -45 1
50 10 4
-8 36 8
-25 42 5
-4 35 8
13 -28 7
49 10 4
10 -28 7
10 -32 7
-5 33 8
-5 35 8
33 32 2
22 -39 9
49 10 4
22 -40 9
-13 -11 9
-17 -45 1
35 35 2
21 -41 9
46 10 4
-13 -45 1
45 10 4
35 -24 0
-30 42 5
-36 -13 6
35 -23 0
37 34 2
21 -41 9
-7 33 8
37 34 2
35 33 2
-29 46 5
25 -40 9
27 17 3
-45 -17 6
-14 -47 1
-15 -45 1
36 -25 0
26 14 3
-6 36 8
10 -31 7
25 17 3
-5 36 8
-43 -14 6
-28 42 5
36 -28 0
24 17 3
12 -25 7
35 36 2
-43 -14 6
-12 5 3
11 -32 7
-8 10 8
34 32 2
44 13 4
22 -42 9
34 35 2
-7 33 8
25 18 3
-30 44 5
32 -24 0
37 32 2
-44 -12 6
22 14 3
27 17 3
-44 -15 6
24 -43 9
-40 -18 6
-8 36 8
-7 19 8
13 -26 7
47 14 4
26 14 3
36 35 2
-29 47 5
14 -27 7
-42 -18 6
22 -41 9
49 12 4
-40 -14 6
-12 -16 9
36 34 2
-37 -11 6
-9 31 8
-36 -13 6
-43 -18 6
34 -25 0
33 31 2
-26 42 5
35 -26 0
10 -32 7
-31 44 5
28 16 3
-8 30 8
22 16 3
-41 -11 6
-41 -17 6
-44 -18 6
-25 41 5
24 -39 9
22 -40 9
-31 43 5
36 -26 0
24 20 3
25 17 3
-16 -44 1
13 -30 7
33 -23 0
-39 -15 6
36 -22 0
32 -24 0
-43 -17 6
-29 40 5
-8 32 8
-5 34 8
26 -41 9
13 -26 7
-27 45 5
-7 33 8
-42 -18 6
42 11 4
-41 -12 6
49 9 4
49 10 4
23 -44 9
13 -27 7
-15 -46 1
12 -26 7
-8 31 8
13 -29 7
-17 -44 1
34 34 2
-44 -14 6
-41 -15 6
-27 41 5
32 30 2
12 -31 7
-25 42 5
-41 -11 6
-18 -44 1
35 -26 0
33 -23 0
46 9 4
25 13 3
-29 43 5
34 -23 0
-4 35 8
-28 47 5
33 35 2
43 13 4
33 30 2
10 -31 7
22 -41 9
34 30 2
-16 -45 1
-29 41 5
-41 -14 6
37 -27 0
26 15 3
34 -21 0
-42 -11 6
23 18 3
-27 43 5
-9 34 8
-29 47 5
11 -32 7
38 -28 0
23 19 3
49 11 4
37 -24 0
-14 -45 1
32 -23 0
45 12 4
-42 -18 6
-42 -17 6
45 13 4
36 -24 0
14 -27 7
-9 32 8
38 -27 0
25 -41 9
33 33 2
-44 -17 6
-43 -16 6
24 17 3
11 -30 7
36 -26 0
-2 -1 3
-30 45 5
9 -29 7
-40 -17 6
44 10 4
-16 -49 1
-16 -49 1
22 18 3
-25 41 5
-16 -45 1
49 10 4
-7 36 8
32 -24 0
38 -23 0
-30 46 5
47 13 4
-15 -46 1
23 -40 9
34 34 2
48 10 4
-9 36 8
42 12 4
23 -44 9
35 -27 0
38 -26 0
26 17 3
21 -42 9
38 -27 0
-1 0 1
25 -40 9
22 -41 9
44 14 4
45 10 4
23 -40 9
22 -39 9
-17 -47 1
32 31 2
45 13 4
33 30 2
21 -40 9
-7 32 8
-29 44 5
46 11 4
9 -31 7
35 35 2
-29 43 5
11 -29 7
25 -39 9
-43 -18 6
47 10 4
22 -39 9
-45 -17 6
-7 32 8
-6 34 8
-16 -43 1
-30 44 5
45 9 4
-27 41 5
-8 31 8
49 11 4
-28 42 5
26 19 3
31 30 2
35 35 2
26 16 3
47 10 4
26 18 3
45 14 4
-29 47 5
23 17 3
-27 45 5
21 17 3
27 15 3
-39 -15 6
25 -41 9
36 -21 0
23 -43 9
24 -39 9
22 15 3
-9 34 8
12 -26 7
22 15 3
-10 31 8
-17 -44 1
-25 41 5
10 -25 4
34 31 2
-6 31 8
-16 -48 1
23 -41 9
48 12 4
46 10 4
43 11 4
24 13 3
25 -43 9
24 12 3
-43 -14 6
-40 -13 6
-26 41 5
35 -22 0
43 10 4
-4 34 8
-40 -11 6
-17 -45 1
45 9 4
36 36 2
-41 -17 6
-42 -18 6
-4 33 8
-16 -44 1
12 -29 7
13 -29 7
-25 42 5
-45 -16 6
32 32 2
-7 34 8
-29 43 5
-7 35 8
36 33 2
24 15 3
22 -41 9
-40 -14 6
37 -22 0
37 -24 0
-8 32 8
49 11 4
35 -23 0
25 -42 9
9 -32 7
-44 -12 6
-17 -43 1
36 -21 0
45 14 4
12 -32 7
-46 1 2
38 -28 0
32 33 2
23 -38 9
24 12 3
11 -29 7
26 18 3
45 14 4
24 -43 9
-42 -13 6
24 14 3
-43 -16 6
-41 -14 6
-17 -46 1
13 -29 7
-6 35 8
47 10 4
-6 34 8
37 35 2
-15 -44 1
-29 45 5
34 35 2
-40 -15 6
-8 32 8
27 17 3
10 -33 7
23 15 3
13 -32 7
13 -30 7
21 -40 9
-40 -14 6
-5 2 5
24 18 3
48 8 4
-6 31 8
26 16 3
-9 34 8
-14 -44 1
35 33 2
-30 42 5
-41 -16 6
44 9 4
-45 -16 6
-39 -14 6
12 -27 7
47 11 4
-28 46 5
9 -31 7
27 19 3
-9 32 8
-41 -13 6
15 -25 7
38 -26 0
-39 -14 6
22 -42 9
25 -40 9
-43 -15 6
24 -41 9
21 -42 9
-5 -1 9
-40 -13 6
44 14 4
13 -27 7
47 13 4
48 11 4
31 30 2
-7 33 8
22 -41 9
-5 34 8
-5 33 8
-43 -16 6
-28 41 5
-6 33 8
32 31 2
49 12 4
-28 42 5
35 31 2
25 13 3
12 -31 7
-15 -48 1
23 17 3
-16 -46 1
-16 -46 1
-14 -46 1
-15 -44 1
11 -32 7
-4 -1 4
22 16 3
46 13 4
-31 45 5
-5 32 8
48 11 4
25 15 3
37 -27 0
14 -26 7
-13 -45 1
36 -23 0
36 -28 0
-14 -44 1
14 -25 7
32 31 2
-3 1 1
24 18 3
-16 -44 1
-14 -45 1
14 -30 7
37 -28 0
-39 -14 6
23 -42 9
-6 33 8
12 -33 7
-14 -44 1
9 -29 7
13 -26 7
36 32 2
33 30 2
24 -40 9
26 15 3
36 34 2
15 -29 7
-15 -45 1
-25 42 5
12 -31 7
36 34 2
-18 -43 1
26 -42 9
-15 -45 1
49 12 4
-25 42 5
-16 -46 1
33 33 2
12 -28 7
13 -28 7
-3 -4 3
43 10 4
8 -31 7
23 -42 9
-6 34 8
22 -40 9
-9 30 8
46 10 4
11 -30 7
-30 46 5
32 32 2
23 -39 9
-16 -47 1
46 9 4
25 19 3
33 33 2
-45 -16 6
34 -23 0
25 -41 9
-11 32 8
-39 -12 6
35 -24 0
24 16 3
36 35 2
-42 -10 6
-40 -14 6
44 10 4
-15 -43 1
12 -31 7
35 33 2
-14 -46 1
26 -42 9
-40 -17 6
35 32 2
13 -27 7
-15 -46 1
26 -42 9
35 -22 0
-14 -48 1
-29 43 5
36 -27 0
12 -29 7
10 -31 7
-45 -15 6
44 10 4
24 -43 9
34 -24 0
-7 31 8
36 34 2
11 -27 7
34 31 2
-27 45 5
13 -26 7
10 -31 7
35 34 2
-5 34 8
-40 -12 6
-40 -13 6
36 32 2
14 -29 7
37 -26 0
45 11 4
48 11 4
23 -40 9
-43 -17 6
37 -22 0
-8 36 8
35 -24 0
-4 34 8
-28 42 5
35 -25 0
26 14 3
-9 32 8
-30 42 5
27 17 3
44 11 4
32 -25 0
26 -44 9
-31 41 5
23 18 3
34 -24 0
-42 -12 6
26 14 3
35 34 2
10 -26 7
9 -29 7
10 -33 7
32 33 2
35 -25 0
34 -27 0
-7 34 8
12 -27 7
49 11 4
23 15 3
-27 41 5
22 -43 9
-42 -10 6
-14 -46 1
13 -29 7
24 14 3
24 -42 9
-26 39 5
14 -27 7
-6 35 8
-14 -48 1
32 32 2
24 14 3
27 19 3
-43 -14 6
13 -30 7
13 -26 7
-7 32 8
27 19 3
-5 34 8
42 14 4
-15 -46 1
-27 43 5
12 -27 7
22 17 3
26 -41 9
-8 34 8
-16 -45 1
-30 41 5
-27 47 5
22 16 3
14 -28 7
47 11 4
14 -30 7
-45 -17 6
-17 -46 1
-31 43 5
43 10 4
32 35 2
23 -41 9
25 -40 9
23 17 3
47 10 4
25 13 3
-27 39 5
-14 -48 1
27 17 3
11 -32 7
-15 -45 1
-29 46 5
35 -25 0
12 -26 7
-39 -17 6
-45 -15 6
33 31 2
-38 -18 5
25 19 3
22 -42 9
-6 32 8
24 -42 9
-27 46 5
47 10 4
-28 41 5
35 -23 0
-27 43 5
24 -42 9
34 34 2
-16 -44 1
36 -25 0
36 33 2
33 34 2
-28 42 5
12 -31 7
-10 31 8
-13 -45 1
-30 46 5
24 17 3
24 19 3
37 -23 0
34 -21 0
-8 31 8
27 17 3
36 -26 0
-27 41 5
35 33 2
13 -31 7
-41 -17 6
49 8 4
43 11 4
-42 -10 6
31 33 2
35 34 2
-41 -17 6
35 -21 0
-5 33 8
37 -27 0
44 12 4
-30 44 5
22 -39 9
38 -25 0
12 -31 7
34 33 2
-14 -46 1
27 17 3
-41 -18 6
22 15 3
-17 -47 1
33 32 2
-44 -15 6
43 13 4
33 30 2
21 -39 9
-39 -14 6
23 16 3
-43 -16 6
35 -21 0
27 18 3
-16 -42 1
26 16 3
32 32 2
-28 41 5
46 11 4
34 30 2
22 -40 9
22 18 3
44 14 4
-44 -14 6
10 -27 7
-17 -44 1
35 32 2
43 11 4
23 13 3
22 -39 9
-30 46 5
-30 41 5
21 -42 9
12 -29 7
24 18 3
23 17 3
27 18 3
36 -27 0
35 35 2
24 -42 9
-44 -16 6
31 30 2
46 13 4
-41 -14 6
35 -26 0
24 15 3
-27 42 5
-13 -45 1
44 12 4
36 31 2
43 11 4
44 11 4
-42 -12 6
49 10 4
-27 42 5
36 -25 0
33 -26 0
23 13 3
12 -29 7
-42 -17 6
12 -28 7
32 29 2
-10 34 8
44 11 4
36 34 2
-6 35 8
-44 -14 6
33 -25 0
34 -22 0
22 -39 9
22 -42 9
35 -24 0
48 11 4
-31 44 5
-43 -18 6
26 15 3
21 -43 9
33 34 2
25 -43 9
37 -24 0
36 -25 0


==> data_pada_2.tex <==
x y label
31.72 28.175 0
-4.8658 30.011 0
-26.615 -5.01 0
25.36 17.213 0
11.194 -23.206 0
-24.363 41.977 0
10.285 0.073909 0
-27.552 -1.7931 0
-42.062 -16.077 0
-26.594 -6.9296 0
-27.255 -2.5674 0
30.551 31.859 0
26.241 -0.93289 0
20.824 3.1046 0
12.557 -13.755 0
4.6892 -43.578 0
-39.657 -14.98 0
-13.294 -46.499 0
-7.6693 29.297 0
21.434 -38.444 0
-24.193 18.702 0
-1.0615 -9.9838 0
2.4536 -2.5102 0
26.715 -1.015 0
16.797 38.334 0
-14.494 10.07 0
26.26 0.30613 0
-30.279 44.824 0
-27.694 -29.199 0
-1.9643 -5.9486 0
-25.997 -30.782 0
5.8361 -49.606 0
10.979 -32.082 0
-24.619 -29.927 0
7.0448 -42.999 0
32.716 29.279 0
-30.296 43.853 0
15.274 -10.405 0
11.318 27.062 0
-5.8311 -0.70962 0
10.929 1.25 0
-5.0948 -25.585 0
-42.477 -16.304 0
11.293 27.723 0
-22.59 18.974 0
24.351 -1.0362 0
-2.3221 8.1791 0
32.673 -24.499 0
6.6119 -44.497 0
43.939 12.742 0
-40.006 20.423 0
26.762 1.5157 0
-0.57538 1.9206 0
-5.9326 0.41385 0
-25.632 -3.7662 0
-0.52419 -9.3122 0
4.2475 -46.346 0
8.9693 1.8937 0
-29.846 44.415 0
-25.723 -28.709 0
24.198 -42.629 0
34.394 32.578 0
-28.39 39.497 0
-40.312 -17.62 0
-4.8592 1.7459 0
-23.165 24.779 0
23.822 13.958 0
-25.148 -1.3639 0
46.523 11.266 0
35.142 -22.944 0
-12.519 -14.46 0
40.035 -6.313 0
0.86139 -46.647 0
-36.469 20.901 0
-30.437 47.924 0
-27.522 42.505 0
-26.458 -3.5604 0
38.755 -6.9487 0
-4.5975 29.128 0
1.0547 59.362 0
-23.789 -2.9301 0
9.5458 -26.844 0
18.426 -11.949 0
17.055 42.427 0
-0.43058 -1.1511 0
-52.793 6.0233 0
11.132 -23.099 0
-19.462 22.055 0
-26.285 40.311 0
-22.693 24.661 0
-11.787 2.69 0
10.043 -30.289 0
-22.571 -25.766 0
24.073 15.055 0
-28.585 44.221 0
3.1586 1.8264 0
11.015 -31.531 0
5.2771 57.438 0
-8.2478 32.922 0
45.222 9.7247 0
4.8173 -48.86 0
14.52 -24.071 0
37.207 -21.659 0
-20.463 24.276 0
12.337 4.0686 0
9.3404 4.7816 0
38.751 -5.1413 0
-53.016 4.4877 0
-12.197 3.4319 0
23.047 14.964 0
10.022 28.396 0
-13.75 10.064 0
-38.308 -9.6747 0
-4.1726 1.2179 0
-15.938 -47.429 0
5.7324 14.926 0
-23.775 20.454 0
27.565 17.339 0
16.256 41.48 0
5.0737 -47.937 0
-15.557 -41.485 0
-41.293 -15.486 0
-39.822 -15.85 0
44.366 12.44 0
-38.26 20.721 0
-4.5973 1.4271 0
-7.9512 30.478 0
32.316 -23.035 0
-8.6031 33.33 0
-39.569 -10.903 0
-11.334 7.5775 0
-4.2217 22.778 0
-38.753 19.508 0
-28.636 -4.6223 0
-25.143 -27.172 0
-7.3159 33.286 0
-16.101 7.4653 0
26.656 14.925 0
34.471 33.584 0
-19.381 23.465 0
-0.092173 4.4315 0
32.741 -23.782 0
-48.689 6.3365 0
-40.88 -12.341 0
-13.835 8.9789 0
-20.258 21.288 0
9.4439 26.99 0
-2.079 -1.7633 0
5.304 -51.536 0
16.532 -12.493 0
-16.887 -16.088 0
-11.65 2.8351 0
-42.273 -15.228 0
-4.8731 0.49206 0
11.202 -30.092 0
16.059 42.877 0
10.765 27.194 0
-6.3428 -26.668 0
23.68 16.019 0
10.18 26.319 0
-4.4544 -2.5946 0
-3.4941 -0.15285 0
-28.183 -6.7311 0
-26.426 -30.154 0
-48.868 1.7092 0
1.4313 -14.16 0
26.267 -42.559 0
38.735 -8.2926 0
14.074 -26.705 0
24.691 14.862 0
2.1329 -14.358 0
-41.587 -12.684 0
-27.917 -29.45 0
15.562 -12.16 0
-21.438 24.151 0
-40.349 21.577 0
-8.5928 -23.955 0
-39.698 21.433 0
-26.992 43.558 0
5.2255 -48.308 0
5.2686 -48.944 0
37.979 -8.4802 0
-16.807 20.87 0
-3.0348 -28.578 0
-32.6 18.779 0
-41.128 -14.617 0
-28.973 44.097 0
-25.454 -24.768 0
-23.835 -27.566 0
-25.91 -3.9587 0
26.888 -0.5428 0
-38.996 18.273 0
24.49 15.812 0
-35.768 19.04 0
12.509 -30.194 0
-27.945 39.986 0
-1.1207 0.10779 0
-22.776 -30.407 0
-26.436 43.066 0
12.224 27.354 0
-2.1986 -0.82258 0
10.22 28.177 0
-40.694 -18.42 0
36.701 -28.154 0
11.152 1.9818 0
37.094 -26.943 0
33.021 31.249 0
1.897 62.29 0
-26.3 -6.128 0
-26.692 -5.6211 0
16.247 43.391 0
-26.589 42.241 0
-0.50832 0.50337 0
-26.113 -6.0992 0
10.029 26.328 0
-15.651 -13.827 0
12.119 1.6539 0
-19.545 23.282 0
11.698 -32.373 0
38.046 -24.574 0
7.0099 25.104 0
2.0793 -14.284 0
-41.23 21.584 0
7.7408 11.413 0
7.1215 12.238 0
-21.522 24.399 0
-20.826 23.475 0
35.951 -27.379 0
39.367 -7.64 0
-42.114 -17.805 0
-14.41 -13.148 0
-15.918 8.2834 0
32.259 29.378 0
-41.454 -16.721 0
-3.3701 31.717 0
-22.012 -30.025 0
10.781 -31.835 0
2.2342 -47.869 0
22.065 18.644 0
33.262 -23.565 0
-12.252 11.119 0
-24.218 -2.2341 0
-3.0578 -21.545 0
1.614 -12.925 0
-1.0686 -9.3168 0
-14.633 -44.269 0
5.153 -51.534 0
-3.7127 2.6594 0
-40.475 -11.217 0
1.3619 -15.508 0
-27.947 -27.634 0
16.068 -14.442 0
13.141 40.263 0
-32.088 12.469 0
-21.049 -4.0474 0
36.07 -23.757 0
16.847 -11.833 0
-6.5321 33.561 0
25.393 -39.5 0
23.8 -39.206 0
34.963 -22.272 0
11.422 -28.912 0
22.805 2.6115 0
31.88 28.847 0
46.778 11.003 0
-21.93 23.191 0
1.7708 -49.895 0
10.616 23.214 0
41.373 10.568 0
38.544 -8.5083 0
6.0221 -49.71 0
-23.765 -25.469 0
46.872 10.96 0
-16.23 8.4989 0
6.3756 -48.406 0
5.2703 -0.53297 0
16.813 -13.797 0
27.189 13.784 0
35.378 -26.762 0
-38.91 -16.851 0
-2.1157 -5.7819 0
36.998 -9.8624 0
-11.533 10.341 0
-38.621 23.484 0
4.8798 -51.2 0
35.237 -23.098 0
12.602 -31.943 0
-21.849 24.43 0
14.306 39.215 0
23.9 15.797 0
-38.425 -18.482 0
34.159 29.985 0
-2.4265 2.1666 0
-25.711 -28.681 0
-23.503 23.823 0
2.891 -44.985 0
-24.688 -28.741 0
-43.394 -16.609 0
-20.89 -3.7218 0
-12.007 5.8701 0
-40.364 19.455 0
-6.9367 18.013 0
6.6383 -45.167 0
-40.766 -15.721 0
-48.766 1.5582 0
4.1945 -50.897 0
9.9292 24.984 0
23.978 -2.7353 0
1.5902 -12.69 0
-28.437 39.662 0
-39.851 -13.391 0
-5.8005 -0.019216 0
-41.61 -15.786 0
-5.2793 -23.518 0
11.379 25.54 0
-21.925 23.641 0
26.756 0.28484 0
23.803 16.786 0
8.574 22.628 0
21.621 -38.831 0
34.853 -23.073 0
-24.02 -28.857 0
9.5021 -30.178 0
-13.907 -48.084 0
-6.695 34.795 0
-1.0752 22.293 0
-13.394 8.9194 0
-25.093 -7.7202 0
12.818 -25.579 0
10.273 27.22 0
2.394 -9.3541 0
35.524 -23.929 0
-27.118 42.051 0
11.412 -24.823 0
-40.378 22.252 0
-7.0843 33.096 0
-22.109 -4.7622 0
-2.2742 -1.9004 0
1.7268 62.379 0
-41.453 -15.702 0
-3.3682 3.4574 0
47.656 12.609 0
-44.652 -17.065 0
-51.499 2.5599 0
-37.768 -15.471 0
40.691 -6.8009 0
-13.773 -15.383 0
-28.965 46.154 0
13.566 -25.299 0
35.3 29.971 0
11.51 -27.451 0
22.615 -40.033 0
5.466 -47.791 0
9.7389 2.2192 0
37.365 33.679 0
-26.917 -26.201 0
-11.84 8.2927 0
39.369 -8.6498 0
12.925 -28.009 0
-26.951 -28.564 0
45.66 11.364 0
-40.918 20.145 0
-14.345 -15.872 0
24.209 1.7784 0
-22.778 24.081 0
15.437 -11.705 0
-27.795 -28.094 0
-21.628 23.857 0
-27.31 -5.328 0
-49.649 -0.031537 0
2.6879 -8.5115 0
-12.805 11.518 0
-0.65075 -0.49709 0
-0.78767 -0.45598 0
-13.937 9.0196 0
-21.982 23.047 0
6.0124 -46.492 0
-16.299 -45.306 0
37.845 -9.1017 0
35.815 35.434 0
-41.191 21.72 0
-12.757 -46.689 0
-27.733 -5.5773 0
41.443 -7.6015 0
5.2497 -45.8 0
2.2499 -12.723 0
-7.5877 33.668 0
-4.2145 1.0662 0
-4.6112 -1.6186 0
36.643 -6.879 0
38.505 -7.9582 0
-41.392 20.673 0
37.602 -24.617 0
1.2089 -15.586 0
36.241 35.08 0
1.4644 -15.224 0
25.075 15.607 0
9.078 -31.677 0
-25.159 -2.0891 0
-3.3979 31.808 0
-17.311 -18.62 0
37.416 -7.0747 0
-0.38351 58.405 0
-5.4045 -24.157 0
33.76 -22.014 0
34.033 -21.914 0
-24.6 -6.1906 0
-51.581 3.8608 0
-48.815 6.1437 0
-7.6898 29.371 0
19.722 -43.504 0
23.238 15.863 0
6.0246 0.089708 0
-5.8518 1.6801 0
23.614 -39.925 0
-6.5513 7.9753 0
12.432 39.6 0
35.887 -27.336 0
25.712 -0.71713 0
-40.468 -11.827 0
10.811 -29.671 0
-14.936 9.5237 0
-24.407 -25.802 0
22.811 16.798 0
37.279 -22.143 0
12.837 1.6877 0
-7.4745 32.564 0
10.803 26.37 0
-23.885 -3.8648 0
-21.254 24.252 0
36.385 -6.8475 0
-41.768 -14.671 0
-2.9369 7.8718 0
36.889 -27.087 0
24.04 -0.90727 0
-14.879 6.1235 0
-39.341 22.454 0
-1.3073 2.3497 0
22.399 -40.934 0
-23.358 -26.976 0
48.615 9.7521 0
-24.277 18.695 0
-20.905 -26.333 0
0.66964 -14.398 0
1.7347 3.2685 0
-24.836 -3.9209 0
4.6993 -51.648 0
-51.567 4.5913 0
24.962 -43.236 0
-20.938 -3.7124 0
-28.346 -2.834 0
-20.422 20.39 0
35.626 -27.14 0
0.4783 -0.35165 0
-0.90641 -6.1119 0
-41.847 -12.737 0
47.453 8.6903 0
-28.886 -3.7736 0
-7.5271 17.217 0
0.20668 -12.937 0
49.561 10.447 0
26.295 14.279 0
39.078 -7.1369 0
45.755 11.475 0
1.7428 -49.743 0
-22.831 19.985 0
-43.008 -15.073 0
-6.245 -27.445 0
31.131 -21.551 0
4.8148 -43.342 0
-46.991 2.2155 0
0.38597 1.6786 0
16.621 42.592 0
12.916 -30.191 0
-7.0254 17.901 0
40.254 -6.3736 0
-14.941 -42.997 0
-50.769 0.60733 0
8.7597 -1.8078 0
-43.572 -15.406 0
-37.833 -15.475 0
-23.939 25.873 0
37.077 -10.865 0
32.917 33.124 0
26.653 16.713 0
17.237 -13.237 0
-14.57 6.6345 0
-41.737 20.006 0
10.241 2.4752 0
14.739 -11.728 0
20.354 -0.61326 0
-13.006 -45.99 0
-8.7721 -24.018 0
26.534 17.781 0
4.5324 13.701 0
7.6487 -49.184 0
-29.589 9.4389 0
27.529 17.339 0
-22.56 25.417 0
10.713 3.0663 0
-13.098 -45.864 0
-23.034 24.225 0
4.4676 58.536 0
32.566 32.357 0
-40.164 -15.707 0
34.966 -23.914 0
10.08 0.73329 0
11.66 23.443 0
25.521 19.643 0
-15.267 -13.784 0
2.8077 57.529 0
5.4738 -48.027 0
10.344 -33.234 0
-24.729 -25.664 0
20.806 16.892 0
11.234 -29.625 0
11.119 -32.207 0
-8.2828 35.27 0
11.207 3.0132 0
1.2284 55.643 0
-12.094 6.1218 0
11.59 -32.728 0
-13.74 -47.041 0
-22.636 -30.411 0
-40.698 -11.378 0
16.801 -13.84 0
9.5457 24.69 0
-11.781 10.411 0
-17.781 -19.192 0
-0.34578 -13.562 0
6.1272 -0.49955 0
44.216 12.102 0
-41.168 21.415 0
33.189 -21.798 0
-15.287 -47.701 0
48.955 9.5323 0
-13.238 -43.845 0
12.449 3.1692 0
-41.726 19.956 0
6.8911 -44.437 0
27.022 -0.43264 0
-38.518 -14.813 0
-42.004 20.122 0
-24.824 -30.365 0
-25.084 -7.8799 0
23.848 -42.977 0
4.3131 56.347 0
14.275 -14.545 0
22.775 13.819 0
-25.762 -29.013 0
43.964 12.992 0
-10.454 8.3524 0
-17.418 8.5458 0
9.8759 2.1029 0
-17.75 -44.531 0
-22.633 24.818 0
42.802 10.805 0
-40.513 -16.098 0
6.1994 0.026426 0
0.76003 -7.9628 0
24.121 1.6488 0
-0.68697 -10.225 0
35.461 -24.096 0
-29.898 44.163 0
-0.97286 -6.0949 0
-45.302 -14.92 0
-7.8184 35.402 0
-15.639 -19.424 0
8.5054 5.2155 0
-26.4 -30.333 0
1.9769 3.7942 0
-4.7397 29.762 0
-51.023 0.89553 0
-28.476 39.834 0
-23.446 -3.0821 0
-6.4477 34.378 0
-2.3155 -1.5842 0
-2.9167 31.062 0
-12.851 10.841 0
38.426 -5.8733 0
-49.289 4.8757 0
42.23 10.635 0
-51.3 3.2673 0
35.445 -21.875 0
15.897 -8.7586 0
36.746 34.241 0
4.8089 -44.495 0
-10.564 8.1801 0
5.9592 15.005 0
-14.293 8.1044 0
23.989 15.573 0
24.942 2.054 0
-24.882 -0.6555 0
32.086 31.618 0
-24.687 -29.442 0
-9.0783 30.857 0
-12.507 8.7159 0
26.629 15.003 0
20.477 -41.7 0
35.971 -27.298 0
-15.237 7.5161 0
44.175 12.762 0
-28.061 -27.112 0
5.0788 -51.748 0
-47.003 3.2515 0
-12.775 -47.462 0
39.402 -6.1182 0
-7.2604 7.4806 0
36.737 -25.359 0
-27.538 -28.765 0
24.964 -2.2879 0
-40.175 20.885 0
-19.768 22.438 0
4.4395 0.34194 0
-24.281 -30.592 0
36.624 -21.714 0
-14.279 -14.637 0
15.043 -25.614 0
41.519 -7.1071 0
-4.3084 1.1751 0
34.194 -22.995 0
24.347 -1.4781 0
10.945 27.161 0
10.876 4.2632 0
-28.987 -5.4834 0
-24.702 -30.494 0
17.491 -13.454 0
-17.656 -44.59 0
45.287 9.9132 0
-12.477 7.8631 0
-14.775 -42.969 0
23.54 16.494 0
-19.501 22.473 0
26.63 -1.0705 0
-24.482 41.772 0
43.829 10.374 0
-6.1877 -24.514 0
-43.495 -17.016 0
-28.174 44.218 0
-39.163 22.656 0
0.2915 1.4819 0
3.0967 -44.237 0
-8.536 -20.598 0
-25.11 -3.6044 0
0.22514 58.921 0
22.743 2.7634 0
12.326 3.1118 0
-14.579 -10.43 0
-29.558 -5.6936 0
-24.915 -6.6327 0
1.4463 -10.38 0
-51.05 0.24722 0
-2.1472 -1.0666 0
4.1068 -46.492 0
-14.664 10.021 0
-29.51 46.819 0
-38.382 -9.9595 0
-23.638 -4.9588 0
35.443 31.583 0
-49.091 2.819 0
-28.309 38.853 0
10.052 28.018 0
7.0881 -47.427 0
-4.7583 -26.025 0
23.178 16.309 0
-5.7571 33.696 0
11.492 -32.566 0
-5.4018 -0.0967 0
-15.919 -15.149 0
8.3818 11.073 0
10.532 23.32 0
-15.859 -15.198 0
9.7424 -30.303 0
3.1896 -49.165 0
-32.823 18.804 0
20.889 16.921 0
-19.238 -21.747 0
3.1487 -44.364 0
12.747 -32.133 0
-49.252 -0.6324 0
-41.469 -13.773 0
-2.0892 -1.7634 0
23.899 -42.743 0
-24.931 -27.66 0
23.442 -4.5922 0
45.719 9.6961 0
-2.0031 -1.9642 0
5.902 -51.296 0
24.806 17.741 0
0.96669 -9.0705 0
-3.5245 -22.751 0
1.7807 5.2126 0
14.944 -25.088 0
-3.5646 1.7206 0
-12.363 4.2194 0
-15.271 -16.383 0
3.7721 -49.474 0
10.244 26.537 0
-50.365 1.1915 0
-15.547 -46.115 0
16.143 36.021 0
22.354 -40.984 0
11.939 -27.074 0
-40.061 -15.441 0
14.632 -24.018 0
12.591 -24.652 0
-12.743 -15.615 0
-8.3579 -22.952 0
36.818 33.772 0
18.593 -11.251 0
-48.783 -0.69913 0
-51.932 4.0681 0
1.9808 -49.841 0
-5.255 -3.4274 0
-3.7158 -21.955 0
32.531 29.449 0
-20.937 23.308 0
4.6104 -51.162 0
-40.346 -17.033 0
5.941 -0.89927 0
-24.485 -24.591 0
-8.0389 -26.231 0
1.634 5.8458 0
31.767 29.11 0
-27.062 40.598 0
-21.914 25.469 0
-43.355 -13.408 0
9.7645 1.0362 0
-43.258 -16.678 0
-27.434 45.862 0
-43.384 -16.691 0
2.3606 -47.345 0
-26.7 -3.2185 0
-26.812 44.129 0
-23.06 24.5 0
32.32 -21.59 0
-15.68 -19.229 0
3.8396 57.464 0
-40.463 -14.552 0
-7.159 34.924 0
25.68 15.165 0
7.0123 25.207 0
1.0723 3.1211 0
-6.3738 33.281 0
-22.012 -27.379 0
17.129 38.758 0
-27.076 38.67 0
-2.3479 -25.503 0
-20.327 20.039 0
-22.614 19.576 0
-41.337 21.357 0
5.2984 16.786 0
-40.879 19.19 0
-43.289 -14.962 0
36.654 -22.855 0
-26.781 43.871 0
21.446 -37.29 0
-26.166 -30.819 0
31.051 -21.386 0
-4.3038 2.9615 0
-26.954 -28.188 0
-25.204 -3.6157 0
-29.144 39.642 0
-4.7826 -21.089 0
10.575 28.279 0
37.429 -7.3188 0
-26.937 44.226 0
-25.268 40.216 0
-28.601 41.098 0
20.359 16.897 0
26.444 15.771 0
-15.326 -42.103 0
-13.31 10.501 0
16.861 -13.286 0
1.8815 57.937 0
-16.104 -13.661 0
9.5818 28.604 0
-41.282 -15.621 0
-14.96 9.2267 0
-1.0657 -10.792 0
-6.1938 4.169 0
-2.9703 -23.362 0
-4.3016 -24.017 0
17.634 -12.057 0
-5.6366 -26.177 0
36.419 -11.233 0
36.975 -6.6428 0
-15.741 -14.581 0
-28.798 8.4085 0
-20.538 23.439 0
40.489 -6.5812 0
31.212 34.272 0
-52.091 1.0172 1
43.709 10.651 1
3.2471 56.585 1
7.2004 1.3177 1
10.775 -31.284 1
-7.3693 32.32 1
-7.5756 34.037 1
-11.257 -12.664 1
-5.0753 34.589 1
-51.928 0.36664 1
22.433 -40.394 1
9.4852 1.5204 1
15.885 -11.157 1
-30.513 7.9086 1
-6.6623 -26.785 1
-2.3063 22.846 1
-38.469 21.958 1
32.921 -22.39 1
-1.5987 -13.259 1
-3.2224 -24.615 1
0.80245 -13.945 1
-13.955 11.746 1
3.4694 14.439 1
16.271 -11.457 1
-3.8345 -28.186 1
-6.6409 -24.084 1
-21.875 24.895 1
-27.858 -5.0195 1
-24.116 -30.726 1
-3.9274 -23.346 1
26.084 -43.782 1
-21.68 24.834 1
-14.555 7.9802 1
-51.336 3.344 1
-9.7244 9.1896 1
32.973 30.724 1
36.278 -8.8275 1
23.667 -38.727 1
-5.1345 -0.55635 1
-15.814 -43.932 1
-11.737 11.832 1
-2.5879 0.60126 1
45.327 13.979 1
0.47741 -12.84 1
8.7459 4.8768 1
-0.55781 -9.515 1
35.253 -25.486 1
-14.478 -46.673 1
2.2727 -14.977 1
11.043 -30.94 1
38.004 -6.3901 1
-26.758 45.141 1
2.2735 -49.479 1
25.489 -1.6605 1
21.907 -39.634 1
-3.0742 -5.0225 1
12.789 -27.153 1
13.938 -30.545 1
24.86 16.454 1
12.506 0.19792 1
11.9 -30.508 1
12.308 0.16927 1
4.0603 57.955 1
37.976 -27.417 1
10.985 27.404 1
-22.347 -4.6592 1
-23.76 -26.463 1
-50.113 4.1715 1
-25.767 -29.607 1
16.492 41.636 1
-26.936 -5.0669 1
-7.4308 -24.816 1
-3.8794 -26.132 1
11.528 -26.403 1
-48.379 0.9131 1
37.743 -10.618 1
-23.982 -26.718 1
-39.12 -12.748 1
-26.906 41.042 1
-5.4182 35.256 1
3.0741 -12.579 1
-11.995 23.298 1
-30.8 45.265 1
-48.76 3.9718 1
24.758 15.792 1
5.6298 16.437 1
11.437 -25.921 1
-1.9991 3.2202 1
32.604 30.449 1
1.9897 3.7398 1
4.4728 -44.977 1
2.2229 -10.849 1
33.113 31.957 1
-31.466 10.453 1
-1.7836 21.736 1
-31.308 45.744 1
-41.676 19.732 1
-11.242 10.563 1
-1.2266 4.8934 1
-38.503 21.191 1
14.356 -11.516 1
6.8045 0.43849 1
5.0812 -48.43 1
-12.923 10.18 1
37.609 -27.398 1
-26.395 -28.958 1
-3.4799 32.28 1
16.951 40.529 1
3.3125 14.654 1
-28.163 -30.976 1
-28.662 -7.5003 1
-13.943 -11.252 1
-8.1059 36.151 1
10.301 1.2477 1
14.791 -11.301 1
7.3697 12.887 1
-7.3186 34.186 1
3.9018 2.3736 1
-26.894 41.926 1
-40.66 19.201 1
11.303 -0.051122 1
-4.8899 -24.496 1
-14.485 -15.35 1
-2.8177 5.0874 1
-14.278 -14.701 1
-23.892 -3.6928 1
-20.517 26.108 1
-23.048 -27.374 1
2.8899 58.281 1
22.843 -42.466 1
-6.5582 35.686 1
34.479 34.038 1
13.954 -14.531 1
-13.99 6.0922 1
-48.011 2.4405 1
-52.586 3.8129 1
46.727 8.3314 1
24.558 2.8419 1
33.48 -25.028 1
-41.118 18.962 1
15.568 39.651 1
12.927 -26.797 1
-11.329 22.498 1
-15.452 -44.348 1
-32.479 10.472 1
-28.567 9.5919 1
24.213 -0.21765 1
8.996 -0.13766 1
-26.22 -1.4879 1
-4.8905 -23.623 1
-30.293 9.5218 1
-12.765 10.162 1
35.047 -24.271 1
3.1209 1.9161 1
38.31 -26.041 1
21.027 -39.156 1
34.494 29.365 1
9.3483 3.121 1
-49.8 3.9195 1
-9.506 31.184 1
0.86484 -10.956 1
13.027 -11.367 1
-14.067 8.1698 1
39.143 -9.3526 1
1.3118 58.869 1
-41.564 21.211 1
9.5312 2.2781 1
-48.773 1.5213 1
1.6731 0.78983 1
6.2992 14.374 1
-14.102 -18.152 1
25.509 17.525 1
-13.326 6.5053 1
-15.797 -44.72 1
-3.8231 -28.148 1
-37.619 23.516 1
5.6131 16.646 1
-12.474 -12.251 1
23.987 19.468 1
26.703 17.3 1
10.227 23.72 1
-39.129 21.06 1
-24.684 -4.5281 1
24.537 16.178 1
25.389 -1.6082 1
-37.515 -13.268 1
16.692 39.857 1
-28.953 46.479 1
-3.3695 1.8975 1
22.842 -42.136 1
21.884 -2.0086 1
36.429 32.755 1
-3.3227 4.9013 1
-5.0029 32.694 1
-19.952 21.46 1
35.326 33.261 1
-9.0062 -25.894 1
33.454 -26.34 1
19.697 -39.278 1
5.5294 -47.332 1
-43.295 -18.621 1
25.387 14.624 1
24.328 -41.625 1
8.7957 -0.80384 1
-7.9242 31.951 1
39.219 -6.5506 1
0.81317 59.084 1
25.574 17.971 1
-25.255 40.559 1
-27.284 -8.3197 1
-21.591 21.419 1
0.15501 -8.6837 1
-49.823 0.43665 1
1.522 -11.408 1
-14.391 -17.852 1
-26.805 -27.936 1
-16.967 -45.868 1
16.312 38.425 1
-23.166 21.962 1
-26.632 41.547 1
21.768 14.28 1
-12.428 -12.961 1
23.634 13.423 1
10.964 0.7944 1
12.553 24.685 1
-1.8607 21.01 1
15.519 -12.179 1
-28.513 -26.827 1
21.716 1.2862 1
-37.146 20.368 1
-24.946 22.494 1
13.656 -13.252 1
36.14 35.863 1
22.497 -0.73526 1
-0.34278 4.3528 1
10.502 29.188 1
-4.6423 -2.6381 1
33.561 -26.529 1
4.1061 56.014 1
47.889 10.216 1
10.35 4.0197 1
-9.0605 -26.343 1
-15.401 -12.649 1
-4.4945 3.1793 1
14.783 38.799 1
-39.875 -14.434 1
-12.716 -45.753 1
-2.3509 3.7616 1
-1.2513 -13.337 1
-23.072 -29.58 1
-2.4758 -24.477 1
-44.57 -15.022 1
-30.575 44.417 1
-0.10273 -11.554 1
14.912 -10.823 1
34.115 -23.887 1
-6.0632 -25.237 1
-39.279 -14.928 1
45.507 11.502 1
-42.988 -13.995 1
1.4046 -46.844 1
-2.7904 23.339 1
16.038 -14.103 1
41.199 14.483 1
-26.409 40.684 1
-22.457 24.128 1
-23.022 -26.36 1
-2.8435 1.2 1
-14.266 6.6635 1
-14.745 9.633 1
6.0198 -49.94 1
-38.423 20.225 1
-4.1604 21.319 1
8.2308 27.053 1
10.724 -27.887 1
-4.7254 30.382 1
-28.137 39.991 1
0.76372 -10.525 1
3.7012 55.95 1
17.601 41.245 1
-22.725 26.553 1
-1.7532 -11.861 1
14.158 -13.685 1
26.091 14.925 1
38.486 -7.706 1
6.4828 -50.554 1
-36.908 20.485 1
-17.934 -15.902 1
-22.85 26.581 1
26.149 -40.685 1
-31.144 8.1418 1
35.257 33.605 1
14.943 40.247 1
-12.021 23.441 1
-14.009 -46.708 1
39.606 -7.1697 1
-11.908 -14.778 1
-51.486 4.1887 1
6.6324 14.232 1
-8.2035 -26.832 1
-47.761 1.506 1
13.133 -30.735 1
-17.074 -43.972 1
35.541 -26.21 1
1.6814 58.29 1
8.7586 -31.378 1
-28.839 45.618 1
21.58 -39.678 1
-18.771 23.904 1
-47.743 1.2852 1
-5.6787 31.295 1
-27.889 -4.9239 1
-29.333 43.451 1
4.4546 -50.701 1
25.717 1.3868 1
-25.642 -25.781 1
-24.513 -6.0582 1
48.229 9.8906 1
-28.65 10.895 1
17.737 -11.194 1
41.799 -5.2449 1
24.47 17.876 1
1.1579 -46.893 1
15.216 -11.815 1
18.183 38.76 1
10.154 28.592 1
-25.588 -6.8035 1
-7.1683 35.199 1
2.0743 -11.755 1
33.922 31.211 1
16.505 40.967 1
-0.40693 -10.927 1
15.139 37.395 1
-31.319 45.768 1
-5.4396 22.652 1
-40.736 20.396 1
6.2104 11.527 1
12.217 -25.945 1
8.9908 5.1984 1
-41.682 22.561 1
3.6879 15.496 1
11.628 -26.268 1
8.9812 1.6469 1
0.64967 -11.085 1
4.0134 58.3 1
0.88415 61.201 1
2.0515 57.442 1
0.33537 58.76 1
2.1319 59.149 1
4.5397 16.116 1
5.8101 14.907 1
33.669 32.033 1
-22.949 21.45 1
11.471 -28.556 1
39.087 -6.9588 1
35.635 -23.742 1
18.348 38.842 1
-30.156 9.7885 1
13.964 40.676 1
8.527 21.49 1
-27.527 41.422 1
-10.677 32.342 1
-40.393 -12.82 1
-25.65 -5.6195 1
3.5627 55.632 1
44.463 9.8156 1
-50.674 5.5544 1
-14.568 -13.135 1
-40.596 19.193 1
-22.806 -6.0203 1
47.088 12.159 1
-38.578 19.262 1
45.142 13.987 1
-31.004 42.183 1
13.411 -11.468 1
7.1371 -49.315 1
9.6429 28.449 1
25.14 -0.40241 1
4.347 12.688 1
10.801 3.8407 1
-28.398 40.731 1
-37.277 21.453 1
1.5864 58.863 1
-23.615 -3.0391 1
-28.717 42.337 1
8.647 0.81836 1
22.634 -0.16874 1
-19.502 19.98 1
-30.244 10.7 1
-38.608 -12.995 1
-5.2938 -25.686 1
-14.219 -14.998 1
-25.471 -26.649 1
2.3759 -10.636 1
26.058 -3.0416 1
-7.2507 32.095 1
-48.091 4.5405 1
10.833 28.309 1
36.943 34.156 1
2.1103 54.658 1
16.192 41.962 1
-1.9023 21.768 1
-16.535 -3.3083 1
-1.8912 0.20008 1
32.829 31.828 1
-40.198 -13.665 1
17.5 -13.928 1
44.559 12.992 1
-26.226 -3.445 1
41.316 -4.7162 1
-16.615 -43.127 1
2.4934 61.507 1
-7.3265 7.7381 1
11.934 25.417 1
10.013 23.796 1
-14.264 -45.725 1
16.987 40.5 1
14.363 -27.908 1
45.977 9.0698 1
-6.4555 34.376 1
-13.2 7.6036 1
45.792 12.771 1
-36.712 -12.996 1
-6.0531 33.023 1
-9.3676 -26.134 1
-5.3511 -1.017 1
7.3581 -47.162 1
-36.66 21.728 1
-23.083 23.12 1
15.572 39.123 1
-53.09 4.2494 1
-38.277 -13.683 1
-30.188 12.596 1
-35.043 17.345 1
-3.1605 33.356 1
-40.741 19.662 1
-22.52 -29.64 1
15.763 -12.83 1
9.5756 24.502 1
-22.994 -28.105 1
16.781 40.7 1
-7.8964 31.069 1
26.135 -3.0781 1
6.5966 -49.863 1
-42.684 -18.328 1
17.33 -10.53 1
-18.003 -14.13 1
3.4081 55.213 1
6.0432 -49.847 1
3.2776 13.602 1
2.1057 -14.157 1
25.151 0.3647 1
11.045 24.96 1
7.1387 -49.911 1
20.884 -39.126 1
2.9207 58.664 1
8.3365 22.769 1
-35.073 20.922 1
-15.94 -43.448 1
0.097093 -7.8098 1
-4.8355 -2.8649 1
-13.528 9.8836 1
-13.844 9.2302 1
-17.301 -14.881 1
11.678 -28.462 1
15.119 -13.484 1
22.537 -43.49 1
37.774 -7.385 1
17.108 40.547 1
-14.374 -43.487 1
10.939 -25.943 1
-5.2662 -24.678 1
0.23694 56.322 1
-52.154 0.11056 1
-13.121 -14.954 1
-13.109 -47.399 1
-14.365 7.3876 1
23.541 0.74665 1
33.773 32.424 1
9.7078 3.0536 1
33.357 31.441 1
7.2495 -0.83569 1
11.37 25.728 1
32.399 -22.012 1
-40.908 22.128 1
9.8059 24.166 1
-4.0779 23.764 1
-22.809 19.159 1
9.2223 24.426 1
-15.695 8.026 1
1.1808 -15.555 1
24.036 -43.996 1
1.1383 -48.792 1
37.138 -10.781 1
-25.806 -29.531 1
2.3065 3.4316 1
-36.443 18.228 1
6.3163 12.918 1
-29.078 10.561 1
-29.422 43.389 1
31.825 30.697 1
41.817 -5.6183 1
-14.295 -13.416 1
-14.444 -47.287 1
-12.76 7.6835 1
14.443 -13.611 1
2.1991 61.157 1
-25.539 -2.4132 1
-9.0931 35.704 1
-25.814 -7.4006 1
-9.2234 30.29 1
-28.973 42.741 1
-11.719 -11.558 1
22.676 -40.425 1
35.051 33.371 1
-49.263 0.45069 1
-2.268 -0.53922 1
25.215 -40.357 1
-48.138 2.8979 1
-14.969 10.573 1
34.111 -21.618 1
-15.654 7.8788 1
-30.215 43.547 1
7.8564 27.519 1
-31.707 8.3611 1
-3.7217 22.485 1
24.875 -41.236 1
-42.269 22.493 1
-3.765 22.958 1
10.281 1.4471 1
-49.318 4.4578 1
-30.394 9.9146 1
8.7042 2.0866 1
13.992 -29.912 1
-27.809 40.483 1
20.389 -42.854 1
-40.537 22.278 1
27.055 16.713 1
-8.1143 31.71 1
34.568 -22.555 1
-14.289 -12.214 1
23.924 -43.28 1
-39.748 -14.389 1
33.991 -24.867 1
39.894 -8.9605 1
0.6653 58.562 1
43.927 10.526 1
36.784 -26.35 1
-15.769 9.4745 1
-17.418 -15.053 1
2.6735 -45.603 1
-12.3 10.067 1
0.68928 -8.794 1
-16.703 -42.157 1
-1.4584 4.4108 1
-2.3608 4.3004 1
10.111 -32.237 1
15.503 41.253 1
3.8121 56.179 1
-21.58 20.956 1
2.2883 -8.8402 1
39.832 -9.4412 1
47.474 8.4374 1
-28.918 42.191 1
10.734 -31.92 1
5.1369 12.206 1
33.988 31.675 1
8.0322 26.977 1
-5.2915 -25.836 1
1.6334 -9.4192 1
-30.622 9.5612 1
-16.172 -48.531 1
37.758 -26.656 1
-2.1754 3.3292 1
43.757 9.3133 1
-1.0182 -5.9809 1
-15.278 -46.626 1
-21.99 -28.663 1
-4.784 -23.36 1
-5.4773 34.973 1
-11.847 8.9228 1
16.168 -15.872 1
-16.437 8.3556 1
6.7877 13.114 1
23.076 -37.851 1
22.161 -42.341 1
9.8555 23.625 1
4.3427 13.271 1
39.525 -9.4604 1
16.15 -12.928 1
-51.817 0.55243 1
10.743 2.2841 1
37.117 -23.759 1
9.3772 0.48482 1
36.259 32.842 1
-50.07 4.8415 1
26.19 17.571 1
-6.2308 30.597 1
37.247 -22.549 1
3.3378 -46.473 1
-16.592 -43.038 1
25.916 1.3295 1
21.664 -1.9104 1
-11.224 6.8376 1
1.6724 59.789 1
-25.223 -7.2591 1
-26.055 -4.3214 1
-29.933 9.1985 1
-39.899 20.17 1
-1.9873 23.673 1
-29.775 -29.152 1
5.5162 -3.3205 1
45.06 12.131 1
-2.1006 23.907 1
-14.309 -45.849 1
13.31 -11.401 1
16.101 40.419 1
46.741 11.577 1
-31.059 45.52 1
-13.289 12.277 1
4.0689 14.165 1
22.625 1.1556 1
1.653 -47.466 1
0.10094 -14.976 1
-36.596 21.99 1
-7.8897 31.329 1
-7.9932 31.766 1
22.744 -0.63712 1
39.082 -9.4789 1
-2.5233 22.56 1
43.984 12.945 1
-25.161 -30.844 1
11.371 -27.29 1
4.0035 -1.8741 1
-30.052 8.7894 1
-3.8801 -28.217 1
-29.185 42.001 1
-5.6493 -22.185 1
-30.66 9.4355 1
1.2302 56.199 1
5.9308 -46.852 1
10.208 27.065 1
-23.961 -26.354 1
-10.282 9.4274 1
24.327 -2.1449 1
-5.4271 33.972 1
-31.887 8.945 1
-38.783 19.115 1
9.959 0.97162 1
7.8582 2.7096 1
-28.516 42.303 1
3.307 -44.906 1
12.934 -28.384 1
-35.955 19.889 1
-28.128 40.878 1
-21.79 21.986 1
6.4106 14.833 1
-12.216 10.957 1
-52.841 4.5146 1
-14.731 8.7387 1
-12.187 -15.15 1
-7.7895 -24.435 1
49.163 12.857 1
40.435 -6.9682 1
-30.513 8.4175 1
22.586 -39.7 1
-27.773 -7.8907 1
-11.1 8.1188 1
-20.798 20.277 1
-31.013 46.267 1
-19.742 25.092 1
22.159 -37.86 1
-23.349 23.505 1
34.923 -23.438 1
2.8796 61.773 1
-29.941 44.871 1
-25.927 -27.433 1
26.344 -41.801 1
23.63 -2.7123 1
23.875 -3.3943 1
-25.332 39.031 1
-36.785 18.716 1
10.829 2.8968 1
27.967 17.595 1
1.6719 -14.452 1
25.897 18.324 1
36.276 -8.704 1
-22.568 -4.5263 1
36.849 34.282 1
24.679 -42.937 1
-41.505 20.133 1
2.8484 -11.901 1
25.74 17.925 1
-16.691 -43.351 1
10.228 1.3113 1
-13.482 -15.791 1
-7.0856 18.898 1
-14.728 23.089 1
1.4767 59.775 1
12.896 -10.229 1
48.069 10.72 1
-23.199 -27.278 1
-27.784 -3.4485 1
-15.261 -46.104 1
17.44 -12.338 1
-43.225 -12.684 1
-7.2117 33.759 1
-2.1577 20.65 1
-14.939 -45.294 1
49.718 9.7302 1
-6.5151 19.1 1
-22.463 -27.793 1
16.105 38.475 1
25.679 -1.2221 1
-7.9354 36.057 1
-25.055 41.828 1
-4.4741 35.108 1
12.934 -27.952 1
-49.378 1.1947 1
48.55 10.033 1
18.13 38.74 1
9.7026 -28.383 1
7.8993 26.388 1
-26.285 -6.8207 1
-7.5923 -23.818 1
-29.655 10.878 1
16.48 -10.95 1
10.091 -31.783 1
26.589 0.35555 1
7.8814 24.864 1
-5.3566 32.775 1
22.373 -3.0165 1
-28.037 -30.13 1
-4.5228 34.772 1
9.4723 26.254 1
33.404 31.724 1
22.196 -39.054 1
-13.254 -15.706 1
48.695 9.9839 1
-10.168 6.6297 1
2.5945 -14.337 1
21.951 -40.138 1
-17.653 -15.439 1
-2.9831 1.0781 1
-12.823 -10.776 1
-16.729 -44.565 1
-29.602 8.2954 1
10.733 1.5104 1
2.2624 -46.436 1
0.37731 -10.488 1
9.3891 0.28564 1
35.02 34.627 1
-9.592 -25.304 1
21.432 -41.443 1
-4.307 -3.7809 1
-9.1701 -26.089 1
45.865 9.7616 1
-26.551 -31.729 1
-12.924 -45.265 1
-0.066472 -12.755 1
38.291 -8.445 1
-5.8022 -23.365 1
-21.6 20.914 1
10.802 24.425 1
-28.052 -3.2235 1
4.2557 14.03 1
44.597 10.013 1
35.291 -23.689 1
-29.768 42.45 1
-3.3918 2.4436 1
-12.197 22.092 1
-36.463 -12.938 1
3.4886 56.163 1
34.63 -22.692 1
8.8082 3.9319 1
5.8881 -47.574 1
8.5279 21.547 1
36.728 33.562 1
0.86854 -11.157 1
21.006 -40.601 1
2.6104 -46.517 1
-6.8877 32.943 1
14.938 -12.038 1
-19.182 19.937 1
25.425 1.6873 1
36.731 33.679 1
17.882 -13.425 1
-11.509 22.545 1
4.6984 -44.956 1
35.457 33.276 1
3.9742 12.305 1
-28.624 46.451 1
-27.353 -27.299 1
25.113 -40.18 1
26.956 17.166 1
-45.351 -16.93 1
11.877 28.485 1
-14.389 -46.999 1
-15.29 -44.844 1
-13.871 -13.464 1
-50.108 -0.13329 1
-15.289 7.8779 1
4.4599 -49.697 1
-19.484 21.143 1
3.9354 14.377 1
36.389 -24.957 1
25.587 14.404 1
36.527 -8.8612 1
-5.7956 35.911 1
-14.12 7.8508 1
-10.332 11.066 1
0.64155 59.726 1
9.9912 -30.73 1
39.739 -9.6263 1
-24.311 -5.9268 1
24.509 17.331 1
4.8349 -44.879 1
-5.366 36.105 1
-42.586 -13.941 1
-27.87 41.766 1
17.295 -12.131 1
35.811 -28.284 1
40.149 -5.7227 1
24.314 17.268 1
-24.125 -4.5821 1
-11.401 25.85 1
12.262 -24.595 1
-11.178 8.9386 1
35.418 35.569 1
-14.811 -11.378 1
10.544 2.327 1
14.218 -13.073 1
-3.63 -23.795 1
0.99221 -10.458 1
16.888 -10.16 1
-20.148 19.396 1
39.693 -5.7984 1
2.5856 -8.811 1
-42.58 -14.121 1
-11.583 5.2366 1
3.1041 -47.975 1
-31.232 9.1283 1
13.307 -10.676 1
16.257 -10.827 1
11.095 -31.742 1
23.281 -1.3734 1
8.934 1.0532 1
-16.382 21.163 1
36.703 -7.3079 1
-7.6586 9.7505 1
16.893 41.916 1
33.549 31.893 1
-5.1937 -23.273 1
-38.308 18.422 1
43.686 12.765 1
22.435 -42.292 1
-21.794 24.688 1
-17.891 -15.855 1
34.094 34.863 1
-26.886 -4.5678 1
-7.2985 32.859 1
-14.29 11.196 1
-5.0228 -23.4 1
4.3342 -45.918 1
25.477 18.273 1
10.243 26.538 1
-11.176 24.377 1
-29.829 43.8 1
10.902 2.7572 1
32.03 -23.599 1
-29.784 -29.134 1
36.977 32.206 1
-43.978 -11.875 1
7.9318 3.751 1
17.217 38.91 1
21.697 14.201 1
6.2775 1.668 1
26.688 17.484 1
-42.067 19.121 1
-26.592 -26.682 1
6.6388 16.649 1
-8.2495 -22.956 1
-29.321 8.7613 1
-41.146 22.47 1
17.216 39.786 1
-43.778 -15.489 1
24.081 -43.481 1
-40.45 -17.674 1
-7.7468 35.937 1
-6.7775 19.306 1
-27.009 -27.418 1
-48.874 3.8169 1
-24.485 -28.931 1
-52.475 3.3015 1
12.928 -26.269 1
4.2296 13.427 1
47.162 13.638 1
8.2505 23.384 1
-40.595 22.692 1
24.213 0.015638 1
25.778 13.754 1
36.298 34.881 1
-29.04 46.713 1
13.802 -27.428 1
0.63473 -13.945 1
-42.131 -18.424 1
21.877 -41.412 1
-17.354 -14.84 1
24.996 -0.42453 1
9.4614 3.722 1
2.0816 58.428 1
21.506 -0.44126 1
-1.039 21.707 1
41.374 -5.159 1
7.0108 14.203 1
48.952 11.727 1
-40.219 -14.262 1
-11.666 -15.605 1
36.176 33.548 1
-37.25 -11.408 1
-8.5542 31.212 1
-3.7579 24.149 1
-1.6498 21.059 1
-38.901 21.749 1
-36.339 -12.955 1
11.471 0.66442 1
-48.525 1.0787 1
0.39609 -8.9484 1
-30.868 9.9682 1
-30.762 10.264 1
-42.957 -18.352 1
34.04 -25.462 1
-22.227 -27.925 1
-14.26 10.951 1
16.171 36.867 1
32.599 31.195 1
7.2389 14.998 1
-26.443 42.303 1
-38.806 24.135 1
-13.135 -13.868 1
35.196 -25.66 1
9.9879 -32.404 1
-14.76 7.8681 1
-3.0003 -27.41 1
-26.238 -1.2745 1
-30.097 9.7629 1
-17.517 23.863 1
-31.219 44.145 1
28.023 16.238 1
-7.7688 29.684 1
-14.173 -10.993 1
22.364 16.1 1
-0.3266 -8.4766 1
9.8655 27.399 1
8.272 28.636 1
-41.177 -11.488 1
15.824 -11.092 1
-24.33 -26.574 1
0.75519 -46.471 1
-48.07 0.53485 1
-41.474 -17.425 1
-44.255 -17.571 1
38.46 -7.2523 1
6.1585 -49.767 1
2.3124 57.291 1
-22.979 23.371 1
17.334 41.681 1
-53.696 2.8511 1
-38.644 23.574 1
15.45 37.904 1
-30.659 11.966 1
-25.04 41.436 1
23.775 -38.667 1
-2.9211 22.605 1
-2.4217 24.546 1
3.8365 14.782 1
-2.8259 1.1879 1
21.92 -40.243 1
-1.9868 0.13589 1
-23.385 22.585 1
4.3884 11.874 1
-31.175 42.72 1
5.6875 -47.77 1
13.861 41.232 1
-10.557 9.8486 1
14.629 39.937 1
36.488 -26.384 1
-25.084 22.451 1
-28.506 10.256 1
-3.4725 -23.899 1
-3.8502 23.555 1
-24.379 -6.1536 1
-11.967 23.837 1
24.064 19.547 1
25.27 16.528 1
-16.417 -44.371 1
2.1554 -47.988 1
16.36 -15.325 1
15.09 42.808 1
-14.455 8.0496 1
12.542 -29.567 1
-4.9997 22.747 1
-51.388 4.484 1
24.217 -3.4121 1
-22.878 -26.356 1
-25.331 -25.873 1
33.279 -22.878 1
-38.528 -15.34 1
36.179 -21.674 1
32.335 -24.474 1
-31.188 9.6372 1
-43.442 -17.429 1
4.9374 12.937 1
-2.3117 24.402 1
3.0597 12.721 1
-29.486 40.242 1
-2.7259 22.252 1
-39.787 20.952 1
-24.232 26.46 1
-13.236 -11.861 1
-7.8766 31.819 1
-4.9947 33.759 1
-37.381 19.031 1
-7.6214 -24.78 1
-21.851 19.759 1
-12.494 7.923 1
24.567 -1.3077 1
26.412 -41.462 1
12.8 -26.069 1
23.933 0.71492 1
-27.034 45.303 1
-3.7058 -28.163 1
-6.7062 33.203 1
-41.654 -17.986 1
42.068 10.681 1
4.3203 -49.815 1
-41.351 -11.793 1
13.688 40.948 1
-26.368 -26.433 1
2.0517 -45.761 1
48.846 8.742 1
23.907 -2.4511 1
-52.672 4.7034 1
48.685 10.482 1
23.342 -43.555 1
-19.884 21.359 1
13.288 -27.131 1
-1.1821 21.443 1
-5.6265 -23.127 1
2.7555 61.669 1
-11.973 22.557 1
-37.819 22.364 1
-4.4261 -26.042 1
-26.744 -7.1069 1
-14.558 -45.727 1
11.631 -26.191 1
-3.2554 22.476 1
-52.534 3.7946 1
-8.2423 31.371 1
-27.577 -4.6573 1
12.84 -28.959 1
20.57 1.6194 1
-10.824 9.6193 1
-16.588 -43.506 1
2.6559 -9.2484 1
34.47 34.21 1
-44.162 -13.866 1
-41.441 -14.709 1
5.9873 13.762 1
-27.502 -8.1917 1
-26.648 41.007 1
-27.524 -3.7673 1
1.9157 3.8631 1
7.0335 13.862 1
31.68 29.534 1
-16.158 -15.496 1
12.179 -31.29 1
-21.642 24.889 1
2.1137 -50.284 1
15.843 37.888 1
-25.286 41.575 1
-46.945 -0.55453 1
22.917 -1.5383 1
-41.058 -10.781 1
2.1576 -10.417 1
-17.769 -44.051 1
35.156 -25.818 1
9.8021 28.174 1
-14.159 -18.072 1
33.001 -23.455 1
46.075 9.365 1
25.033 13.094 1
-3.3417 -24.58 1
-8.2616 -26.916 1
-28.402 -27.493 1
-29.494 43.497 1
24.981 -2.822 1
15.636 -13.472 1
-5.5318 -26.456 1
8.2093 1.2708 1
12.071 -25.199 1
33.733 -23.395 1
-4.3316 21.791 1
-4.2687 35.385 1
-37.212 19.83 1
9.0757 1.3175 1
-3.3011 23.747 1
-27.131 -4.461 1
-27.795 46.953 1
32.517 34.92 1
-5.778 -1.7418 1
6.3573 -0.75767 1
43.158 12.856 1
32.622 29.893 1
0.39749 56.352 1
-35.274 17.934 1
6.3945 12.315 1
-22.696 19.261 1
10.364 -31.218 1
-5.2988 -26.648 1
22.166 -40.792 1
34.093 29.603 1
-15.633 -44.575 1
1.5482 57.72 1
-26.433 -25.689 1
4.9259 13.342 1
-22.181 25.251 1
-28.887 40.87 1
-41.023 -14.035 1
2.6158 55.501 1
-20.075 26.098 1
-23.212 -26.491 1
36.734 -27.446 1
-30.994 11.533 1
17.837 -13.639 1
-0.91122 -10.509 1
-39.927 21.068 1
7.8385 0.38311 1
26.402 15.007 1
33.84 -21.283 1
-42.412 -10.62 1
-12.88 -12.27 1
-13.891 -16.127 1
-5.4195 -22.841 1
-50.507 2.0077 1
8.8368 28.953 1
23.467 17.847 1
5.8505 -50.467 1
-14.663 -15.822 1
20.826 -0.43764 1
-27.384 43.31 1
40.476 -8.6772 1
-51.132 2.4426 1
-8.5226 33.93 1
6.8455 -49.08 1
-29.281 46.759 1
3.8138 15.172 1
-27.019 -31.647 1
-27.785 -6.0506 1
10.517 -31.715 1
37.908 -27.936 1
-27.713 -6.3736 1
-0.60417 23.339 1
-48.626 2.3218 1
23.236 19.088 1
48.839 11.046 1
-19.376 22.951 1
17.731 -13.979 1
-18.249 -16.171 1
16.363 42.263 1
37.038 -23.678 1
-3.8142 -28.191 1
-29.369 8.0401 1
22.934 -2.3124 1
-30.508 8.1891 1
-13.87 -45.168 1
32.313 -22.76 1
3.6923 61.598 1
44.924 11.754 1
-41.793 -17.641 1
-17.713 -14.387 1
2.2517 -13.251 1
-42.031 -16.501 1
44.644 12.951 1
39.608 -4.7545 1
0.67957 -6.1404 1
-9.3459 7.2794 1
11.353 26.216 1
35.58 -24.136 1
13.688 -27.45 1
-23.191 25.527 1
25.822 -2.3439 1
-9.2248 32.344 1
-3.7275 -26.162 1
38.135 -26.525 1
9.7949 4.5879 1
-10.6 11.282 1
24.717 -40.827 1
32.832 33.331 1
8.5571 4.2728 1
39.209 -4.5679 1
-12.342 22.556 1
10.841 26.022 1
26.078 1.4959 1
-16.533 -16.145 1
-44.451 -17.316 1
-42.833 -16.458 1
-13.518 9.7933 1
0.89023 -11.632 1
-24.791 -28.293 1
23.951 17.03 1
41.471 -4.8342 1
-11.374 22.304 1
15.546 -10.56 1
-15.687 6.8728 1
3.1807 -14.379 1
40.559 -6.3341 1
11.268 -30.277 1
-27.753 -2.9513 1
-14.185 -11.066 1
35.637 -25.755 1
-2.1931 -0.8968 1
-22.791 23.192 1
-30.1 8.105 1
-29.939 45.47 1
8.8993 -29.259 1
-39.928 -17.108 1
44.437 10.278 1
-16.141 -48.62 1
-38.998 21.194 1
16.577 40.929 1
-27.211 9.9808 1
1.6998 56.764 1
-30.576 13.413 1
-16.182 -48.55 1
-24.733 -24.767 1
-6.7269 -23.81 1
21.938 18.043 1
-49.698 1.3048 1
37.278 -8.3197 1
-52.631 2.3405 1
-24.655 40.654 1
-16.009 -45.007 1
48.938 9.6432 1
-26.195 -3.7466 1
1.6989 -44.866 1
8.8079 29.169 1
-6.7164 36.34 1
3.5276 -44.181 1
-50.614 3.6378 1
9.2547 3.8808 1
31.869 -23.563 1
-20.327 22.743 1
-27.541 -26.567 1
38.066 -22.733 1
-29.664 45.747 1
-26.566 -4.0901 1
46.587 12.922 1
-14.958 -45.641 1
23.427 -40.407 1
11.34 26.53 1
33.511 33.961 1
2.7012 61.573 1
-15.451 -15.904 1
48.261 10.058 1
-50.918 1.7367 1
-13.074 -15.899 1
8.5648 23.574 1
4.9764 56.935 1
-11.066 24.578 1
-8.8498 35.686 1
-51.806 3.4374 1
12.637 0.87467 1
42.469 11.993 1
-24.774 -26.791 1
-25.539 -26.752 1
22.992 -43.917 1
1.3606 -12.447 1
40.295 -7.7466 1
-13.834 -11.047 1
-14.689 -17.546 1
35.452 -27.224 1
-28.179 -3.8781 1
37.918 -26.283 1
25.629 16.5 1
20.875 -41.736 1
-13.135 7.6548 1
-3.7472 -27.945 1
23.921 -0.77301 1
-14.816 8.4557 1
40.987 -8.6922 1
37.9 -26.964 1
-9.1968 -26.376 1
-14.125 -18.135 1
11.057 24.961 1
6.216 -48.776 1
-48.353 2.0731 1
-1.391 0.1051 1
4.1134 -48.135 1
25.129 -39.663 1
-36.014 19.26 1
14.906 -14.31 1
22.054 -41.271 1
43.556 13.897 1
6.2638 1.466 1
11.552 24.159 1
-3.3253 23.494 1
44.931 10.205 1
-12.67 9.3237 1
-28.773 11.997 1
3.2992 14.53 1
3.2941 58.865 1
-13.74 -13.821 1
26.382 -1.4618 1
22.938 -39.96 1
30.474 29.988 1
21.849 -39.053 1
-16.544 -47.163 1
-22.351 -4.861 1
-23.586 -25.564 1
-47.857 4.6537 1
9.0682 0.34335 1
-29.031 10.486 1
5.7057 14.103 1
32.308 31.045 1
13.664 42.135 1
3.4677 56.632 1
44.95 12.77 1
23.359 -1.3635 1
-0.27374 -7.6541 1
-4.4705 -24.214 1
11.175 26.801 1
32.649 29.934 1
20.711 -40.22 1
-6.7192 31.965 1
-20.495 19.638 1
1.3503 -13.496 1
-51.994 0.55841 1
-29.449 43.645 1
45.905 10.869 1
-5.7289 -23.599 1
3.4104 -50.527 1
-13.692 9.5195 1
8.8267 -31.491 1
-50.222 4.1814 1
-15.469 -14.499 1
34.748 35.409 1
13.361 -10.931 1
39.116 -6.7015 1
-1.6136 -10.235 1
2.0791 57.194 1
-17.596 -15.001 1
25.116 -0.50652 1
-22.477 -28.566 1
-28.798 42.552 1
-2.0054 0.2937 1
11.15 -28.886 1
25.337 -38.922 1
3.3056 56.637 1
-3.0836 -24.25 1
24.437 -3.8784 1
1.6108 57.056 1
-42.957 -18.446 1
47.255 10.358 1
21.678 -39.228 1
-22.897 -28.663 1
-49.939 1.5312 1
-45.15 -17.057 1
-11.179 22.315 1
6.3469 -46.96 1
-39.396 23.022 1
-7.0334 32.459 1
-5.7758 34.334 1
4.1724 -49.005 1
-22.724 24.381 1
-16.141 -42.569 1
4.3904 -45.216 1
-26.602 -4.3477 1
-50.815 3.7543 1
-8.4168 -24.826 1
-14.217 -13.411 1
-29.522 43.999 1
-17.101 -13.98 1
-12.859 -11.592 1
40.398 -7.5613 1
1.3277 57.271 1
23.1 2.6721 1
17.666 -10.407 1
-1.2005 19.297 1
5.2492 16.979 1
-21.95 23.221 1
23.728 -2.3035 1
23.73 -1.2444 1
-11.65 11.781 1
44.706 8.6146 1
-41.155 21.467 1
-27.239 41.297 1
5.224 15.554 1
15.54 -9.5205 1
-15.647 -15.031 1
-8.1333 31.405 1
3.1055 58.794 1
-2.2548 22.014 1
49.32 10.881 1
-28.398 -30.288 1
8.0749 2.7002 1
-27.738 42.464 1
25.873 19.03 1
-51.894 3.5642 1
31.313 30.081 1
35.6 -6.6802 1
35.314 35.442 1
25.767 15.943 1
-3.0592 1.8676 1
46.862 9.9681 1
7.6404 26.876 1
-30.373 10.14 1
23.495 -3.8684 1
25.675 18.092 1
45.093 13.674 1
-29.489 46.732 1
3.4795 -47.548 1
22.274 -3.0749 1
-28.686 9.5408 1
22.671 17.48 1
-39.835 23.645 1
-27.268 45.246 1
-4.2865 -28.324 1
21.186 17.058 1
7.8517 14.343 1
7.691 1.9213 1
-42.185 21.495 1
22.752 -1.7441 1
1.7396 -46.357 1
-49.58 3.1291 1
26.866 14.574 1
-38.974 -14.58 1
-24.192 -2.8923 1
38.278 -6.7602 1
25.283 -41.433 1
35.642 -21.159 1
22.819 -42.864 1
23.714 -39.411 1
21.604 15.212 1
-16.837 -15.337 1
-21.412 23.38 1
-1.4985 3.8807 1
0.73727 -10.346 1
-9.4217 34.067 1
6.7453 -48.454 1
-13.432 -14.844 1
-4.122 -26.448 1
15.788 -12.177 1
14.297 -12.75 1
11.765 -26.164 1
4.5343 14.385 1
21.894 15.006 1
-22.585 -5.9775 1
15.547 38.599 1
-9.9476 30.559 1
0.084102 -9.8148 1
-16.973 -43.602 1
13.83 37.431 1
4.5943 14.294 1
2.6786 58.087 1
-24.568 40.512 1
9.9236 -25.464 1
-35.89 17.83 1
33.953 31.159 1
-6.6308 19.319 1
9.0543 26.803 1
-50.654 -0.69137 1
-26.773 -1.4926 1
2.174 -8.9767 1
10.419 -0.74078 1
17.277 39.633 1
13.584 40.784 1
-26.043 -30.014 1
-6.4319 30.565 1
-23.359 25.54 1
-15.677 -47.615 1
23.427 -41.103 1
-15.215 22.126 1
15.516 40.217 1
7.7663 11.72 1
47.65 11.556 1
45.966 10.255 1
3.6057 57.096 1
5.6866 -47.501 1
1.7203 -12.668 1
-13.327 -14.414 1
-24.042 -24.89 1
15.68 -13.499 1
-7.653 7.858 1
1.5342 -46.708 1
-22.823 -5.9934 1
-30.591 7.682 1
42.691 11.456 1
24.279 13.273 1
17.543 -14.593 1
25.335 -42.784 1
38.566 -6.6248 1
-21.718 -25.814 1
24.283 12.417 1
-11.756 22.406 1
-42.745 -14.441 1
1.9264 56.914 1
-25.14 -31.156 1
3.6639 12.32 1
-40.245 -13.276 1
-1.4262 4.1724 1
-6.026 -22.96 1
0.033822 57.393 1
-26.205 41.047 1
34.81 -22.126 1
-21.622 20.822 1
-39.162 20.585 1
1.5427 57.567 1
-31.099 10.018 1
42.748 10.067 1
-3.842 34.306 1
-14.343 7.4469 1
-40.161 -11.332 1
-16.824 -45.451 1
4.828 56.885 1
45.461 9.3004 1
36.089 35.703 1
9.1423 26.416 1
-12.979 9.7274 1
17.217 38.415 1
-48.077 2.2545 1
-24.83 21.517 1
-29.479 -30.803 1
-37.03 22.352 1
2.9557 -14.095 1
-41.443 -16.762 1
-28.605 -29.397 1
-42.472 -17.853 1
-3.5013 33.238 1
-16.05 -43.926 1
11.715 -28.522 1
12.696 -29.315 1
-27.994 -5.4492 1
-29.55 10.31 1
-25.334 41.679 1
-45.032 -16.255 1
15.769 43.396 1
31.649 32.292 1
-7.1735 33.755 1
-35.944 -12.893 1
-22.144 -3.1091 1
8.3422 2.0273 1
3.2131 -48.479 1
-29.253 43.421 1
-7.2714 35.128 1
36.036 33.091 1
-0.15766 18.759 1
-13.293 22.567 1
-52.453 2.6203 1
-3.8892 24.316 1
11.81 24.196 1
-11.757 6.3145 1
11.076 24.999 1
-10.077 9.7438 1
-3.1085 24.719 1
15.66 38.383 1
-49.172 4.1562 1
23.564 15.026 1
-13.332 -15.185 1
-26.271 -27.65 1
3.5469 14.221 1
1.0182 -9.9828 1
21.614 -40.585 1
2.7928 61.71 1
-39.954 -14.137 1
-36.922 18.786 1
37.248 -22.082 1
36.502 -24.157 1
-8.1363 31.786 1
-49.366 3.75 1
-26.535 -27.248 1
49.245 10.738 1
3.8421 -43.988 1
7.2994 12.04 1
34.978 -22.548 1
24.648 -41.562 1
9.1454 -31.638 1
-24.64 -5.4575 1
-43.954 -11.759 1
41.103 -7.9855 1
37.612 -5.8684 1
-14.018 -12.404 1
-16.997 -42.835 1
14.113 -10.686 1
2.6268 -48.249 1
35.631 -21.12 1
0.61355 -11.482 1
45.17 13.968 1
12.029 -32.317 1
6.2655 16.371 1
15.213 37.848 1
-51.558 5.1604 1
-46.409 0.68845 1
37.974 -27.795 1
17.112 39.956 1
32.261 33.111 1
8.5942 22.987 1
22.895 -38.312 1
39.572 -8.6905 1
24.395 12.01 1
5.6755 15.954 1
-28.133 -6.9208 1
5.6753 -44.447 1
10.504 -28.793 1
25.992 18.041 1
0.45036 -10.107 1
45.19 13.92 1
-13.118 6.4589 1
23.676 -42.759 1
-48.358 0.71352 1
-41.996 -13.498 1
16.417 -15.107 1
10.106 25.838 1
-29.607 11.263 1
23.926 13.572 1
-43.198 -15.731 1
-40.564 -13.963 1
3.902 1.5812 1
-21.093 22.276 1
-16.682 -46.475 1
16.093 40.127 1
-26.979 -7.8427 1
-30.116 12.519 1
7.6118 11.704 1
12.718 26.191 1
-22.203 22.621 1
1.3121 58.833 1
1.8003 -11.217 1
12.751 -28.77 1
2.6095 -47.771 1
-6.3046 34.837 1
2.1766 -44.243 1
-15.27 -13.983 1
47.276 10.175 1
10.787 25.732 1
-52.356 2.089 1
-49.944 1.4932 1
41.187 -5.2589 1
9.4619 26.137 1
-5.9986 34.069 1
-37.473 21.364 1
-30.335 11.685 1
37.618 -9.4557 1
-38.742 22.979 1
37.948 -7.9087 1
-27.676 -5.2708 1
1.1438 -46.041 1
37.09 35.017 1
2.8831 -46.056 1
-15.271 -43.907 1
9.8546 25.443 1
-27.993 11.195 1
3.4199 -48.779 1
-28.806 45.051 1
-7.4197 -27.004 1
-27.83 -3.2252 1
21.463 -0.69488 1
34.146 35.233 1
-36.54 21.545 1
-26.204 -2.502 1
-40.056 -14.511 1
-8.2898 31.843 1
-50.349 3.7128 1
6.4764 2.4922 1
26.867 16.803 1
1.058 -6.8103 1
5.0665 16.094 1
10.292 -33.103 1
16.15 -13.004 1
-13.782 -14.819 1
-23.644 24.055 1
-11.176 -12.594 1
22.756 14.982 1
-9.644 10.146 1
-12.555 23.503 1
-4.0224 23.088 1
-25.142 -5.2936 1
16.331 -10.392 1
5.5039 -47.906 1
9.5544 25.8 1
12.88 -31.53 1
-26.063 -28.897 1
6.7971 16.04 1
25.923 0.34585 1
13.191 -29.853 1
6.5002 15.736 1
-50.433 3.5003 1
-3.8042 23.681 1
0.39509 -12.176 1
-49.588 3.5018 1
16.472 -13.535 1
21.249 -39.812 1
-3.315 -22.256 1
-39.887 -13.887 1
10.852 0.53985 1
-5.2483 1.5498 1
-1.426 21.251 1
3.4854 56.84 1
17.584 -11.011 1
15.82 -12.577 1
24.117 18.495 1
5.0193 17.174 1
12.627 2.8161 1
48.387 8.3944 1
40.827 -4.3031 1
-16.542 8.2406 1
-6.2189 31.081 1
-3.8331 23.778 1
-46.941 -0.62559 1
-24.118 -27.363 1
-21.7 25.384 1
-26.073 -4.7514 1
-40.228 18.076 1
25.711 15.898 1
-25.305 -6.389 1
1.9229 -14.536 1
-9.0773 33.934 1
5.8315 13.965 1
-13.877 -43.995 1
34.521 32.85 1
13.785 -15.687 1
1.7391 57.282 1
7.1556 12.795 1
-30.351 42.349 1
-49.587 1.4029 1
-50.699 -0.76081 1
-41.096 -16.268 1
43.975 9.4257 1
-44.941 -16.207 1
19.145 -12.411 1
-39.38 -13.721 1
12.076 -26.978 1
47.098 10.865 1
2.6403 -12.756 1
-38.775 19.484 1
-6.1201 -22.879 1
-23.442 25.652 1
27.123 1.4469 1
-28.442 45.789 1
-2.8433 1.2 1
33.94 29.474 1
8.687 -31.151 1
-3.1893 -4.5872 1
27.017 18.585 1
-8.7214 31.853 1
-40.832 -13.234 1
-24.393 -6.6215 1
-37.984 20.42 1
14.653 -25.218 1
37.995 -25.735 1
-39.126 -13.658 1
-3.9434 24.293 1
38.672 -6.5914 1
22.859 1.0831 1
-31.394 9.4487 1
22.085 -42.375 1
5.5412 12.693 1
39.349 -5.1835 1
3.5036 56.038 1
24.5 -40.388 1
4.7119 1.8346 1
-12.427 -16.514 1
-42.51 -14.684 1
-23.669 -7.1421 1
23.215 1.4827 1
-1.5094 -13.31 1
-24.019 -7.092 1
24.036 -40.967 1
20.925 -42.084 1
-4.5086 -0.80498 1
0.55815 2.9822 1
-52.418 0.51089 1
24.982 2.6341 1
40.59 -7.7093 1
-39.943 -13.372 1
-7.7082 -23.732 1
-2.7334 5.1513 1
23.798 -0.24062 1
8.1894 24.293 1
15.812 -12.064 1
-16.834 -16.127 1
43.647 13.869 1
12.926 -26.867 1
15.515 -14.942 1
9.8985 24.962 1
47.472 13.337 1
4.7947 -49.09 1
48.096 10.554 1
30.864 29.594 1
-7.4951 32.96 1
9.826 -0.3237 1
22.258 -40.638 1
-12.809 23.333 1
13.262 -10.617 1
-4.7224 34.016 1
3.1565 -13.306 1
-3.6586 -27.933 1
-5.004 33.125 1
-42.62 -15.868 1
-28.407 40.685 1
-6.3617 32.972 1
32.428 31.272 1
-3.9747 -3.9704 1
-40.556 19.037 1
-53.661 3.1907 1
49.495 12.416 1
-27.71 42.206 1
34.564 30.888 1
25.21 13.149 1
-4.5038 -24.906 1
-24.951 21.62 1
-53.095 2.0853 1
-29.184 10.338 1
14.977 37.16 1
12.286 -31.123 1
-28.018 -25.66 1
-14.582 -48.192 1
23.393 16.693 1
14.069 -14.733 1
-16.103 -45.71 1
2.2541 -14.894 1
-35.505 17.518 1
-15.565 -46.264 1
-14.378 -45.971 1
22.59 1.1767 1
14.975 37.242 1
-15.336 -44.048 1
-20.416 22.847 1
10.525 -32.226 1
-4.0938 -1.1651 1
3.5269 -8.0757 1
16.791 -11.624 1
22.295 15.684 1
46.481 12.768 1
1.3566 -48.014 1
2.905 -13.903 1
-16.652 -16.278 1
-3.3593 -25.883 1
-25.392 -27.895 1
-37.544 20.579 1
2.9765 58.701 1
8.7159 25.485 1
-4.1987 21.517 1
-31.378 44.794 1
-40.483 19.953 1
-5.2932 31.823 1
-26.454 -6.9273 1
39.057 -6.9629 1
47.597 11.046 1
-3.7076 -23.971 1
24.696 14.751 1
-0.41179 -13.429 1
36.62 -27.208 1
-7.23 -23.321 1
-20.808 22.487 1
-24.565 -5.6479 1
7.9771 2.7692 1
13.942 -26.32 1
18.966 -12.426 1
2.1058 -9.5182 1
15.409 -9.6505 1
-20.381 25.248 1
-13.242 -44.772 1
-2.148 -12.788 1
-23.562 -30.906 1
35.875 -22.764 1
-50.083 0.56967 1
-28.636 9.566 1
8.8623 2.359 1
3.2594 -47.823 1
-14.983 -13.835 1
12.066 28.353 1
-22.382 22.223 1
36.009 -27.983 1
-9.701 29.494 1
-14.333 -44.341 1
23.894 -2.7686 1
-14.315 -10.963 1
-3.8891 -28.098 1
-26.846 -30.645 1
13.537 -25.422 1
32.128 30.72 1
-28.86 -4.9005 1
-2.7757 1.2358 1
-24.992 -6.2573 1
-13.825 -16.689 1
-2.3212 -23.563 1
-4.5646 -1.615 1
-35.09 20.975 1
6.7623 14.277 1
-11.287 6.9349 1
23.734 18.333 1
-49.566 2.225 1
-24.858 -31.359 1
-8.16 -23.21 1
-37.597 23.355 1
-15.845 -43.526 1
-50.233 4.7584 1
-13.902 -44.907 1
4.6912 13.889 1
14.179 -30.214 1
2.0914 56.429 1
-16.873 -14.252 1
36.502 -28.203 1
2.9098 -47.876 1
38.148 -7.9482 1
-39.734 19.723 1
-39.438 -13.734 1
23.009 -42.101 1
-3.3673 24.356 1
-42.25 22.529 1
-27.863 -29.297 1
-5.5847 33.129 1
-13.017 -13.791 1
21.308 0.12019 1
-17.456 20.824 1
1.6007 57.861 1
18.101 -11.982 1
12.268 -33.067 1
-14.324 -44.498 1
15.278 40.007 1
16.502 39.111 1
8.8354 -29.226 1
15.929 40.582 1
12.715 -26.024 1
-13.389 7.9602 1
18.988 -12.667 1
7.7767 10.979 1
1.682 60.74 1
3.6618 -26.372 1
6.0915 -51.057 1
35.729 32.436 1
-42.268 21.417 1
33.001 30.4 1
-5.2047 20.855 1
2.9883 58.78 1
23.918 -39.959 1
25.882 14.906 1
-2.3793 20.661 1
38.131 -8.7745 1
9.8871 24.061 1
35.564 33.892 1
14.811 -29.063 1
-14.953 -45.35 1
-49.89 1.5576 1
8.2991 25.392 1
7.1793 -1.1508 1
-24.774 41.509 1
11.556 -30.917 1
-2.7884 -4.9635 1
-50.875 1.6244 1
14.832 -9.9959 1
-38.94 18.314 1
35.993 33.625 1
22.942 -1.7655 1
-17.514 -43.309 1
25.917 -41.961 1
-25.548 -2.4655 1
-22.707 -4.1139 1
2.0768 56.391 1
-15.145 9.1451 1
-15.035 -44.716 1
-30.459 8.7501 1
49.09 11.789 1
-25.366 41.868 1
-22.353 19.261 1
-15.636 -45.696 1
32.605 32.668 1
11.629 -27.962 1
12.544 -28.067 1
-14.084 10.033 1
-27.504 -24.842 1
-3.3729 -4.1915 1
43.087 10.417 1
8.4482 -30.882 1
3.7068 61.712 1
-7.7315 -25.773 1
3.8954 16.161 1
-25.643 -5.2687 1
21.749 0.1028 1
-1.2131 4.1842 1
-26.147 -26.667 1
23.454 -42.072 1
-5.8146 34.058 1
10.748 1.2259 1
-30.474 10.008 1
5.1042 -49.102 1
-11.713 -13.734 1
0.53179 56.548 1
-37.193 22.683 1
3.5458 -46.555 1
-30.583 8.109 1
-25.57 -5.4721 1
-11.972 23.755 1
22.206 -40.158 1
-9.3459 30.26 1
-39.723 23.049 1
45.947 10.119 1
10.939 -29.728 1
-28.231 10.448 1
-29.941 45.609 1
1.1993 -13.372 1
31.568 31.746 1
-4.7534 -23.087 1
23.087 -39.285 1
-16.139 -46.587 1
-50.631 3.6748 1
-50.173 2.3243 1
5.3807 16.11 1
-36.558 22.11 1
-1.2209 -9.8026 1
17.837 -13.032 1
45.979 9.1236 1
25.1 18.733 1
-23.165 -26.491 1
-30.529 9.7334 1
14.583 -12.451 1
33.057 33.107 1
-44.775 -16.071 1
0.13733 58.426 1
-12.766 5.1696 1
3.4334 -44.849 1
6.2976 0.34808 1
2.017 -45.951 1
-12.255 22.325 1
-21.905 22.326 1
-15.306 22.05 1
15.437 37.64 1
40.311 -6.0628 1
-1.1603 -12.311 1
5.2107 17.088 1
6.3139 0.29011 1
33.619 -23.117 1
9.1951 4.0507 1
25.219 -41.086 1
-53.023 3.6607 1
-11.019 32.317 1
-39.106 -12.351 1
-21.571 21.293 1
34.775 -24.132 1
2.4062 -48.946 1
-11.132 7.1911 1
8.4759 4.172 1
24.4 15.659 1
-39.466 21.531 1
35.937 34.885 1
-24.548 -26.981 1
-41.808 -10.218 1
-21.645 21.743 1
-40.282 -14.254 1
38.767 -6.8547 1
-12.818 9.5832 1
43.558 10.339 1
-1.3391 -12.56 1
-24.194 26.486 1
1.5084 57.106 1
14.237 -14.951 1
-15.425 -42.719 1
12.082 -31.442 1
15.429 41.953 1
-4.9728 -23.152 1
24.005 1.6083 1
34.987 32.732 1
41.295 14.424 1
-13.781 -46.06 1
25.946 -42.325 1
-3.6881 23.499 1
-25.241 -29.908 1
-40.351 -17.453 1
-25.872 -27.594 1
35.148 31.888 1
13.377 -26.958 1
-14.65 -46.156 1
22.752 -0.16991 1
17.591 -13.794 1
26.299 -41.543 1
35.244 -21.645 1
24.442 1.4808 1
-0.53076 23.283 1
-6.741 -25.715 1
-11.998 22.189 1
5.8222 15.757 1
-14.572 -15.673 1
1.8673 -46.67 1
17.787 -14.718 1
-13.968 -48.057 1
-17.347 -15.719 1
-28.561 43.045 1
-25.128 -3.0807 1
35.554 -27.058 1
11.92 -29.075 1
10.495 -31.221 1
11.679 27.345 1
-12.693 23.244 1
-7.9464 -26.915 1
14.487 43.128 1
7.6419 0.047411 1
-45.152 -15.007 1
-21.406 21.808 1
-51.189 5.5028 1
3.186 61.742 1
3.7691 -46.491 1
-28.646 -30.174 1
43.839 9.9245 1
-12.294 22.114 1
-5.3546 -24.516 1
-47.814 3.6758 1
-15.579 -19.139 1
23.896 -42.543 1
-13.115 -11.746 1
3.884 -51.434 1
-12.992 11.94 1
15.975 -8.3661 1
-26.798 -1.6953 1
6.8165 -48.243 1
34.012 -24.162 1
-24.045 -27.691 1
1.5223 -12.876 1
-6.9212 31.406 1
2.3753 -10.517 1
15.424 -14.79 1
-22.572 22.971 1
35.553 33.893 1
-23.46 22.072 1
10.57 -27.305 1
7.5296 -49.455 1
10.34 0.14656 1
14.074 -12.333 1
-20.196 24.421 1
-37.153 18.019 1
-6.8356 22.84 1
-11.089 8.6776 1
23.815 1.2295 1
-30.365 9.3295 1
15.293 41.674 1
-18.241 24.3 1
-40.761 23.491 1
15.159 -9.7895 1
-6.2641 22.948 1
34.447 31.378 1
-1.6588 -12.001 1
4.8146 56.915 1
-7.2985 -24.801 1
-27.204 45.479 1
12.637 -26.076 1
10.488 -31.257 1
34.814 33.557 1
-4.7631 33.774 1
13.735 -15.777 1
-40.146 -12.423 1
14.9 -24.636 1
-39.791 -13.461 1
8.2221 28.802 1
0.65878 -13.429 1
9.7035 24.237 1
-21.331 22.331 1
40.729 -4.498 1
35.899 31.533 1
-51.547 1.4105 1
14.093 -29.042 1
37.026 -26.256 1
44.812 10.887 1
4.9118 56.501 1
48.155 11.238 1
-5.5914 22.695 1
24.423 -3.6042 1
23.048 -39.91 1
-42.784 -16.893 1
-4.1288 -25.704 1
11.344 27.983 1
36.756 -22.405 1
-8.1154 35.642 1
34.81 -23.554 1
-4.189 34.263 1
9.8751 4.7364 1
1.7594 55.871 1
-3.0359 0.81034 1
6.7248 0.57599 1
15.231 40.043 1
-51.338 5.3438 1
6.7749 -48.621 1
-27.854 41.856 1
34.999 -24.912 1
26.083 13.982 1
-8.7198 32.396 1
-29.939 42.466 1
-27.784 11.427 1
-2.8439 23.809 1
27.118 16.799 1
15.425 38.857 1
2.4962 -46.516 1
5.2977 -46.664 1
-24.329 -26.523 1
18.164 -12.46 1
13.633 -8.3797 1
-2.5517 0.76491 1
-14.253 -17.997 1
-9.5327 9.0458 1
44.238 11.095 1
31.989 -25.391 1
5.5149 13.305 1
-18.28 24.228 1
-42.699 20.352 1
26.027 -43.734 1
1.1744 -48.203 1
25.817 -2.5408 1
-30.773 40.939 1
23.483 17.976 1
-2.616 5.1624 1
25.161 0.29563 1
34.172 -23.968 1
-41.666 -12.487 1
25.593 14.078 1
-2.4874 -23.719 1
34.92 34.074 1
1.8602 -14.704 1
9.8971 -26.079 1
17.044 -9.9457 1
12.621 2.5561 1
-19.179 20.114 1
8.9137 -29.165 1
10.043 1.642 1
0.9229 -44.967 1
-1.4214 -2.3114 1
39.79 -5.1557 1
10.166 -32.794 1
-28.121 -5.1236 1
31.788 33.215 1
-23.114 21.173 1
35.139 -25.442 1
-40.868 19.269 1
-29.319 8.2681 1
33.807 -26.717 1
-6.6452 33.53 1
-28.211 -28.388 1
-52.528 1.5597 1
11.733 -27.06 1
49.34 10.824 1
-7.2979 -24.833 1
22.958 14.609 1
25.561 1.509 1
3.9129 61.7 1
-12.288 23.165 1
-26.592 41.025 1
-9.5374 -25.221 1
1.8922 5.4803 1
22.164 -42.927 1
23.299 -0.5197 1
-41.675 -10.088 1
40.213 -5.998 1
1.954 57.606 1
-14.436 -45.874 1
-26.476 -28.036 1
-13.271 11.365 1
-13.773 6.7955 1
13.208 -28.602 1
-25.061 -29.43 1
-39.055 20.409 1
24.229 14.036 1
24.444 -42.344 1
-25.7 39.292 1
39.542 -4.4627 1
13.964 -27.334 1
-13.497 -14.484 1
3.4308 2.1419 1
-6.029 34.838 1
-14.057 -47.812 1
-6.6386 -24.236 1
1.7703 -43.674 1
31.641 32.212 1
-13.894 11.713 1
-2.5542 24.359 1
24.212 13.9 1
5.5152 14.503 1
26.54 19.27 1
-24.154 -27.278 1
-27.075 -6.0445 1
-25.28 -28.286 1
-42.939 -13.884 1
13.437 -29.954 1
8.4027 1.3447 1
12.787 -26.343 1
-6.8384 31.978 1
-52.17 1.4797 1
-0.41649 23.309 1
40.149 -4.4324 1
-40.31 21.922 1
-2.477 20.669 1
8.8925 4.115 1
27.033 18.953 1
22.443 -2.4154 1
8.3146 28.868 1
-4.6518 33.695 1
-38.556 20.068 1
-26.661 -31.743 1
-32.527 13.032 1
12.213 26.782 1
41.874 13.984 1
-5.0108 -22.801 1
-14.584 -46.101 1
-27.398 43.238 1
11.884 -27.496 1
4.8438 56.938 1
-36.445 18.094 1
-0.1998 -11.398 1
22.071 17.259 1
-2.8433 1.2 1
-0.82012 -6.6559 1
4.5864 14.868 1
15.626 40.84 1
-41.074 20.908 1
25.988 -41.233 1
-7.9222 34.38 1
15.141 42.677 1
-15.703 -44.809 1
-30.025 41.325 1
-20.357 24.848 1
16.492 37.335 1
-27.491 46.853 1
-15.814 -14.534 1
21.872 15.758 1
3.1804 -44.376 1
-37.011 22.918 1
-13.54 10.978 1
13.864 -28.155 1
39.192 -5.801 1
4.6775 -45.396 1
47.347 11.167 1
24.816 -3.6422 1
1.1295 -46.794 1
13.697 -29.739 1
11.319 25.764 1
-11.076 6.8544 1
4.6968 14.747 1
13.995 -13.066 1
25.969 -1.7547 1
8.0159 14.376 1
21.395 0.6498 1
8.7862 2.8751 1
-24.989 22.834 1
14.652 41.492 1
-30.096 12.134 1
-10.559 7.476 1
-20.788 22.768 1
-1.4633 22.441 1
-38.449 20.051 1
-44.936 -17.106 1
-16.868 -46.035 1
-31.123 42.919 1
-17.649 -15.239 1
-17.1 23.865 1
22.336 -2.7074 1
43.379 9.9257 1
32.399 34.783 1
-48.088 3.2023 1
16.399 -14.751 1
2.8131 59.126 1
-4.4422 -28.23 1
-11.425 6.785 1
-38.377 19.13 1
12.962 1.3562 1
14.985 40.243 1
-22.865 -29.711 1
-47.544 2.7471 1
5.0521 12.097 1
22.718 -41.362 1
-50.316 4.2232 1
24.921 -39.51 1
-7.017 -24.792 1
22.808 17.177 1
-14.2 5.1952 1
-6.9458 22.816 1
-37.868 22.008 1
47.47 10.13 1
-5.481 -23.48 1
16.895 39.879 1
25.279 13.448 1
5.1469 -47.208 1
3.5437 -2.2167 1
2.3704 -10.649 1
-27.083 39.065 1
-14.152 -47.503 1
11.972 0.028037 1
27.098 16.752 1
15.211 41.455 1
11.257 -32.476 1
2.7145 61.616 1
-15.007 -45.392 1
0.81273 58.345 1
-29.36 46.351 1
34.793 -24.761 1
-23.712 23.05 1
12.109 -25.98 1
-27.403 -4.0269 1
-0.69326 -12.536 1
3.5893 55.448 1
-52.935 3.9581 1
-39.423 -16.854 1
23.043 1.0832 1
-44.7 -15.323 1
32.527 30.937 1
-38.464 -18.434 1
-12.181 23.007 1
-6.1247 -24.576 1
37.598 -8.1697 1
0.54125 -11.99 1
24.958 18.697 1
-13.062 8.8311 1
21.51 -41.925 1
-6.48 31.852 1
16.323 -11.491 1
-3.7116 24.267 1
24.127 -41.535 1
2.2967 -12.582 1
-27.258 46.151 1
47.234 9.7847 1
2.9831 61.683 1
-27.964 41.198 1
35.156 -22.638 1
7.5716 -0.27125 1
-26.773 43.22 1
12.578 26.894 1
-28.655 -7.5428 1
-21.467 26.024 1
-12.366 8.8886 1
24.17 -41.882 1
-20.954 -3.7236 1
33.898 33.72 1
-15.787 -44.377 1
36.081 -25.358 1
35.979 32.929 1
38.766 -5.9395 1
-15.537 -15.502 1
-3.7934 -24.795 1
15.592 40.708 1
32.86 33.737 1
-27.648 42.14 1
-1.6946 24.295 1
12.048 -31.303 1
-9.995 31.376 1
-26.304 -30.714 1
0.62554 -0.14271 1
-0.24546 -11.81 1
-12.749 -44.812 1
4.3282 -49.964 1
-30.491 45.934 1
-25.149 -6.0018 1
7.7962 0.04983 1
23.722 16.707 1
1.3634 -43.504 1
24.025 19.356 1
-28.875 -6.5444 1
39.818 -7.9148 1
14.53 -12.945 1
22.663 -2.8565 1
-15.532 9.2853 1
-9.5851 9.2288 1
9.2173 -0.86517 1
36.917 -22.594 1
-8.3864 -23.098 1
0.82019 -14.23 1
-27.147 -31.089 1
33.774 -20.858 1
6.0101 13.582 1
-8.4437 31.48 1
-14.904 10.734 1
16.603 39.618 1
26.621 17.492 1
-3.4197 -23.134 1
24.628 -3.6224 1
-36.323 17.882 1
-0.98578 0.89867 1
35.919 -26.043 1
2.8009 56.507 1
-27.476 40.689 1
15.031 -12.779 1
5.8842 14.534 1
0.025531 -13.516 1
-26.61 -25.922 1
-22.056 19.32 1
15.122 -12.441 1
34.756 32.821 1
2.3406 58.086 1
13.474 -30.926 1
-40.468 19.435 1
14.242 43.264 1
23.415 1.4868 1
-41.477 -16.727 1
-20.35 -23.823 1
48.782 8.4513 1
15.893 37.893 1
4.0784 -49.569 1
43.345 11.224 1
0.25245 1.7774 1
8.1071 3.3819 1
-41.803 -10.209 1
31.188 32.827 1
11.576 1.3546 1
34.612 33.767 1
-41.58 19.955 1
-40.948 -16.58 1
34.567 -20.876 1
-3.7259 2.5209 1
-24.25 -29.931 1
-4.9435 32.773 1
40.941 -7.0908 1
25.076 2.5959 1
-52.446 2.9609 1
15.102 -13.621 1
-5.6806 -23.469 1
-23.959 -28.956 1
36.72 -26.611 1
-29.09 10.763 1
25.018 0.23003 1
-25.852 -3.3813 1
44.133 12.142 1
-2.7726 0.41364 1
-49.554 2.9797 1
-23.043 25.525 1
-30.167 44.364 1
21.979 -39.08 1
38.065 -24.837 1
11.801 -31.424 1
41.52 -4.9744 1
12.799 -13.255 1
9.4344 26.419 1
38.044 -8.7292 1
10.322 23.778 1
34.339 32.881 1
4.725 13.192 1
15.242 39.988 1
3.2483 -11.952 1
-14.37 -46.287 1
-47.903 2.1842 1
27.1 17.109 1
-0.88772 1.8356 1
4.2347 58.854 1
11.872 1.351 1
-40.727 -18.355 1
21.558 15.44 1
14.249 40.747 1
-16.645 -47.131 1
1.8184 59.019 1
-23.945 -25.208 1
33.276 32.242 1
-44.307 -15.248 1
42.647 12.961 1
33.483 29.644 1
17.283 41.367 1
20.664 -39.179 1
-30.183 9.4868 1
-39.05 -13.729 1
-3.6441 23.427 1
-26.09 -2.3063 1
6.3306 -46.144 1
39.561 -4.9867 1
6.3309 -45.86 1
15.022 41.087 1
-16.94 -15.23 1
22.704 15.552 1
22.994 0.014775 1
-15.018 -13.174 1
-42.948 -16.008 1
34.687 -21.184 1
27.018 18.343 1
5.8203 16.464 1
10.529 2.1914 1
16.081 -10.074 1
40.408 -4.8807 1
11.729 26.212 1
-15.759 -42.34 1
-5.5931 36.155 1
-10.779 11.41 1
25.641 15.6 1
-25.66 -6.6825 1
31.989 31.534 1
1.8696 57.113 1
-27.533 41.324 1
-14.001 6.2641 1
-17.215 23.328 1
4.3613 15.314 1
-16.131 8.9269 1
-15.163 -13.679 1
45.867 11.144 1
-1.9391 -3.728 1
34.02 30.334 1
-28.495 -5.5992 1
-4.4017 -25.981 1
-28.326 8.5452 1
-2.7638 4.337 1
8.8032 5.0676 1
-28.134 -7.6645 1
21.988 -40.36 1
4.184 59.546 1
21.96 18.28 1
-7.4456 -25.331 1
4.1298 11.985 1
-26.728 -4.9128 1
43.761 13.547 1
-46.774 0.71313 1
-44.084 -14.013 1
10.317 -26.779 1
-10.056 8.4317 1
0.94101 -6.4342 1
-17.255 -43.568 1
23.066 0.43927 1
-12.522 -12.064 1
-23.253 25.586 1
9.006 25.075 1
-11.023 8.5706 1
1.4729 -13.369 1
34.571 31.693 1
42.826 11.227 1
23.273 13.366 1
21.859 1.2133 1
22.167 -38.708 1
-35.859 19.43 1
27.032 1.3552 1
-39.602 21.648 1
-29.851 46.125 1
-29.851 41.435 1
1.4291 -11.758 1
-37.559 23.682 1
10.002 25.853 1
-9.3802 7.2925 1
-27.255 -29.517 1
21.202 -42.084 1
-28.593 -27.848 1
11.83 -28.881 1
-14.147 -18.101 1
24.048 17.651 1
4.8628 -48.264 1
13.663 -13.184 1
22.889 17.191 1
12.209 2.6597 1
-12.784 -14.124 1
-49.104 2.6461 1
27.363 18.461 1
15.71 40.09 1
15 39.067 1
35.812 -26.829 1
34.917 34.893 1
24.357 -41.846 1
-23.936 -29.232 1
-43.948 -15.676 1
-29.588 9.2379 1
31.329 30.478 1
-47.887 1.9492 1
-6.932 -27.56 1
46.142 12.585 1
-41.441 -13.643 1
34.524 -25.771 1
2.7167 59.171 1
14.073 -8.882 1
24.701 2.7201 1
23.995 15.007 1
-26.842 41.99 1
-1.7114 3.9471 1
-13.221 -44.903 1
6.6205 13.101 1
43.677 12.141 1
-51.127 1.7585 1
5.5573 15.911 1
-13.429 -15.581 1
-8.8621 8.4159 1
2.0121 -43.809 1
35.676 31.226 1
-20.222 21.113 1
-1.5445 4.3928 1
4.2816 1.594 1
25.095 2.2226 1
3.4557 14.156 1
16.25 40.993 1
-3.8392 -24.188 1
43.259 10.53 1
44.112 10.924 1
-4.1517 24.539 1
14.793 41.413 1
-41.807 -11.861 1
-47.214 2.6785 1
-27.242 -3.5982 1
-28.367 8.5277 1
48.532 10.053 1
14.938 42.793 1
7.1798 -0.070269 1
5.8075 16.33 1
5.1728 -46.515 1
-23.606 -4.8794 1
17.945 -12.571 1
-27.074 41.514 1
39.092 -6.9999 1
36.274 -25.081 1
8.4714 0.45104 1
-28.61 -30.372 1
39.695 -4.3451 1
32.673 -25.624 1
-4.7882 -25.126 1
-11.806 7.1002 1
7.7957 28.129 1
-25.641 -5.4188 1
-29.377 10.764 1
-30.784 9.7357 1
-3.8568 24.258 1
3.7425 -48.933 1
22.916 13.42 1
14.834 -10.992 1
10.53 26.638 1
12.16 -28.777 1
-13.059 22.58 1
-37.781 20.799 1
-37.968 19.067 1
-41.792 -17.275 1
5.3461 13.46 1
14.239 41.868 1
-3.5465 22.68 1
1.6105 -11.827 1
7.9273 26.346 1
4.0082 -46.851 1
12.02 -28.006 1
-14.488 -12.89 1
32.001 28.969 1
-22.164 19.297 1
9.0221 4.8849 1
-9.6225 34.059 1
44.229 10.543 1
-49.492 2.2158 1
-3.273 22.613 1
1.9096 4.3814 1
-26.924 -29.145 1
-5.8494 3.3669 1
7.6486 -49.733 1
3.4403 59.244 1
36.199 34.409 1
41.042 -8.7326 1
-24.463 -5.6126 1
-6.3531 34.65 1
3.4311 -44.979 1
-43.63 -14.351 1
24.439 0.35563 1
-24.566 -27.066 1
33.483 -24.648 1
-25.075 -29.255 1
-27.905 -5.3987 1
8.5946 4.8195 1
-22.963 -29.382 1
-12.731 -14.578 1
-5.4225 -25.239 1
15.349 43.32 1
-20.462 21.21 1
-3.5576 22.646 1
-17.226 -14.931 1
-20.058 19.409 1
34.4 -21.858 1
-11.571 2.7046 1
-21.01 25.73 1
21.806 -39.424 1
6.4251 -50.372 1
-25.985 -27.33 1
-16.928 -16.97 1
3.2491 61.926 1
-13.24 11.544 1
-3.5917 21.515 1
22.462 -41.868 1
-13.393 -15.419 1
13.008 -10.441 1
35.394 -23.606 1
-17.667 -16.249 1
48.185 11.203 1
-20.481 19.976 1
-23.893 -2.3091 1
-9.8175 29.12 1
-25.703 -26.316 1
1.127 58.026 1
-13.069 11.497 1
-21.676 22.775 1
2.511 -14.58 1
-13.051 8.6616 1
-35.462 18.711 1
-30.722 44.367 1
-43.083 -18.354 1
25.707 14.51 1
21.243 -43.28 1
-16.426 -14.521 1
14.75 -13.706 1
11.495 27.578 1
-21.534 25.129 1
-30.579 8.0861 1
33.264 34.463 1
25.054 -42.521 1
16.261 41.51 1
-23.125 -5.9538 1
5.5133 -45.616 1
17.084 -11.471 1
-2.8434 1.1964 1
36.521 -24.366 1
11.181 3.5717 1
36.39 -24.943 1
0.73174 -13.431 1


==> data_san_1.tex <==
x y label
44 -1 0
-13 -40 6
-37 -14 8
-36 -22 8
-7 -28 6
49 -2 0
12 -2 5
26 -40 4
10 28 9
-35 -22 8
44 2 0
-13 -41 6
-12 -44 6
-37 -41 1
11 24 9
45 3 0
16 11 5
17 -7 5
10 28 9
27 -42 4
45 -1 0
-8 -39 5
-38 -21 8
-8 -27 6
-7 -29 6
25 -38 4
-39 -43 1
-13 -11 8
44 -29 2
-13 38 7
47 -23 2
28 -40 4
-12 -41 6
-16 3 9
-14 40 7
-14 38 3
-6 -29 6
-12 -40 6
-14 -41 6
48 -2 0
-37 -19 8
43 -26 2
27 -44 4
-41 -39 1
25 -41 4
-13 -40 6
25 -42 4
47 0 0
-10 41 7
-27 22 3
44 -24 2
-34 -19 8
-36 -21 8
12 -4 5
13 -9 5
-26 24 3
-11 40 7
27 -42 4
-12 -40 6
47 0 0
-8 42 7
-13 -45 6
45 -24 2
-37 -20 8
-10 -43 6
-15 -38 6
12 -4 5
-35 -42 1
-10 40 7
-34 -17 8
-39 -42 1
-37 -41 1
-31 25 3
-38 -43 1
-28 23 3
14 25 9
-9 40 7
-12 -39 6
27 -40 4
-13 42 7
-9 -38 6
-38 -41 1
-37 -21 8
-13 1 9
-36 -44 1
-6 -29 6
11 48 6
-40 -38 1
-29 26 3
-40 -39 1
14 -5 5
47 -22 2
45 2 0
45 -23 2
-29 21 3
-10 -38 6
28 -42 4
28 -40 4
7 25 9
-40 -42 1
-17 -42 6
26 -41 4
46 -2 0
-9 39 7
14 -8 5
-40 -41 1
47 -28 2
-9 18 5
-8 41 7
47 -29 2
-11 -38 6
-38 -16 8
45 -21 2
-12 -39 6
-41 -40 1
12 26 9
-16 -45 6
28 -40 4
43 -23 2
15 -4 5
-12 37 7
-27 22 3
-36 -20 8
47 0 0
-26 23 3
24 -39 4
-15 42 7
46 1 0
-25 22 3
-27 25 3
45 -3 0
11 -3 5
-29 27 3
14 -8 5
-12 36 4
46 -23 2
45 -29 2
26 -44 4
-25 22 3
15 -5 5
17 12 9
45 2 0
-37 -19 8
44 2 0
-35 -22 8
-30 23 3
-14 -42 6
12 -4 5
12 -5 5
-7 39 7
12 -9 5
13 25 9
-11 41 7
25 -40 4
-27 22 3
-7 -30 6
44 -26 2
-8 -1 5
15 28 9
22 1 6
-6 39 7
29 -41 4
-37 -16 8
12 -9 5
46 -21 2
11 24 9
43 -25 2
27 -41 4
-37 -22 8
13 -6 5
48 -5 0
11 28 9
27 -42 4
-12 -39 6
-29 22 3
10 28 9
-14 39 7
26 -41 4
46 -22 2
-12 44 7
46 0 0
-8 -27 6
-26 26 3
-28 24 3
43 -21 2
-14 -46 6
16 -6 5
-26 23 3
-11 41 7
-25 22 3
-25 -28 0
45 -23 2
-17 -6 3
43 -22 9
-38 -22 8
45 -1 0
-10 42 7
46 -23 2
10 26 9
-10 41 7
45 -23 2
-38 -21 8
-42 -38 1
53 12 9
45 -2 0
15 -5 5
-35 -23 8
43 -24 2
-15 -44 6
10 25 9
49 -2 0
-37 -20 8
-40 -41 1
-31 26 3
27 -42 4
-27 24 3
-12 -3 9
-11 -43 6
-12 42 7
25 -41 4
-16 3 9
-9 -3 6
11 24 9
-3 -27 6
46 1 0
-40 -40 1
12 28 9
-38 -42 1
-38 -42 1
26 -41 4
-13 42 7
16 -7 5
41 -25 2
16 -6 5
46 0 0
-37 -21 8
-14 -45 6
-9 41 7
44 -22 2
14 31 9
13 25 9
-12 -40 6
-12 42 7
-9 41 7
-9 42 7
-35 -42 1
-38 -20 8
14 -6 5
10 27 9
46 -23 2
-13 -39 6
14 -5 5
44 2 0
46 2 0
-37 -43 1
47 -24 2
-9 42 7
47 -1 0
13 -3 5
-37 -18 8
45 0 0
-36 -21 8
-12 -40 6
58 15 9
16 -5 5
-11 -38 6
26 -37 4
41 -24 2
-28 22 3
-14 -42 6
22 1 6
17 12 9
43 -23 2
-16 3 9
12 -4 5
44 2 0
48 -4 0
27 -43 4
-28 22 3
47 -22 2
47 -24 2
26 -38 4
-8 40 7
-13 -40 6
-28 23 3
-37 -16 8
-8 40 7
11 28 9
-37 -20 8
-11 -43 6
13 -5 5
10 26 9
45 -21 2
-30 26 3
10 26 9
-27 22 3
19 12 5
-27 20 3
-36 -17 8
12 -2 5
28 -39 4
12 29 9
-9 39 7
43 -29 2
-26 25 3
-28 27 3
-25 22 3
12 29 9
44 -29 2
14 28 9
-9 43 7
27 -42 4
-13 41 7
-14 42 7
45 -27 2
-12 40 7
-40 -43 1
42 -27 2
23 -40 4
27 -39 4
14 -8 5
-41 -38 1
12 27 9
-27 21 3
45 -25 2
13 28 9
43 1 0
-13 -38 6
-37 -19 8
-2 -3 1
-14 -45 6
15 -7 5
44 -27 2
-40 -42 1
24 -41 4
-14 -41 6
-11 39 7
45 3 0
45 -23 2
-35 -17 8
14 -3 5
13 28 9
42 -27 2
26 -41 4
-10 38 7
47 -3 0
11 -5 5
-40 -41 1
-9 -38 6
-40 -41 1
12 -5 5
-26 21 3
-13 -45 6
-13 44 7
-37 -18 8
13 29 9
-40 -39 1
-41 -40 1
-13 38 7
45 3 0
-29 23 3
-28 21 3
30 -41 4
-27 22 3
-15 -43 6
-13 43 7
-36 -17 8
-8 41 7
13 29 9
-10 39 7
47 -26 2
-41 -39 1
44 -24 2
44 -25 2
11 -5 5
-43 -42 1
-37 -42 1
48 -25 2
43 -2 0
26 -44 4
14 27 9
43 -27 2
-12 -40 6
27 -36 4
-15 -43 6
-9 42 7
16 -7 5
-38 -22 8
-30 24 3
-15 -46 6
12 -4 5
29 -39 4
-8 40 7
14 -5 5
45 -29 2
-23 23 3
-34 -22 8
-10 42 7
-10 40 7
42 -26 2
45 0 0
-30 24 3
-29 23 3
-14 -44 6
25 -39 4
-7 40 7
-12 42 7
45 -26 2
-12 -38 6
12 -5 5
27 -43 4
-37 -21 8
14 27 9
-38 -15 8
-14 43 7
-27 27 3
29 -40 4
-25 24 3
-9 41 7
11 -7 5
12 -7 5
46 -2 0
14 26 9
11 26 9
43 -2 0
12 29 9
10 -6 5
14 30 9
-14 -45 6
-27 23 3
-42 -39 1
-36 -22 8
-36 -16 8
16 28 9
47 -23 2
-28 25 3
-10 43 7
10 28 9
-35 -21 8
13 -8 5
-2 -3 7
11 25 9
13 -6 5
15 29 9
-31 26 3
45 2 0
-25 25 3
-41 -39 1
47 -5 0
-37 -21 8
46 0 0
-36 -41 1
27 -42 4
-26 19 3
-38 -41 1
-27 21 3
15 28 9
12 26 9
-9 -39 6
46 1 0
11 -10 5
30 -38 4
12 29 9
29 -43 4
-35 -21 8
14 25 9
-42 -38 1
14 26 9
-27 22 3
-41 -38 1
29 -41 4
-32 25 3
-8 40 7
-10 39 7
45 -2 0
41 -25 2
45 -24 2
43 0 0
49 -2 0
-37 -41 1
27 -38 4
11 -3 5
12 -3 5
-27 20 3
11 25 9
46 -22 2
48 -4 0
-37 -20 8
-11 -39 6
-13 -39 6
-37 -19 8
46 -25 2
-27 21 3
47 -4 0
-29 25 3
-28 24 3
-34 -17 8
13 31 9
11 29 9
46 -24 2
29 -38 4
-12 -38 6
12 -4 5
17 -7 5
-11 43 7
-11 37 7
46 2 0
-40 -38 1
41 -24 2
26 -38 4
46 2 0
-35 -23 8
46 -4 0
47 -26 2
29 -39 4
-38 -15 8
12 26 9
-37 -18 8
-8 39 7
31 -40 4
14 28 9
43 -29 2
-13 -44 6
44 -23 2
45 -23 2
-14 43 7
-13 40 7
46 -22 2
-39 -41 1
26 -37 4
-11 40 7
-11 43 7
10 -6 5
12 -9 5
45 1 0
14 -9 5
-28 25 3
-11 41 7
-14 -43 6
-34 -21 8
-9 42 7
-12 -42 6
-13 41 7
27 -38 4
-31 26 3
-38 -15 8
-12 -40 6
25 -43 4
13 31 9
9 27 9
44 -3 0
14 -5 5
47 -1 0
15 27 9
-8 39 7
45 -21 2
14 -8 5
-12 -40 6
15 -5 5
44 -3 0
-13 -40 6
16 -5 5
44 -24 2
11 26 9
-12 -40 6
15 29 9
14 31 9
15 -7 5
13 27 9
13 -5 5
15 29 9
44 1 0
13 -7 5
14 -5 5
44 -25 2
-13 -45 6
14 -5 5
-26 21 3
-42 -40 1
-11 39 7
49 -4 0
-9 -37 6
-7 39 7
30 -42 4
30 -39 4
27 -41 4
-13 -43 6
43 -25 2
-11 -39 6
47 -2 0
-13 -38 6
26 -39 4
-29 25 3
45 -28 2
11 -3 5
-39 -41 1
46 0 0
-11 -41 6
-36 -18 8
45 -23 2
-1 -2 8
-8 42 7
42 -26 2
-12 -39 6
-29 26 3
48 -1 0
47 -27 2
-7 39 7
-14 43 7
15 -9 5
-30 24 3
-13 -41 6
-26 24 3
29 -41 4
-38 -14 8
13 -3 5
12 -4 5
-36 -15 8
-36 -42 1
-39 -39 1
-10 39 7
-37 -15 8
-37 -42 1
14 29 9
45 0 0
11 -6 5
24 -41 4
-28 25 3
-13 -45 6
-30 22 3
-26 24 3
-12 -38 6
26 -37 4
43 -5 0
26 -43 4
-42 -39 1
-37 -22 8
14 -10 5
-37 -19 8
-29 24 3
-35 -16 8
11 -5 5
15 28 9
-37 -42 1
-38 -14 8
-14 -46 6
-37 -21 8
-10 43 7
12 28 9
14 30 9
-2 -5 4
-37 -2 5
-37 -42 1
44 0 0
-29 27 3
16 28 9
-32 26 3
-37 -3 6
-39 -20 8
27 -40 4
48 -3 0
-28 26 3
12 -9 5
-12 -42 6
-38 -15 8
44 -21 2
30 -42 4
-10 42 7
-13 -45 6
-23 9 3
12 -3 5
29 -39 4
-34 -19 8
-38 -14 8
29 -43 4
-36 -43 1
46 2 0
-38 -21 8
42 -25 2
-13 -39 6
-8 41 7
46 2 0
-37 -22 8
-38 -40 1
43 -26 2
46 0 0
-12 39 7
-9 -38 6
46 1 0
-37 -15 8
46 2 0
-38 -40 1
-15 -41 6
11 -4 5
11 -5 5
-7 39 7
13 -3 5
47 -22 2
-43 -38 1
-13 43 7
45 -4 0
14 28 9
-38 -16 8
-38 -22 8
47 -21 2
-39 -41 1
47 -27 2
-10 37 7
30 -40 4
-13 -40 6
46 2 0
46 -2 0
46 0 0
-34 -19 8
-29 23 3
29 -41 4
-36 -43 1
44 -24 2
-38 -16 8
28 -37 4
16 29 9
15 -9 5
46 -1 0
-14 -39 6
45 -1 0
12 -2 5
-38 -15 8
46 1 0
43 -28 2
-33 -18 3
-31 26 3
-29 25 3
-37 -15 8
-29 27 3
-36 -20 8
29 -41 4
27 -43 4
13 -7 5
-38 -20 8
-15 -42 6
14 27 9
30 -42 4
-39 -41 1
45 -25 2
-11 -42 6
46 -4 0
-38 -43 1
46 -4 0
-37 -42 1
42 -23 2
13 -9 5
-9 39 7
-28 23 3
15 30 9
-9 -39 6
-11 -38 6
-7 41 7
-5 -9 9
-13 43 7
-9 41 7
-42 -40 1
-37 -19 8
15 29 9
-4 -8 9
48 -2 0
-9 40 7
44 -3 0
-16 -45 6
-38 -16 8
-17 -43 6
11 -3 5
-9 39 7
-39 -40 1
-36 -17 8
13 -8 5
45 -1 0
-9 39 7
42 -24 2
-27 23 3
-30 26 3
41 -24 2
26 -44 4
15 27 9
24 -42 4
-3 -6 9
-14 -42 6
-7 39 7
-12 40 7
27 -43 4
-40 -40 1
-41 -40 1
27 -38 4
13 -5 5
-26 22 3
48 -3 0
14 -10 5
15 28 9
13 28 9
27 -42 4
13 -5 5
14 30 9
10 -4 5
-38 -18 8
-37 -15 8
47 -23 2
46 -2 0
13 29 9
-12 -38 6
-13 43 7
47 -2 0
42 -26 2
46 -22 2
44 -22 2
-12 -38 6
13 30 9
43 -29 2
11 -6 5
-6 39 7
45 -5 0
11 25 9
26 -41 4
44 -26 2
-38 -40 1
-3 -3 4
-15 -43 6
28 -42 4
47 -4 0
11 -10 5
-11 -41 6
16 -6 5
45 -1 0
26 -42 4
-29 23 3
-31 25 3
8 25 9
-8 41 7
13 26 9
25 -40 4
-28 27 3
-26 23 3
29 -42 4
45 -26 2
-29 26 3
46 -3 0
26 -41 4
-38 -42 1
-13 -44 6
13 -9 5
45 -28 2
47 -2 0
-38 -20 8
13 -5 5
13 29 9
-34 -19 8
-38 -18 8
29 -38 4
-29 27 3
-12 44 7
-15 -43 6
-28 26 3
-10 42 7
-28 23 3
-36 -22 8
44 -26 2
27 -40 4
-38 -41 1
-34 -21 8
29 -41 4
11 26 9
42 -24 2
-28 25 3
-28 24 3
11 -3 5
-39 -16 8
10 28 9
-14 -44 6
-13 -44 6
-16 -43 6
-25 23 3
-26 26 3
25 -42 4
17 -7 5
-36 -18 8
-40 -38 1
-34 -21 8
12 -7 5
45 1 0
11 -6 5
15 -6 5
-38 -21 8
-9 40 7
-28 22 3
-37 -42 1
10 -6 5
-42 -39 1
43 -28 2
10 30 9
13 -7 5
14 29 9
14 -3 5
-8 39 7
42 -24 2
-39 -41 1
-8 40 7
49 -4 0
41 -25 2
-38 -39 1
46 -21 2
-30 21 3
24 -38 4
-12 -42 6
30 -39 4
-36 -19 8
-8 39 7
12 -5 5
12 29 9
-15 -44 6
11 -4 5
-9 41 7
-12 40 7
11 -3 5
-36 -17 8
-8 42 7
-39 -39 1
13 24 9
-30 25 3
-39 -42 1
-36 -43 1
-37 -42 1
11 -3 5
-41 -38 1
-31 24 3
45 1 0
-11 38 7
-42 -38 1
-42 -38 1
-15 -44 6
-27 26 3
-30 26 3
-26 23 3
10 -9 5
15 -7 5
12 26 9
-12 41 7
-36 -43 1
-33 -21 8
12 28 9
8 25 9
44 -29 2
-13 -43 6
0 -2 5
47 -3 0
10 27 9
25 -38 4
12 30 9
-13 -41 6
-38 -21 8
47 -1 0
12 -8 5
0 -2 5
-37 -16 8
-38 -14 8
47 -3 0
15 28 9
16 -6 5
14 28 9
-13 39 7
-36 -15 8
29 -41 4
12 27 9
25 -39 4
46 -1 0
45 -3 0
27 -40 4
43 -29 2
13 -5 5
44 -24 2
46 -5 0
11 29 9
-38 -15 8
-27 23 3
-10 43 7
14 -5 5
-36 -19 8
-31 26 3
-12 -43 6
-28 24 3
23 -39 4
-10 -39 6
12 -6 5
31 -39 4
45 -23 2
45 -22 2
-37 -14 8
-38 -22 8
-42 -41 1
-15 -44 6
14 27 9
-40 -41 1
-39 -19 8
-15 -38 6
13 -5 5
14 -9 5
12 -9 5
24 -37 4
-14 40 7
-29 26 3
28 -39 4
29 -40 4
-10 38 7
43 -27 2
47 -5 0
-24 23 3
9 26 9
-40 -40 1
-13 -41 6
-30 25 3
14 29 9
10 24 9
-40 -40 1
28 -41 4
-40 -40 1
26 -43 4
-36 -43 1
49 -5 0
28 -43 4
46 -26 2
-12 41 7
-7 40 7
14 -5 5
-13 -44 6
49 -5 0
-27 22 3
-12 42 7
-37 -16 8
46 -5 0
-10 41 7
14 26 9
-38 -19 8
-8 42 7
-10 -38 6
-42 -38 1
-14 39 7
-30 24 3
-37 -19 8
-31 23 3
14 26 9
-13 -38 6
-30 27 3
-14 -41 6
-8 42 7
-10 40 7
14 -6 5
-34 -21 8
25 -40 4
-29 27 3
48 -2 0
16 29 9
-12 42 7
44 -3 0
28 -39 4
14 28 9
-15 -38 6
-14 -44 6
46 -27 2
-36 -17 8
14 -5 5
-41 -40 1
27 -38 4
47 -21 2
26 -39 4
48 -5 0
25 -41 4
28 -42 4
26 -38 4
-38 -14 8
-42 -40 1
13 -4 5
-12 39 7
-36 -42 1
-13 43 7
27 -38 4
43 -22 2
27 -43 4
-38 -19 8
43 -24 2
10 25 9
46 -24 2
-14 -43 6
-4 -5 7
46 -23 2
45 1 0
30 -41 4
30 -40 4
-13 -42 6
15 28 9
-38 -39 1
26 -44 4
-16 -41 6
45 -21 2
-14 -43 6
25 -42 4
-38 -39 1
-13 -42 6
-15 -44 6
-12 43 7
-28 25 3
16 -9 5
44 -29 2
44 -24 2
-14 -42 6
-12 -43 6
-39 -19 8
15 -7 5
-12 39 7
13 26 9
27 -37 4
-11 -39 6
-27 20 3
12 29 9
-27 25 3
-9 -39 6
-37 -15 8
-27 23 3
-27 23 3
11 28 9
-11 42 7
-30 23 3
-27 22 3
46 1 0
-39 -39 1
11 27 9
29 -41 4
44 -27 2
48 -6 0
-12 -40 6
30 -42 4
-28 22 3
47 -22 2
48 -5 0
-38 -42 1
-16 -41 6
-13 43 7
46 -4 0
-26 24 3
48 -25 2
-13 37 7
-37 -20 8
25 -43 4
-26 20 3
-36 -16 8
-11 40 7
-36 -43 1
46 -24 2
-38 -16 8
45 2 0
-14 43 7
44 -3 0
-37 -14 8
-37 -17 8
-32 26 3
13 26 9
14 -8 5
26 -41 4
13 28 9
43 -26 2
-42 -41 1
-38 -15 8
29 -41 4
-39 -40 1
44 -1 0
-37 -15 8
12 -9 5
-17 -42 6
25 -37 4
28 -41 4
-16 -45 6
-37 -18 8
-36 -19 8
14 27 9
-38 -22 8
16 -9 5
-14 42 7
46 -25 2
-14 -41 6
46 -22 2
47 -1 0
-11 -42 6
-13 -41 6
26 -39 4
-38 -41 1
15 29 9
43 -24 2
-27 23 3
-16 -41 6
25 -42 4
-26 22 3
-16 -44 6
46 2 0
-11 42 7
10 25 9
-10 -37 6
-36 -42 1
-12 -39 6
-38 -40 1
-39 -41 1
47 -27 2
45 -24 2
43 -25 2
13 -4 5
48 -5 0
-37 -14 8
-13 39 7
-43 -41 1
26 -40 4
13 26 9
48 -3 0
-8 41 7
-39 -42 1
-9 38 7
11 -3 5
-30 24 3
-14 -39 6
46 -2 0
-37 -42 1
45 -29 2
-3 -4 9
-29 26 3
10 -3 5
44 -21 2
47 -4 0
-27 27 3
46 0 0
-14 -43 6
25 -37 4
12 -6 5
-14 -41 6
-14 39 7
10 26 9
12 -10 5
47 -2 0
45 -27 2
45 -5 0
-37 -14 8
46 -5 0
28 -39 4
43 -24 2
-15 -42 6


==> data_san_2.tex <==
x y label
44.071 -1.1572 0
34.501 36.464 0
7.8491 40.672 0
-14.561 -2.9214 0
4.5095 -47.946 0
-13.029 -39.581 0
-37.204 -14.487 0
-11.429 4.722 0
0.064064 -12.709 0
-36.157 -22.183 0
-0.024301 -13.867 0
14.732 22.392 0
1.1667 10.569 0
-42.749 -4.0427 0
27.425 -16.717 0
-6.745 -28.32 0
48.594 -2.0073 0
33.362 18.867 0
12.237 -1.9804 0
-11.512 22.639 0
26.123 -18.404 0
25.703 -39.95 0
10.433 27.602 0
-27.657 -20.035 0
-35.169 -21.614 0
43.603 1.7822 0
55.192 15.45 0
-13.136 -40.892 0
31.242 20.897 0
29.192 -15.821 0
-11.904 -43.912 0
-29.301 38.874 0
2.58 12.996 0
29.839 17.702 0
-36.879 -41.319 0
25.819 -15.693 0
-11.269 21.541 0
9.2864 42.702 0
29.16 0.4068 0
-11.64 23.304 0
44.108 -4.9835 0
11.186 23.987 0
30.789 15.963 0
45.095 2.6743 0
-1.013 13.566 0
44.886 -25.942 0
15.808 11.068 0
16.62 -6.6029 0
10.346 27.688 0
-19.023 -9.809 0
27.098 -42.247 0
29.03 -17.418 0
45.428 -0.87147 0
-8.3968 -38.673 0
33.149 17.225 0
-13.405 21.936 0
-38.061 -21.118 0
8.9076 43.224 0
29 -1.2401 0
11.883 46.174 0
-28.207 40.337 0
-7.7422 -27.044 0
-6.895 -28.763 0
24.743 -37.559 0
-38.811 -42.525 0
-13.353 -10.992 0
44.052 -28.934 0
0.82409 -16.532 0
27.219 15.048 0
-12.867 37.829 0
46.929 -23.056 0
30.723 32.954 0
-47.321 15.836 0
-25.581 5.3949 0
13.937 10.692 0
-27.65 -19.437 0
-27.417 4.6375 0
14.418 -29.661 0
-47.403 15.269 0
30.688 20.023 0
28.132 -39.972 0
55.52 11.103 0
-12.481 -40.661 0
-15.63 2.7585 0
32.728 16.95 0
1.9744 -14.718 0
-13.637 39.984 0
-13.575 37.766 0
32.48 15.385 0
-5.7851 -28.845 0
51.658 13.045 0
-18.14 -10.377 0
-12.986 -9.629 0
-11.835 -39.659 0
-30.721 38.078 0
-14.374 -41.221 0
48.346 -2.1314 0
-37.265 -19.456 0
31.3 18.228 0
29.611 1.8897 0
42.596 -26.463 0
-12.62 3.7907 0
18.757 5.668 0
29.256 17.28 0
-40.403 2.747 0
0.70144 -14.11 0
-17.404 -8.8093 0
-12.998 19.326 0
16.431 10.016 0
26.622 -43.752 0
13.141 10.129 0
-40.643 -38.724 0
-32.475 -18.15 0
25.234 -40.855 0
28.52 15.764 0
-12.676 -40.499 0
24.621 -42.334 0
6.3075 43.686 0
-15.845 1.4417 0
-31.29 42.779 0
28.346 -0.60646 0
-7.188 -9.0686 0
55.969 13.687 0
-30.218 42.602 0
46.775 -0.16158 0
-1.5925 -10.032 0
47.456 -5.9796 0
4.677 -53.491 0
-9.6746 40.717 0
1.157 -13.589 0
-27.108 21.545 0
-10.271 -2.0111 0
43.624 -24.26 0
-19.021 -10.704 0
-26.713 -25.953 0
-31.213 39.617 0
9.07 44.627 0
-34.448 -19.057 0
-7.8258 -28.734 0
28.795 1.3704 0
-42.71 -0.10218 0
-36.308 -21.1 0
11.703 -3.6633 0
-41.311 -3.1048 0
-42.528 2.6602 0
2.5011 -47.641 0
12.536 -8.6028 0
-27.254 -20.732 0
-6.1055 -27.544 0
-25.997 24.353 0
-11.432 40.34 0
26.907 -42.364 0
-12.426 -40.115 0
-28.392 42.764 0
46.943 0.0092432 0
-9.7018 4.8605 0
-11.34 22.528 0
-7.9256 41.904 0
-42.925 -0.90796 0
11.219 45.421 0
-13.377 -45.027 0
45.072 -23.59 0
-14.158 2.8626 0
10.914 46.092 0
35.94 35.438 0
28.087 -18.335 0
-37.199 -19.966 0
2.6067 -50.167 0
-10.412 -42.552 0
1.2199 -16.371 0
-15.008 -38.13 0
7.9298 43.79 0
32.886 35.919 0
31.085 15.908 0
-8.7102 -26.828 0
11.526 -4.3583 0
-35.225 -42.203 0
-13.395 -7.5818 0
-11.138 4.7281 0
-9.6739 39.665 0
-41.031 0.53904 0
18.317 9.8228 0
-34.052 -16.96 0
-39.382 -41.811 0
33.493 33.387 0
5.1616 -46.607 0
-31.215 -20.78 0
-36.673 -40.736 0
-30.584 25.339 0
31.545 19.797 0
-44.78 -1.2275 0
-37.502 -42.542 0
-27.826 22.931 0
14.145 24.979 0
4.0327 -50.936 0
-28.821 6.7069 0
-8.748 40.112 0
4.3249 -51.884 0
-12.007 -39.42 0
27.924 -0.41539 0
-9.9039 -25.775 0
-8.0175 19.988 0
26.573 -39.708 0
-12.599 41.985 0
-2.6373 -15.313 0
5.3057 -46.814 0
-9.1759 -37.537 0
16.158 13.863 0
16.078 -29.105 0
2.2877 -53.14 0
32.615 16.669 0
-37.868 -40.858 0
14.695 12.758 0
-36.847 -20.508 0
-12.607 1.3957 0
3.0539 -47.492 0
-35.73 -43.753 0
-7.2927 -9.9647 0
44.044 -27.665 0
-9.5963 25.807 0
27.131 -19.29 0
-14.489 4.378 0
-5.8483 -28.969 0
-3.9583 12.395 0
11.475 47.606 0
27.527 -17.665 0
-40.379 -38.209 0
-27.343 -20.352 0
5.2127 -46.977 0
-25.736 -20.225 0
5.3016 -47.767 0
4.2196 -51.336 0
-29.33 26.332 0
35.484 36.032 0
-39.813 -38.553 0
14.25 -4.8553 0
46.57 -21.658 0
2.2531 9.7732 0
-10.726 22.663 0
31.635 -0.51589 0
29.485 2.7104 0
44.559 1.9949 0
-37.468 -2.2115 0
44.682 -22.927 0
-31.222 38.911 0
5.6652 -50.212 0
-29.387 21.463 0
-10.146 -38.155 0
-28.594 42.96 0
1.8824 8.6877 0
28.496 -41.574 0
-43.824 -1.6844 0
-40.208 3.3216 0
-25.571 -20.61 0
5.0094 -46.924 0
28.025 -19.711 0
-33.116 -18.278 0
33.454 18.516 0
-12.23 -8.3152 0
26.718 -0.57806 0
28.195 -40.394 0
7.4735 25.23 0
-39.589 -42.467 0
-17.183 -42.164 0
0.50796 -14.247 0
7.0348 -47.239 0
26.144 -40.89 0
45.806 -2.0793 0
27.009 -18.279 0
-24.903 7.2246 0
-26.748 -19.81 0
-39.985 0.30707 0
9.7572 48.56 0
-9.0561 38.697 0
13.623 -8.323 0
36.693 34.294 0
32.502 35.904 0
-7.7941 1.2063 0
-31.132 40.07 0
31.541 -2.7435 0
-40.333 -41.234 0
27.073 -19.157 0
47.218 -27.551 0
-9.2511 17.781 0
-29.486 38.214 0
-28.255 4.8459 0
-7.8164 41.153 0
9.2739 49.106 0
29.223 -1.9834 0
46.581 -28.978 0
-11.347 -38.092 0
-37.606 -15.932 0
16.56 9.9789 0
31.354 -14.133 0
45.152 -21.492 0
-28.934 -30.621 0
-11.814 -39.132 0
0.76094 9.798 0
-41.414 -39.508 0
12.418 26.487 0
-15.671 -45.324 0
-9.4114 22.057 0
-17.481 -10.594 0
10.701 42.61 0
28.067 -40.081 0
-10.446 3.201 0
-11.586 23.466 0
43.405 -23 0
14.562 -3.7241 0
-12.064 37.194 0
33.119 34.178 0
-26.945 21.551 0
-35.583 -20.278 0
30.786 18.602 0
57.262 16.153 0
47.018 0.12284 0
-43.747 -2.6194 0
-25.555 22.983 0
24.158 -38.573 0
-14.538 42.415 0
3.7541 -53.056 0
-36.975 -0.40047 0
45.724 1.3758 0
43.966 -4.7969 0
25.221 1.0549 0
9.0398 40.442 0
-29.554 40.822 0
33.895 18.355 0
-25.44 21.577 0
-27.418 25.211 0
-25.754 -28.349 0
4.4487 -51.092 0
44.672 -2.9687 0
43.528 -25.826 0
11.41 -2.9051 0
-43.908 -2.4776 0
30.354 -16.56 0
-28.91 26.619 0
14.142 -7.7485 0
-11.385 -2.1987 0
-12.237 36.252 0
29.224 -16.035 0
46.408 -22.644 0
7.1292 -47.572 0
44.994 -29.426 0
-41.58 -3.1386 0
-7.097 -26.971 0
25.669 -43.802 0
9.0866 41.877 0
28.771 16.601 0
27.337 -17.604 0
-25.356 21.982 0
15.357 -4.6379 0
17.427 11.798 0
-8.9546 25.134 0
44.622 2.3717 0
1.2774 9.2085 0
13.773 13.402 0
-2.8889 -11.618 0
-37.156 -18.906 0
34.531 36.989 0
-14.656 5.2363 0
15.624 10.172 0
43.963 2.4537 0
-37.05 -1.34 0
-34.625 -21.833 0
-30.082 22.574 0
-14.491 -41.88 0
-14.777 -12.449 0
11.673 -3.8578 0
-47.519 15.742 0
12.007 -5.1129 0
-7.4469 38.915 0
-28.205 4.8599 0
6.8831 -48.513 0
0.32132 12.411 0
-6.3701 -23.632 0
34.284 38.852 0
0.42895 13.681 0
11.834 -9.0304 0
-42.131 0.38088 0
13.237 25.407 0
8.5408 48.798 0
-28.36 8.3737 0
-14.986 3.7031 0
-26.803 -30.327 0
30.792 -14.328 0
-10.632 41.094 0
25.008 -39.644 0
-16.255 1.7281 0
-12.972 0.94115 0
-26.694 22.142 0
-7.436 -30.152 0
44.476 -26.053 0
-7.8743 -1.1847 0
14.53 28.337 0
22.279 1.0097 0
29.44 -14.325 0
-29.849 41.607 0
-39.955 -3.4094 0
-6.1131 39.104 0
1.9142 10.693 0
-39.906 -0.59651 0
-15.856 -10.78 0
-29.803 39.387 0
28.643 -41.279 0
4.6477 -50.79 0
-37.116 -15.8 0
-0.054665 -11.249 0
15.472 -28.593 0
-2.8987 12.259 0
57.256 14.702 0
11.915 -8.5462 0
33.482 18.976 0
44.499 -25.855 0
46.194 -20.689 0
27.309 -14.455 0
-41.394 1.6741 0
55.138 10.213 0
-30.911 -17.155 0
46.859 -3.4745 0
0.50636 12.051 0
-7.2142 -27.025 0
-14.118 38.345 0
1.8759 12.156 0
-9.9845 25.688 0
-30.074 40.931 0
11.441 24.45 0
-29.076 36.793 0
51.545 16.375 0
-4.9167 -26.491 0
-43.086 0.02361 0
42.695 -25.054 0
1.8755 -12.377 0
27.37 -40.896 0
27.681 -15.199 0
-41.578 1.2159 0
-39.964 -3.3825 0
28.519 15.247 0
-9.1966 22.481 0
-42.993 -1.1075 0
-30.074 38.517 0
-37.188 -22.486 0
-28.81 40.812 0
-0.25283 -13.789 0
0.82396 16.978 0
-0.81341 13.02 0
-1.4651 -12.502 0
-7.4874 -25.695 0
12.722 -5.6233 0
-1.2619 12.587 0
27.65 -0.69194 0
-28.717 42.167 0
-1.8318 -15.825 0
48.349 -5.2753 0
11.066 28.389 0
29.753 19.584 0
13.822 -29.685 0
27.222 -42.206 0
-11.712 -39.077 0
-40.362 2.7041 0
54.155 13.906 0
-29.186 22.395 0
8.9893 46.925 0
-5.9828 -28.649 0
45.908 -3.4681 0
10.075 27.654 0
14.502 9.7814 0
-14.111 38.831 0
16.418 -29.612 0
27.596 17.625 0
26.444 -41.38 0
30.571 16.686 0
28.167 1.1269 0
2.3495 15.355 0
27.172 15.054 0
-42.708 -0.22858 0
45.702 -21.666 0
-27.523 6.2545 0
27.038 -19.241 0
-28.764 -31.033 0
-30.379 39.324 0
31.245 -1.8694 0
-12.174 43.708 0
-11.369 1.1692 0
26.461 -0.82919 0
45.882 0.20268 0
-10.609 -0.76555 0
0.68404 10.162 0
-7.9033 -26.67 0
-25.507 25.521 0
-27.664 23.88 0
47.133 -5.7923 0
-26.222 7.8917 0
43.459 -21.459 0
-14.033 -46.018 0
15.665 -5.8078 0
33.709 36.739 0
-12.354 4.1221 0
-14.707 -12.247 0
6.4994 -48.516 0
-27.145 8.8428 0
-25.5 22.647 0
-1.1106 10.223 0
-10.619 41.276 0
28.985 15.667 0
-25.393 21.757 0
-30.067 43.866 0
-24.977 -27.824 0
-17.071 2.753 0
1.747 -12.51 0
45.007 -22.866 0
-5.4151 -25.756 0
-16.796 -6.2055 0
42.887 -21.685 0
-30.797 39.138 0
36.89 36.519 0
-25.686 8.9285 0
-37.789 -22.259 0
44.852 -0.71233 0
-9.7446 41.7 0
12.059 -27.818 0
-27.307 -20.513 0
-16.736 4.0104 0
1.9723 -53.203 0
45.538 -22.883 0
-28.351 11.236 0
10.304 25.805 0
-43.923 0.21727 0
47.716 -23.43 0
3.2908 -13.314 0
-14.612 -3.1595 0
-10.097 41.291 0
46.087 -26.153 0
9.2205 44.434 0
3.4174 -45.387 0
43.972 -27.604 0
1.0469 -14.963 0
-1.9445 12.985 0
1.1181 -13.838 0
3.2618 -54.589 0
57.253 16.295 0
-8.463 25.222 0
31.354 -16.11 0
44.703 -22.573 0
28.021 -2.8858 0
1.9312 15.621 0
-2.0305 16.456 0
-38.301 -20.698 0
-43.85 -0.85401 0
-26.994 6.6388 0
13.261 10.136 0
-40.946 -2.2206 0
-42.251 -38.325 0
52.844 12.306 0
-0.1817 10.74 0
45.185 -2.0983 0
5.0636 -49.714 0
30.413 -1.3721 0
15.025 -5.2419 0
27.888 0.77904 0
13.58 -29.524 0
14.759 10.899 0
-4.8932 -27.686 0
-15.325 -10.093 0
-35.075 -23.271 0
52.162 14.848 0
42.544 -23.89 0
-15.144 -43.739 0
-28.173 9.0334 0
-28.552 -28.233 0
2.4639 14.574 0
-49.669 14.17 0
10.169 25.074 0
54.765 10.923 0
48.724 -1.8268 0
-36.762 -19.57 0
0.76029 9.7092 0
-25.978 -27.178 0
3.1514 -49.53 0
0.35207 -15.066 0
35.993 34.971 0
-28.594 39.63 0
8.7615 45.362 0
11.204 42.502 0
-40.251 -41.273 0
8.3661 47.939 0
-30.808 25.973 0
47.859 -23.181 0
27.331 -42.05 0
-0.33017 10.295 0
-27.015 23.892 0
-12.095 -2.5281 0
-11.369 -42.528 0
1.6329 -15.966 0
-42.733 -0.8431 0
-11.529 41.842 0
-42.804 1.7755 0
56.869 16.037 0
25.083 -41.103 0
-15.601 3.216 0
-17.901 -9.3266 0
-9.4102 -3.1234 0
-29.701 -29.46 0
10.924 23.801 0
-18.672 -11.093 0
9.1997 46.222 0
-42.084 0.29431 0
27.536 -2.6341 0
1.3046 13.487 0
-1.4719 11.551 0
-29.248 40.838 0
2.6759 14.031 0
52.661 14.906 0
-3.3062 -27.319 0
45.872 0.79734 0
-9.5617 -28.756 0
-40.06 -40.248 0
-43.544 2.4272 0
30.551 16.599 0
54.349 12.606 0
-8.8102 24.895 0
27.856 1.8352 0
-0.22318 12.13 0
11.765 27.952 0
17.311 -29.505 0
-37.853 -41.795 0
-37.565 -41.607 0
1.4455 -51.118 0
25.638 -40.828 0
-12.802 42.393 0
-11.377 21.824 0
16.01 -6.7334 0
41.043 -24.868 0
16.157 -6.3988 0
-27.705 9.5045 0
27.789 0.52153 0
46.276 0.11186 0
57.38 14.859 0
-19.711 -10.984 0
-7.5158 -25.13 0
-8.4789 25.555 0
-37.045 -20.704 0
-13.899 -45.467 0
-8.835 41.146 0
43.617 -21.746 0
-26.781 -20.563 0
43.512 -28.367 0
13.535 30.785 0
-15.734 -7.5397 0
12.841 25.251 0
-11.986 -39.605 0
-26.607 -19.962 0
-11.699 41.916 0
9.9716 46.801 0
28 16.407 0
43.879 -28.092 0
54.084 15.526 0
-9.2339 41.016 0
-9.3964 41.692 0
49.165 -3.6784 0
-35.5 -41.724 0
-27.33 -29.501 0
-12.641 1.0271 0
-2.0876 -13.447 0
-37.61 -19.649 0
-14.87 -6.9441 0
25.77 -1.7211 0
5.1098 -45.864 0
-43.972 3.3665 0
-9.9218 22.695 0
-11.533 6.225 0
13.837 -6.3935 0
10.327 27.321 0
45.861 -23.08 0
-13.42 -39.377 0
13.554 -4.5428 0
47.325 1.1841 0
44.29 1.9371 0
45.549 2.4574 0
-42.549 -3.4146 0
-36.909 -42.724 0
-0.63614 10.076 0
46.526 -23.694 0
-2.7698 -16.187 0
-8.7415 41.743 0
5.3453 -47.766 0
46.75 -0.61411 0
12.899 -2.7157 0
-36.529 -1.5531 0
0.40063 -49.738 0
-16.083 -9.2383 0
-41.675 1.2192 0
-27.655 41.713 0
-37.269 -17.62 0
-40.279 2.6227 0
45.406 0.46767 0
46.319 -5.6056 0
-36.415 -20.649 0
27.505 -15.568 0
29.324 1.6357 0
-12.169 -40.174 0
-13.554 2.101 0
58.454 15.046 0
11.251 46.293 0
-12.158 -2.7216 0
-1.1347 -16.085 0
3.7237 -48.921 0
-7.1971 23.34 0
6.2471 -50.353 0
15.986 -4.7066 0
0.5629 -14.232 0
27.131 -1.8101 0
-10.889 -38.109 0
25.516 -36.504 0
41.425 -24.293 0
28.209 15.286 0
-47.639 15.266 0
-10.983 22.612 0
-28.254 21.981 0
-13.74 -42.435 0
22.439 1.0576 0
2.5059 -52.226 0
43.411 -26.613 0
-24.169 -26.813 0
0.40197 12.093 0
27.746 -0.18538 0
1.0715 -9.2743 0
16.855 11.671 0
43.199 -22.952 0
30.27 1.9694 0
49.058 -3.5111 0
-27.774 -19.896 0
-15.778 3.1852 0
-12.835 36.918 0
11.755 -4.2812 0
-4.9283 -27.618 0
44.442 1.7504 0
48.425 -4.1182 0
26.922 -42.749 0
-27.679 21.902 0
-26.563 41.756 0
-11.911 22.719 0
-16.616 -6.4108 0
-5.5263 -8.1398 0
46.916 -21.913 0
27.37 -2.1038 0
31.917 19.328 0
-27.487 9.2766 0
33.23 19.652 0
46.92 -23.668 0
28.481 2.3814 0
26.004 -37.614 0
-7.573 39.973 0
-10.078 20.84 0
-47.975 15.361 0
28.323 -19.596 0
-0.68893 12.279 0
-13.375 -40.056 0
-28.485 22.826 0
-36.73 -15.821 0
-5.6144 -25.182 0
17.916 -28.423 0
32.665 16.803 0
6.4326 -48.028 0
-8.0924 40.481 0
-12.148 -8.4812 0
46.486 -4.3153 0
10.663 27.848 0
-41.072 2.1364 0
-36.845 -19.554 0
2.5067 10.449 0
16.375 10.89 0
-27.835 -29.369 0
2.3183 10.177 0
-11.348 -42.937 0
-27.262 7.5166 0
30.451 -19.438 0
-18.395 -8.2868 0
14.36 -27.94 0
12.916 -4.6561 0
10.324 26.009 0
-29.559 7.9823 0
45.396 -21.4 0
2.0445 -49.928 0
-29.695 25.768 0
13.628 12.924 0
3.5172 -12.293 0
-6.005 -26.009 0
54.896 14.751 0
5.1774 -45.831 0
5.2174 -47.061 0
3.2556 -51.33 1
10.206 25.89 1
-25.921 7.7242 1
-26.789 21.928 1
-3.0816 -13.717 1
25.898 -0.3409 1
-45.069 1.9508 1
5.9307 -49.636 1
30.904 19.166 1
55.821 15.821 1
1.5382 14.431 1
19.212 11.825 1
-26.593 19.998 1
-35.59 -17.466 1
11.883 -2.3716 1
52.955 14.574 1
-5.1097 -26.357 1
0.69608 -12.799 1
6.8139 -48.042 1
28.261 -38.661 1
5.532 -50.952 1
12.426 28.853 1
10.958 44.161 1
-51.266 10.948 1
-12.122 24.992 1
30.282 -16.483 1
1.2343 9.7032 1
4.872 -49.314 1
-24.718 -20.22 1
-42.41 2.6023 1
-13.942 5.1223 1
36.144 36.01 1
29.99 13.872 1
32.676 35.706 1
16.301 -28.863 1
3.7148 -13.467 1
-8.9965 39.15 1
-27.189 7.2179 1
-14.169 -8.5711 1
2.9877 11.178 1
43.192 -29.369 1
29.81 17.838 1
28.818 -2.3852 1
4.8061 -52.266 1
31.405 32.997 1
53.89 13.931 1
7.882 45.631 1
-15.181 -10.734 1
15.411 9.145 1
-24.724 6.1307 1
33.361 36.91 1
-32.397 -17.656 1
-26.237 -30.331 1
34.094 38.946 1
34.815 33.255 1
-29.247 40.479 1
5.141 -50.925 1
-1.8386 -2.7316 1
34.95 33.918 1
-3.0926 15.378 1
34.312 35.529 1
-50.268 10.204 1
52.078 15.008 1
-26.306 24.731 1
-28.104 27.179 1
-24.94 21.878 1
12.088 29.007 1
43.517 -29.014 1
-27.529 7.3575 1
17.06 13.079 1
-9.5206 21.9 1
8.0521 47.345 1
14.373 27.952 1
-26.357 8.938 1
-9.1574 42.94 1
26.782 -41.615 1
-26.786 -28.883 1
-13.453 40.952 1
-9.9238 21.185 1
-9.9535 4.6576 1
-13.551 42.138 1
15.657 10.479 1
44.746 -27.159 1
-11.919 40.359 1
-25.614 -28.086 1
31.042 -14.967 1
-4.0291 -28.016 1
28.211 17.202 1
-39.844 -42.674 1
27.071 -1.752 1
-1.0238 15.172 1
42.229 -27.173 1
55.859 13.162 1
1.3606 10.538 1
23.377 -39.567 1
31.601 -16.149 1
-8.9966 -0.42433 1
-48.068 12.626 1
31.417 -14.469 1
27.267 -38.545 1
29.271 1.794 1
-13.28 3.9625 1
-26.862 6.8678 1
50.741 13.73 1
14.34 -8.2128 1
4.5118 -50.38 1
-47.651 15.355 1
4.135 -49.023 1
-40.501 -38.264 1
12.485 27.11 1
-23.802 -28.106 1
25.575 -0.29547 1
19.756 -28.112 1
28.526 -16.904 1
14.162 -26.956 1
-27.096 20.976 1
-30.614 39.021 1
1.2673 10.047 1
-28.781 41.174 1
32.274 16.152 1
45.282 -25.468 1
13.294 28.202 1
43.253 1.1038 1
8.4823 43.723 1
29.304 15.909 1
4.0562 -47.776 1
15.814 6.5412 1
30.267 16.927 1
-12.589 -37.901 1
6.419 -49.298 1
-36.94 -18.552 1
-1.9235 -3.2225 1
-10.552 22.941 1
-13.899 -45.431 1
32.958 37.829 1
15.01 -6.9195 1
43.72 -27.143 1
-40.727 0.67895 1
-39.794 -42.067 1
24.124 -40.928 1
14.598 4.8736 1
-7.6329 24.174 1
-8.7479 -24.62 1
-14.486 -41.343 1
12.938 7.3971 1
-25.873 -30.112 1
-11.296 39.297 1
24.916 -2.8034 1
26.692 -17.907 1
-37.756 0.94595 1
33.522 32.052 1
15.109 10.965 1
36.023 35.1 1
-4.1389 -6.1097 1
-44.548 -0.072607 1
-29.41 8.2774 1
44.9 2.5994 1
44.868 -23.139 1
-4.0624 -29.916 1
-35.006 -16.921 1
13.841 -3.2731 1
12.925 27.728 1
-43.369 -0.68091 1
11.721 44.74 1
54.127 14.642 1
-12.345 21.738 1
26.243 0.14357 1
-8.9069 23.898 1
-6.8057 -6.0682 1
31.083 -2.4789 1
-2.5293 -28.367 1
41.671 -27.235 1
26.216 -40.869 1
-29.146 38.363 1
10.786 42.955 1
-27.982 42.502 1
32.869 32.785 1
4.4412 -45.791 1
-40.554 3.6096 1
3.4695 -13.557 1
30.241 14.9 1
-9.7519 38.173 1
46.845 -3.4617 1
-31.151 42.633 1
-3.0387 12.226 1
35.454 35.094 1
-26.394 -30.724 1
17.296 7.5842 1
11.234 -4.8737 1
34.773 35.265 1
-29.927 42.465 1
15.455 -28.361 1
-40.234 -41.095 1
-9.2676 -38.452 1
-40.374 -41.09 1
34.682 36.311 1
12.477 -4.6413 1
-26.163 21.379 1
5.4123 -49.434 1
-4.6317 -28.035 1
-12.654 -45.194 1
4.5566 -49.554 1
29.261 20.243 1
9.817 43.821 1
-14.968 -8.8223 1
13.222 -28.039 1
18.518 -28.527 1
-13.491 43.596 1
-9.8559 -26.41 1
-37.466 -18.292 1
-16 -8.0683 1
12.66 29.234 1
-1.1111 15.002 1
-16.3 -7.6606 1
-16.181 2.6472 1
-1.046 -11.99 1
-39.858 -39.432 1
-41.379 -40.355 1
36.176 33.284 1
1.6227 11.545 1
-12.829 37.856 1
44.945 2.862 1
-28.685 22.825 1
8.2802 46.675 1
-28.824 9.1964 1
-28.29 21.127 1
31.04 17.977 1
-1.8353 -2.7341 1
2.3468 14.129 1
28.546 0.24828 1
-17.436 -9.2487 1
-2.9525 10.467 1
30.299 -40.974 1
-12.533 1.411 1
-50.426 12.765 1
-9.8395 2.1856 1
9.1245 41.037 1
16.657 11.073 1
-6.2866 -26.959 1
-15.458 -9.4288 1
-10.904 20.367 1
-26.878 22.411 1
29.628 15.725 1
4.1321 -12.917 1
-14.57 -42.962 1
17.383 8.5875 1
-1.873 -3.743 1
-13.102 43.033 1
-36.125 -16.577 1
-49.994 11.74 1
-23.201 5.4932 1
-27.261 40.507 1
-7.9134 40.959 1
-23.625 8.2181 1
12.971 28.986 1
-9.7032 39.365 1
46.736 -26.185 1
-40.62 -39.448 1
-49.529 13.204 1
44.191 -23.714 1
44.172 -25.471 1
11.056 -5.384 1
-12.634 21.568 1
-10.422 -28.401 1
-42.524 -41.504 1
-36.98 -41.984 1
54.623 13.101 1
48.077 -25.212 1
42.903 -1.8745 1
26.384 -43.87 1
-9.2101 2.169 1
1.6263 15.959 1
-6.4157 -27.293 1
29.712 -2.1616 1
-26.33 -19.18 1
13.821 26.627 1
42.993 -26.668 1
-17.318 -6.5409 1
-11.817 -40.493 1
-51.353 10.892 1
27.322 -35.852 1
-24.053 -31.072 1
13.834 -27.549 1
-50.626 11.379 1
18.822 5.7408 1
14.809 -27.524 1
-46.753 12.872 1
33.175 30.841 1
-14.727 -42.944 1
14.881 8.9547 1
29.543 -2.584 1
-9.1399 42.469 1
-11.462 1.6749 1
-13.643 2.0603 1
27.45 -15.078 1
16.087 -6.6425 1
-22.933 6.7101 1
1.0225 -48.802 1
-23.813 6.2044 1
-14.917 -9.1709 1
-27.323 7.3807 1
35.588 33.743 1
-38.093 -22.099 1
-0.3317 11.182 1
54.976 12.429 1
-27.641 7.4031 1
-39.731 -1.9233 1
12.264 43.142 1
34.013 36.314 1
-29.992 24.224 1
9.4493 46.614 1
31.522 17.55 1
2.1335 14.848 1
34.432 38.212 1
0.16779 15.24 1
16.124 -26.99 1
-14.562 -45.724 1
33.223 36.426 1
12.231 -3.5954 1
28.749 -38.877 1
-1.098 -11.263 1
-7.8254 39.999 1
13.617 -5.1441 1
-8.0024 3.6524 1
-30.21 38.094 1
45.187 -29.353 1
-23.128 23.333 1
-11.204 -4.5541 1
-23.763 -20.211 1
31.023 -14.229 1
33.801 18.253 1
0.83572 -12.424 1
35.739 36.063 1
32.825 37.816 1
-8.4893 25.474 1
-33.699 -22.045 1
-10.228 42.438 1
-9.9718 40.338 1
42.128 -25.723 1
54.039 10.036 1
44.752 -0.11698 1
-0.86611 10.704 1
-28.257 -28.915 1
-30.38 24.055 1
-16.404 3.1128 1
1.1233 13.576 1
-28.914 23.172 1
-41.678 -0.33555 1
-13.967 -44.493 1
25.437 -38.991 1
-7.0102 40.207 1
-50.567 11.977 1
-11.765 42.375 1
-12.132 17.876 1
45.253 -26.247 1
-41.202 -2.2901 1
-50.377 11.783 1
-4.0401 -7.4299 1
0.43193 10.741 1
-10.023 1.3542 1
-7.6367 1.0214 1
-24.98 -28.684 1
5.2516 -52.833 1
1.9265 8.3376 1
-11.83 -38.275 1
29.672 -1.5096 1
12.295 -5.209 1
26.55 -42.715 1
-37.116 -20.757 1
48.19 -25.588 1
25.934 -18.029 1
3.4585 -13.3 1
-23.596 -29.399 1
-13.939 2.9662 1
13.936 27.232 1
-38.064 -14.997 1
-13.725 42.528 1
-30.543 40.101 1
-27.168 27.279 1
28.382 17.247 1
29.467 -39.543 1
-25.275 23.754 1
-30.512 38.745 1
-9.7088 3.6744 1
-13.565 -5.4327 1
-0.11745 -15.106 1
55.412 11.146 1
10.525 47.625 1
-9.489 40.913 1
0.39413 -10.811 1
-14.495 5.3148 1
-27.127 40.689 1
10.713 -7.0085 1
-40.417 2.0485 1
-0.90464 -12.486 1
-45.192 1.7587 1
15.784 8.165 1
55.798 15.571 1
11.81 -6.7233 1
45.957 -2.1827 1
14.102 26.122 1
10.81 26.408 1
42.827 -1.68 1
11.583 29.464 1
10.484 -6.2588 1
-27.78 10.414 1
13.941 29.556 1
31.113 14.194 1
-16.288 -9.2247 1
-14.3 -45.468 1
-15.195 -9.8053 1
-12.286 21.86 1
15.082 11.749 1
-26.981 23.076 1
29.304 1.9345 1
-42.495 -39.043 1
-36.071 -22.173 1
-36.232 -15.878 1
-31.423 39.872 1
15.768 27.559 1
-7.8488 -28.668 1
-2.3252 -3.4407 1
29.788 -18.787 1
29.315 -19.294 1
47.256 -22.827 1
9.0129 48.576 1
-28.08 24.504 1
-9.8626 42.53 1
-40.863 2.1655 1
4.738 -48.695 1
10.259 27.751 1
-35.264 -21.277 1
-26.408 5.7356 1
13.161 -7.5724 1
-1.8353 -2.7343 1
29.139 17.63 1
56.223 10.444 1
52.906 16.152 1
-25.637 -29.308 1
16.269 7.4738 1
-15.777 2.8943 1
9.2259 41.803 1
29.164 17.272 1
-1.438 -12.641 1
9.0277 44.078 1
11.443 24.878 1
2.2517 -52.1 1
-10.444 23.928 1
28.496 -18.265 1
13.415 -5.9132 1
16.44 -26.894 1
14.575 28.926 1
1.8034 -16.384 1
-30.776 25.788 1
-13.867 -8.333 1
26.004 -2.4929 1
45.222 1.9982 1
-25.449 24.849 1
1.2856 11.912 1
-40.737 -38.742 1
46.927 -4.9627 1
16.154 13.661 1
-24.459 -19.438 1
-10.108 1.9962 1
-36.95 -21.446 1
0.17035 13.947 1
-8.9381 2.2549 1
46.067 -0.055822 1
3.8524 -50.023 1
5.4197 -48.732 1
-5.6385 -25.994 1
-43.202 -1.0316 1
-36.205 -41.398 1
-43.482 -2.008 1
-38.673 -0.018116 1
26.99 -41.861 1
2.2025 12.134 1
-25.673 19.45 1
-2.0269 16.48 1
-11.901 19.7 1
-37.652 -41.146 1
14.241 -28.181 1
-26.545 20.725 1
14.662 28.058 1
33.688 36.037 1
-0.36521 -14.978 1
33.092 31.896 1
11.86 25.614 1
-31.384 43.04 1
-3.4687 -8.1162 1
-9.3898 -39.263 1
-28.588 -28.508 1
32.597 34.175 1
56.071 13.391 1
46.335 1.0952 1
11.186 -9.8959 1
-26.268 6.3716 1
30.474 -38.24 1
-3.8317 -26.807 1
-18.38 -12.21 1
12.377 28.539 1
28.778 -42.779 1
-35.376 -20.561 1
26.658 0.36184 1
33.146 34.153 1
9.9814 43.37 1
13.897 25.254 1
-18.571 -10.547 1
-41.908 -38.203 1
13.77 26.013 1
-27.233 21.896 1
14.377 -28.563 1
-43.266 1.1467 1
-41.476 -38.209 1
-27.132 9.5976 1
29.497 -17.628 1
-43.244 1.2062 1
28.863 0.076714 1
3.3474 -54.039 1
28.693 -41.229 1
-31.538 25.353 1
-7.6281 40.378 1
-27.267 11.219 1
-9.6002 39.387 1
56.082 13.401 1
33.222 34.998 1
-27.476 42.209 1
33.242 37.867 1
44.574 -2.0914 1
-27.861 7.2252 1
41.292 -25.4 1
-17.463 -7.7329 1
19.734 -28.059 1
31.58 -16.336 1
-27.457 10.426 1
-8.1344 -16.749 1
50.704 13.753 1
29.63 -3.5123 1
17.086 5.7898 1
27.978 -1.1878 1
45.174 -24.445 1
-27.41 10.7 1
43.006 -0.17635 1
54.077 16.304 1
57.491 15.371 1
48.547 -2.3168 1
-36.799 -41.308 1
1.4343 -52.163 1
14.873 -27.755 1
27.394 -37.725 1
-29.175 8.317 1
-8.7183 25.084 1
28.405 -18.435 1
15.568 6.6966 1
28.85 -1.2003 1
10.879 -2.813 1
11.563 -2.5986 1
-26.873 42.179 1
-26.766 20.341 1
11.408 25.19 1
25.682 -0.46017 1
-1.7523 -10.495 1
45.899 -22.253 1
48.199 -4.0677 1
-27.306 -21.014 1
-36.599 -19.764 1
-28.77 -29.474 1
16.579 9.4815 1
-11.409 -38.675 1
-29.238 -29.701 1
30.568 -18.967 1
-13.305 -38.849 1
-12.649 18.306 1
-36.616 -19.44 1
28.425 15.139 1
-38.881 0.15641 1
0.21749 -49.889 1
26.91 -19.317 1
34.889 35.222 1
18.944 -28.119 1
45.535 -25.28 1
-39.024 3.4079 1
-27.393 20.592 1
28.077 -17.261 1
47.221 -4.3526 1
-18.738 -11.57 1
25.852 -16.604 1
-29.06 25.068 1
9.4276 44.698 1
-28.198 23.576 1
-0.45176 -14.415 1
52.302 15.194 1
-33.968 -16.907 1
-23.813 -28.205 1
-48.91 12.337 1
12.838 30.826 1
10.574 29.241 1
27.965 17.138 1
14.976 5.7074 1
-7.1807 -27.712 1
46.093 -24.145 1
25.28 0.1476 1
-7.5053 -5.2161 1
9.8979 45.631 1
-1.2389 14.212 1
33.436 19.966 1
28.964 -37.624 1
26.974 -14.663 1
-15.328 -7.8558 1
-13.702 3.545 1
-1.8553 -2.7485 1
10.672 46.984 1
-17.557 -10.374 1
-11.506 -37.776 1
-26.892 -29.094 1
0.79831 -10.782 1
12.384 -4.3724 1
35.136 34.233 1
-23.366 10.276 1
55.554 12.024 1
1.5229 -12.415 1
2.5945 -12.556 1
16.701 -6.6192 1
-11.45 43.267 1
-11.268 25.52 1
17.894 -26.395 1
-11.276 37.377 1
-10.903 4.7659 1
-39.208 2.7436 1
45.612 1.6085 1
-38.918 2.8207 1
-3.7211 -3.4335 1
-39.77 -38.347 1
41.486 -24.048 1
26.054 -37.821 1
46.291 1.6478 1
-35.288 -23.075 1
46.359 -4.4277 1
55.258 11.4 1
47.157 -26.113 1
-40.93 -0.48924 1
29.153 -17.039 1
28.503 -39.026 1
-37.723 -15.403 1
31.634 35.506 1
-46.168 13.357 1
12.264 26.072 1
8.6705 42.925 1
25.626 -1.3565 1
32.21 35.951 1
-41.164 2.5296 1
-36.86 -17.998 1
15.011 6.7843 1
-26.828 4.9197 1
-12.151 21.374 1
-7.6559 38.976 1
-13.49 -7.9358 1
-50.001 12.672 1
30.522 -40.191 1
-13.922 -8.318 1
-30.162 40.516 1
13.943 27.833 1
-25.316 -19.235 1
-42.912 -0.23064 1
56.78 11.431 1
-6.8213 -27.86 1
-15.01 5.1548 1
54.075 13.445 1
-25.69 -29.549 1
5.3667 -46.585 1
43.213 -28.511 1
-13.156 -43.559 1
-12.138 -9.2265 1
-25.195 -28.134 1
-14.379 -7.5349 1
25.479 -16.842 1
24.433 -16.468 1
-29.394 -29.942 1
43.76 -22.984 1
-25.707 7.0839 1
8.0005 44.439 1
44.752 -22.613 1
-13.823 42.905 1
0.086097 -11.679 1
-12.618 39.617 1
31.893 -1.731 1
0.50434 16.831 1
-2.7307 -26.894 1
-2.2147 -15.75 1
45.926 -21.637 1
-10.646 -7.9259 1
-39.316 -40.588 1
-0.72876 14.536 1
26.316 -36.557 1
-10.84 39.875 1
13.869 -27.303 1
-14.393 -8.6652 1
-50.631 12.177 1
-11.475 42.569 1
0.43974 -15.189 1
10.265 -6.2913 1
-0.98314 11.815 1
11.913 -8.6758 1
44.535 0.83295 1
13.835 -9.018 1
-28.185 25.006 1
-10.561 40.655 1
-13.996 -42.892 1
15.278 7.7713 1
-34.238 -21.494 1
-9.7102 -26.152 1
-10.508 3.6405 1
-8.9554 42.165 1
56.727 13.578 1
-11.574 -42.157 1
16.565 13.054 1
17.048 6.6059 1
-13.082 41.099 1
26.977 -38.245 1
-29.21 43.984 1
-30.951 26.101 1
-38.012 -14.757 1
2.4855 11.864 1
11.753 47.248 1
-12.308 -40.202 1
24.656 -42.554 1
15.883 10.552 1
12.639 30.656 1
8.5407 27.415 1
2.6379 12.489 1
44.275 -2.6288 1
14.459 -4.8574 1
46.654 -1.2953 1
15.43 26.803 1
-8.3733 38.538 1
44.888 -21.225 1
-41.987 -1.4551 1
26.083 -18.634 1
14.385 -7.9434 1
-11.897 -40.45 1
-42.145 -2.9951 1
-9.8035 -7.2816 1
14.805 -5.4841 1
44.126 -2.8097 1
-12.782 -39.646 1
33.033 34.516 1
-25.558 -20.015 1
15.706 -5.4042 1
43.892 -24.362 1
11.492 26.222 1
8.7801 42.795 1
56.102 11.091 1
-11.711 -39.749 1
15.129 28.816 1
28.878 14.86 1
11.288 44.761 1
13.937 31.023 1
3.4489 13.962 1
14.697 -6.856 1
55.279 13.864 1
12.765 27.413 1
-16.853 2.8794 1
17.014 13.152 1
-24.365 7.1624 1
-9.9395 22.153 1
-4.7085 -8.8788 1
-24.007 7.432 1
-25.127 7.3215 1
12.668 -4.633 1
-1.7536 -28.245 1
30.675 -4.8263 1
14.862 28.946 1
44.316 1.0603 1
13.477 -7.4932 1
-31.23 38.881 1
14.458 -5.1001 1
43.894 -25.055 1
27.886 -16.702 1
-12.711 -45.085 1
-44.253 1.6062 1
33.785 19.653 1
-10.806 24.728 1
-15.06 4.6773 1
-3.9728 -7.908 1
13.634 -4.528 1
-3.3402 -5.4643 1
-41.49 3.3355 1
-15.513 -8.1702 1
54.306 16.532 1
9.8582 40.465 1
14.994 9.4315 1
-12.654 -8.9195 1
-28.509 41.744 1
-1.8353 -2.7343 1
56.427 9.9073 1
19.101 -28.106 1
-24.91 39.833 1
-26.204 21.263 1
14.435 -25.755 1
29.507 -4.1812 1
-41.895 -40.262 1
-10.769 38.519 1
30.804 17.215 1
31.703 35.774 1
14.774 10.542 1
26.689 -2.6868 1
-29.692 40.018 1
29.711 -15.677 1
9.1036 43.853 1
9.5448 41.32 1
54.701 9.4249 1
48.592 -3.9624 1
-9.1742 -37.254 1
-7.3297 39.259 1
-25.444 -19.769 1
30.808 0.11491 1
11.448 43.565 1
32.762 34.223 1
29.716 -42.451 1
30.402 -38.674 1
-9.7945 19.528 1
27.209 -41.031 1
36.237 35.893 1
26.483 1.979 1
-28.68 7.7136 1
-1.9501 -13.3 1
-17.461 -6.4222 1
-10.061 25.329 1
-12.6 -42.612 1
42.896 -25.066 1
-10.661 -39.152 1
46.614 -1.9219 1
-13.076 -38.028 1
2.1567 11.609 1
-48.075 13.695 1
-43.496 -0.093935 1
-37.671 0.0058538 1
-27.482 8.2322 1
25.698 -38.924 1
-29.274 25.309 1
44.941 -27.897 1
15.634 9.6574 1
10.554 -3.4359 1
-1.6211 -11.571 1
-10.497 -27.64 1
7.1075 -48.106 1
-38.594 -40.95 1
46.22 -0.42356 1
-11.352 -41.34 1
-36.467 -18.42 1
-12.327 19.705 1
-12.096 19.646 1
44.97 -22.723 1
-1.1161 -2.3969 1
-7.5731 41.727 1
54.331 16.506 1
-24.948 -28.739 1
53.998 14.433 1
41.665 -26.345 1
1.2669 -10.871 1
26.486 -18.927 1
-23.919 -20.095 1
0.75774 14.845 1
54.461 12.853 1
32.653 17.498 1
-28.663 10.181 1
-12.268 1.9985 1
-9.5336 25.299 1
-11.777 -38.688 1
-28.475 -30.092 1
28.193 -16.072 1
0.82869 -10.808 1
5.2436 -48.401 1
-17.85 -10.407 1
30.383 -3.4274 1
54.194 11.877 1
33.259 36.759 1
55.495 12.934 1
-28.832 26.006 1
47.535 -1.2528 1
-29.219 -29.694 1
46.53 -26.861 1
36.957 36.424 1
-7.2085 39.277 1
-9.5213 26.465 1
32.501 33.562 1
-10.191 26.039 1
-13.815 42.731 1
-0.91704 8.7637 1
9.039 45.239 1
-24.624 8.7566 1
29.993 17.337 1
15.015 -8.8812 1
-29.788 23.816 1
-12.871 -40.766 1
-28.597 9.1478 1
-26.288 23.816 1
15.486 7.6624 1
-8.6861 -28.671 1
28.091 12.443 1
29.371 -41.467 1
-37.769 -14.173 1
6.8725 -48.202 1
13.476 -2.9812 1
27.332 1.7769 1
-15.336 -9.1578 1
-7.2006 -9.778 1
11.712 -4.041 1
55.202 10.747 1
-1.0024 9.9816 1
-5.5854 -29.703 1
9.1054 44.866 1
-36.096 -14.628 1
30.078 -1.4084 1
30.594 -14.2 1
-14.845 -9.7013 1
-7.4966 -25.551 1
-12.162 23.438 1
17.753 -28.881 1
-12.136 25.098 1
-4.654 -6.2244 1
-11.392 21.1 1
-9.3754 25.061 1
-27.54 9.1299 1
-28.024 -29.516 1
-12.87 19.829 1
-23.989 -31.07 1
-36.205 -42.398 1
31.031 19.493 1
-49.951 13.159 1
-44.911 -1.8682 1
-39.699 -0.43065 1
-39.063 -39.258 1
29.198 -3.5343 1
-10.414 39.389 1
-25.72 6.2578 1
16.966 6.397 1
-7.0194 -26.166 1
-37.25 -15.371 1
-36.955 -41.735 1
14.335 29.38 1
3.8024 -49.28 1
19.207 -28.038 1
33.261 18.543 1
44.672 -0.25016 1
-26.636 -20.143 1
19.515 -27.707 1
10.961 -6.3456 1
57.091 12.246 1
-10.956 0.69199 1
-42.741 0.77193 1
24.284 -40.564 1
-17.543 -10.647 1
-46.909 14.593 1
-27.708 25.225 1
-25.75 7.0934 1
-12.761 -45.376 1
26.603 -18.474 1
34.879 37.512 1
1.0885 -10.35 1
-30.446 21.914 1
29.434 -16.348 1
-26.404 23.669 1
-14.232 4.7263 1
-40.494 2.2421 1
-12.297 -38.352 1
3.9687 13.321 1
-18.658 -9.4287 1
34.295 33.479 1
25.826 -37.327 1
4.085 -47.743 1
43.241 -4.9945 1
-14.695 3.8788 1
-9.192 22.324 1
26.43 -43.368 1
-42.261 -39.424 1
-11.518 20.412 1
4.4045 -47.07 1
-16.299 -7.6311 1
-36.981 -21.736 1
14.356 -9.7168 1
30.251 16.153 1
-37.28 -18.887 1
-9.9803 4.1257 1
27.089 15.065 1
-5.0979 -28.018 1
-29.48 23.792 1
-35.147 -15.926 1
-27.774 9.2598 1
2.483 13.674 1
-18.895 -11.738 1
-15.88 1.4297 1
-10.968 25.55 1
54.472 15.005 1
2.4371 -52.824 1
11.48 -4.9494 1
-9.4403 3.6314 1
-28.965 37.892 1
-9.8076 23.862 1
56.926 14.918 1
-23.578 -20.157 1
31.006 18.438 1
-49.33 12.464 1
14.532 27.824 1
-30.48 39.031 1
-27.825 -30.108 1
19.587 -27.774 1
27.752 -15.993 1
-10.826 2.9421 1
-37.479 -41.806 1
-37.875 -14.146 1
15.107 -29.003 1
-3.4449 -12.796 1
-4.9989 -7.547 1
-28.683 -29.493 1
-8.4351 -5.8951 1
28.95 -3.2986 1
4.8217 -46.196 1
2.2274 -16.954 1
-14.095 -45.641 1
-36.782 -20.589 1
-9.8724 43.283 1
-16.763 -10.323 1
12.338 27.691 1
14.415 29.63 1
-0.97898 11.391 1
55.752 15.45 1
-2.1157 -4.7665 1
6.2854 -47.799 1
-36.668 -1.8595 1
-36.694 -42.245 1
43.994 -0.28387 1
-29.383 27.364 1
15.677 27.721 1
7.9913 44.807 1
-28.122 43.707 1
-10.088 19.53 1
-31.913 25.656 1
10.568 44.162 1
33.907 18.2 1
-12.458 -8.8855 1
-25.182 6.6949 1
-40.516 0.54094 1
-13.62 1.2164 1
-37.458 -3.0393 1
-38.801 -19.938 1
27.224 -39.998 1
48.345 -3.4553 1
26.264 -2.9667 1
17.529 -28.305 1
-28.267 25.671 1
-8.3948 22.848 1
11.521 -8.6296 1
9.8435 44.694 1
33.583 31.845 1
2.5268 -51.62 1
-29.128 -27.797 1
52.954 12.898 1
-1.5436 -14.889 1
-12.235 -42.358 1
-38.268 -15.268 1
-49.907 12.917 1
-12.472 20.985 1
11.103 41.134 1
32.958 33.159 1
44.078 -21.315 1
-28.428 39.301 1
-43.649 1.6248 1
-24.584 7.4191 1
30.283 -41.942 1
15.637 10.705 1
-10.411 41.992 1
-10.498 2.0383 1
-42.103 -0.99784 1
-12.72 -45.29 1
-3.5101 -29.152 1
-28.924 40.307 1
-9.8089 22.88 1
54.82 9.6522 1
-11.348 3.3107 1
-22.932 9.117 1
-37.01 -0.66719 1
-26.499 6.1666 1
27.899 -14.681 1
11.569 -2.7277 1
28.504 -39.309 1
7.6893 43.71 1
-33.807 -19.2 1
-1.6775 -2.668 1
-37.801 -14.317 1
28.895 -42.796 1
28.029 1.973 1
-2.2709 14.941 1
8.4345 42.328 1
-36.232 -43.296 1
11.128 43.941 1
-41.462 -0.27875 1
-7.9551 1.4369 1
-2.8915 -26.848 1
45.866 1.7742 1
-2.5431 -28.622 1
-16.172 -7.4725 1
-38.447 -21.202 1
35.378 34.903 1
-49.597 11.765 1
0.40377 -49.863 1
41.681 -25.021 1
-12.547 -38.9 1
-24.756 -19.575 1
-7.8369 41.178 1
34.06 38.693 1
-2.8588 -2.4802 1
-40.303 0.46345 1
45.762 2.2693 1
-37.452 -22.01 1
-38.084 -40.251 1
-24.984 8.0575 1
43.341 -25.706 1
-1.2394 -9.922 1
-26.408 -30.274 1
27.944 13.943 1
46.123 0.23871 1
-11.982 38.715 1
3.0249 -12.373 1
9.4631 49.166 1
-1.5434 -2.3383 1
4.3119 -53.97 1
-9.407 -38.035 1
0.85942 -13.092 1
45.512 0.55337 1
-36.781 -15.423 1
-38.862 -1.3582 1
-27.901 -28.414 1
45.861 1.6151 1
-30.071 43.416 1
-37.672 -39.522 1
31.138 19.491 1
-10.368 21.323 1
-15.176 -41.055 1
27.738 -1.5526 1
3.5657 -14.046 1
15.364 9.0583 1
55.207 10.105 1
17.236 -26.772 1
34.862 37.783 1
-31.133 39.212 1
2.1086 -14.828 1
-44.099 -2.4005 1
10.531 -3.6942 1
26.229 -17.576 1
10.524 -4.696 1
-7.1973 38.931 1
13.445 -2.7974 1
46.714 -21.928 1
-3.6027 -29.017 1
-9.9039 4.7296 1
18.01 -24.049 1
-50.957 12.154 1
-0.98603 10.591 1
7.1536 42.74 1
29.834 14.388 1
-13.975 1.2834 1
-42.55 -38.343 1
-13.304 42.728 1
3.6554 13.374 1
55.309 9.4183 1
44.658 -4.1008 1
-30.63 42.593 1
-29.023 -28.235 1
0.58988 -15.619 1
-18.111 -12.15 1
-5.5871 -25.076 1
3.8194 11.584 1
-30.901 37.589 1
13.806 28.314 1
-9.7714 4.3243 1
-0.048768 -15.545 1
-38.286 -16.418 1
-37.847 -22.159 1
31.674 -1.9407 1
-26.802 10.182 1
17.302 -28.944 1
1.841 -15.986 1
46.97 -21.405 1
-38.784 -40.59 1
-31.356 41.424 1
27.758 0.17907 1
46.574 -27.213 1
-11.968 3.2932 1
-10.391 37.084 1
-26.578 -18.147 1
-26.255 9.7734 1
29.16 -14.631 1
30.477 -40.338 1
-25.03 9.9157 1
-27.642 -30.525 1
12.499 43.868 1
-27.7 -29.597 1
-29.707 41.067 1
-29.33 40.973 1
-12.812 -39.676 1
45.671 2.3548 1
-10.199 21.619 1
46.499 -1.5128 1
-3.558 -29.447 1
46.094 -0.31365 1
3.4254 -46.313 1
-33.972 -18.538 1
-28.602 22.615 1
29.313 -40.507 1
-35.825 -42.544 1
15.473 8.9199 1
-48.778 13.041 1
17.752 -27.273 1
-51.162 10.647 1
4.7572 -51.487 1
43.702 -24.216 1
33.415 32.215 1
3.4293 -13.244 1
-12.073 21.063 1
-24.603 24.878 1
13.933 10.879 1
-38.175 -16.177 1
28.118 -37.337 1
24.68 -18.331 1
-25.25 8.8018 1
15.536 28.554 1
35.383 36.012 1
-15.851 -11.941 1
-10.003 1.9334 1
14.426 -28.113 1
14.795 -9.3709 1
46.476 -1.3739 1
1.0578 -51.17 1
-13.676 -38.639 1
-4.2499 -28.943 1
44.71 -1.4105 1
30.528 16.874 1
9.1609 47.343 1
-29.775 38.565 1
-45.222 -1.5138 1
11.786 -2.3468 1
-37.658 -14.914 1
46.033 0.81244 1
42.919 -27.514 1
-32.621 -17.525 1
29.644 18.437 1
13.702 -29.629 1
-31.468 25.585 1
-30.108 39.98 1
0.39952 15.608 1
-10.644 23.085 1
-28.931 25.024 1
-37.248 -15.499 1
-29.243 26.953 1
30.764 -15.172 1
6.9973 -48.516 1
-35.579 -20.28 1
-42.587 -0.97248 1
0.13567 15.425 1
10.859 41.823 1
1.3128 16.478 1
28.907 0.0035425 1
29.283 -40.679 1
53.87 10.484 1
26.601 -42.738 1
-9.478 -26.055 1
12.651 -6.9078 1
-38.049 -19.664 1
-15.419 -42.489 1
-8.8551 21.765 1
-16.056 -10.71 1
-28.055 41.031 1
27.5 -19.294 1
13.598 27.027 1
8.4852 42.095 1
-6.7181 -27.202 1
26.274 -17.305 1
-27.7 -19.88 1
11.396 46.694 1
29.886 -41.666 1
-26.837 42.073 1
27.666 15.166 1
-38.842 -40.571 1
-17.457 -10.527 1
45.257 -25.133 1
1.5546 -11.408 1
-16.127 -10.552 1
-10.682 -42.196 1
45.665 -4.3391 1
1.79 -52.082 1
24.781 0.087195 1
-37.887 -42.754 1
46.216 -4.2102 1
-36.519 -41.943 1
42.372 -23.45 1
-3.0852 -26.684 1
12.935 -9.2116 1
-7.2902 -28.511 1
-8.855 38.671 1
-28.152 23.346 1
9.5981 46.263 1
11.054 45.62 1
14.877 30.028 1
-0.86647 -13.456 1
-9.2139 -38.649 1
-27.048 9.8817 1
-11.408 -37.831 1
-18.264 -8.1413 1
8.4087 46.946 1
26.003 12.479 1
55.234 9.4976 1
-7.2491 -25.702 1
-6.7769 41.33 1
25.28 -1.495 1
-41.255 0.3422 1
25.435 -17.284 1
-6.7426 -25.869 1
53.502 11.504 1
-4.7175 -8.8897 1
-24.821 7.7178 1
1.9359 8.5294 1
-13.604 -9.9334 1
33.124 34.062 1
8.4121 41.632 1
-13.231 43.162 1
-7.4314 -28.007 1
56.763 15.307 1
-9.4009 -29.14 1
15.114 7.4102 1
-23.579 8.0816 1
34.221 35.052 1
-11.381 18.869 1
-1.3179 -11.312 1
-9.3843 3.7191 1
-9.2912 40.846 1
-16.419 -7.9946 1
10.167 39.768 1
56.238 12.495 1
-2.2948 -0.68968 1
-26.72 10.198 1
-27.94 39.911 1
-7.3972 -6.5662 1
7.2256 45.348 1
27.422 -19.345 1
-42.394 -40.22 1
-36.626 -19.286 1
-9.2502 -27.667 1
-18.985 -10.727 1
14.802 28.873 1
-7.5451 -29.611 1
-0.60072 14.24 1
-4.3307 -8.0945 1
11.11 42.05 1
-50.148 13.9 1
48.433 -2.127 1
56.182 16.316 1
-30.378 42.84 1
0.82 -9.9172 1
15.156 8.2976 1
28.711 -19.556 1
-43.324 -2.2521 1
-11.32 19.917 1
-8.6913 40.441 1
44.237 -3.3117 1
-15.65 -44.61 1
28.894 -17.809 1
-37.671 -16.148 1
-9.5392 25.677 1
33.065 34.103 1
-47.817 15.626 1
-16.854 -42.526 1
-10.573 -28.355 1
33.698 33.718 1
-0.055988 -14.861 1
-25.15 -19.253 1
10.558 -2.9028 1
-9.3702 39.337 1
-50.077 12.678 1
15.162 7.5146 1
55.211 14.154 1
-38.65 -40.415 1
17.55 -29.059 1
0.9765 10.126 1
30.113 -2.2164 1
29.045 -16.1 1
-3.5106 -3.1961 1
-36.3 -17.494 1
-4.2645 -26.059 1
-42.664 -2.1945 1
12.641 -8.1006 1
-18.899 -9.0875 1
45.089 -0.91796 1
31.156 34.703 1
-9.4131 39.076 1
-28.648 -30.878 1
18.92 -28.859 1
-11.277 25.426 1
-30.005 -29.42 1
8.9116 44.322 1
-28.338 -19.808 1
42.491 -24.348 1
-27.441 23.029 1
-29.668 26.473 1
-8.9752 -28.051 1
-42.47 -2.1453 1
-24.979 -19.392 1
-26.945 -29.664 1
3.6532 -48.84 1
-6.7278 -5.5466 1
11.796 47.47 1
41.412 -24.141 1
-12.551 23.721 1
4.9719 -46.235 1
-14.277 4.7798 1
26.263 -43.657 1
12.626 45.949 1
-24.449 -20.117 1
-47.959 13.764 1
-39.784 1.1631 1
15.227 26.957 1
-9.2565 20.048 1
24.46 -41.735 1
-43.904 0.25224 1
-19.797 -9.9876 1
-3.039 -5.614 1
-6.8283 -5.5565 1
-14.449 -41.748 1
55.917 10.55 1
-6.7178 39.258 1
-11.797 39.976 1
26.796 -43.303 1
9.399 45.958 1
-40.152 -40.491 1
3.8947 -51.977 1
54.787 9.2215 1
-28.601 44.25 1
-40.833 -39.526 1
-0.27586 -16.27 1
27.218 -38.386 1
-3.8583 -29.465 1
58.35 15.092 1
1.8996 -50.609 1
34.24 32.573 1
12.747 -4.6271 1
23.998 -1.8881 1
-25.917 21.788 1
48.052 -2.9014 1
0.6763 -12.064 1
-9.7495 23.473 1
56.546 16.279 1
14.255 -9.5856 1
-9.9749 -27.085 1
28.071 14.781 1
-1.5403 -10.875 1
-7.5149 -29.503 1
31.667 32.651 1
15.366 28.224 1
13.251 27.671 1
-11.368 -8.1813 1
11.363 46.022 1
-25.589 8.7668 1
31.165 34.144 1
18.083 -24.885 1
26.718 -41.764 1
1.7232 16.339 1
56.589 12.808 1
12.601 -4.6293 1
-0.60151 -13.992 1
13.986 30.177 1
10.231 -3.8497 1
-37.939 -18.353 1
28.557 -19.43 1
31.32 0.26166 1
52.5 15.004 1
-36.733 -15.292 1
46.935 -22.725 1
46.313 -1.8504 1
13.484 28.891 1
-11.886 -37.785 1
-3.0109 -30.045 1
-11.687 5.776 1
31.221 0.6757 1
-26.17 -19.853 1
-13.269 42.788 1
46.9 -2.4309 1
41.577 -26.177 1
26.746 1.971 1
13.341 -29.85 1
-28.022 38.654 1
46.286 -22.335 1
8.144 42.32 1
0.79019 -11.008 1
-10.058 19.783 1
1.0555 10.558 1
-11.843 18.553 1
-14.209 2.0064 1
3.3097 -49.382 1
14.926 -28.923 1
3.5933 -49.941 1
2.5586 11.766 1
1.7227 -11.363 1
34.267 33.068 1
-40.587 3.3907 1
-11.297 4.3679 1
44.121 -22.183 1
-11.519 -38.121 1
-17.115 -12.03 1
34.657 38.312 1
12.837 29.551 1
8.6627 48.589 1
31.991 35.306 1
43.122 -28.695 1
16.414 8.1521 1
-6.1954 -24.749 1
10.551 -6.1723 1
-6.4828 39.191 1
-5.9 -26.959 1
-3.5558 -25.435 1
19.276 -27.117 1
-10.68 2.7562 1
4.1411 -46.556 1
-39.735 -1.3126 1
45.06 -5.3171 1
11.401 24.777 1
13.442 12.619 1
14.088 10.931 1
17.534 -24.604 1
-51.186 10.734 1
2.9226 13.472 1
18.055 -24.159 1
25.525 -41.346 1
-16.947 -8.3045 1
43.804 -26.003 1
3.443 -53.997 1
-40.591 1.9757 1
-42.175 2.5564 1
26.668 -18.751 1
17.449 -28.601 1
-37.946 -40.342 1
56.143 13.071 1
-48.308 11.87 1
-2.5918 -2.9193 1
25.997 -18.694 1
-15.284 -42.974 1
32.975 32.501 1
27.642 -41.939 1
34.581 38.925 1
-10.533 1.0502 1
-5.5894 -30.7 1
15.736 9.4588 1
1.5319 -51.413 1
46.625 -3.63 1
2.6624 -52.052 1
56.405 11.313 1
-26.688 39.916 1
-1.2636 -12.238 1
19.008 -27.282 1
11.47 -9.6571 1
17.968 8.4873 1
-11.479 -41.107 1
15.593 -6.3059 1
2.5954 -53.374 1
44.852 -0.67276 1
26.222 -41.979 1
-29.043 22.759 1
-30.6 25.233 1
7.5825 25.182 1
-8.3117 40.737 1
1.9663 -50.234 1
-27.451 41.027 1
12.95 25.817 1
24.905 -40.127 1
-28.274 26.731 1
-25.739 22.611 1
31.588 -14.233 1
28.591 -42.015 1
15.686 8.415 1
45.14 -25.726 1
-28.817 25.84 1
3.6958 -53.332 1
-8.0732 -16.75 1
45.773 -3.4066 1
25.965 -41.047 1
26.831 -13.829 1
25.255 1.1372 1
56.439 15.537 1
56.861 12.407 1
-38.231 -41.502 1
-25.884 10.167 1
-10.593 26.211 1
-12.566 -44.368 1
13.083 -8.9493 1
44.957 -27.741 1
-7.7863 24.777 1
30.451 -2.9548 1
-11.824 20.648 1
-14.852 4.7743 1
-26.891 5.2685 1
-28.462 39.467 1
28.416 2.4014 1
46.631 -2.0729 1
-9.3187 23.077 1
-37.57 -20.202 1
-50.343 13.338 1
30.07 1.8245 1
12.647 -4.8399 1
-24.722 -19.345 1
-47.092 15.69 1
-12.037 18.097 1
-9.1155 23.263 1
-18.149 -11.25 1
13.393 29.428 1
33.261 38.153 1
5.5366 -46.916 1
-12.279 21.28 1
-16.544 2.8835 1
-0.46412 -1.4085 1
-30.691 38.258 1
7.2215 46.28 1
-34.046 -18.609 1
-37.88 -18.24 1
-8.3399 -28.653 1
35.905 34.407 1
15.606 -27.776 1
28.881 -37.538 1
-28.764 27.154 1
-12.345 44.052 1
-50.963 10.921 1
-15.423 -43.498 1
-28.087 26.046 1
15.57 10.922 1
30.257 -3.015 1
-10.136 41.771 1
-27.92 23.381 1
-36.194 -22.466 1
-43.965 2.1491 1
43.611 -25.793 1
-4.1881 -6.3097 1
-0.63467 14.642 1
-11.657 3.2151 1
29.61 16.161 1
26.789 -40.077 1
-12.54 0.80654 1
-37.588 -41.166 1
-13.486 2.154 1
26.062 12.562 1
-33.897 -20.883 1
29.449 -41.165 1
8.8053 41.931 1
11.347 26.265 1
7.5128 45.035 1
41.547 -23.991 1
32.247 34.416 1
-23.051 8.0574 1
-27.662 24.829 1
27.228 -0.045084 1
-27.715 23.832 1
16.711 12.337 1
10.504 -3.0458 1
-38.579 -15.711 1
-7.4741 -6.6894 1
9.5377 28.228 1
18.541 11.654 1
-24.973 5.8626 1
12.768 -28.584 1
15.642 7.6526 1
-50.864 11.858 1
-14.021 -44.079 1
30.311 -16.231 1
33.099 18.185 1
-12.583 -43.763 1
-16.888 3.1821 1
15.365 -29.245 1
-17.112 -7.5073 1
-15.58 -43.099 1
-25.678 -28.526 1
-1.9218 -16.006 1
-2.0868 -11.72 1
-29.005 6.3452 1
-25.851 -30.668 1
17.608 8.3708 1
-25.28 22.552 1
27.8 13.793 1
14.698 8.5569 1
0.059354 -16.299 1
-25.662 25.578 1
-47.207 14.149 1
30.291 14.093 1
-31.136 42.562 1
24.555 -41.634 1
30.179 -18.739 1
34.084 37.804 1
13.776 11.856 1
1.8123 15.172 1
-39.005 2.4317 1
19.446 -28.064 1
-39.92 1.4489 1
16.87 -6.7805 1
-31.443 38.701 1
15.47 10.562 1
-11.59 19.194 1
5.0084 -52.48 1
-35.545 -18.495 1
27.924 -16.706 1
-40.493 2.4235 1
-7.9326 -27.413 1
-40.19 -38.289 1
53.816 11.425 1
29.025 14.264 1
-18.513 -11.942 1
27.02 1.7235 1
30.045 -16.922 1
-4.1897 -5.8539 1
17.944 -24.426 1
-49.461 13.118 1
30.679 -15.315 1
31.028 -0.40878 1
-50.812 11.327 1
2.5781 14.605 1
31.875 15.44 1
-49.813 10.877 1
-33.864 -20.951 1
12.078 -6.9471 1
45.488 1.3883 1
0.52753 -51.255 1
1.7912 13.965 1
-23.951 -27.696 1
1.1845 14.726 1
11.27 -5.9145 1
-37.94 0.10739 1
-27.485 9.4393 1
14.659 -5.8448 1
15.326 7.0161 1
12.679 45.36 1
15.251 8.564 1
-26.279 -19.729 1
-38.445 -20.798 1
-9.2021 40.112 1
28.278 -15.221 1
-1.8353 -2.7341 1
-27.759 21.52 1
-37.409 -42.354 1
-38.982 3.6853 1
10.242 -5.7373 1
26.751 -1.1931 1
-42.455 -38.819 1
1.8358 8.4449 1
28.686 -3.182 1
-27.938 43.971 1
-23.404 -29.298 1
15.28 7.804 1
3.9 -50.536 1
-50.544 12.655 1
43.408 -27.645 1
9.7709 29.767 1
12.806 -6.7617 1
11.997 -28.221 1
-1.8433 -2.7305 1
30.789 16.412 1
-27.113 42.368 1
28.625 14.465 1
33.415 32.125 1
-51.989 10.402 1
55.049 10.176 1
13.998 28.888 1
-26.641 -30.996 1
13.586 -3.0958 1
-10.836 0.23648 1
28.95 0.57892 1
-7.5292 -6.756 1
-7.7956 39.408 1
-25.615 -29.326 1
41.826 -23.953 1
1.0243 8.0596 1
2.1808 10.501 1
-40.346 -1.7866 1
53.998 13.426 1
-4.7324 -25.359 1
-37.655 1.437 1
28.099 -18.55 1
-11.336 2.8378 1
-38.912 -40.793 1
1.2566 -14.026 1
-7.781 40.09 1
49.166 -3.8519 1
40.915 -24.835 1
31.638 -0.33508 1
-37.627 -39.108 1
-25.279 -19.964 1
46.075 -21.333 1
-29.837 21.241 1
-28.062 9.7172 1
-38.125 1.4225 1
-38.968 3.3812 1
7.549 46.12 1
-19.031 -10.258 1
-31.234 42.845 1
57.537 13.356 1
24.461 -38.184 1
-12.165 -42.298 1
-12.723 0.63047 1
30.235 -38.903 1
-36.398 -18.507 1
-8.3039 39.478 1
-4.4066 -28.553 1
11.524 -5.4193 1
-6.7393 -25.819 1
12.002 29.277 1
-14.748 -43.862 1
10.715 -3.585 1
1.2719 14.492 1
-8.9752 41.139 1
-12.146 40.23 1
11.334 -3.4452 1
-11.003 21.911 1
-43.51 -0.59826 1
32.13 34.525 1
-10.936 3.7619 1
13.58 -29.54 1
-13.267 20.726 1
52.967 11.744 1
-15.864 -9.9196 1
-35.771 -17.234 1
31.615 19.145 1
17.789 -27.198 1
12.316 43.201 1
-11.99 -6.664 1
55.359 13.591 1
-8.3168 41.771 1
3.5936 -53.546 1
24.925 -2.9438 1
-5.852 -24.873 1
-3.4535 -27.522 1
-12.04 4.8899 1
2.88 -46.547 1
-39.373 -38.905 1
12.533 24.119 1
-29.928 24.763 1
-39.325 -42.11 1
-36.194 -42.54 1
-43.069 -1.9865 1
-29.52 40.284 1
-37.276 -41.685 1
33.634 19.393 1
11.229 -3.1505 1
-13.65 -8.0833 1
-41.175 -38.256 1
-0.39466 9.538 1
-31.346 24.185 1
45.127 0.73405 1
-10.742 38.487 1
52.521 12.91 1
-2.3962 -28.089 1
-41.55 -38.213 1
-9.154 -26.851 1
-41.511 -37.909 1
6.4019 -48.523 1
-13.628 -10.267 1
-14.54 -44.432 1
-26.923 26.283 1
28.272 -0.66252 1
-30.05 25.575 1
0.32115 -50.493 1
28.379 -2.07 1
-26.487 22.621 1
32.377 15.681 1
29.353 16.478 1
10.204 -8.7554 1
14.993 -7.2013 1
-10.103 21.978 1
-11.929 4.7714 1
2.5519 13.175 1
14.471 14.083 1
12.297 26.064 1
-12.295 40.858 1
-35.797 -42.728 1
-32.927 -21.31 1
-10.402 23.75 1
12.431 28.305 1
33.131 34.039 1
25.766 12.686 1
7.501 25.259 1
43.848 -28.914 1
-12.903 -42.765 1
-25.129 -29.113 1
-15.662 -9.2057 1
-2.3706 -15.948 1
0.48481 -2.1457 1
46.945 -2.5672 1
16.925 -25.592 1
9.9027 26.751 1
-27.045 9.1264 1
-11.752 -6.5934 1
-41.093 3.1724 1
3.9258 -52.292 1
-3.8565 -3.2247 1
-50.789 11.126 1
16.907 -28.061 1
25.338 -38.266 1
12.122 29.603 1
-12.747 -41.131 1
-11.114 20.727 1
-38.141 -21.08 1
47.418 -1.1803 1
-13.726 -10.746 1
11.953 -8.2974 1
-0.52415 10.212 1
0.3024 -2.1773 1
-36.947 -15.992 1
-42.744 -3.3633 1
-38.164 -13.812 1
46.719 -3.095 1
6.239 -48.3 1
28.632 -17.02 1
57.007 14.645 1
-7.1389 -6.1097 1
9.8428 44.088 1
15.148 28.161 1
15.909 -5.6248 1
-12.577 2.6337 1
-6.5718 -24.758 1
-39.473 2.9461 1
13.688 27.982 1
-1.9806 11.062 1
9.8619 43.081 1
-12.738 39.329 1
-0.83243 -1.5693 1
32.154 33.077 1
-9.576 21.702 1
28.437 -15.753 1
15.912 6.8158 1
32.26 32.901 1
14.38 11.854 1
-11.883 2.8151 1
-44.041 2.4174 1
-36.42 -15.179 1
55.161 13.083 1
-24.462 -20.213 1
-29.48 -29.397 1
34.87 34.645 1
1.9463 8.3729 1
1.1045 13.859 1
35.114 37.058 1
18.944 8.6364 1
-15.951 -8.6178 1
29.104 -40.69 1
11.615 27.303 1
-43.687 0.29695 1
25.188 -38.504 1
-12.458 1.8384 1
46.433 -1.2576 1
45.035 -3.3132 1
-10.294 24.413 1
-9.5444 20.167 1
26.915 -40.355 1
-11.445 1.578 1
25.906 -2.1743 1
-24.56 -19.842 1
43.456 -28.967 1
53.586 12.71 1
5.3026 -50.414 1
12.512 -5.1804 1
-27.548 6.4788 1
43.971 -24.045 1
6.3753 -49.816 1
46.177 -5.0191 1
11.426 29.372 1
10.076 42.931 1
-17.236 -8.4355 1
-38.168 -14.883 1
-2.4602 -0.34821 1
-49.234 14.653 1
-27.444 22.551 1
-9.5109 42.925 1
14.498 -4.6652 1
-35.969 -19.045 1
3.7805 -48.187 1
-8.8195 -5.8016 1
31.033 -18.021 1
-31.091 25.706 1
-12.133 -43.468 1
14.721 -27.923 1
-0.94906 11.794 1
-27.675 23.813 1
33.157 35.328 1
15.538 -27.675 1
17.867 6.3662 1
23.267 -39.496 1
-10.403 -38.642 1
-50.801 12.327 1
-27.977 5.7331 1
-10.591 4.6 1
-41.708 3.1063 1
25.401 -1.8477 1
-29.691 41.396 1
12.295 -6.2269 1
30.833 -39.173 1
44.84 -23.49 1
45.145 -22.274 1
28.817 16.501 1
34.552 18.494 1
16.632 -29.335 1
-15.263 4.8083 1
-37.092 -14.006 1
-25.213 6.1571 1
29.151 0.17914 1
56.471 11.637 1
-37.506 -22.193 1
16.834 -27.797 1
-41.508 -40.971 1
-14.917 -43.64 1
30.472 18.865 1
14.312 27.302 1
1.83 -17.503 1
-40.232 -41.188 1
1.0228 8.3018 1
-27.351 -30.461 1
-38.561 -18.847 1
-15.011 -37.815 1
12.863 -4.6816 1
25.138 0.61612 1
19.66 -27.93 1
7.6356 44.833 1
32.761 33.469 1
-9.3319 3.991 1
13.719 -8.6169 1
-11.818 23.587 1
12.149 -8.7288 1
-10.91 18.29 1
-2.4132 -2.6657 1
13.956 12.991 1
-27.478 10.96 1
-10.264 19.453 1
-0.66433 14.643 1
-42.107 1.0699 1
24.027 -37.391 1
13.949 -28.341 1
23.763 -37.31 1
-42.181 1.8476 1
4.159 -45.53 1
-12.196 19.707 1
-13.675 40.491 1
12.391 44.783 1
-2.5141 -9.8089 1
-28.541 8.449 1
-24.145 7.5372 1
-24.722 6.9769 1
3.8912 -49.982 1
-28.559 25.754 1
1.6414 16.286 1
33.113 34.928 1
-12.251 -5.7513 1
-2.7274 -4.1701 1
28.488 -39.016 1
29.357 -40.074 1
-10.452 37.59 1
0.77604 -10.022 1
30.245 -17.754 1
-11.839 22.388 1
32.335 17.648 1
42.884 -27.073 1
-1.6956 -14.441 1
-11.82 22.109 1
-0.62513 -1.5586 1
1.7229 11.849 1
46.813 -4.8946 1
28.862 18.052 1
0.058811 -10.936 1
-23.92 23.111 1
9.384 26.123 1
-26.157 -30.077 1
-29.194 -27.69 1
17.932 -28.261 1
-7.7734 -25.665 1
1.0623 15.001 1
-10.934 4.9213 1
-9.9604 1.201 1
-39.559 -40.45 1
-12.951 -41.465 1
-30.137 25.302 1
-14.145 19.359 1
-4.9783 -28.655 1
-39.604 -1.2596 1
-16.445 2.8859 1
13.781 29.147 1
-6.0476 -26.042 1
-5.1525 -29.682 1
-0.76867 -11.939 1
-26.579 -18.268 1
-30.103 41.978 1
10.413 23.949 1
-14.84 3.8343 1
-39.599 -40.262 1
-4.7283 -27.948 1
-17.458 -9.0239 1
28.214 -40.68 1
17.819 -28.848 1
56.784 12.34 1
-40.247 -39.563 1
26.419 -43.439 1
9.8741 44.488 1
-35.878 -42.719 1
-44.356 -1.0098 1
-25.431 -20.077 1
49.49 -5.2127 1
27.833 -42.968 1
8.728 42.671 1
-23.302 5.7182 1
-40.325 -1.722 1
16.367 -29.089 1
-15.253 -10.275 1
-23.972 -31.089 1
33.101 19.345 1
45.898 -25.866 1
-29.436 -29.536 1
-11.862 40.606 1
-13.439 22.742 1
12.737 7.0897 1
-26.202 6.6901 1
2.9824 9.9652 1
-6.995 -28.256 1
-17.452 -8.8671 1
9.4797 48.722 1
25.777 -1.3014 1
-1.917 -15.667 1
-7.245 39.559 1
14.206 -5.0566 1
-13.302 -43.73 1
25.455 -0.019869 1
-14.991 -4.0218 1
-12.543 18.033 1
-4.8856 -28.119 1
16.324 7.1536 1
-12.027 5.4787 1
49.023 -4.7496 1
29.377 14.152 1
8.8216 47.233 1
7.0057 45.367 1
1.8489 12.493 1
-27.483 21.888 1
16.23 9.2875 1
15.712 12.114 1
-0.93781 -13.015 1
-26.454 -29.841 1
-26.468 -19.349 1
-12.385 42.208 1
-12.621 2.8773 1
-37.096 -16.439 1
-28.162 44.041 1
55.982 12.495 1
-11.06 -8.0257 1
30.438 0.9723 1
-12.375 2.0733 1
31.62 20.096 1
46.133 -4.8637 1
-8.1937 -26.508 1
-26.685 -19.288 1
14.904 9.4978 1
-9.5167 40.674 1
-48.599 13.518 1
-4.0572 -26.999 1
-23.079 6.5672 1
17.394 5.8208 1
57.695 13.45 1
-27.303 -29.885 1
-28.947 41.587 1
5.4807 -49.414 1
-2.6062 -5.6068 1
-10.056 21.763 1
-41.433 3.0788 1
14.883 12.023 1
14.102 26.132 1
-10.582 20.778 1
57.386 13.552 1
-38.187 -18.862 1
-7.5419 42.233 1
0.33896 -16.565 1
-46.923 12.842 1
13.357 -27.962 1
-0.22132 9.1588 1
-11.915 2.7937 1
0.72869 11.908 1
27.072 -19.216 1
-50.162 10.3 1
27.996 13.996 1
-2.2691 -12.287 1
16.825 -27.858 1
16.797 8.2494 1
9.531 49.217 1
-9.7402 -38.034 1
3.6744 -51.773 1
12.358 43.325 1
-41.567 -37.817 1
-9.9712 23.536 1
3.354 13.311 1
5.4939 -45.806 1
-13.98 39.109 1
-15.918 -11.987 1
-30.48 24.162 1
-37.143 -18.651 1
-29.905 43.408 1
30.951 15.255 1
-30.765 23.101 1
-1.002 12.504 1
13.783 25.88 1
-39.697 0.97727 1
-13.078 -37.535 1
5.7174 -48.294 1
-26.366 6.5078 1
-30.484 26.868 1
-0.76905 -13.836 1
-13.845 -40.949 1
-1.8353 -2.7343 1
-0.69668 -16.625 1
-4.2494 -28.71 1
0.39365 -51.249 1
-7.7328 42.118 1
30.168 -18.69 1
-9.922 40.446 1
-26.293 -29.324 1
28.978 -14.576 1
13.932 -5.7802 1
-33.94 -21.045 1
13.393 11.697 1
15.39 -27.485 1
1.6039 12.751 1
29.463 0.30724 1
-24.982 5.9525 1
25.026 -39.821 1
-28.885 26.687 1
-23.678 8.4136 1
28.13 -1.6032 1
15.396 14.116 1
47.512 -2.4673 1
15.525 28.614 1
-12.215 42.423 1
9.9855 48.194 1
16.183 11.915 1
27.417 -17.894 1
44.298 -3.008 1
-40.629 -1.5342 1
-19.579 -10.253 1
27.535 -38.805 1
14.186 27.548 1
-28.747 40.787 1
0.7343 -12.388 1
-8.9528 3.7392 1
-11.647 24.484 1
9.7761 42.251 1
54.495 15.259 1
0.21472 15.613 1
53.128 16.41 1
-9.2932 21.42 1
-14.959 -37.973 1
55.706 15.593 1
-16.478 -9.7547 1
55.097 11.394 1
24.631 0.10708 1
-13.226 19.206 1
32.308 18.965 1
1.3299 14.473 1
-51.669 11.054 1
-14.27 -43.528 1
17.137 -27.667 1
-1.3868 -14.266 1
-3.8861 -8.1006 1
27.659 2.0204 1
1.8386 -15.05 1
46.269 -27.345 1
-35.565 -17.253 1
14.439 -5.001 1
-7.4801 -29.038 1
-41.153 -40.477 1
-12.808 24.073 1
-25.982 9.401 1
15.42 -28.904 1
-47.666 15.592 1
26.894 -38.447 1
28.528 -18.441 1
46.904 -20.966 1
26.388 -2.3045 1
26.093 -38.97 1
-18.576 -10.776 1
33.971 37.791 1
-11.774 19.52 1
48.085 -4.8226 1
8.5694 45.919 1
-50.574 10.328 1
-3.9884 -26.614 1
25.284 -40.82 1
-12.74 18.019 1
31.001 -2.4973 1
30.632 -15.259 1
27.678 -41.838 1
-24.927 -19.607 1
26.096 -37.849 1
-15.896 -7.4717 1
-38.072 -13.933 1
-41.546 -40.283 1
-27.059 -20.237 1
12.63 -3.6591 1
10.45 45.236 1
18.09 -23.874 1
1.2971 -50.814 1
8.5389 48.25 1
15.439 6.84 1
-27.035 -30.135 1
-7.9021 24.889 1
18.864 -27.251 1
27.182 1.0152 1
-11.861 39.214 1
-24.654 6.372 1
-36.25 -41.859 1
-12.591 43.088 1
27.068 -38.267 1
43.427 -22.44 1
26.154 -2.5349 1
26.618 -43.483 1
-25.476 -20.126 1
14.739 7.5948 1
-42.78 2.0899 1
-11.628 2.5449 1
-29.972 43.731 1
29.692 2.473 1
-37.972 -19.123 1
-17.144 -8.1702 1
42.777 -23.809 1
4.1097 -13.075 1
27.923 -0.47356 1
10.076 25.316 1
-25.524 -27.929 1
7.7357 41.886 1
45.847 -23.567 1
-44.785 -0.40939 1
-14.281 -42.612 1
27.635 13.582 1
-3.6038 -4.7756 1
34.816 38.53 1
45.515 -23.467 1
45.004 1.2423 1
30.081 -40.847 1
16.374 -28.924 1
31.349 17.372 1
3.2242 -12.209 1
29.896 -40.139 1
-29.297 8.3418 1
56.904 12.402 1
13.911 13.38 1
33.909 18.199 1
-13.411 -41.877 1
15.397 28.262 1
-38.485 -39.205 1
-51.856 10.435 1
-28.925 42.172 1
26.484 -44.187 1
17.08 9.6196 1
-16.071 -41.057 1
44.929 -21.122 1
-14.134 -43.253 1
-47.924 15.334 1
34.456 37.713 1
25.146 -42.237 1
-29.466 7.9603 1
-38.098 -39.403 1
14.384 -27.183 1
-11.575 3.7107 1
-28.885 39.266 1
34.218 17.38 1
0.84317 -12.43 1
-12.767 -41.71 1
7.4077 47.518 1
-12.552 20.665 1
16.358 12.012 1
28.767 19.5 1
-8.1244 -1.0158 1
-1.5555 -10.534 1
-12.089 3.5375 1
55.056 10.759 1
-15.254 -43.941 1
-11.746 42.865 1
-3.5768 -7.9915 1
-8.0389 -27.238 1
27.851 1.656 1
27.111 11.044 1
-27.933 24.878 1
16.127 -8.6601 1
44.334 -28.965 1
16.35 -29.256 1
30.081 14.058 1
-0.12852 -14.525 1
43.777 -24.451 1
-50.376 12.378 1
-13.504 -42.449 1
-31.098 41.627 1
-12.492 -43.061 1
14.221 13.56 1
-41.356 3.1801 1
-38.506 -19.461 1
-51.48 10.958 1
28.81 -18.533 1
29.888 -17.446 1
-2.2415 -10.402 1
3.0754 -51.994 1
15.339 -7.0345 1
-50.52 13.619 1
4.8163 -48.43 1
-11.501 39.422 1
14.558 11.466 1
13.08 25.965 1
-49.506 12.687 1
-27.132 -30.624 1
26.541 -36.624 1
36.349 33.308 1
0.84138 -16.915 1
-30.93 43.631 1
-46.333 13.66 1
-2.4026 -11.952 1
15.993 12.494 1
-11.48 -39.108 1
56.974 15.538 1
-10.646 3.4718 1
-11.846 21.511 1
17.638 -28.374 1
31.384 17.085 1
-13.379 20.423 1
-12.448 0.64167 1
13.352 13.417 1
54.159 11.379 1
-26.629 20.136 1
53.234 13.875 1
14.042 12.671 1
-47.951 12.895 1
30.15 16.36 1
-27.253 -30.103 1
12.169 28.772 1
19.617 -27.56 1
-40.306 -1.5709 1
-27.047 25.239 1
16.064 12.729 1
-13.594 -8.7445 1
53.867 13.423 1
-9.2058 -39.181 1
56.943 14.46 1
-37.253 -14.517 1
-26.818 23.2 1
-26.594 23.146 1
25.915 -17.461 1
11.446 28 1
-10.608 42.114 1
2.0969 11.463 1
-6.0146 -27.868 1
-29.515 23.279 1
-27.498 22.309 1
-28.411 7.4995 1
45.913 0.84889 1
-41.305 -0.82997 1
28.965 -18.603 1
9.9462 44.774 1
55.4 15.401 1
-4.5632 -26.157 1
-38.887 -39.448 1
-27.485 -28.965 1
11.045 27.37 1
28.677 -41.245 1
4.838 -49.878 1
43.877 -27.438 1
55.514 10.226 1
47.803 -6.1324 1
-12.215 -39.561 1
29.524 -41.601 1
28.838 -1.5189 1
-27.893 21.821 1
32.9 17.964 1
-9.9286 5.111 1
-51.469 10.66 1
-12.715 -8.6097 1
32.216 -1.2952 1
15.881 6.443 1
47.448 -21.553 1
48.302 -4.8019 1
-4.5804 -27.33 1
-25.171 -20.502 1
-37.611 -41.995 1
-25.215 9.2318 1
11.214 47.703 1
30.226 -16.167 1
-15.991 -41.046 1
10.089 45.992 1
4.7453 -52.953 1
-12.928 21.552 1
-39.339 1.9818 1
-13.013 42.858 1
34.212 19.197 1
28.975 -3.5686 1
-10.772 -27.594 1
-11.401 24.862 1
18.041 -27.874 1
46.064 -3.775 1
-48.953 11.559 1
-26.278 23.548 1
-47.366 14.102 1
18.427 -28.486 1
-17.714 -12.199 1
47.849 -24.738 1
-2.3025 -27.924 1
-12.709 37.23 1
-14.5 5.0907 1
-37.083 -20.463 1
-14.546 -8.4976 1
25.495 -43.238 1
-6.495 -26.014 1
-16.599 -9.3815 1
35.259 35.562 1
-26.374 20.099 1
-10.129 0.54264 1
31.369 -14.05 1
-13.246 -8.5033 1
26.601 -1.0343 1
-36.1 -16.195 1
-10.511 39.927 1
-36.218 -42.552 1
45.646 -23.758 1
-37.771 -15.913 1
2.2181 -52.024 1
13.979 13.352 1
-47.654 14.026 1
-3.8375 -29.462 1
44.626 2.2195 1
-14.369 42.739 1
25.217 -2.5673 1
-1.6835 -14.519 1
-26.389 -30.541 1
-26.539 5.847 1
-9.0982 -26.89 1
-27.916 42.635 1
27.078 10.937 1
44.189 -3.4458 1
-19.808 -11.195 1
-37.301 -13.761 1
-37.378 -17.095 1
-28.59 -28.047 1
-9.6725 -27.26 1
2.2569 9.4943 1
-31.732 25.81 1
-30.383 40.563 1
16.891 5.9619 1
12.736 26.47 1
13.951 -8.2847 1
4.0262 -54.394 1
36.389 34.91 1
13.372 -29.487 1
25.883 -41.134 1
52.822 16.197 1
28.856 14.945 1
13.047 28.322 1
42.845 -26.41 1
30.777 -1.1487 1
-41.674 -41.423 1
7.9656 43.467 1
16.157 13.448 1
-37.681 -15.363 1
28.309 18.141 1
-41.508 0.06608 1
-25.899 -29.725 1
29.29 -40.708 1
-39.323 -39.808 1
44.437 -0.97264 1
-14.643 -9.6097 1
-37.147 -14.591 1
16.902 9.5172 1
54.348 14.517 1
7.0719 45.253 1
-13.506 -9.7406 1
30.817 19.251 1
11.728 -8.8165 1
14.656 14.494 1
-9.381 -26.839 1
-50.157 11.165 1
-17.15 -42.215 1
14.281 -27.66 1
-14.383 -7.0625 1
51.482 16.426 1
-6.2734 -29.707 1
-43.753 2.0075 1
25.488 -36.621 1
0.67816 -11.441 1
29.97 -17.337 1
28.354 -40.626 1
-26.571 8.8432 1
-15.52 -44.769 1
-49.436 11.35 1
-36.676 -17.729 1
-7.0628 -30.408 1
14.16 -27.592 1
12.155 45.456 1
-35.888 -19.047 1
-13.865 -6.7598 1
13.859 27.316 1
-37.634 -22.251 1
-30.748 39.992 1
0.015574 9.3368 1
-28.46 44.026 1
16.157 -8.6378 1
31.232 -18.571 1
-14.004 41.695 1
46.247 -25.125 1
-14.23 -41.46 1
-2.1397 -28.17 1
-12.694 18.709 1
-5.2883 -26.282 1
-39.332 2.7141 1
27.327 0.62146 1
45.675 -21.927 1
47.479 -1.3811 1
18.358 -27.104 1
-10.815 -41.948 1
-29.082 9.869 1
2.5311 11.778 1
-1.4903 13.419 1
-12.712 -41.124 1
-10.63 2.8907 1
-14.886 3.5136 1
-47.996 13.814 1
-9.9395 -0.09387 1
25.93 -39.058 1
55.364 14.5 1
-11.429 2.9421 1
-3.2426 -8.8035 1
-9.9769 20.843 1
-2.6348 -15.457 1
-38.415 -41.068 1
-29.664 40.896 1
3.332 -51.706 1
3.1451 12.03 1
15.19 29.158 1
28.969 -1.0467 1
30.543 -18.722 1
-7.9869 -28.356 1
43.419 -23.717 1
29.484 14.055 1
-27.11 22.864 1
14.277 10.28 1
-16.035 -40.959 1
25.445 -41.804 1
-25.857 21.56 1
-15.707 -44.012 1
28.083 16.615 1
16.538 -27.22 1
8.5075 46.295 1
-1.2144 -13.912 1
35.492 35.195 1
46.466 1.6673 1
-3.4017 -25.778 1
17.687 6.0029 1
15.411 10.063 1
-29.949 39.137 1
30.235 -1.8824 1
-7.2939 -29.075 1
27.785 -3.5617 1
-10.63 41.655 1
10.276 24.688 1
-18.862 -10.204 1
2.0822 -17.131 1
32.777 32.848 1
-25.5 -29.833 1
-9.8612 -37.343 1
-35.913 -42.387 1
-12.064 2.2778 1
9.5218 42.473 1
-26.129 8.5355 1
-11.905 -38.609 1
-26.119 7.7337 1
4.767 -53.094 1
-0.42047 -11.814 1
-0.54025 -14.56 1
9.0465 47.47 1
28.69 -14.998 1
-37.891 -39.898 1
-12.207 -6.8277 1
31.808 17.84 1
7.7977 41.592 1
56.644 11.423 1
-39.397 -41.197 1
32.115 15.142 1
35.854 37.721 1
46.778 -27.326 1
29.001 16.678 1
18.646 -26.06 1
44.691 -24.164 1
1.1774 9.0725 1
4.8743 -49.858 1
42.878 -25.281 1
13.493 -3.6444 1
53.558 12.706 1
4.2808 -49.764 1
47.946 -5.3644 1
56.356 13.364 1
28.532 1.2281 1
-1.9721 13.977 1
32.633 35.881 1
-14.218 1.5008 1
-0.49458 -1.1942 1
32.738 32.931 1
-3.9778 -6.3267 1
-37.461 -14.36 1
-13.046 38.517 1
-42.569 -41.426 1
-26.131 8.8568 1
-19 -10.192 1
0.32094 11.019 1
-1.829 -11.062 1
-4.4659 -7.8503 1
25.762 -39.988 1
12.604 25.844 1
47.504 -2.9902 1
-8.4896 41.294 1
-39.325 -41.745 1
-8.9736 38.411 1
-17.093 -12.085 1
-8.2762 -25.875 1
10.647 -2.5511 1
34.86 35.138 1
-15.104 -6.9838 1
-30.294 24.137 1
31.086 17.356 1
-13.54 -38.862 1
46.02 -2.4096 1
28.635 -17.14 1
17.775 -26.137 1
-48.404 11.974 1
34.231 34.253 1
-3.5476 -3.5645 1
-27.753 -19.767 1
18.971 -27.706 1
-50.554 11.629 1
-5.2282 -27.469 1
-6.5109 -28.66 1
-36.997 -42.139 1
-1.0798 -16.72 1
8.6066 48.186 1
-29.731 42.368 1
-50.785 11.473 1
2.5236 11.927 1
44.576 -28.529 1
-2.9142 10.478 1
29.516 14.06 1
17.016 -28.648 1
9.7252 44.77 1
-2.5126 -4.4916 1
7.1731 43.21 1
-29.132 26.351 1
27.76 0.091951 1
29.374 20.045 1
-23.417 -29.204 1
10.307 -3.3366 1
17.904 -27.752 1
44.465 -21.486 1
47.323 -3.5672 1
30.157 1.013 1
-30.298 40.27 1
29.148 -0.59648 1
31.51 17.079 1
14.616 14.504 1
-0.4306 15.871 1
-26.86 26.504 1
4.8982 -53.309 1
3.6906 -45.438 1
45.632 0.20197 1
-14.29 -43.125 1
15.769 7.2576 1
-14.249 1.696 1
25.375 -37.125 1
-30.808 37.845 1
12.228 -6.295 1
0.77381 -16.564 1
-14.3 -40.934 1
3.9774 -52.881 1
-41.478 -0.38231 1
54.749 9.9999 1
16.889 6.7707 1
31.667 15.226 1
-39.002 -1.0698 1
27.189 -19.397 1
-13.863 39.089 1
-41.844 -3.0854 1
-25.029 -19.993 1
4.6074 -49.426 1
-8.8352 21.297 1
10.179 25.678 1
10.831 43.166 1
-13.161 3.6313 1
11.662 -9.5067 1
47.388 -2.3586 1
45.469 -27.41 1
27.795 -0.0047831 1
29.71 -17.334 1
45.272 -4.9454 1
-12.275 3.6563 1
-37.328 -14.311 1
46.164 -5.1039 1
27.762 -38.628 1
16.194 12.461 1
-0.45012 -14.995 1
43.18 -24.302 1
54.465 10.095 1
7.1366 46.409 1
-15.331 -41.959 1


==> data_us_1.tex <==
x y label
64 1 2
64 1 2
64 1 2
60 0 2
60 -1 2
65 1 2
59 -1 2
65 0 2
65 1 2
65 1 2
60 0 2
61 2 2
63 1 2
62 1 2
63 0 2
61 2 2
60 1 2
63 0 2
62 1 2
63 1 2
60 1 2
63 1 2
62 2 2
63 1 2
15 -14 2
63 2 2
62 3 2
62 1 2
64 1 2
65 2 2
64 1 2
-27 -52 4
-27 -52 4
-36 -53 4
-35 -53 4
-35 -53 4
-34 -53 4
-34 -53 4
-33 -52 4
-34 -52 4
-35 -52 4
-34 -54 4
-34 -54 4
-34 -52 4
-34 -52 4
-31 -54 4
-31 -54 4
-31 -54 4
-30 -53 4
-31 -54 4
-30 -54 4
-31 -54 4
-31 -54 4
-30 -54 4
-29 -53 4
-30 -53 4
-30 -53 4
-30 -53 4
34 -35 5
34 -35 5
34 -35 5
31 -34 5
31 -34 5
31 -35 5
29 -34 5
32 -35 5
32 -34 5
31 -37 5
34 -34 5
31 -35 5
32 -34 5
32 -34 5
32 -35 5
34 -33 5
33 -35 5
32 -35 5
30 -34 5
32 -36 5
30 -36 5
33 -36 5
32 -36 5
31 -36 5
30 -37 5
29 -36 5
29 -36 5
30 -36 5
30 -36 5
29 -37 5
13 48 7
18 43 7
15 50 7
15 50 7
14 49 7
13 48 7
13 49 7
14 49 7
15 49 7
15 49 7
15 49 7
16 49 7
16 51 7
16 52 7
16 51 7
16 51 7
16 51 7
16 52 7
14 51 7
14 51 7
15 52 7
15 52 7
15 51 7
14 51 7
15 51 7
15 52 7
17 50 7
17 49 7
17 50 7
17 50 7
31 6 6
31 5 6
30 6 6
29 7 6
28 8 6
28 7 6
30 6 6
31 7 6
32 6 6
32 6 6
32 6 6
32 7 6
32 7 6
28 8 6
31 4 6
31 7 6
27 9 6
31 5 6
27 9 6
32 7 6
32 5 6
31 5 6
32 5 6
31 7 6
26 8 6
35 0 6
35 0 6
30 7 6
31 7 6
30 7 6
31 7 6
30 8 6
27 0 6
30 7 6
27 0 6
33 6 6
33 6 6
32 6 6
28 9 6
28 9 6
26 0 6
27 0 6
29 9 6
-37 42 8
-37 41 8
-37 42 8
-36 41 8
-37 42 8
-40 41 8
-40 41 8
-40 41 8
-39 41 8
-40 41 8
-38 42 8
-38 42 8
-38 42 8
-38 42 8
-38 42 8
-39 41 8
-39 42 8
-39 40 8
-39 42 8
-39 42 8
-39 41 8
-37 40 8
-37 40 8
-37 40 8
-37 39 8
-37 41 8
-37 40 8
-56 10 1
-58 9 1
-57 10 1
-57 13 1
-58 12 1
-57 14 1
-57 14 1
-58 10 1
-57 12 1
-56 11 1
-57 11 1
-57 11 1
-58 12 1
-58 12 1
-57 12 1
-58 10 1
-58 11 1
-58 11 1
-58 10 1
-58 11 1
-58 10 1
-59 -18 0
-59 -18 0
-59 -18 0
-61 -20 0
-61 -19 0
-59 -20 0
-59 -19 0
-61 -18 0
-61 -18 0
-59 -19 0
-59 -19 0
-59 -18 0
-61 -19 0
-61 -19 0
-61 -19 0
-59 -19 0
-61 -18 0
-59 -20 0
-59 -19 0
-59 -19 0
-61 -19 0
-61 -19 0
-61 -19 0
-61 -19 0
-59 -19 0
-61 -19 0
-59 -20 0
-59 -20 0
-59 -19 0
-8 -33 9
-8 -34 9
-7 -33 9
-5 -34 9
-8 -32 9
-9 -34 9
-8 -33 9
-8 -33 9
-8 -35 9
-9 -38 9
-10 -38 9
-10 -38 9
-9 -38 9
-9 -37 9
-9 -38 9
-10 -38 9
-9 -38 9
-10 -39 9
-10 -39 9
-10 -39 9
-10 -39 9
-9 -36 9
-8 -36 9
-12 -40 9
-12 -40 9
-12 -40 9
-12 -40 9
-12 -39 9
-12 -35 9
-12 -40 9
16 24 3
15 23 3
15 24 3
16 24 3
15 24 3
17 21 3
17 22 3
16 22 3
16 22 3
16 22 3
16 23 3
16 22 3
16 23 3
16 23 3
16 24 3
16 24 3
18 23 3
17 21 3
17 22 3
17 22 3
17 21 3
17 21 3
17 24 3
17 24 3
18 23 3
18 23 3
18 24 3
-36 -50 4
24 47 7
17 47 7
-35 -48 4
-14 -38 9
20 45 7
54 9 2
41 -36 5
36 2 6
-31 -49 4
37 -3 6
-64 11 1
12 25 3
21 46 7
-43 34 8
23 47 7
-55 -17 0
-36 -47 4
-44 39 8
-12 -44 9
28 0 6
-42 33 8
12 26 3
36 -34 5
-43 40 8
-63 11 1
-31 -49 4
38 0 6
11 26 3
59 6 2
28 0 6
-64 9 1
-8 -45 9
25 47 7
-59 13 1
-46 38 8
10 27 3
8 31 3
-34 -48 4
-46 39 8
28 0 6
-65 8 1
-50 -15 0
-39 34 8
14 29 3
56 1 2
-64 11 1
-59 12 1
-41 34 8
53 11 2
35 -32 5
-47 35 8
-66 14 1
-45 32 8
-11 -45 9
11 26 3
36 2 6
13 26 3
-43 32 8
12 26 3
-11 -41 9
52 8 2
30 0 6
-64 8 1
-43 37 8
36 -30 5
-67 14 1
26 50 7
17 31 3
54 11 2
-54 -16 0
41 -36 5
-14 -41 9
-14 -41 9
41 -33 5
-67 13 1
-9 -43 9
-36 -45 4
-47 37 8
37 -35 5
-47 39 8
63 -2 2
-30 -47 4
24 46 7
-43 35 8
59 6 2
37 0 6
-38 -48 4
-43 36 8
26 44 7
-35 -49 4
55 7 2
-43 38 8
-13 -42 9
38 -36 5
10 29 3
-46 39 8
55 -3 2
-31 -48 4
-38 -50 4
-63 10 1
28 0 6
-11 -43 9
53 11 2
40 -36 5
-43 37 8
-12 -41 9
-61 13 1
-36 -48 4
36 0 6
20 47 7
-53 -20 0
-42 39 8
-36 -45 4
-34 -50 4
-53 -18 0
-37 -49 4
-55 -19 0
37 -3 6
56 8 2
52 10 2
16 30 3
26 44 7
-32 -46 4
-43 40 8
-55 -16 0
22 49 7
34 -37 5
-29 -52 4
-67 10 1
8 31 3
37 1 6
53 4 2
10 33 3
-56 -13 0
-45 38 8
19 44 7
-54 -20 0
-50 -16 0
39 -33 5
11 29 3
26 46 7
-57 -16 0
-36 -47 4
19 44 7
-41 36 8
53 10 2
-47 38 8
-40 41 8
39 -31 5
23 47 7
-44 34 8
54 9 2
-53 -16 0
-67 9 1
50 10 2
-44 34 8
22 46 7
58 8 2
-12 -41 9
-32 -47 4
62 -2 2
28 0 6
58 2 2
34 -30 5
40 -28 5
34 -31 5
36 -32 5
24 49 7
-45 37 8
21 47 7
-11 -39 9
57 12 2
10 24 3
-13 -41 9
-17 -22 0
36 -2 6
-55 -12 0
-46 36 8
52 10 2
-11 -44 9
33 0 6
-44 33 8
-41 38 8
-40 34 8
-33 -47 4
25 48 7
33 0 6
-64 10 1
-52 -18 0
-53 -16 0
32 -1 6
28 -1 6
-45 38 8
-31 -49 4
36 -30 5
-56 -17 0
11 23 3
37 -1 6
36 -28 5
-9 -44 9
-53 -17 0
31 -30 5
-38 -49 4
39 -33 5
38 -36 5
40 -29 5
-54 -16 0
12 25 3
-9 -43 9
38 -29 5
24 49 7
-52 -11 0
53 9 2
36 -33 5
-54 -20 0
38 -34 5
33 -1 6
41 -33 5
-55 -17 0
20 49 7
22 45 7
13 29 3
-56 -17 0
-61 13 1
54 8 2
-35 -49 4
36 -34 5
33 -1 6
-43 37 8
54 5 2
28 -1 6
11 27 3
6 29 3
52 8 2
-53 -15 0
-13 -44 9
20 45 7
-55 -16 0
-51 -13 0
13 24 3
-30 -48 4
22 48 7
-60 13 1
-12 -42 9
-32 -50 4
16 47 7
34 -1 6
53 10 2
12 30 3
35 -1 6
38 0 6
-56 -18 0
-12 -43 9
12 29 3
41 -36 5
-12 -42 9
-30 -48 4
-64 12 1
-55 -20 0
56 1 2
39 -31 5
-11 -45 9
-44 38 8
55 -3 2
-53 -17 0
-46 36 8
9 28 3
-45 36 8
13 31 3
11 28 3
39 -30 5
25 44 7
-41 34 8
54 10 2
57 -1 2
38 -28 5
35 -2 6
54 11 2
52 8 2
-43 40 8
-38 33 8
-67 13 1
16 47 7
59 8 2
33 -39 5
-57 -15 0
20 46 7
-7 -28 0
-47 43 8
26 45 7
51 12 2
52 11 2
58 5 2
-35 -46 4
-39 -48 4
10 27 3
58 1 2
-37 -45 4
-36 -45 4
23 47 7
38 -34 5
-57 -17 0
-45 39 8
10 24 3
-52 -16 0
-42 32 8
25 47 7
-35 -48 4
35 1 6
-37 -49 4
41 -32 5
22 43 7
-36 -49 4
30 -2 6
-32 -40 4
8 31 3
-31 -50 4
-66 13 1
-47 40 8
36 -33 5
-11 -45 9
23 47 7
-12 -43 9
-43 32 8
-66 10 1
-54 -17 0
13 29 3
13 25 3
54 11 2
-43 32 8
50 12 2
16 43 7
36 -0 6
33 -0 6
57 3 2
15 30 3
-66 14 1
-64 8 1
55 4 2
53 9 2
54 12 2
-51 -16 0
28 0 6
-42 37 8
38 0 6
12 32 3
-55 -15 0
36 0 6
25 50 7
36 -32 5
21 49 7
-39 37 8
37 -29 5
-63 15 1
-51 -15 0
-32 -46 4
-63 8 1
-47 38 8
11 29 3
25 48 7
-38 40 8
-60 16 1
14 33 3
-10 -43 9
-44 39 8
33 -1 6
56 1 2
26 49 7
58 2 2
-32 -49 4
24 49 7
-30 -50 4
40 -32 5
58 2 2
-17 -22 0
35 -1 6
14 33 3
-54 -20 0
-39 35 8
-64 12 1
-11 -39 9
-59 13 1
-55 -14 0
57 -2 2
11 32 3
-10 -42 9
41 -37 5
-63 9 1
27 0 6
-30 -48 4
-55 -19 0
24 47 7
11 33 3
-34 35 8
-30 -48 4
-57 -15 0
9 28 3
34 -31 5
-15 -43 9
51 10 2
37 0 6
12 29 3
26 47 7
-11 -44 9
14 26 3
55 4 2
-37 -46 4
34 -39 5
33 0 6
-38 33 8
-55 -12 0
37 -36 5
-65 9 1
-12 -39 9
11 32 3
21 47 7
-56 -16 0
-37 -47 4
-65 13 1
-27 -50 2
-55 -17 0
13 25 3
12 30 3
-31 -50 4
-42 34 8
35 -1 6
20 45 7
-52 -18 0
58 8 2
40 -29 5
-57 -17 0
10 29 3
-13 -40 9
6 29 3
-33 -50 4
-63 9 1
12 23 3
37 -31 5
-64 11 1
38 -29 5
25 44 7
22 43 7
18 49 7
11 28 3
-46 38 8
-43 33 8
14 27 3
36 2 6
-46 38 8
-65 11 1
-36 -49 4
-58 -15 0
-43 37 8
-41 39 8
36 -30 5
-53 -14 0
-13 46 1
-29 -49 4
25 45 7
-29 -50 4
38 -33 5
23 46 7
-35 -48 4
-9 -43 9
-38 -48 4
-65 11 1
-41 37 8
-47 43 8
24 49 7
41 -33 5
26 44 7
-65 14 1
-31 -48 4
26 47 7
-34 -54 4
56 13 2
-58 -15 0
-63 13 1
-29 -49 4
-11 -39 9
-46 35 8
-54 -14 0
-43 36 8
-64 10 1
-10 -45 9
-65 11 1
36 -28 5
-60 16 1
39 -31 5
34 -39 5
7 31 3
33 -1 6
57 4 2
33 0 6
39 -33 5
36 -30 5
-41 34 8
21 46 7
37 1 6
-43 39 8
33 0 6
-36 -48 4
40 -36 5
34 -38 5
-29 -50 4
13 25 3
13 31 3
30 0 6
-66 11 1
27 46 7
-31 -47 4
22 45 7
10 25 3
11 25 3
37 -1 6
12 26 3
38 -31 5
-34 -48 4
-45 37 8
-30 -48 4
-53 -20 0
41 -28 5
-64 14 1
35 0 6
8 28 3
-34 -50 4
10 32 3
-52 -11 0
-39 36 8
37 -30 5
-11 -42 9
12 32 3
53 12 2
56 -3 2
18 49 7
28 -1 6
13 29 3
39 -31 5
-44 40 8
-14 -40 9
28 -1 6
10 30 3
-64 11 1
57 4 2
-57 -17 0
59 0 2
26 47 7
55 10 2
-56 -13 0
-54 -18 0
12 29 3
12 30 3
41 -36 5
37 -29 5
36 2 6
9 26 3
-47 40 8
-9 -41 9
25 49 7
40 -36 5
33 -39 5
58 4 2
-60 16 1
51 11 2
16 47 7
13 25 3
40 -34 5
59 7 2
19 42 7
36 1 6
37 1 6
-48 38 8
11 27 3
49 7 2
-64 11 1
-65 11 1
13 29 3
-52 -14 0
-55 -12 0
-34 -49 4
-65 14 1
57 -1 2
37 -33 5
-36 -48 4
-37 -46 4
52 11 2
-15 -44 9
40 -29 5
-65 14 1
15 30 3
22 45 7
54 4 2
38 -31 5
-9 -45 9
-13 -44 9
-65 10 1
-65 8 1
-65 13 1
25 48 7
-60 16 1
-46 39 8
-34 -48 4
-40 33 8
-54 -17 0
28 0 6
26 48 7
-50 -16 0
57 12 2
40 -29 5
-59 11 1
58 8 2
36 -31 5
37 0 6
-10 -40 9
37 -35 5
56 9 2
-10 -45 9
-55 -15 0
59 8 2
-42 38 8
-12 -43 9
-42 38 8
33 -4 6
27 0 6
21 49 7
56 0 2
9 28 3
-52 -14 0
-56 -18 0
10 32 3
12 23 3
-64 10 1
-40 34 8
56 8 2
54 12 2
28 2 6
-62 12 1
-54 -16 0
-38 -46 4
37 -1 6
13 24 3
-42 32 8
-63 15 1
59 6 2
14 33 3
28 0 6
26 43 7
58 4 2
-34 -47 4
26 48 7
38 -34 5
34 2 6
-52 -16 0
59 1 2
36 1 6
55 11 2
-35 -50 4
11 24 3
57 3 2
55 10 2
-30 -50 4
-50 -16 0
54 6 2
16 21 3
30 0 6
14 28 3
36 -30 5
33 -39 5
-67 10 1
53 3 2
30 -2 6
18 48 7
-63 15 1
-32 -48 4
13 30 3
19 42 7
33 1 6
35 2 6
25 45 7
41 -29 5
-13 -46 9
24 47 7
-45 40 8
36 -30 5
-37 -49 4
38 -36 5
-8 -45 9
26 43 7
-57 -15 0
27 47 7
36 -33 5
14 26 3
-42 39 8
56 7 2
37 -30 5
-11 -45 9
20 45 7
-45 36 8
20 47 7
56 13 2
24 46 7
52 11 2
36 1 6
19 44 7
24 47 7
30 -1 6
-51 -17 0
54 7 2
10 27 3
-65 8 1
-8 -44 9
13 27 3
35 -36 4
14 29 3
-65 14 1
-44 33 8
-33 41 8
-10 -44 9
-44 40 8
-64 7 1
8 26 3
33 -1 6
12 26 3
37 -28 5
-46 35 8
-44 39 8
-45 32 8
33 1 6
12 30 3
-9 -42 9
18 48 7
37 0 6
-45 38 8
-51 -15 0
-66 14 1
30 0 6
22 47 7
32 -13 4
37 -32 5
35 -32 5
34 -0 6
6 29 3
-9 -44 9
-33 -44 4
18 48 7
-30 -47 4
-33 -44 4
9 28 3
26 44 7
10 24 3
-36 -49 4
38 0 6
58 4 2
-44 40 8
-14 -41 9
52 12 2
-63 10 1
-14 -41 9
-41 32 8
31 0 6
37 -30 5
-13 46 1
-45 39 8
51 10 2
-15 -44 9
-14 -42 9
-60 16 1
-54 -16 0
-53 -14 0
-7 -28 0
58 -2 2
33 1 6
25 48 7
-13 -43 9
14 31 3
-66 12 1
39 -36 5
16 21 3
26 48 7
-36 -49 4
26 45 7
50 8 2
40 -34 5
-37 -45 4
20 47 7
-39 34 8
38 2 6
51 11 2
-38 -45 4
25 45 7
40 -36 5
-40 33 8
52 10 2
30 2 6
33 0 6
55 7 2
54 10 2
-14 -44 9
13 29 3
57 12 2
26 44 7
-66 13 1
-66 10 1
27 45 7
38 -36 5
-56 -16 0
39 -32 5
-13 -38 9
39 -34 5
55 4 2
53 10 2
-45 38 8
-46 34 8
58 2 2
54 8 2
-14 -44 9
13 31 3
-64 8 1
20 49 7
-55 -19 0
-64 11 1
19 48 7
-47 35 8
-9 -42 9
40 -36 5
-11 -41 9
-29 -48 4
-54 -16 0
-35 -48 4
33 -0 6
37 -32 5
41 -27 5
53 3 2
-52 -19 0
-13 -43 9
39 -34 5
39 -33 5
35 -1 6
59 6 2
-14 -42 9
-11 -42 9
39 -31 5
-10 -42 9
27 46 7
-35 -46 4
-64 10 1
12 26 3
-13 -45 9
-53 -17 0
-63 8 1
33 -1 6
37 -29 5
-36 -46 4
-9 -45 9
-8 -46 9
-64 10 1
-41 35 8
-42 37 8
-10 -42 9
-32 -50 4
-39 31 8
18 48 7
-55 -18 0
19 44 7
-66 13 1
13 -6 2
57 3 2
-60 16 1
-66 14 1
54 7 2
39 -36 5
21 43 7
-11 -44 9
35 -33 5
32 4 6
-45 32 8
-11 -43 9
12 32 3
23 46 7
25 48 7
35 0 6
59 1 2
-54 -17 0
37 -30 5
63 -2 2
-43 32 8
-46 38 8
-21 -3 9
42 -32 5
36 -28 5
-54 -17 0
41 -29 5
-12 -44 9
10 26 3
-34 -48 4
21 43 7
-35 -48 4
37 -28 5
-11 -39 9
42 -30 5
33 1 6
36 -34 5


==> data_us_2.tex <==
x y label
46.795 -8.1869 0
47.377 -4.0054 0
46.078 -7.6067 0
48.209 -4.631 0
49.59 -5.2835 0
46.82 -8.8044 0
49.496 -5.6494 0
47.001 -8.6954 0
47.374 -8.9131 0
47.867 -9.2124 0
48.346 -7.65 0
48.098 -1.3415 0
46.17 -6.7123 0
47.063 -4.6894 0
46.15 -5.6046 0
48.037 -1.7868 0
47.667 -6.861 0
46.277 -6.1949 0
47.694 -5.0728 0
46.28 -6.5649 0
48.095 -1.5386 0
46.258 -6.2867 0
47.739 -6.9293 0
46.773 -7.2758 0
47.69 -4.9869 0
47.341 -7.6205 0
47.975 -2.922 0
47.528 -7.5884 0
47.207 -8.1618 0
46.783 -7.8493 0
46.882 -7.9846 0
-18.748 -52.993 0
-18.402 -52.822 0
-17.661 -52.978 0
-16.234 -50.687 0
-16.022 -50.132 0
-16.182 -50.512 0
-15.944 -50.398 0
-16.288 -49.776 0
-17.72 -51 0
-16.628 -50.925 0
-17.195 -51.519 0
-17.379 -51.759 0
-16.829 -51.126 0
-17.612 -52.55 0
-15.501 -51.934 0
-15.655 -52.144 0
-15.472 -51.863 0
-16.588 -52.354 0
-15.122 -52.129 0
-15.001 -52.364 0
-15.063 -52.06 0
-15.244 -51.898 0
-18.41 -51.842 0
-18.763 -52.061 0
-17.05 -49.866 0
-17.299 -50.502 0
-18.451 -51.777 0
29.865 -34.48 0
29.635 -34.456 0
28.965 -34.657 0
26.872 -31.631 0
26.764 -31.668 0
26.437 -33.337 0
26.056 -31.535 0
27.998 -34.318 0
27.231 -34.163 0
27.007 -32.654 0
2.7378 -45.34 0
27.012 -33.324 0
29.852 -32.353 0
30.332 -32.915 0
26.649 -33.496 0
31.224 -32.897 0
28.418 -34.081 0
27.081 -34.277 0
27.114 -34.261 0
27.558 -34.717 0
27.672 -33.487 0
28.935 -34.568 0
27.885 -34.295 0
27.669 -33.818 0
27.526 -30.491 0
26.994 -33.093 0
30.017 -32.206 0
27.856 -34.261 0
27.254 -32.89 0
27.627 -30.249 0
-0.35568 22.047 0
-3.7345 22.038 0
-4.065 21.941 0
-4.4537 21.448 0
-4.2831 21.337 0
-0.48419 22.028 0
-2.9908 21.693 0
-4.097 21.753 0
-4.5576 21.529 0
-4.8078 21.187 0
-4.2366 21.896 0
-3.0124 21.963 0
-4.7827 23.501 0
-4.2611 23.524 0
-5.3666 23.611 0
-3.8275 23.314 0
-5.056 23.558 0
-4.9455 23.54 0
-3.0056 23.608 0
-3.2962 23.723 0
-5.4308 23.667 0
-2.0673 24.015 0
-4.399 22.396 0
-1.5923 23.937 0
-3.7665 23.671 0
-3.9144 24.179 0
-2.455 22.503 0
-4.6874 21.049 0
-2.4734 22.295 0
-5.2783 20.703 0
20.509 -22.346 0
19.718 -21.991 0
20.243 -22.668 0
21.879 -23.695 0
22.469 -24.949 0
22.493 -24.192 0
19.706 -22.382 0
22.192 -21.626 0
21.364 -21.476 0
21.808 -21.397 0
21.097 -21.314 0
21.965 -21.515 0
22.384 -21.941 0
24.159 -25.143 0
22.051 -20.775 0
22.224 -23.284 0
20.862 -24.428 0
21.223 -21.955 0
19.211 -22.579 0
22.587 -22.808 0
20.727 -21.17 0
20.502 -22.013 0
20.591 -21.53 0
23.309 -23.678 0
23.762 -25.205 0
25.08 -25.636 0
24.85 -25.569 0
22.334 -23.823 0
21.003 -22.967 0
21.026 -22.986 0
21.163 -23.033 0
22.931 -24.546 0
22.807 -25.962 0
22.751 -24.005 0
22.287 -25.543 0
21.877 -22.121 0
22.141 -21.829 0
22.046 -23.126 0
23.025 -25.341 0
23.176 -25.519 0
23.074 -26.065 0
22.669 -25.969 0
21.998 -24.549 0
-34.263 31.465 0
-34.347 31.197 0
-34.213 31.554 0
-34.428 31.07 0
-34.403 31.175 0
-31.631 31.71 0
-31.8 31.39 0
-31.546 31.494 0
-31.871 31.425 0
-31.872 31.109 0
-32.996 30.569 0
-32.959 30.925 0
-33.033 31.003 0
-32.475 31.193 0
-33.428 30.407 0
-33.692 29.131 0
-33.746 29.364 0
-32.012 30.032 0
-32.379 31.795 0
-33.76 29.324 0
-33.637 29.297 0
-33.381 32.598 0
-33.406 32.655 0
-33.458 32.675 0
-33.39 32.612 0
-33.636 31.57 0
-33.459 32.397 0
-50.814 30.896 0
-50.579 29.414 0
-50.766 30.137 0
-50.149 31.105 0
-50.408 30.219 0
-50.222 30.973 0
-50.346 31.026 0
-51.469 29.239 0
-52.794 27.352 0
-51.006 31.075 0
-51.842 28.689 0
-51.715 29.065 0
-51.015 29.094 0
-51.501 29.359 0
-51.209 30.035 0
-49.537 30.318 0
-50.857 29.775 0
-50.764 29.893 0
-50.56 29.019 0
-51.138 28.478 0
-51.2 28.202 0
-19.151 38.004 0
-18.921 37.707 0
-18.668 37.998 0
-20.058 39.066 0
-19.527 37.742 0
-19.654 37.638 0
-19.853 40.133 0
-19.845 40.733 0
-19.989 40.293 0
-19.805 40.158 0
-19.85 40.53 0
-19.386 40.567 0
-18.434 39.847 0
-19.489 39.418 0
-19.285 37.781 0
-19.248 38.203 0
-19.384 41.083 0
-19.577 39.136 0
-18.972 41.536 0
-17.99 41.222 0
-15.447 43.508 0
-17.968 40.237 0
-18.241 39.207 0
-18.041 40.065 0
-18.216 40.228 0
-18.362 40.12 0
-16.195 40.282 0
-17.628 39.733 0
-18.423 40.766 0
4.3801 -46.185 0
3.1421 -46.092 0
3.4609 -45.552 0
3.0067 -45.731 0
3.9748 -45.679 0
4.6108 -46.895 0
4.3651 -46.172 0
4.2077 -46.204 0
-10.554 -2.9301 0
4.5462 -47.559 0
5.6166 -49.562 0
5.4886 -48.718 0
5.2733 -47.927 0
4.6493 -47.59 0
5.209 -49.026 0
5.5299 -49.869 0
4.9217 -47.695 0
6.686 -51.508 0
6.445 -50.869 0
6.4606 -50.311 0
5.522 -49.303 0
3.7378 -47.465 0
3.5618 -47.532 0
1.1484 -48.486 0
1.0785 -48.338 0
1.5941 -48.776 0
1.2922 -48.5 0
1.0871 -48.344 0
2.1468 -49.142 0
0.70326 -48.131 0
0.83861 37.842 0
3.2764 38.302 0
4.1252 38.373 0
0.67228 37.778 0
3.0719 37.517 0
3.703 39.716 0
3.2926 39.484 0
4.9385 39.304 0
3.8654 39.133 0
3.222 39.36 0
4.2125 41.253 0
4.2554 41.23 0
4.6287 41.058 0
4.4327 40.996 0
4.2815 40.212 0
3.2285 39.796 0
4.6332 40.512 0
2.3048 39.314 0
3.3388 39.335 0
2.8657 39.219 0
2.7328 39.579 0
2.3989 39.625 0
4.9663 40.025 0
4.7474 40.209 0
5.1248 40.336 0
5.2306 40.249 0
5.1885 40.13 0
8.0392 -28.643 1
44.858 -8.5823 1
-1.1583 -9.0313 1
10.282 17.372 1
4.8431 20.25 1
8.0111 -26.663 1
7.703 -25.634 1
-1.7222 20.401 1
4.2263 -13.384 1
-30.798 19.396 1
-29.619 -49.439 1
-11.946 -1.9633 1
-3.2001 18.774 1
50.057 11.026 1
34.92 -29.809 1
-0.72853 -20.632 1
25.853 -10.829 1
-5.6336 12.289 1
-13.046 -17.606 1
-27.719 -48.207 1
12.807 -37.291 1
-23.252 -6.7483 1
8.3433 -31.97 1
23.21 4.1625 1
-32.872 7.7436 1
-21.33 -4.3243 1
25.907 -9.1768 1
-30.095 19.879 1
-54.169 17.882 1
23.846 5.2562 1
4.8702 32.049 1
18.534 24.78 1
33.096 6.3939 1
-7.139 -19.587 1
29.083 21.992 1
26.201 -13.012 1
-0.3498 11.944 1
-14.482 40.045 1
-32.15 -31.64 1
22.24 -0.32141 1
-18.261 21.326 1
-27.555 0.3538 1
-1.4604 32.851 1
-6.2192 60.141 1
11.242 34.675 1
-21.359 -51.515 1
34.15 10.271 1
-3.0497 56.13 1
-31.184 23.399 1
33.452 21.389 1
-2.2167 -21.808 1
24.685 1.6688 1
-17.373 -13.602 1
-32.033 -31.691 1
9.1933 -54.889 1
21.444 -8.5376 1
-19.462 21.132 1
-8.7535 1.1706 1
30.859 22.731 1
4.811 34.116 1
31.837 -36.433 1
-31.983 22.485 1
-28.379 -2.7384 1
32.05 9.922 1
31.504 -8.9595 1
-24.574 18.294 1
-52.919 21.344 1
25.402 24.635 1
-27.673 -48.189 1
29.719 -5.3839 1
41.669 7.3713 1
-33.101 -32.118 1
21.139 30.707 1
2.527 34.413 1
-30.852 -5.3563 1
53.274 -2.1255 1
-9.5665 0.90136 1
4.4838 -11.52 1
21.532 -8.3784 1
-7.5004 61.358 1
-54.536 17.834 1
9.003 -57.155 1
2.8099 19.01 1
3.2901 -17.35 1
-50.09 29.392 1
-13.614 -26.711 1
-31.561 27.286 1
-24.911 1.262 1
-17.985 -54.297 1
-31.731 4.3646 1
-7.0041 2.6098 1
11.217 -37.42 1
25.197 2.528 1
11.726 -28.422 1
7.2288 26.342 1
32.176 8.5482 1
9.4235 -49.333 1
20.719 2.5488 1
-28.898 -48.709 1
35.839 23.066 1
-12.778 8.8138 1
-23.299 -6.6715 1
-8.0067 60.499 1
-18.814 -8.2342 1
1.0855 30.877 1
-0.19361 -11.026 1
21.746 -16.936 1
3.9713 -5.8379 1
54.107 -10.328 1
8.3414 -27.903 1
42.469 8.3386 1
2.4524 3.7355 1
37.38 5.901 1
-21.603 15.908 1
-31.699 25.803 1
13.094 -35.739 1
27.796 -4.5472 1
-12.596 9.2213 1
-8.3648 -0.16103 1
10.482 -8.9648 1
-30.725 -3.4489 1
-52.096 22.161 1
-33.306 -7.2386 1
-12.581 -17.28 1
-1.46 -19.311 1
-7.5628 16.653 1
-11.824 43.146 1
-12.434 -6.4557 1
-34.662 -32.161 1
29.3 9.696 1
11.585 -12.633 1
18.084 11.697 1
-33.103 6.1129 1
11.15 -16.942 1
12.573 -35.033 1
-36.239 7.1366 1
31.45 20.468 1
-28.107 19.871 1
-34.999 -12.318 1
-3.2871 -14.045 1
-28.802 26.474 1
6.5759 -9.8717 1
6.8597 -26.344 1
5.1962 -18.85 1
6.1557 31.213 1
10.463 -8.9288 1
-19.984 -2.5791 1
37.492 7.361 1
-27.816 -7.7301 1
50.363 -4.7952 1
-54.113 17.885 1
34.075 10.322 1
-53.004 26.293 1
-29.498 27.485 1
49.588 9.8838 1
35.853 -35.777 1
27.798 -0.21773 1
13.906 -6.9501 1
31.512 24.316 1
-51.307 22.477 1
-32.812 7.453 1
-29.84 19.382 1
-7.6262 62.79 1
22.207 30.367 1
-7.7686 62.204 1
0.70894 -27.474 1
54.624 -11.465 1
29.245 22.052 1
-6.9074 -36.228 1
-13.814 -31.029 1
-25.748 17.763 1
7.0064 -44.761 1
3.966 33.678 1
-3.0085 7.8418 1
-19.413 -4.3903 1
-11.273 0.81007 1
25.787 -10.91 1
56.418 -10.897 1
-6.1668 -17.777 1
-16.471 -2.8668 1
-27.738 1.4686 1
32.792 21.148 1
11.679 -36.039 1
-9.2504 -15.329 1
-33.133 -25.883 1
-28.164 -28.289 1
2.8366 8.9364 1
4.852 34.136 1
7.4888 -53.589 1
48.294 0.040424 1
-3.6305 2.6277 1
53.833 -10.352 1
-26.271 6.5115 1
24.941 -6.5121 1
-54.716 18.095 1
-34.556 4.6321 1
-21.015 -46.294 1
-29.658 29.341 1
-34.089 -26.859 1
35.087 -36.116 1
-54.695 17.072 1
-35.686 -29.568 1
25.94 38.092 1
17.455 23.879 1
-11.217 0.85333 1
8.5231 -7.4342 1
54.905 -10.534 1
-27.804 -25.511 1
7.2262 26.208 1
51.498 6.2877 1
16.034 2.6143 1
-12.471 39.914 1
35.361 -29.548 1
-2.6835 60.077 1
-0.69017 30.282 1
7.6079 -46.96 1
-29.412 4.2899 1
-15.988 -9.1647 1
-34.231 -13.442 1
11.28 -37.488 1
8.0438 -46.081 1
38.2 -31.848 1
38.009 -27.702 1
10.403 -34.766 1
1.2297 -10.148 1
-50.958 22.06 1
7.9799 -52.439 1
-26.312 -3.0036 1
-25.27 -8.9567 1
-25.972 -51.764 1
-30.217 26.757 1
33.263 -36.282 1
-26.916 30.77 1
22.928 28.331 1
52.246 -9.2294 1
27.215 38.496 1
-18.795 -12.253 1
30.294 -1.0475 1
17.654 5.3494 1
25.529 6.5839 1
-21.181 -53.405 1
-20.382 -11.357 1
18.223 23.465 1
11.53 -14.791 1
31.026 22.777 1
-6.5039 -32.919 1
52.356 0.80451 1
28.451 -7.0691 1
-23.797 -51.13 1
-27.724 31.313 1
9.9531 -18.737 1
-0.69382 -10.772 1
19.351 21.732 1
-1.0258 6.6453 1
-24.55 -50.747 1
-33.124 -3.76 1
50.599 1.4563 1
-12.034 -33.118 1
-30.741 26.312 1
8.7097 -49.324 1
-1.1658 -19.434 1
32.236 -33.638 1
18.309 35.305 1
6.1673 32.675 1
-27.141 30.89 1
-24.434 17.451 1
54.733 -5.1552 1
36.397 8.3549 1
-23.855 -49.982 1
40.64 8.3986 1
0.71117 -7.0237 1
-27.512 13.655 1
-19.535 -49.022 1
-1.7817 -27.507 1
-50.406 25.278 1
-21.092 21.248 1
10.623 22.077 1
21.715 -8.3426 1
9.3569 -2.0072 1
-14.537 -31.925 1
9.2845 -34.162 1
8.8329 -53.396 1
40.008 7.9212 1
49.495 10.053 1
34.622 -30.148 1
-16.331 -18.063 1
-30.228 28.325 1
-4.0383 -1.7526 1
9.2534 -50.279 1
-13.276 -29.605 1
-14.462 -33.128 1
-51.384 24.715 1
-12.356 -19.449 1
-25.149 -50.563 1
-12.197 18.795 1
21.394 4.9696 1
2.4523 3.7569 1
6.5987 -9.8364 1
-19.675 -15.091 1
9.627 -1.9888 1
-5.8741 -31.626 1
-37.5 -29.295 1
26.525 39.68 1
-10.538 53.095 1
8.6349 -44.315 1
22.107 -15.007 1
-34.136 4.9497 1
-3.8815 17.78 1
21.17 30.641 1
-5.7356 -17.058 1
-15.283 35.668 1
-11.8 -38.037 1
36.846 6.4509 1
-10.288 53.229 1
-28.746 25.063 1
-26.837 -50.853 1
-29.824 -8.9413 1
-13.238 -29.613 1
-7.7939 62.961 1
7.9637 2.3107 1
28.679 -8.9717 1
-26.292 6.5156 1
10.441 -35.381 1
-15.501 4.0547 1
-14.932 -33.31 1
-35.293 -13.456 1
-7.8518 54.737 1
20.507 -4.206 1
52.935 -9.5874 1
-6.9991 -26.493 1
-19.19 -48.698 1
-12.299 -6.5302 1
-9.247 -15.368 1
-5.0123 -9.4018 1
-4.786 -12.882 1
-18.577 -13.536 1
-13.915 38.759 1
-17.351 3.7087 1
30.656 20.856 1
16.746 4.0742 1
-35.014 7.5632 1
-20.472 -49.534 1
24.552 40.309 1
7.8923 -15.094 1
9.8435 5.7565 1
-8.0936 -1.8262 1
-24.758 1.7804 1
-14.967 37.616 1
7.3863 9.7048 1
25.522 -9.3028 1
-19.014 2.6947 1
51.442 10.459 1
-5.501 12.205 1
49.931 10.399 1
12.281 20.656 1
57.635 -12.534 1
-7.2604 -16.84 1
-20.791 19.284 1
-5.7281 12.375 1
20.05 29.898 1
19.244 21.795 1
26.889 1.8541 1
-8.7139 -10.755 1
-28.737 -49.794 1
-22.013 18.6 1
-31.963 22.561 1
-29.705 20.543 1
-14.835 40.004 1
23.021 14.029 1
48.79 -10.413 1
-6.8437 -26.167 1
2.591 20.118 1
-33.644 -8.8692 1
-32.985 5.2146 1
-26.833 -9.941 1
-13.704 -30.932 1
-13.807 -18.757 1
33.381 8.8642 1
-9.0328 3.0194 1
29.642 -10.152 1
-28.668 -12.855 1
-36.136 -31.734 1
-31.536 -26.121 1
-26.234 -5.0399 1
-18.067 -49.95 1
35.338 22.541 1
-17.583 3.7954 1
1.0278 6.4372 1
7.0182 26.52 1
-6.4785 -32.87 1
-5.4018 12.327 1
27.995 -6.5196 1
-17.084 -9.8524 1
-0.10907 0.072594 1
-29.66 -29.323 1
-23.795 0.72129 1
36.243 7.5202 1
21.265 4.8876 1
51.309 -10.608 1
50.034 3.0017 1
-6.9124 -36.278 1
-29.966 -6.6829 1
54.708 -10.282 1
-13.793 -31.726 1
-33.886 -9.5136 1
-9.3112 -10.921 1
24.209 35.251 1
-27.802 3.448 1
-11.498 45.301 1
-12.084 -22.798 1
23.432 21.849 1
-26.434 27.32 1
-20.342 19.751 1
-25.223 19.702 1
-12.105 -25.172 1
-30.905 19.288 1
-8.2698 -11.026 1
-30.916 25.889 1
-3.099 18.042 1
-35.04 -12.639 1
-5.3753 -17.966 1
11.678 14.451 1
4.478 -11.572 1
-10.932 -22.179 1
14.238 15.887 1
-12.042 -33.249 1
9.1341 -33.344 1
-14.367 35.179 1
-13.194 37.591 1
25.892 41.435 1
-8.9047 -25.555 1
21.029 3.1497 1
22.482 9.0111 1
37.569 -32.804 1
0.97292 34.041 1
10.463 -2.0512 1
-24.554 -14.662 1
-13.594 -26.665 1
17.771 22.278 1
32.51 17.595 1
-19.556 4.1776 1
-18.848 4.4401 1
31.617 9.4046 1
57.632 -12.638 1
-21.286 21.266 1
-11.739 44.611 1
25.438 24.628 1
-31.36 -28.523 1
-21.041 -51.102 1
27.819 40.552 1
-3.9582 -29.096 1
-1.2073 17.11 1
-29.379 -2.4732 1
-19.068 2.6908 1
28.822 21.176 1
-10.157 -32.71 1
-9.7284 2.4282 1
49.721 9.7755 1
26.004 40.4 1
48.762 -10.394 1
-5.8032 55.349 1
8.4695 1.1891 1
-29.618 29.096 1
11.501 13.793 1
-12.36 -19.41 1
40.822 -29.282 1
-25.474 -15.244 1
-1.2063 -25.197 1
-3.0733 -35.92 1
6.3256 4.0784 1
25.965 32.465 1
-10.708 53.012 1
1.2083 19.987 1
32.659 22.301 1
3.617 12.128 1
49.148 8.3377 1
-12.877 40.649 1
-53.919 16.999 1
-3.4036 9.7642 1
-13.865 6.1359 1
-10.063 8.6217 1
48.079 7.6854 1
-28.659 21.596 1
34.121 10.282 1
32.836 22.297 1
22.077 5.8501 1
11.987 -4.6214 1
-0.58107 18.317 1
18.98 -32.813 1
49.031 6.0578 1
20.624 39.176 1
10.642 22.032 1
8.5459 -53.116 1
-12.326 -19.538 1
-3.5601 -35.889 1
-23.45 19.251 1
-19.661 -2.8121 1
24.111 35.326 1
-28.441 -49.61 1
0.37268 35.254 1
49.743 -9.3264 1
-14.439 -18.664 1
-36.487 -29.449 1
-5.8971 -35.04 1
37.753 6.5766 1
23.221 5.8858 1
51.522 -3.5366 1
34.173 -35.725 1
41.316 -26.382 1
6.1335 -18.913 1
28.004 9.6631 1
-35.835 -12.133 1
53.402 -8.7183 1
-29.724 -26.097 1
34.14 -36.513 1
-3.4014 19.231 1
-29.366 31.272 1
15.659 1.2822 1
-2.4573 19.506 1
9.2682 -46.094 1
0.053551 -10.986 1
-13.014 -32.342 1
51.758 8.7953 1
4.8901 28.688 1
-28.94 -29.865 1
9.0299 14.568 1
6.8311 33.955 1
1.3983 -5.1005 1
0.30152 42.226 1
-6.9552 -26.133 1
-11.771 35.493 1
-1.0494 9.7124 1
26.596 -9.015 1
16.465 -7.2579 1
-12.264 45.464 1
-29.173 31.711 1
-23.638 -5.8256 1
11.095 -16.938 1
49.732 8.832 1
-3.3777 58.341 1
8.4529 -49.551 1
-19.073 15.49 1
-29.025 -29.406 1
-9.8095 -11.353 1
51.623 -12.118 1
22.231 -16.992 1
31.207 22.551 1
33.691 19.946 1
-27.877 28.298 1
-28.095 -49.775 1
8.824 -12.698 1
-1.3552 18.663 1
21.269 -17.684 1
-7.8152 17.857 1
-26.609 31.601 1
-52.65 20.253 1
-5.6166 55.631 1
-12.653 38.109 1
-9.7609 10.015 1
-11.894 41.273 1
18.806 -19.18 1
-5.5659 -27.561 1
24.423 37.933 1
21.808 -8.312 1
-0.63813 5.9046 1
30.607 9.3511 1
-30.951 25.622 1
-36.619 4.7194 1
-29.629 -12.047 1
-19.947 -50.307 1
-4.1539 57.399 1
34.918 -35.917 1
-14.372 38.194 1
6.7407 31.722 1
27.089 -6.796 1
31.911 8.305 1
-1.8018 -11.628 1
36.381 -33.653 1
-5.88 -35.118 1
9.0062 -56.164 1
20.696 29.264 1
-7.7984 55.993 1
-5.8658 -10.621 1
-15.492 36.483 1
-26.528 -0.83373 1
21.495 5.0815 1
31.16 -9.0625 1
-14.34 -21.508 1
31.763 -7.0469 1
-15.382 -12.278 1
-36.876 8.4748 1
-20.933 -49.872 1
6.6247 17.273 1
-32.1 -31.676 1
-5.1804 53.75 1
-30.568 -2.7476 1
28.039 9.6397 1
37.933 -32.372 1
20.7 39.065 1
32.281 -36.207 1
19.903 -31.341 1
8.7037 1.3963 1
-4.3074 5.6117 1
-27.868 4.9332 1
-34.811 -30.472 1
41.242 -27.712 1
-11.501 42.929 1
-32.11 0.033822 1
5.8008 33.386 1
-13.874 -2.4651 1
-8.9624 18.71 1
7.8445 -54.868 1
-10.571 -11.986 1
39.524 7.4622 1
-19.79 22.752 1
-34.588 5.6663 1
40.27 -28.779 1
-36.637 -30.362 1
26.996 40.469 1
-5.9332 60.568 1
-24.91 -2.5761 1
23.796 13.049 1
-3.9038 20.319 1
8.1952 -30.598 1
-34.706 7.7529 1
-5.0265 -0.81311 1
21.878 19.235 1
50.627 10.04 1
-2.2439 -21.823 1
55.855 -13.665 1
-4.8798 -19.379 1
34.88 -36.735 1
51.234 -9.6884 1
-31.014 19.183 1
11.564 -35.732 1
24.12 35.341 1
-34.5 -8.3081 1
27.744 38.578 1
-19.335 20.573 1
-25.122 -10.106 1
58.737 -12.388 1
-11.449 52.513 1
-16.364 -18.037 1
-31.33 -9.0048 1
-14.265 35.138 1
-3.011 8.114 1
55.834 -13.664 1
-2.5325 -25.816 1
-8.8735 -8.0907 1
36.274 -33.305 1
-4.9866 -14.104 1
24.858 -11.827 1
38.289 -31.638 1
-13.814 38.59 1
5.2724 18.363 1
-30.129 3.8436 1
-32.049 -26.563 1
16.05 23.744 1
3.777 32.528 1
-13.436 -16.871 1
-14.398 37.821 1
-51.673 24.322 1
-6.5539 -14.658 1
24.548 39.917 1
48.36 7.7023 1
9.4746 -26.087 1
0.69186 -7.0547 1
-11.102 1.7045 1
-21.084 -49.943 1
-14.735 -35.717 1
8.9213 -7.1944 1
15.565 1.2498 1
32.184 -36.425 1
9.6337 3.2978 1
21.04 -17.766 1
-30.24 28.323 1
-25.183 -12.877 1
-23.552 29.482 1
50.636 4.8897 1
10.756 -35.372 1
-3.3872 9.773 1
-35.391 4.0988 1
21.526 -8.4608 1
1.8189 34.821 1
-1.5248 -29.355 1
10.335 -6.1523 1
-0.61039 -9.8597 1
-7.1657 -19.37 1
-14.79 -4.1867 1
23.083 13.761 1
-16.782 -1.2032 1
52.616 -8.9578 1
-34.615 5.647 1
-8.9695 18.749 1
-15.954 -9.1351 1
-24.92 -2.122 1
-14.467 4.9987 1
-24.726 0.01961 1
10.957 24.574 1
48.296 -0.31541 1
-13.614 -7.437 1
-10.108 -29.839 1
-5.1342 -14.198 1
-14.632 -32.787 1
34.8 20.244 1
1.671 0.59762 1
-7.4327 7.7269 1
23.845 37.893 1
-11.917 41.311 1
-26.052 15.501 1
26.27 38.298 1
8.5547 -48.272 1
0.6477 18.732 1
-27.339 14.208 1
-14.901 38.696 1
-15.269 35.459 1
0.86378 35.89 1
17.179 -23.315 1
-36.99 -29.482 1
-14.728 -3.9277 1
-29.394 -27.893 1
-31.172 6.5271 1
51.067 -10.491 1
-24.796 17.133 1
11.776 -36.908 1
-18.808 -48.327 1
-7.3496 58.298 1
-9.3901 -37.417 1
-19.032 15.456 1
1.4552 20.296 1
-50.069 28.696 1
8.5474 -53.608 1
10.941 -20.367 1
-11.684 -15.498 1
-19.508 -51.122 1
-3.0508 15.443 1
-32.453 -2.7461 1
-5.8732 61.605 1
23.441 -13.432 1
-35.864 -12.126 1
48.769 9.6923 1
2.4743 32.593 1
-11.864 -37.144 1
24.308 -10.49 1
-13.767 -27.333 1
-10.807 -6.768 1
35.358 8.4105 1
-13.339 -34.593 1
-27.437 -24.231 1
29.521 -5.2261 1
-12.81 -35.944 1
-35.749 -14.125 1
21.116 4.6343 1
12.526 17.595 1
-15.641 36.226 1
27.248 1.988 1
8.7521 -54.377 1
-9.7734 10.018 1
38.866 6.818 1
-24.748 -14.767 1
25.301 36.3 1
-5.7069 -4.1573 1
-11.338 -24.871 1
-10.193 -2.2238 1
6.7479 -29.419 1
-18.895 -7.837 1
5.4786 9.8208 1
-21.09 -15.336 1
3.571 32.819 1
34.991 -29.86 1
-19.16 19.52 1
-12.341 -8.631 1
8.2322 -51.808 1
-22.571 -50.023 1
-54.395 17.437 1
-14.55 35.852 1
11.119 -38.09 1
1.2161 10.891 1
-33.883 -9.539 1
-18.006 -14.336 1
51.12 -5.0855 1
27.522 -8.8046 1
-16.831 1.9891 1
40.973 -29.183 1
10.381 8.1747 1
8.936 14.755 1
-35.546 -31.669 1
-11.937 -37.021 1
-2.8788 -3.7078 1
23.356 14.262 1
-20.053 20.02 1
7.013 -44.763 1
-31.655 24.971 1
-19.469 -0.70907 1
-0.98141 -13.769 1
19.59 -30.307 1
29.664 1.2321 1
54.683 -5.1002 1
27.972 38.57 1
-28.812 -12.604 1
27.645 40.54 1
-13.225 39.986 1
-29.319 31.415 1
12.002 19.076 1
5.3918 30.306 1
21.331 4.8823 1
-12.956 -30.872 1
-37.09 -12.754 1
-5.9566 -35.135 1
-14.346 -8.4488 1
-28.967 30.467 1
-17.359 -13.768 1
-3.6184 -35.891 1
4.5827 31.087 1
1.6721 34.213 1
39.198 -29.468 1
23.979 2.7016 1
6.3536 4.1083 1
0.93479 17.835 1
-3.8487 5.8065 1
-8.7078 -8.072 1
-6.0453 61.342 1
5.9483 12.53 1
-34.596 -32.084 1
-31.475 -15.492 1
-16.465 -3.3223 1
-6.6121 -19.679 1
8.8895 -7.1803 1
20.553 30.125 1
-28.684 28.988 1
50.079 9.3557 1
51.279 -10.557 1
10.789 1.9683 1
51.259 -5.456 1
8.2891 -18.45 1
23.123 -10.748 1
51.408 6.102 1
49.78 8.1832 1
-12.629 -36.414 1
-5.4091 -17.951 1
-31.516 23.05 1
-25.682 29.462 1
-50.949 22.137 1
1.9848 13.101 1
21.276 -4.4159 1
-23.744 -5.3563 1
-19.354 -4.4996 1
4.7572 2.1539 1
-5.3146 -16.864 1
-2.8905 15.464 1
22.693 0.85134 1
-2.716 -28.004 1
-1.4574 32.842 1
52.493 7.6146 1
-31.257 -4.3204 1
-28.121 -2.7903 1
31.702 -7.6369 1
38.96 6.8594 1
-26.767 -22.459 1
31.303 -8.1848 1
35.494 4.9061 1
-6.6825 59.574 1
22.743 13.071 1
-24.549 0.16589 1
-31.541 6.8474 1
-10.627 46.107 1
4.1021 -5.7089 1
-35.976 -35.004 1
19.064 -32.916 1
-16.389 -18.033 1
-32.575 -29.911 1
-0.42832 11.88 1
-30.11 19.819 1
6.0794 6.9217 1
3.5867 -8.7565 1
33.276 24.843 1
-12.612 -31.57 1
56.358 -11.092 1
16.581 22.385 1
47.459 10.615 1
-36.973 4.8222 1
-37.543 -29.364 1
-10.641 -6.7959 1
-9.2672 -10.933 1
50.324 7.4774 1
-13.851 -34.171 1
50.999 4.8064 1
-29.04 -50.044 1
-23.971 -51.426 1
24.711 37.809 1
-6.4002 -26.816 1
-25.678 5.506 1
51.954 -5.1468 1
-3.1385 -28.11 1
-6.1331 53.87 1
7.3918 9.7015 1
-28.67 -51.281 1
-14.625 -16.989 1
-25.882 -51.86 1
1.1781 19.964 1
-9.0142 -8.1238 1
16.247 -3.5645 1
11.731 -32.651 1
36.341 -33.246 1
26.25 -13.003 1
-2.7097 -28.373 1
-0.91708 36.658 1
19.245 -33.188 1
-14.622 41.457 1
0.76775 -14.434 1
-30.784 24.532 1
6.7189 33.976 1
-5.1595 55.484 1
-6.4641 3.7153 1
-15.406 35.888 1
-7.1084 59.648 1
32.935 20.809 1
10.371 8.1141 1
-28.637 -9.3947 1
-13.565 3.9627 1
39.039 7.092 1
-6.1989 18.03 1
-21.282 -50.665 1
24.483 -13.122 1
-14.652 -35.77 1
-21.247 -50.224 1
-14.734 -34.211 1
-24.086 0.10924 1
41.094 -28.115 1
20.758 29.347 1
-35.738 -29.473 1
18.074 24.109 1
-20.999 -1.2508 1
-0.4941 5.9772 1
23.608 14.161 1
23.432 37.821 1
-29.316 -23.569 1
18.82 -5.703 1
-22.665 -51.138 1
21.278 -14.753 1
-28.855 -51.813 1
-26.524 27.197 1
37.373 6.8218 1
7.1874 26.425 1
-11.335 13.306 1
-17.872 -48.415 1
3.7803 -26.752 1
-32.019 -28.46 1
-53.623 17.542 1
-13.568 -9.2796 1
33.242 24.834 1
24.696 38.222 1
34.354 -36.543 1
-27.086 16.038 1
-34.746 6.2122 1
-35.681 6.6224 1
-31.176 -27.336 1
5.1836 -24.166 1
9.5332 -56.439 1
-26.733 -22.414 1
26.837 2.8667 1
0.04098 -7.3279 1
1.1126 19.984 1
-31.591 -27.849 1
10.032 -48.305 1
54.143 -9.4474 1
33.061 20.377 1
-18.715 -24.35 1
-53.923 21.147 1
20.958 -7.5013 1
-8.903 59.901 1
-10.314 17.441 1
-14.216 39.347 1
-3.3054 58.247 1
4.1698 32.345 1
18.488 25.975 1
4.8485 -25.435 1
-33.831 -3.8805 1
-27.856 3.3808 1
-13.95 -21.823 1
-25.924 17.074 1
25.883 32.537 1
4.4511 -12.087 1
51.454 6.1154 1
-6.3303 -1.8471 1
-0.28429 -9.8022 1
-2.7394 60.19 1
32.615 21.23 1
11.606 -12.563 1
2.2368 -12.801 1
-1.6325 3.2742 1
3.8104 5.6412 1
-27.254 26.289 1
-6.8939 4.7351 1
48.591 11.791 1
19.334 25.048 1
-7.5292 -10.803 1
-19.449 19.345 1
26.522 -8.1702 1
26.101 -12.95 1
-29.473 -3.8755 1
52.872 -2.811 1
-1.5515 -27.496 1
38.937 4.543 1
-8.2442 -27.267 1
4.6162 36.142 1
-50.486 22.191 1
22.889 28.331 1
-54.627 19.712 1
51.862 3.1799 1
-6.5923 -26.655 1
49.691 8.2507 1
51.896 11.234 1
16.24 -3.5519 1
12.017 -28 1
-37.549 -29.382 1
-13.341 10.476 1
-20.477 2.4529 1
3.6316 -18.547 1
8.5783 -35.197 1
-25.812 -6.9309 1
-15.079 -9.1002 1
-12.642 38.443 1
5.4386 1.0999 1
0.94023 -7.0573 1
-13.547 4.0861 1
-27.553 30.112 1
-11.35 13.305 1
-34.527 -8.3156 1
-1.139 61.789 1
-32.672 -6.2431 1
29.019 -4.7506 1
-14.757 -34.102 1
11.518 2.2012 1
8.0679 28.643 1
-23.235 -18.038 1
-14.963 6.7423 1
-13.752 -0.10981 1
-11.082 -21.67 1
-13.754 36.464 1
21.99 -15.049 1
-34.007 -28.898 1
-28.528 21.548 1
53.008 -9.6437 1
38.203 7.6479 1
-29.626 -24.121 1
19.993 7.5769 1
-11.81 -38.117 1
-21.84 15.489 1
-7.7016 57.137 1
3.0489 19.897 1
10.626 -36.536 1
20.902 -32.455 1
-14.134 -0.056269 1
-16.381 -18.031 1
-13.947 13.602 1
36.052 -36.034 1
34.933 20.2 1
-12.812 -35.47 1
1.9484 -0.1902 1
17.893 24.898 1
3.2871 4.6107 1
-4.1244 -27.751 1
3.7711 -26.753 1
-18.613 15.339 1
-29.565 23.476 1
-15.1 -30.023 1
8.1061 -8.3419 1
40.816 9.4305 1
-30.901 -6.5556 1
-13.256 -34.885 1
35.085 9.0457 1
-6.1097 58.726 1
-32.985 -6.9252 1
3.084 29.001 1
38.807 -29.557 1
-25.651 -7.4521 1
-32.311 -10.24 1
-5.4716 -27.098 1
35.867 23.064 1
57.531 -10.632 1
-16.452 -3.3322 1
-8.454 17.651 1
-19.07 0.58685 1
-9.249 -0.99472 1
-50.969 25.832 1
-35.068 -12.537 1
-33.765 3.5928 1
28.001 38.528 1
-11.103 42.575 1
-11.731 -32.513 1
-26.389 27.327 1
-27.694 -49.971 1
36.227 22.712 1
40.411 8.3928 1
-7.0357 59.408 1
-6.9709 2.2107 1
-54.905 18.453 1
-28.878 30.423 1
6.1654 32.651 1
22.141 30.36 1
-31.861 -4.8525 1
28.223 38.547 1
39.319 9.9348 1
-2.3195 -1.5142 1
-22.917 18.061 1
9.0517 14.701 1
-15.954 -9.1758 1
-1.619 18.231 1
7.9809 0.69794 1
-12.764 -36.013 1
-6.0229 53.889 1
-1.3185 6.6344 1
-49.383 30.117 1
56.079 -10.419 1
12.175 20.575 1
8.5702 -53.868 1
-0.69142 5.7704 1
-31.182 23.283 1
5.4061 14.495 1
18.913 -19.165 1
50.765 -5.0302 1
17.287 23.808 1
51.545 -4.1512 1
-34.68 5.7107 1
-7.0234 -33.245 1
-12.579 -18.081 1
-26.605 -2.5557 1
-25.806 -49.816 1
-3.6327 19.287 1
-1.0396 9.7029 1
-18.014 -48.725 1
40.441 -27.95 1
51.748 -4.0153 1
-11.76 35.515 1
-13.897 -50.053 1
9.453 -26.161 1
-30.756 -11.813 1
9.2169 -2.1282 1
21.263 -13.913 1
12.162 20.603 1
-27.239 18.823 1
-14.332 35.14 1
24.085 7.314 1
1.8056 -12.797 1
51.633 -12.032 1
15.637 -11.119 1
-0.69372 -0.67234 1
15.949 15.503 1
18.265 -7.0694 1
-4.0278 -1.763 1
-14.137 -7.2326 1
-52.825 20.448 1
-15.475 -1.7855 1
-0.86292 -19.025 1
-14.002 10.267 1
-33.903 -28.558 1
20.633 30.223 1
8.1223 -51.082 1
0.2227 6.6433 1
26.692 39.776 1
-52.817 26.414 1
-30.004 -26.369 1
-13.62 36.302 1
-20.324 -11.384 1
-10.144 -32.659 1
23.263 5.9163 1
-19.157 2.5468 1
53.038 -6.2009 1
-19.082 2.5969 1
-10.938 -22.131 1
20.752 2.6039 1
8.8735 27.649 1
23.845 13.721 1
8.1476 -54.845 1
19.861 -31.56 1
41.561 -26.303 1
22.178 39.68 1
-29.554 -12.034 1
-30.868 -8.9088 1
-52.225 22.634 1
0.8264 -7.0422 1
-18.855 -7.8745 1
29.897 -2.6939 1
-22.73 -50.023 1
-14.953 37.942 1
11.611 -36.02 1
-8.3131 -1.8447 1
9.6111 3.3089 1
-7.5564 5.1651 1
-6.201 18.067 1
-30.947 -3.592 1
7.4454 29.488 1
12.622 3.9616 1
11.557 -7.6421 1
-2.7382 -14.008 1
20.633 39.275 1
-26.828 17.01 1
-4.8256 -18.974 1
-27.807 -48.477 1
-21.925 15.404 1
-1.5579 -27.486 1
-29.849 -24.808 1
-32.495 -9.4119 1
-26.986 0.71271 1
51.57 -11.997 1
-33.42 -27.921 1
-12.067 44.115 1
-1.9325 -8.2713 1
10.23 -15.098 1
-34.093 -7.8712 1
10.973 -37.037 1
-6.7291 61.265 1
5.0225 30.423 1
38.966 4.4813 1
5.9853 12.533 1
35.053 -35.397 1
-34.52 -7.1135 1
-31.198 -8.8484 1
9.992 -48.311 1
29.323 9.6066 1
-34.595 9.7014 1
-16.38 19.903 1
18.275 -7.06 1
48.517 10.842 1
9.5924 -31.279 1
-32.013 -26.681 1
27.099 -6.8359 1
-32.029 -4.8905 1
2.2629 32.452 1
13.267 11.761 1
2.1137 18.86 1
8.2484 -50.278 1
10.693 -34.367 1
3.7232 34.113 1
-16.862 -1.4624 1
51.873 3.2294 1
-23.299 -51.809 1
-29.536 -24.224 1
-2.0013 -19.121 1
25.496 39.735 1
-35.963 -34.949 1
-3.0142 -35.914 1
29.749 -10.091 1
-34.066 -26.799 1
-15.343 -29.801 1
9.4442 23.19 1
35.181 9.6256 1
-36.858 8.4556 1
21.324 -16.593 1
-26.468 28.985 1
-3.5568 18.021 1
-2.6438 -15.103 1
-8.5441 -37.343 1
21.966 -0.12134 1
2.87 8.955 1
-12.442 45.456 1
36.387 6.7734 1
-35.173 -30.972 1
32.314 -35.942 1
18.128 5.7072 1
-34.48 -11.033 1
10.062 -16.997 1
-52.101 20.659 1
28.807 7.9114 1
8.9952 27.445 1
-2.7939 5.3493 1
-26.746 -1.2923 1
-14.414 -6.7466 1
21.097 30.603 1
-5.9591 56.924 1
7.8485 22.37 1
-7.0307 59.205 1
0.24501 6.6135 1
-14.733 -4.2086 1
-7.0436 -34.181 1
-1.7407 17.972 1
-27.861 -7.6195 1
-14.202 42.162 1
-0.85958 36.736 1
-13.917 -27.748 1
5.1899 -24.109 1
10.376 -8.915 1
-28.503 -50.669 1
-25.216 -12.867 1
-2.5761 -25.647 1
-52.906 19.045 1
56.003 -8.559 1
24.65 30 1
14.069 0.75081 1
-22.835 17.997 1
-16.384 19.902 1
-34.131 -29.936 1
35.408 22.596 1
-3.5779 5.8666 1
-1.2053 -25.173 1
-5.215 59.906 1
-13.469 39.889 1
32.578 11.211 1
53.082 -8.4956 1
0.80004 35.908 1
27.725 -12.143 1
3.1492 32.869 1
-35.384 -15.368 1
1.8105 -11.435 1
-17.684 -47.977 1
-28.366 29.262 1
-26.675 -15.177 1
20.366 -16.589 1
0.44293 18.689 1
-25.64 -25.444 1
-12.582 38.231 1
-13.101 -30.629 1
11.577 -7.704 1
23.285 25.317 1
-0.19537 -1.3238 1
-27.057 15.922 1
48.974 6.2953 1
41.281 -26.688 1
-31.439 -4.4604 1
-0.38134 14.702 1
-24.018 -12.312 1
27.705 -12.149 1
-5.5951 -33.409 1
-4.9015 61.245 1
-14.711 40.633 1
-4.5779 8.2405 1
17.207 -23.342 1
-15.292 -22.238 1
-31.16 6.4826 1
7.9859 31.34 1
36.677 5.0646 1
-4.7072 -8.6197 1
9.4073 -50.932 1
-36.507 -1.48 1
10.989 24.538 1
23.433 21.849 1
-30.954 -3.7666 1
54.679 -9.9006 1
-20.255 -49.925 1
-14.662 -1.8483 1
-50.476 25.193 1
0.35263 36.504 1
40.537 9.3201 1
-26.151 15.571 1
19.199 -5.3826 1
49.444 7.9234 1
50.297 -7.8017 1
-26.012 -8.4126 1
25.96 32.451 1
35.055 -36.719 1
-53.388 19.237 1
57.288 -9.9147 1
40.486 -28.69 1
4.6997 -2.6221 1
-26.825 -1.1402 1
23.385 4.7633 1
-3.6329 2.5958 1
-21.611 15.856 1
4.503 -11.621 1
1.4867 17.459 1
17.814 24.005 1
-5.8292 18.81 1
9.3501 -2.0954 1
1.622 34.335 1
-11.418 14.435 1
7.3322 -30.338 1
-31.932 -28.517 1
10.345 21.192 1
-31.649 27.122 1
32.364 21.597 1
-7.975 -26.662 1
-2.8794 -13.814 1
4.5696 33.148 1
25.724 -10.976 1
55.814 -8.2503 1
-31.553 27.269 1
3.8471 27.636 1
-5.5225 -27.154 1
25.058 40.112 1
-1.5849 3.2684 1
-22.051 21.708 1
-52.196 21.21 1
-5.9492 -35.133 1
-8.8703 59.704 1
-22.504 -51.089 1
-14.898 4.7534 1
-10.481 45.042 1
-29.541 29.417 1
23.114 14.162 1
-11.145 1.7467 1
-12.554 -32.098 1
-33.78 -7.7229 1
-28.653 25.156 1
35.201 -35.895 1
-30.537 -25.137 1
-29.511 4.061 1
-3.4314 -10.242 1
-15.328 -29.781 1
24.864 0.63822 1
25.499 24.63 1
-13.236 43.512 1
-7.0028 -10.693 1
-19.094 15.467 1
-2.3008 62.289 1
19.25 8.0374 1
-8.8712 59.608 1
12.012 19.058 1
-17.964 -47.214 1
9.0812 18.407 1
-16.327 19.907 1
-34.337 -10.468 1
-7.1932 2.8513 1
-1.3445 -19.357 1
-34.468 -10.792 1
-28.16 -10.327 1
-35.198 -27.873 1
12.431 -35.17 1
15.363 8.5976 1
31.753 -8.7646 1
-18.856 -8.0155 1
0.7873 -14.476 1
37.575 -32.569 1
-22.803 -12.239 1
13.936 -6.9585 1
17.568 23.34 1
-21.92 -17.375 1
-8.3973 -3.4619 1
-22.686 -0.48868 1
-0.49351 -1.8402 1
1.8017 -20.055 1
12.051 -35.442 1
37.48 9.7001 1
-33.408 -8.6996 1
25.948 38.141 1
22.876 13.72 1
-5.7435 -32.052 1
-9.3885 -29.001 1
-25.739 -50.6 1
-6.3183 -34.384 1
-15.308 -12.361 1
-0.28444 -1.3404 1
-34.238 -7.3981 1
7.8624 -54.981 1
22.443 9.0352 1
20.3 -33.131 1
5.4323 9.8177 1
-28.043 -26.298 1
-27.381 -50.468 1
-52.512 20.177 1
25.736 24.739 1
13.724 14.925 1
7.9559 -13.542 1
-1.1888 6.6518 1
1.3108 8.1966 1
19.236 -31.745 1
33.289 24.844 1
-4.1372 18.958 1
38.741 -30.937 1
19.349 21.751 1
-12.711 -35.711 1
-2.2603 -4.6626 1
-36.609 -33.61 1
1.3447 2.6012 1
-0.30931 14.658 1
-50.253 23.552 1
-24.999 -50.176 1
7.8486 22.353 1
-35.453 -5.7364 1
-11.367 -0.90967 1
-3.3989 -11.975 1
1.7463 18.145 1
-4.3004 0.39438 1
-31.851 -8.714 1
48.291 11.723 1
20.423 36.767 1
-10.588 44.967 1
-50.677 21.423 1
-13.638 -26.789 1
50.468 -7.7781 1
-12.614 -33.015 1
35.82 6.5753 1
-31.291 6.4868 1
-21.366 18.796 1
-18.028 -47.435 1
29.574 40.014 1
9.335 -46.074 1
-27.622 -2.6193 1
29.895 23.881 1
-12.909 -1.1888 1
-19.16 2.4985 1
-28.942 -29.233 1
-34.435 5.0292 1
14.086 -0.64729 1
3.8499 -9.8011 1
37.375 6.7611 1
-12.6 44.801 1
-10.6 53.037 1
-27.245 31.453 1
-14.535 -22.475 1
-53.144 20.521 1
9.3939 -55.41 1
13.983 1.9146 1
-35.229 -27.931 1
-8.241 57.23 1
-14.487 -21.652 1
-50.881 23.792 1
9.3968 -2.0161 1
5.0645 -8.3194 1
18.091 11.678 1
-49.301 30.209 1
-35.624 4.0378 1
-2.4601 4.9295 1
54.458 -10.451 1
40.991 -29.158 1
-13.658 -10.323 1
37.95 4.1513 1
-2.767 6.8941 1
8.9019 -32.557 1
29.726 -10.074 1
7.2669 26.147 1
-35.503 -5.715 1
-8.302 -9.3582 1
-25.937 -12.268 1
22.1 -16.961 1
-13.444 6.1493 1
51.435 0.55056 1
22.447 -14.946 1
14.317 15.929 1
23.812 4.237 1
-7.0189 2.6332 1
37.616 -32.653 1
0.79155 -6.8634 1
-14.251 2.1156 1
34.405 -36.88 1
-26.242 -5.0282 1
-28.077 29.009 1
-10.298 -33.252 1
-11.067 -0.46494 1
20.318 -33.356 1
-30.238 3.4554 1
-1.711 -21.603 1
23.812 13.978 1
36.884 8.5257 1
9.9875 -18.93 1
-4.8609 60.619 1
-29.828 -11.757 1
-0.44037 19.017 1
11.266 22.511 1
11.687 -32.651 1
-36.613 -33.545 1
27.635 -12.346 1
49.075 -10.447 1
-14.774 -34.226 1
-29.346 -5.6756 1
-6.5945 -14.649 1
-17.568 3.7798 1
23.474 14.436 1
20.358 -33.222 1
12.263 -8.2288 1
-32.422 -29.74 1
9.8302 5.7215 1
-27.34 -26.273 1
8.0367 -8.4167 1
29.382 -5.8804 1
18.244 -30.391 1
29.668 1.2018 1
6.103 7.0301 1
10.652 -36.583 1
-30.079 23.846 1
16.141 -12.066 1
22.188 -15.51 1
-25.443 -50.455 1
-31.427 -27.682 1
15.37 8.6038 1
34.995 -29.853 1
29.607 -10.145 1
-15.439 4.7268 1
-29.928 -6.8104 1
-17.637 -47.699 1
-27.827 3.4077 1
3.2542 -17.365 1
-8.2129 -9.4374 1
4.4472 31.246 1
-16.636 -2.0948 1
3.8501 -26.629 1
23.318 -7.645 1
9.9668 -33.488 1
-25.935 17.086 1
30.268 -1.0701 1
26.93 38.77 1
-53.768 17.534 1
52.657 -10.539 1
33.81 21.765 1
35.876 23.048 1
9.9067 -18.746 1
-33.281 -27.742 1
18.329 22.913 1
-24.899 -50.141 1
15.872 23.69 1
7.9601 -26.505 1
5.5945 34.364 1
48.374 -0.72711 1
-24.011 3.6559 1
25.218 -9.4495 1
-14.6 4.8971 1
4.7746 33.486 1
16.227 -3.5521 1
6.6239 -18.912 1
52.349 -9.4409 1
-27.521 -49.17 1
-23.932 -12.239 1
-29.377 31.241 1
-27.912 -48.53 1
-4.0614 55.362 1
13.81 -7.0289 1
-14.107 36.477 1
12.666 -35.018 1
8.447 -27.167 1
-29.172 -24.257 1
-29.432 -29.675 1
42.064 -27.66 1
-53.091 18.851 1
24.479 -12.392 1
-21.018 -15.317 1
3.9473 30.585 1
-24.052 -52.05 1
-19.82 22.886 1
-30.229 -24.908 1
23.444 14.422 1
31.15 9.0164 1
8.3152 -30.842 1
-15.331 -12.247 1
-12.075 -22.765 1
9.4639 26.699 1
10.935 -36.114 1
-15.064 4.9918 1
21.853 19.243 1
-15.389 3.9149 1
-29.047 23.69 1
-24.319 -1.1094 1
-30.799 -5.5708 1
7.0836 0.17801 1
-34.676 7.6615 1
22.81 0.72476 1
9.273 -33.542 1
-3.54 7.3615 1
8.6353 -44.289 1
-27.347 -8.1369 1
-5.7494 -4.1573 1
22.45 39.7 1
5.4708 -18.863 1
-6.9291 61.237 1
8.4218 -27.432 1
23.118 4.1349 1
-23.911 -12.273 1
7.9826 -53.754 1
-22.707 -0.55129 1
-11.41 14.407 1
9.4359 26.753 1
-15.373 4.0301 1
-7.6536 -26.727 1
-13.918 2.4738 1
51.307 11.949 1
14.36 15.955 1
32.086 9.9344 1
54.696 -5.0761 1
-4.3014 18.637 1
55.861 -13.63 1
27.02 -5.0104 1
5.3891 30.927 1
40.944 -29.203 1
23.948 2.6544 1
-2.2699 -4.6694 1
-31.421 23.195 1
9.7755 -50.164 1
27.839 -4.5966 1
24.206 6.3606 1
-24.445 -1.3154 1
0.32536 42.127 1
7.989 31.303 1
16.759 4.1217 1
12.59 -36.647 1
-3.5741 -28.307 1
-33.084 -6.9362 1
-52.561 21.369 1
3.5842 -18.524 1
53.492 -3.0648 1
-6.9423 -33.174 1
-21.499 15.942 1
-14.614 41.669 1
50.937 -9.8093 1
51.657 -4.9965 1
-13.628 -10.371 1
-25.101 18.052 1
55.591 -8.8938 1
-27.863 -7.705 1
3.0524 18.715 1
-36.898 -12.486 1
49.331 11.577 1
-31.774 -15.023 1
-3.0099 56.268 1
24.082 35.36 1
-11.157 45.542 1
-20.227 19.843 1
-13.933 38.742 1
5.7466 31.977 1
-30.619 -3.3925 1
-16.317 19.902 1
-32.205 -8.3024 1
-7.8279 5.1525 1
0.089947 41.898 1
-32.111 0.047416 1
2.2206 32.582 1
23.721 1.1905 1
31.52 8.6195 1
-8.3623 -11.3 1
-5.2573 -18.014 1
25.294 40.152 1
-28.224 -28.43 1
-25.553 -25.505 1
35.331 -29.562 1
7.078 -17.787 1
-4.7157 60.993 1
26.515 -8.1972 1
0.89234 -14.417 1
4.2217 29.643 1
-28.36 -28.64 1
1.8795 -20.049 1
4.6831 -2.6441 1
-5.9039 -10.603 1
33.213 24.795 1
8.7926 -55.259 1
10.353 21.291 1
-1.3456 18.696 1
-4.9039 51.812 1
35.3 -29.652 1
31.389 -8.0251 1
53.485 -2.9327 1
-9.7747 -0.17645 1
-50.038 27.603 1
-3.2798 -13.358 1
6.7815 -29.392 1
49.412 9.6043 1
-3.198 15.424 1
9.4201 -2.078 1
-18.778 -8.3238 1
1.2532 35.479 1
24.211 40.304 1
-35.719 -13.16 1
38.021 -32.708 1
35.392 8.3316 1
9.5979 11.236 1
52.196 2.063 1
-30.292 3.3034 1
9.5499 11.249 1
0.14984 41.883 1
23.765 33.905 1
11.993 -54.683 1
24.628 -10.64 1
24.101 1.3036 1
4.6928 2.1614 1
24.796 -10.667 1
-26.712 29.108 1
-29.797 20.51 1
6.5733 -9.8762 1
-10.517 -30.226 1
-11.905 -37.05 1
-3.2741 55.896 1
-34.512 -8.6662 1
22.798 28.267 1
-7.4887 16.579 1
8.6879 25.042 1
42.143 8.303 1
31.149 10.311 1
1.8786 34.793 1
49.832 -3.5961 1
-9.9838 -0.43552 1
-32.315 -9.3073 1
-51.621 22.76 1
-30.269 5.9974 1
-37.329 -13.654 1
-53.394 18.978 1
38.039 6.8731 1
4.7668 31.509 1
-13.152 43.639 1
-12.497 45.455 1
34.972 20.144 1
-6.7779 57.269 1
0.25578 42.037 1
-29.31 -7.3573 1
-20.46 -49.763 1
-50.388 24.012 1
51.444 -5.6821 1
55.803 -13.627 1
-3.207 56.032 1
3.1283 -20.221 1
-23.021 1.6233 1
-36.658 -29.414 1
-9.902 -29.687 1
-7.5687 -10.767 1
31.712 -2.7008 1
-31.686 -26.276 1
-24.885 -1.4792 1
-24.804 -16.394 1
36.83 -33.273 1
-27.969 -49.939 1
-24.01 -51.952 1
-33.04 -3.5811 1
-5.4146 62.13 1
26.809 40.687 1
49.907 9.3185 1
-16.934 -11.442 1
-12.449 -29.544 1
32.458 11.096 1
-23.337 17.317 1
-20.151 19.889 1
8.5911 -46.919 1
-29.8 20.596 1
41.005 -26.93 1
-50.24 23.589 1
36.242 22.764 1
-9.7553 -7.8508 1
-11.206 -21.67 1
-8.0767 61.312 1
-8.5194 -1.7626 1
4.5937 36.128 1
54.557 -10.254 1
-35.319 -27.93 1
11.442 -14.818 1
-5.2974 0.16917 1
-2.9175 -3.6941 1
6.5113 -26.238 1
22.718 6.3033 1
1.0719 -7.0745 1
15.783 23.655 1
50.694 4.6558 1
6.6523 -18.771 1
-13.94 2.5017 1
9.0017 -56.433 1
0.11486 41.844 1
8.5098 -47.966 1
-20.185 19.933 1
-27.378 14.008 1
-53.441 19.924 1
27.523 -12.481 1
-1.5268 -12.399 1
-34.431 -13.121 1
-2.4011 -1.555 1
-12.354 8.8337 1
41.329 7.8377 1
-51.507 24.201 1
53.092 -11.721 1
-50.511 24.641 1
-30.755 -25.661 1
-16.327 -18.072 1
2.7364 19.532 1
-50.09 27.544 1
-4.6521 -12.811 1
-20.313 -11.308 1
-30.911 25.061 1
-4.8815 -27.414 1
-20.013 -0.82959 1
2.2083 -10.24 1
-26.637 -49.807 1
0.2545 42.045 1
23.844 -14.776 1
24.045 7.2233 1
11.936 15.01 1
-7.6068 58.977 1
-14.176 39.292 1
31.567 -8.7586 1
-27.411 13.847 1
-15.05 -6.5991 1
9.1677 -9.5425 1
6.0941 7.0388 1
-14.438 -18.632 1
-6.5175 56.106 1
-36.285 7.6269 1
1.8587 19.363 1
-31.882 -26.267 1
-11.779 43.126 1
-12.759 8.8168 1
-7.2967 61.445 1
51.651 8.9066 1
-26.298 -0.24083 1
23.101 12.826 1
41.293 -27.929 1
-50.924 27.108 1
49.035 6.0525 1
35.716 -36.586 1
24.308 4.4024 1
23.542 -11.181 1
8.5055 -48.779 1
22.438 9.102 1
16.155 3.1282 1
-4.3076 -27.708 1
-4.1451 -27.749 1
32.561 -36.341 1
50.157 11.126 1
18.126 0.56059 1
-14.221 39.122 1
52.491 7.5422 1
17.129 -23.357 1
-29.825 24.906 1
-33.41 4.9137 1
16.74 -7.3758 1
8.0167 -52.758 1
-29.876 24.857 1
-8.1164 -9.3748 1
-19.217 19.555 1
-7.8571 2.0896 1
-12.371 -8.5971 1
-29.804 20.55 1
19.586 -2.5552 1
-10.156 -2.1958 1
22.57 -14.853 1
24.084 -6.4234 1
17.835 24.809 1
-16.082 -12.357 1
4.2323 -13.419 1
-5.0512 60.767 1
3.4855 10.092 1
10.417 15.24 1
-28.251 -7.8241 1
-5.6777 -28.096 1
53.628 -3.9935 1
3.4482 31.114 1
22.462 8.9883 1
-13.175 43.619 1
-13.56 40.723 1
-25.052 18.005 1
9.5568 26.546 1
10.08 -16.99 1
-13.93 -27.688 1
33.335 8.87 1
0.31826 36.562 1
-53.161 21.189 1
-27.882 28.264 1
16.434 18.363 1
51.439 10.417 1
51.877 11.546 1
-7.55 -10.822 1
-30.488 6.1705 1
11.747 -28.449 1
18.912 -32.654 1
-8.0673 61.346 1
42.236 8.4172 1
22.097 30.328 1
-29.766 -8.8993 1
-19.753 -2.8865 1
-36.86 8.4727 1
21.41 -8.5871 1
-51.81 23.844 1
41.305 7.1613 1
-12.599 40.093 1
-27.927 -51.452 1
-19.855 -3.7305 1
-17.231 -2.3351 1
2.1245 12.063 1
-14.591 4.9705 1
52.505 -12.623 1
-34.594 9.7337 1
26.987 -7.0059 1
12.351 23.181 1
-4.0458 -1.7288 1
2.0159 36.179 1
33.517 20.593 1
-52.187 25.299 1
-0.92197 -0.6405 1
-22.125 -17.309 1
53.471 -2.0523 1
24.155 35.306 1
12.168 20.569 1
29.861 -2.6941 1
-10.316 17.444 1
-24.715 -15.29 1
6.6427 17.243 1
12.761 -34.626 1
19.326 25.076 1
-21.854 -17.489 1
57 -9.4435 1
-7.4943 7.7324 1
53.528 -2.8663 1
-28.399 -49.802 1
-9.7794 -28.262 1
-32.802 -27.239 1
1.8615 19.355 1
35.476 -34.341 1
10.403 -8.8748 1
-27.602 -8.1188 1
-6.7443 -17.378 1
41.488 8.1723 1
21.44 -18.012 1
11.382 6.3046 1
7.3763 9.7028 1
-12.382 42.39 1
52.33 -4.085 1
5.4123 14.487 1
-34.105 4.4719 1
24.653 -10.703 1
-28.933 -10.156 1
51.634 6.5098 1
-18.698 -50.069 1
2.4641 34.628 1
38.061 10.19 1
0.98631 -26.617 1
7.6406 -15.67 1
51.559 -2.8702 1
-12.285 -16.764 1
-34.119 -31.515 1
25.96 32.443 1
-14.611 -21.682 1
50.48 11.596 1
7.9753 -15.21 1
-17.714 -47.644 1
-1.1298 6.6512 1
18.112 11.69 1
-4.939 51.933 1
23.321 25.278 1
-20.485 15.584 1
-1.0583 6.5962 1
-11.721 43.143 1
-31.302 -8.4314 1
-26.894 2.1629 1
48.88 0.8573 1
-0.82612 -13.808 1
6.4897 23.989 1
22.839 39.66 1
24.912 -6.5576 1
-21.328 -4.316 1
11.753 -32.622 1
17.797 -5.7373 1
-10.121 4.0553 1
-35.945 -34.792 1
5.0291 32.479 1
-32.775 -8.6659 1
-6.641 63.433 1
14.262 14.343 1
-6.8626 57.836 1
-19.339 20.947 1
35.592 -35.804 1
10.272 17.351 1
29.898 -9.6733 1
-1.0606 6.581 1
23.938 14.467 1
31.958 5.3825 1
-21.288 16.412 1
51.785 -10.903 1
-54.026 17.022 1
-24.35 1.2978 1
-34.476 4.4921 1
53.039 -1.2064 1
23.663 -8.9223 1
-6.038 19.555 1
25.677 6.657 1
-35.438 -5.7155 1
27.663 8.4524 1
-52.163 25.387 1
-29.877 -48.097 1
1.9847 33.58 1
11.228 34.676 1
9.2432 -33.548 1
6.0805 12.777 1
22.473 8.8242 1
-13.954 13.602 1
18.843 -5.6556 1
7.8179 -29.662 1
7.2785 -13.407 1
11.989 -54.673 1
-10.911 9.4683 1
18.789 -32.454 1
-6.9335 -17.136 1
-26.064 15.603 1
19.999 -18.113 1
24.638 30.024 1
-21.353 4.7522 1
23.179 -10.785 1
-4.4691 -11.273 1
-7.5733 3.6998 1
9.1024 18.403 1
24.738 39.812 1
-27.535 0.23883 1
-13.672 -31.056 1
41.263 -27.264 1
55.878 -13.622 1
-11.535 -31.363 1
-32.136 8.217 1
11.602 -26.583 1
2.1298 -1.0147 1
32.656 11.169 1
-14.82 4.7613 1
4.8336 20.248 1
11.222 34.673 1
-31.085 24.109 1
35.194 -36.255 1
-21.188 -49.91 1
-36.263 6.9994 1
32.408 -33.107 1
-5.9057 58.197 1
6.8478 -29.484 1
8.9951 -57.12 1
2.0728 17.131 1
20.496 39.282 1
-18.935 -1.7665 1
-10.708 46.192 1
1.1355 30.981 1
-1.2469 20.509 1
34.714 -36.551 1
-28.093 19.407 1
4.5367 33.399 1
55.712 -9.1339 1
-23.447 -15.585 1
-29.814 23.99 1
49.458 10.077 1
20.359 -32.19 1
-7.3883 -34.79 1
32.517 9.2618 1
-7.6608 61.899 1
-3.1048 58.467 1
-25.129 -12.843 1
-10.013 -18.086 1
9.4101 -55.934 1
-3.2795 18.777 1
-34.412 -11.047 1
13.232 -0.59241 1
-6.1979 3.9428 1
-11.076 1.7331 1
1.4735 -27.45 1
-18.994 -1.7336 1
48.696 -10.442 1
-29.189 30.171 1
11.711 -26.822 1
-13.127 -6.0113 1
-0.42018 11.905 1
48.277 11.619 1
16.885 23.948 1
49.909 5.6221 1
-5.1627 55.683 1
24.667 -10.713 1
-11.727 -29.829 1
-5.2301 17.563 1
11.727 -35.929 1
3.0473 19.558 1
21.692 38.496 1
20.983 -15.648 1
-11.852 43.036 1
-33.079 -7.4808 1
3.8137 -26.736 1
-25.089 -1.7228 1
-5.9761 59.833 1
49.767 7.5274 1
55.69 -9.0304 1
-25.677 5.5057 1
-5.1587 52.638 1
52.98 -11.536 1
2.5157 -24.423 1
-52.283 21.469 1
-31.562 -15.375 1
5.3363 -24.321 1
-36.995 -12.975 1
20.816 30.683 1
-10.382 0.78834 1
-17.374 -13.755 1
-4.1751 -9.0249 1
8.3692 -56.012 1
-27.626 -26.877 1
57.415 -9.8188 1
17.048 4.4095 1
-14.756 -33.908 1
21.129 30.637 1
-37.811 -13.94 1
10.467 -8.9571 1
4.4026 33.901 1
19.289 -15.815 1
4.5799 -13.664 1
-12.002 -22.009 1
18.741 -30.314 1
5.6431 32.032 1
-22.899 -7.1431 1
29.514 39.986 1
-4.4027 -22.037 1
18.277 -30.536 1
-15.015 6.761 1
-1.1461 61.79 1
-33.091 -4.0095 1
-28.719 -2.8508 1
-26.704 17.395 1
-50.229 23.907 1
30.875 21.583 1
40.54 9.4164 1
25.506 39.576 1
15.749 13.797 1
-24.729 29.668 1
9.4234 23.167 1
8.0082 -52.287 1
-31.89 22.238 1
-52.615 22.427 1
4.4625 29.49 1
21.935 -17.756 1
-15.564 3.6929 1
-11.727 -29.986 1
5.4339 33.422 1
-3.7364 -35.886 1
-5.2871 56.072 1
-36.064 -32.967 1
-7.4543 3.9171 1
58.69 -9.9333 1
-28.404 -3.3948 1
1.5579 2.9641 1
38.877 -29.416 1
8.135 -30.304 1
-7.2362 -9.374 1
-9.8675 -7.8287 1
29.895 23.87 1
25.009 2.5554 1
-10.473 -11.934 1
-35.009 -33.057 1
-1.527 -19.292 1
-30.989 23.474 1
-13.861 -35.425 1
29.176 21.993 1
-9.4983 13.033 1
-15.489 -1.9963 1
21.01 -18.248 1
4.9279 -25.366 1
-27.019 -9.9574 1
2.8091 33.465 1
10.75 2.01 1
7.9506 -53.153 1
-6.3405 19.609 1
-5.8767 57.974 1
-3.7599 -10.567 1
-26.049 0.21778 1
-21.928 18.654 1
-13.301 10.526 1
23.923 -11.047 1
-31.248 25.028 1
10.383 4.4682 1
-34.082 -7.5308 1
-11.058 42.542 1
11.333 22.487 1
-52.058 20.029 1
21.895 -11.993 1
-6.2028 12.327 1
14.253 15.999 1
-21.957 15.378 1
-14.645 -22.425 1
-33.608 4.4511 1
16.237 23.018 1
-32.555 3.849 1
41.59 6.5539 1
-32.189 -2.7462 1
-16.445 2.9869 1
-6.2171 57.271 1
-4.1398 0.41344 1
-16.768 5.4533 1
-34.574 9.728 1
-18.621 -12.414 1
26.16 -12.987 1
-14.25 -6.3727 1
-24.627 1.4738 1
36.061 -36.318 1
6.3384 4.0945 1
39.068 4.5126 1
34.676 -35.823 1
22.564 -13.924 1
10.959 24.567 1
9.1145 -55.83 1
-9.5243 -37.441 1
-5.5566 61.962 1
-1.3499 -8.9664 1
-29.982 -48.451 1
-5.9387 19.471 1
-28.154 -48.232 1
-29.99 -48.469 1
-11.668 -29.888 1
8.978 13.804 1
11.514 2.1941 1
5.4028 30.171 1
9.8222 5.718 1
22.965 -1.1616 1
13.094 16.817 1
41.299 7.7156 1
2.0759 17.796 1
-8.1032 45.09 1
-18.329 2.3167 1
-33.824 -32.962 1
4.2316 -13.431 1
-4.4171 56.987 1
-33.528 4.7397 1
-32.143 -0.064124 1
-15.629 3.6523 1
7.1288 33.82 1
8.5853 -35.126 1
-5.5353 54.667 1
-12.346 -8.7042 1
17.347 -9.4782 1
-34.076 -31.397 1
4.0279 -5.7911 1
-22.673 -50.981 1
29.708 -5.3145 1
53.251 -3.0064 1
-12.386 -33.929 1
-31.842 24.242 1
8.0507 -46.158 1
51.073 11.817 1
-36.501 -1.5003 1
-50.306 25.388 1
-5.5913 -33.533 1
-31.135 -6.6513 1
22.134 30.371 1
-9.3203 1.1282 1
26.608 0.9869 1
-36.499 -29.195 1
-9.6728 -11.218 1
8.089 -46.21 1
-31.741 -8.7022 1
-24.398 18.409 1
29.277 21.861 1
20.748 -18.43 1
14.907 14.619 1
-10.086 -18.035 1
37.31 6.0613 1
-2.3092 62.273 1
-8.8527 55.674 1
-31.113 24.146 1
-26.843 -14.418 1
48.537 10.627 1
19.963 -33.353 1
8.5861 -47.064 1
-26.725 -14.69 1
52.56 -10.405 1
-22.982 -1.8084 1
7.2791 -47.205 1
37.721 6.2477 1
-5.8095 57.22 1
-20.54 0.29449 1
24.847 -9.0533 1
-4.6092 3.3513 1
-49.791 27.689 1
-12.64 39.752 1
22.808 37.361 1
-22.346 21.852 1
-13.168 43.544 1
3.4671 -8.8821 1
-14.739 -34.296 1
54.802 -5.3256 1
-18.718 -24.351 1
22.721 13.089 1
20.104 -18.013 1
26.863 0.72921 1
36.759 8.1893 1
-25.274 19.658 1
-1.7027 18.645 1
-6.8985 -36.255 1
-18.358 -13.425 1
-6.6465 -10.553 1
-6.788 1.0022 1
32.534 18.847 1
8.629 -51.728 1
16.575 15.754 1
3.0389 -20.122 1
-34.614 -32.321 1
-32.471 -29.709 1
-9.3458 -28.893 1
6.4087 27.066 1
-27.84 4.8933 1
1.3046 -27.412 1
-12.715 -17.233 1
-51.673 20.581 1
-34.161 -13.372 1
-7.9702 54.852 1
-25.92 -8.0172 1
25.493 38.779 1
-34.46 -10.978 1
-11.491 -25.084 1
-16.849 -1.5777 1
-32.357 -29.7 1
-6.5439 62.175 1
32.565 -33.096 1
-28.392 -2.8395 1
7.7113 -13.416 1
58.751 -11.423 1
-23.023 -15.838 1
6.4587 24.038 1
-11.447 3.7812 1
-11.281 -32.701 1
-6.3697 54.04 1
-13.455 -16.861 1
22.469 39.776 1
28.442 38.551 1
-33.806 -32.961 1
24.228 40.999 1
1.5008 19.641 1
-3.2034 58.178 1
-30.638 -6.1935 1
4.74 2.1238 1
31.65 -8.7843 1
-5.6344 55.07 1
-21.011 -50.188 1
-26.731 -22.399 1
26.225 -12.996 1
-34.127 -3.1084 1
-6.3753 -34.558 1
-35.637 -13.201 1
3.4852 18.515 1
38.092 5.4278 1
-12.975 -6.3624 1
37.913 -32.097 1
-15.431 -2.0026 1
-28.725 -51.251 1
-0.34076 11.928 1
-27.87 -7.555 1
-7.0125 6.355 1
-35.976 3.905 1
-23.217 17.434 1
-9.4227 2.0811 1
-28.805 26.499 1
-19.55 4.1532 1
29.421 -4.6129 1
49.843 5.6503 1
-5.0426 60.864 1
-8.5834 2.9005 1
-6.357 -7.1679 1
-28.398 -51.587 1
-33.023 3.6468 1
9.0683 18.418 1
34.514 -30.289 1
30.508 22.187 1
-12.763 -36.189 1
-27.376 -28.403 1
-28.217 -28.404 1
49.925 7.4192 1
-8.3885 17.306 1
-3.1253 58.126 1
21.17 -14.89 1
-34.351 4.8599 1
20.786 -17.87 1
-26.998 18.818 1
-12.991 -15.783 1
-34.145 6.8235 1
-4.643 12.192 1
-21.138 -15.349 1
3.793 5.658 1
-29.604 -3.9136 1
-31.599 -7.1956 1
-23.834 -2.5496 1
9.0628 -12.941 1
50.604 1.1849 1
0.99904 -27.394 1
-18.733 -24.321 1
18.336 -30.462 1
-33.899 -3.7388 1
-8.3995 -0.30581 1
5.7418 1.8601 1
8.5675 -44.206 1
-23.984 -12.293 1
-35.251 -7.8327 1
50.26 9.5454 1
-1.4644 32.852 1
8.7961 -48.131 1
3.2657 32.829 1
51.839 8.6114 1
-29.529 19.586 1
-12.175 18.784 1
22.857 0.75861 1
19.263 21.806 1
-51.307 21.096 1
13.191 -0.61601 1
20.08 7.5041 1
-53.765 20.716 1
-13.842 6.1302 1
-5.7188 -16.466 1
18.334 22.586 1
-28.077 19.413 1
9.25 -2.0879 1
-4.3995 -12.539 1
-7.898 60.5 1
26.146 1.3308 1
-14.247 2.11 1
20.858 30.838 1
32.166 -33.563 1
-35.483 -5.7828 1
-14.163 42.032 1
27.75 -12.214 1
9.6649 -19.22 1
51.025 -10.448 1
40.389 -28.016 1
-7.8578 0.30056 1
-0.9045 -13.774 1
1.4226 -5.084 1
34.963 -34.541 1
36.537 4.9657 1
-11.283 52.621 1
32.516 17.56 1
-2.0181 -13.223 1
16.587 15.752 1
51.878 3.0985 1
-36.71 -29.377 1
49.112 9.8646 1
-31.007 25.808 1
58.75 -12.416 1
26.871 2.7755 1
-18.277 -14.571 1
-13.601 -26.61 1
29.785 23.446 1
-24.656 2.0189 1
0.8486 -11.21 1
-30.941 -25.729 1
51.805 -3.8598 1
48.26 10.142 1
11.221 34.678 1
-30.852 -25.539 1
11.966 -4.6503 1
-29.443 -27.909 1
-24.959 14.421 1
19.629 -30.615 1
8.7389 -48.035 1
-35.411 -14.439 1
31.15 10.312 1
4.8829 30.901 1
-21.981 -17.403 1
-20.839 19.104 1
-10.978 -22.163 1
-35.747 4.4289 1
-18.252 21.326 1
24.326 40.435 1
5.2785 17.871 1
-14.417 -6.5392 1
2.525 -24.432 1
-53.651 18.999 1
-27.765 1.2452 1
-28.12 -28.187 1
-5.6485 54.97 1
16.471 18.373 1
5.4632 9.8139 1
5.3877 18.274 1
-15.359 39.714 1
11.961 -4.6447 1
0.56314 -27.521 1
-5.1959 59.858 1
-34.478 5.3312 1
19.583 -2.5395 1
-3.1928 -27.968 1
-53.912 18.535 1
-30.162 -26.688 1
10.364 8.1081 1
8.7828 -12.731 1
-0.41123 5.9896 1
-5.4317 19.309 1
54.11 -10.681 1
31.504 24.319 1
-20.326 18.601 1
30.759 8.6001 1
8.0003 -55.438 1
35.01 -29.841 1
9.2769 -49.812 1
-18.363 -47.863 1
22.066 39.915 1
-12.631 39.673 1
-13.864 -27.561 1
-10.994 -21.732 1
-5.3375 -33.309 1
17.086 -23.374 1
-4.1258 -8.9657 1
-25.384 -50.36 1
-33.43 5.2577 1
-26.015 -8.7619 1
-37.443 -13.767 1
23.143 -14.528 1
35.708 -36.616 1
27.504 -8.9058 1
41.536 -26.343 1
52.983 -0.96625 1
-15.467 34.88 1
-13.671 -10.395 1
8.0602 -46.078 1
20.546 39.296 1
36.958 -32.444 1
-5.1446 -0.93917 1
0.097016 -9.645 1
-15.95 -19.943 1
37.706 -32.539 1
22.315 -14.123 1
23.097 11.944 1
-10.045 -29.772 1
8.8626 -32.501 1
52.436 0.5006 1
8.7005 1.5751 1
6.5713 17.262 1
-30.299 -10.003 1
8.2162 -48.603 1
7.3068 -54.767 1
41.072 -29.166 1
8.1198 -53.837 1
18.336 22.846 1
-29.054 -49.973 1
-51.791 22.569 1
6.3124 30.028 1
-4.9286 -19.425 1
28.789 8.344 1
23.432 21.844 1
2.0231 -12.757 1
18.959 -30.237 1
8.5912 -44.248 1
20.224 -31.826 1
8.5914 -48.242 1
-13.203 38.768 1
-54.897 18.415 1
24.758 0.6707 1
-18.629 0.089419 1
15.337 8.6064 1
36.278 7.977 1
-21.407 -1.3491 1
-29.331 -12.235 1
-26.918 2.2167 1
22.513 -15.924 1
-12.177 -6.5754 1
-2.9993 17.456 1
2.2416 10.742 1
-10.702 12.688 1
-7.0013 -17.94 1
11.509 2.2085 1
7.1643 -17.813 1
-8.4193 17.523 1
-11.68 -37.35 1
-5.8692 -31.773 1
-21.027 -50.794 1
9.3334 -55.199 1
2.1244 -1.0224 1
33.123 6.4221 1
15.371 1.154 1
25.128 35.642 1
-1.5057 -29.25 1
23.877 35.618 1
4.6748 2.18 1
42.645 8.3158 1
-53.237 19.648 1
-27.949 31.655 1
27.764 -0.19159 1
-8.2608 7.806 1
2.9128 -15.181 1
-27.452 30.18 1
8.2278 -54.375 1
-19.686 -51.086 1
29.682 1.2251 1
29.213 23.478 1
-32.157 0.079248 1
13.03 16.907 1
-20.199 18.675 1
-5.8585 19.6 1
1.1395 -26.461 1
-4.1301 4.3691 1
-14.907 37.083 1
-5.1718 17.487 1
9.5823 -35.232 1
8.8896 14.79 1
-51.804 20.37 1
-1.6061 0.10001 1
-19.416 -4.4099 1
9.3549 1.1842 1
50.355 0.35136 1
48.376 -0.8217 1
3.6393 12.132 1
-50.141 27.282 1
20.382 36.746 1
-33.593 -31.767 1
-7.1395 -17.119 1
-52.142 19.937 1
12.146 -27.041 1
-14.029 -6.3201 1
49.977 6.7232 1
-11.059 10.991 1
12.568 -6.7603 1
24.504 37.003 1
42.483 8.7469 1
1.2006 -10.177 1
-18.823 -8.1684 1
51.64 -11.339 1
-15.474 -1.8888 1
21.491 -12.383 1
-34.688 -12.668 1
-27.394 13.951 1
52.729 -8.8406 1
6.079 6.9402 1
-36.546 -13.504 1
37.623 9.825 1
-4.7453 -12.799 1
57.536 -10.653 1
21.225 24.462 1
-5.9067 57.625 1
8.5914 -49.23 1
35.692 -36.347 1
-2.2043 -15.279 1
29.731 22.131 1
29.551 8.7394 1
-19.014 0.57023 1
-14.79 -4.2163 1
-4.739 51.175 1
3.2914 -21.141 1
-0.72519 30.3 1
8.4272 -50.173 1
-10.961 9.48 1
-26.572 -0.79068 1
-27.452 -24.222 1
-14.685 -3.8742 1
-20.302 -3.8279 1
16.683 -7.3494 1
-23.066 -15.574 1
24.218 33.354 1
9.9917 -18.906 1
58.25 -11.722 1
12.512 0.033042 1
-21.295 4.7302 1
-24.786 29.569 1
-7.3484 58.425 1
1.2718 8.1649 1
23.962 37.737 1
0.84921 -27.483 1
9.2854 27.036 1
25.496 39.734 1
-25.926 -4.7035 1
24.659 30.026 1
51.836 -11.555 1
17.059 24.175 1
3.047 -20.334 1
-33.41 -8.9346 1
-7.02 -34.195 1
17.22 -7.7248 1
-1.8745 18.205 1
-2.8819 -3.6884 1
14.665 4.9321 1
-29.352 -12.119 1
24.626 -12.201 1
10.083 -16.907 1
52.285 -4.1601 1
-9.5388 13.035 1
-30.511 -2.4996 1
-4.9328 -14.118 1
25.094 36.793 1
37.972 7.5228 1
-5.5949 54.779 1
-13.064 40.372 1
-10.041 -18.069 1
-18.703 -10.508 1
56.167 -10.675 1
49.67 -9.3201 1
33.202 20.496 1
-33.512 -29.732 1
-1.0733 35.841 1
-14.067 -6.3408 1
-24.988 -14.643 1
-26.956 2.3258 1
-7.768 56.116 1
3.8203 -26.714 1
11.543 -26.714 1
35.465 22.581 1
-30.397 27.845 1
31.75 -2.7039 1
11.789 11.287 1
-28.626 -0.28396 1
8.5083 25.123 1
41.107 -28.467 1
5.0823 -8.3023 1
-26.337 -13.266 1
-28.879 -9.9514 1
-18.159 3.4063 1
-36.839 -29.946 1
-26.032 -1.8028 1
-14.177 38.124 1
-4.8996 -0.80799 1
41.162 -27.336 1
-11.607 -1.2281 1
-29.25 -23.067 1
8.8944 -51.663 1
17.854 5.6313 1
3.0646 33.982 1
25.091 1.5907 1
10.271 11.082 1
-3.3362 58.412 1
-26.678 -49.747 1
-6.3621 -7.1636 1
-28.34 -0.18319 1
21.219 24.457 1
21.035 3.1646 1
-27.348 -49.242 1
-18.245 -9.9704 1
9.8629 5.7609 1
-15.574 3.7182 1
-11.871 9.4199 1
-8.4059 -0.27598 1
38.82 -29.403 1
8.1492 -50.898 1
41.91 -27.832 1
21.244 -18.007 1
6.0341 6.9172 1
8.9746 14.846 1
-14.142 13.641 1
32.333 -36.363 1
12.382 23.195 1
33.047 6.301 1
-7.04 -17.149 1
4.6992 -2.6299 1
9.713 -35.176 1
-3.2032 -10.13 1
-5.8791 -31.644 1
-6.1841 59.825 1


==> res.tex <==
x	y_s	y_p	y_e	y_u
0	1	0.95849	0.077966102	0.006779661
500	0.273081761	0.21006	0.084745763	0.006779661
1000	0.203899371	0.18491	0.074576271	0.006779661
1500	0.177421384	0.21761	0.06779661	0.003389831
2000	0.158553459	0.2239	0.06779661	0.003389831
2500	0.153522013	0.20755	0.06779661	0.003389831
3000	0.159811321	0.2	0.06779661	0.003389831
3500	0.152264151	0.17484	0.06779661	0.003389831
4000	0.152264151	0.18239	0.06779661	0.003389831
4500	0.142201258	0.18239	0.06779661	0.003389831
5000	0.147232704	0.19245	0.06779661	0.003389831
5500	0.143459119	0.19119	0.06779661	0.003389831
6000	0.143459119	0.18239	0.06779661	0.003389831
6500	0.138427673	0.19245	0.06779661	0.003389831
7000	0.138427673	0.19748	0.06779661	0.003389831
7500	0.138427673	0.19371	0.06779661	0.003389831
8000	0.123459119	0.18491	0.06779661	0.003389831
8500	0.123459119	0.18742	0.06779661	0.003389831
9000	0.122201258	0.18616	0.06779661	0.003389831
9500	0.112012579	0.17987	0.06779661	0.003389831
10000	0.114591195	0.18491	0.06779661	0.003389831
10500	0.091012579	0.18868	0.06779661	0.003389831
11000	0.089457627	0.19119	0.06779661	0.003389831
11500	0.087457627	0.18491	0.06779661	0.003389831
12000	0.084745763	0.18868	0.06779661	0.003389831
12500	0.083231	0.18616	0.06779661	0.003389831
13000	0.083745763	0.18868	0.06779661	0.003389831
13500	0.081745763	0.18742	0.06779661	0.003389831
14000	0.080745763	0.18491	0.06779661	0.003389831
14500	0.080745763	0.18491	0.06779661	0.003389831
15000	0.080745763	0.18491	0.06779661	0.003389831

